SIPOMDPLite-Net: Lightweight, Self-Interested Learning and Planning in POSGs with Sparse Interactions

This work introduces sIPOMDPLite-net, a deep neural network (DNN) architecture for decentralized, self-interested agent control in partially observable stochastic games (POSGs) with sparse interactions between agents. The network learns to plan in contexts modeled by the interactive partially observable Markov decision process (I-POMDP) Lite framework and uses hierarchical value iteration networks to simulate the solution of nested MDPs, which I-POMDP Lite attributes to the other agent to model its behavior and predict its intention. We train sIPOMDPLite-net with expert demonstrations on small two-agent Tiger-grid tasks, for which it accurately learns the underlying I-POMDP Lite model and near-optimal policy, and the policy continues to perform well on larger grids and real-world maps. As such, sIPOMDPLite-net shows good transfer capabilities and offers a lighter learning and planning approach for individual, self-interested agents in multiagent settings.

==> plots/docs/595142f9-809a-4354-8218-28db58f80e34 <==
{"id":"n0.27567949884143794","lines":[{"id":"n0.040192133545799535","blocks":[]},{"id":"n0.9895876271290234","blocks":[{"id":"n0.9173890258494699","text":"\\diagram","type":"composite","elements":{"de11223966794022666":{"id":"de11223966794022666","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.7905678483945358"}],"id":"n0.19836934953297547"}],"id":"n0.3697409210978573"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.431063176229344"}],"id":"n0.45841864014718414"}],"shape":{"data":{"p":{"x":43.51719895786459,"y":44.62593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9324197589956453":{"id":"de9324197589956453","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"K","id":"n0.7854313636540744"}],"id":"n0.985214144221201"}],"id":"n0.6661812810602377"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.40559890186951475"},{"text":"-recurrence","style":{"fontSize":{"value":0.4}},"id":"n0.003152585387300899"}],"style":{"align":"center"},"id":"n0.061334301092576204"}],"shape":{"data":{"p":{"x":40.48858574589599,"y":50.62593476262708},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8259787715425368":{"id":"de8259787715425368","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"U","id":"n0.6399712608665704"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"0","id":"n0.3151872604159556"}],"id":"n0.47592403312866116"}],"id":"n0.39645060429578693"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5919786388654495"}],"id":"n0.27736361760795636"}],"id":"n0.8097852380933599"}},"id":"n0.02702932545878034"},{"type":"single","text":"(","id":"n0.5606333216341286"},{"text":"s","id":"n0.2292691114706389"},{"type":"single","text":")","id":"n0.04269859187998892"}],"id":"n0.9283375581593811"}],"id":"n0.89449632340263"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5147011925460008"}],"style":{"align":"center"},"id":"n0.4152486386943557"}],"shape":{"data":{"p":{"x":15.006408691406207,"y":47.249469301363774},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8042430803808909":{"id":"de8042430803808909","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"R","id":"n0.5002283888487531"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7783614614964984"}],"id":"n0.297961339951891"}],"id":"n0.06678040051567691"}},"id":"n0.14844533386117065"}],"id":"n0.4081166751938259"}],"id":"n0.811386407261955"}},"id":"n0.3493723863456686"},{"type":"single","text":"(","id":"n0.46907936726833777"},{"text":"s","id":"n0.805370084609033"},{"id":"n0.12240558766567688","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6473433520604324","lines":[{"id":"n0.6655299740628118","blocks":[{"id":"n0.6759078268102778","text":"i"}]}]}}},{"text":",a","id":"n0.7948022804344625"},{"id":"n0.6913558726770317","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.39601115625214267","lines":[{"id":"n0.5983353018248478","blocks":[{"id":"n0.9802798100220826","text":"i"}]}]}}},{"type":"single","text":")","id":"n0.6212127400771796"}],"id":"n0.8011604082776529"}],"id":"n0.5585144594769098"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6409273035569256"}],"style":{"align":"center"},"id":"n0.5580434371713094"}],"shape":{"data":{"p":{"x":105.62584124487336,"y":234.71144772630112},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de23431970431903837":{"id":"de23431970431903837","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.1170102216432789"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K-1","id":"n0.2677685535824075"}],"id":"n0.2888280766334479"}],"id":"n0.10385750759248502"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.1512838805908041"}],"id":"n0.45970722336055814"}],"id":"n0.4227015986382636"}},"id":"n0.8477961955365088"},{"type":"single","text":"(","id":"n0.25677412994056237"},{"text":"s,a","id":"n0.9172064599053886"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4704409906674023"}],"id":"n0.7906745514798215"}],"id":"n0.21186906296159402"}},"id":"n0.38745424536614315"},{"type":"single","text":")","id":"n0.8400134290375487"}],"id":"n0.0860315124689226"}],"id":"n0.03458318572511776"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9650773898812901"}],"style":{"align":"center"},"id":"n0.3927604683534769"}],"shape":{"data":{"p":{"x":88.99999999999994,"y":28.307382940085972},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de9220101954817366":{"id":"de9220101954817366","lines":[{"blocks":[{"style":{"fontSize":"\\tiny"},"text":"max","id":"n0.5759991411766465"}],"id":"n0.17437563620620256"}],"shape":{"data":{"p":{"x":132.9161720677406,"y":43.48307625737806},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2451984776153353":{"id":"de2451984776153353","lines":[{"blocks":[{"text":"over ","style":{"fontSize":{"value":0.4}},"id":"n0.18585304985235784"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.35282676690819437"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.261625646233296"}],"id":"n0.8542118915203367"}],"id":"n0.9393992909034548"}},"id":"n0.6361202043302763"}],"id":"n0.9225802517691526"}],"id":"n0.6358514931961325"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.13620027133852997"}],"style":{"align":"center"},"id":"n0.5598413358017083"}],"shape":{"data":{"p":{"x":130.02611356688283,"y":57.07236067739149},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1899635654055294":{"id":"de1899635654055294","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"U","id":"n0.006068972938334527"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K-1","id":"n0.30327497430878814"}],"id":"n0.6266768437911552"}],"id":"n0.6259082828332134"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.05812691300451456"}],"id":"n0.5793854272311463"}],"id":"n0.6155248479809592"}},"id":"n0.1756386388594553"},{"type":"single","text":"(","id":"n0.6122476690348917"},{"text":"s","id":"n0.779005463770509"},{"type":"single","text":")","id":"n0.5228856643868618"}],"id":"n0.6037200504114792"}],"id":"n0.5587516503235763"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.19403745428148667"}],"style":{"align":"center"},"id":"n0.10508473415509534"}],"shape":{"data":{"p":{"x":173.0064086914062,"y":48.249469301363774},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de13873359332904545":{"id":"de13873359332904545","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.5747433247274787"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.8035317098087782"}],"id":"n0.6941594324020373"}],"id":"n0.5354791515466708"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.19124892957484718"}],"id":"n0.03189260206184197"}],"id":"n0.4123760353214514"}},"id":"n0.20407435975599109"},{"type":"single","text":"(","id":"n0.39395424899370446"},{"text":"s,a","id":"n0.9496317673458718"},{"type":"single","text":")","id":"n0.6571442186758487"}],"id":"n0.8042656885336161"}],"id":"n0.7264028620765699"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.06254498850303825"}],"style":{"align":"center"},"id":"n0.5971366396022255"}],"shape":{"data":{"p":{"x":434,"y":32.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8441154366127299":{"id":"de8441154366127299","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.146835922766952"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.4090732188892696"}],"id":"n0.31365306684005234"}],"id":"n0.40282909853865134"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.08719815994861824"}],"id":"n0.0908462187955954"}],"id":"n0.740663028209978"}},"id":"n0.11371273039382412"},{"type":"single","text":"(","id":"n0.6107997469772355"},{"text":"s,a","id":"n0.8706452099791198"},{"type":"single","text":")","id":"n0.688112252668329"}],"id":"n0.49246669600141635"}],"id":"n0.04583797116036181"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.003118688884779619"}],"style":{"align":"center"},"id":"n0.11301351693347028"}],"shape":{"data":{"p":{"x":627,"y":185.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de5537087275522437":{"id":"de5537087275522437","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"id":"n0.7694279464781144","text":"X"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.8126849532753888"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.9976485833903799"}],"id":"n0.20559309011582427"}],"id":"n0.15112809974544295"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.3556677777254764"}],"id":"n0.12221687328765296"}],"id":"n0.4633494985314448"}},"id":"n0.8614895912338203"}],"id":"n0.1361849523883183"}],"id":"n0.8873242276899993"}},"id":"n0.21849965246663694"},{"type":"single","text":"(","id":"n0.23386516712588956"},{"text":"s,a","id":"n0.31656162311839675"},{"type":"single","text":")","id":"n0.5296909722044236"}],"id":"n0.25330121363332925"}],"id":"n0.5175725534760129"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4369764114799277"}],"style":{"align":"center"},"id":"n0.13265684890715912"}],"shape":{"data":{"p":{"x":485.58166565657575,"y":105.83474321560152},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6990293149639712":{"id":"de6990293149639712","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1-","id":"n0.8220898377435071"},{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.03681549327761591"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.42292628840796764"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.6360884816366903"}],"id":"n0.6075766201412931"}],"id":"n0.1831481499402674"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.3255229490058702"}],"id":"n0.45556410972655126"}],"id":"n0.6017480792671808"}},"id":"n0.1374571125358317"}],"id":"n0.9273496428839458"}],"id":"n0.3620504825259647"}},"id":"n0.29790768148228053"}],"id":"n0.5159037234950323"}],"id":"n0.8764715381876009"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.2441893047384185"}],"style":{"align":"center"},"id":"n0.9480269161627728"}],"shape":{"data":{"p":{"x":545.5816656565758,"y":106.30738294008597},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8785973636687534":{"id":"de8785973636687534","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.9171824590138633"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.44672021196848055"}],"id":"n0.7818607430779412"}],"id":"n0.2424766441816495"}},"id":"n0.8387742053728955"},{"text":"|","id":"n0.02119829929289274"}],"id":"n0.19818936353891803"}],"id":"n0.10534765439253158"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.32943218763312565"}],"style":{"align":"center"},"id":"n0.507418967455411"}],"shape":{"data":{"p":{"x":-4,"y":2.983856201171875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de706628072537445":{"id":"de706628072537445","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.8759636294784048"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.22156309198850188"}],"id":"n0.866329597589272"}],"id":"n0.3327842032733004"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.01853059314001615"}],"id":"n0.41932018945465765"}],"id":"n0.36034326364212843"}},"id":"n0.608825440438538"},{"type":"single","text":"(","id":"n0.9080770702919103"},{"text":"s,a","id":"n0.19498244033844703"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5678821319862739"}],"id":"n0.9238863149011765"}],"id":"n0.5554338636934399"}},"id":"n0.49702652107349476"},{"type":"single","text":")","id":"n0.4577386658511726"}],"id":"n0.3821079040693218"}],"id":"n0.7324353081628885"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8702381870656417"}],"style":{"align":"center"},"id":"n0.5788367918750632"}],"shape":{"data":{"p":{"x":314.4011224293617,"y":33.68144817745889},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de3825894104169385":{"id":"de3825894104169385","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.028112752972151878"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.4472931034526244"}],"id":"n0.9460204965180818"}],"id":"n0.929472850259067"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.28759584258667403"}],"id":"n0.7787886247668507"}],"id":"n0.21699811384766154"}},"id":"n0.8602692990204304"},{"type":"single","text":"(","id":"n0.6777985648016569"},{"text":"s,a","id":"n0.2706690081177474"},{"type":"single","text":")","id":"n0.5167559890629587"}],"id":"n0.8353405095841582"}],"id":"n0.7820935964803029"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.023554338098733085"}],"style":{"align":"center"},"id":"n0.5130102994810564"}],"shape":{"data":{"p":{"x":325,"y":150.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de3664569806969358":{"id":"de3664569806969358","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"R","id":"n0.6926896140574603"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.17437436458251"}],"id":"n0.500450634251201"}],"id":"n0.5707162910337331"}},"id":"n0.8753640369280276"},{"type":"single","text":"(","id":"n0.3654602825647988"},{"text":"s,a","id":"n0.8464509719784241"},{"type":"single","text":")","id":"n0.21823688730695134"}],"id":"n0.8957631635704928"}],"id":"n0.43208464797421753"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8053380576443636"}],"style":{"align":"center"},"id":"n0.506790653356602"}],"shape":{"data":{"p":{"x":106.99999999999994,"y":149.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de6614622216116961":{"id":"de6614622216116961","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.4016781716870128"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.7877869983749566"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.5103569650418229"}],"id":"n0.10297667539010713"}],"id":"n0.24180552040286263"},"indexValue":{"lines":[{"blocks":[{"id":"n0.34845711097347976","text":"R"}],"id":"n0.41998310362694125"}],"id":"n0.645825499301385"}},"id":"n0.270161409778235"}],"id":"n0.8589650799408448"}],"id":"n0.4728382713070429"}},"id":"n0.07072152856983616"},{"type":"single","text":"(","id":"n0.5616600331440771"},{"text":"s,a","id":"n0.17714782829713904"},{"type":"single","text":")","id":"n0.022167164478694046"}],"id":"n0.16188097070730345"}],"id":"n0.2601044691611345"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.995238850418787"}],"style":{"align":"center"},"id":"n0.10232456325390626"}],"shape":{"data":{"p":{"x":267.58166565657575,"y":283.8347432156015},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6133498609024188":{"id":"de6133498609024188","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1-","id":"n0.7130969737888468"},{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.07721349329427385"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.35828667211669396"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.7749033135304042"}],"id":"n0.2482949363799123"}],"id":"n0.3471541028459606"},"indexValue":{"lines":[{"blocks":[{"id":"n0.5448587495264856","text":"R"}],"id":"n0.2807781437837287"}],"id":"n0.44844167584069505"}},"id":"n0.7952041490495199"}],"id":"n0.3574751371814284"}],"id":"n0.09241515757786978"}},"id":"n0.39464029862294425"}],"id":"n0.14935564515850985"}],"id":"n0.1395073386628325"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7253802699131924"}],"style":{"align":"center"},"id":"n0.9517478242664072"}],"shape":{"data":{"p":{"x":197.5816656565757,"y":285.8347432156015},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2819300277576777":{"id":"de2819300277576777","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"R","id":"n0.5080333992027091"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.05988815671987924"}],"id":"n0.8677746219753883"}],"id":"n0.3330801148958591"}},"id":"n0.04931305154863108"},{"type":"single","text":"(","id":"n0.7438265313295498"},{"text":"s,a","id":"n0.9416925031222689"},{"type":"single","text":")","id":"n0.27548838127387"}],"id":"n0.8304290040433637"}],"id":"n0.8840114401506087"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6375920278393064"}],"style":{"align":"center"},"id":"n0.9746471312645337"}],"shape":{"data":{"p":{"x":374.99999999999994,"y":234.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de9417082366336318":{"id":"de9417082366336318","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.03835443573157615"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.24142218287449624"}],"id":"n0.5162121360533385"}],"id":"n0.6195838386917736"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9092287203107567"}],"id":"n0.5174839387703523"}],"id":"n0.6673525200226891"}},"id":"n0.7347679435219794"},{"type":"single","text":"(","id":"n0.28843414602820805"},{"text":"s,a","id":"n0.6083528317729592"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6610000866890124"}],"id":"n0.8139612448440854"}],"id":"n0.5390876427499873"}},"id":"n0.23308836377708442"},{"type":"single","text":")","id":"n0.5120386048257137"}],"id":"n0.14721663159612897"}],"id":"n0.6997469764205988"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.2885185327931037"}],"style":{"align":"center"},"id":"n0.9110026451703763"}],"shape":{"data":{"p":{"x":616,"y":62.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de4462760249275344":{"id":"de4462760249275344","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.6097464845282279"}],"id":"n0.8832627046842543"}],"id":"n0.8247489543416093"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.2450296951090163"}],"id":"n0.2552966683935185"}],"shape":{"data":{"p":{"x":615.5171989578646,"y":131.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8948224066984556":{"id":"de8948224066984556","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.10857956305467842"}],"id":"n0.421574138797302"}],"id":"n0.7424021727233538"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6055471072451277"}],"id":"n0.7705004067186279"}],"shape":{"data":{"p":{"x":280.16577825936406,"y":232.6259652802052},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4331374139554627":{"id":"de4331374139554627","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.5027133070605017"}],"id":"n0.5355959891214823"}],"id":"n0.005551580701313341"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6075118873025613"}],"id":"n0.0914600554525753"}],"shape":{"data":{"p":{"x":253.5171989578646,"y":209.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de26192952769719957":{"id":"de26192952769719957","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.8888688572006751"}],"id":"n0.3267010850773666"}],"id":"n0.8041508784277376"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7720336149755831"}],"id":"n0.1346588330455778"}],"shape":{"data":{"p":{"x":487.5171989578646,"y":185.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6035267197891458":{"id":"de6035267197891458","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.6543152002270076"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7334742889692814"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.3242040524010321"}],"id":"n0.32644845688640456"}],"id":"n0.6312958751544981"}},"id":"n0.8409088613073215"}],"id":"n0.42302298582626086"}],"id":"n0.779041171275882"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.6188405926277076"}],"id":"n0.3493043981926587"}],"id":"n0.8508007860753459"}},"id":"n0.49707329322549"}],"id":"n0.6768200944743077"}],"id":"n0.976576704540332"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9023187988105708"}],"id":"n0.16337623688328828"}],"shape":{"data":{"p":{"x":9.99359130859375,"y":-3.4417227080760426}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de9760449880962501":{"id":"de9760449880962501","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.7644474351444859"}],"id":"n0.38534861850241797"}],"id":"n0.03316696426389476"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.35057284840972147"}],"id":"n0.5048663397251856"}],"shape":{"data":{"p":{"x":535.5171989578646,"y":43.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8954529408852401":{"id":"de8954529408852401","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.848393679454543"}],"id":"n0.25456691959311417"}],"id":"n0.8389529357060233"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8813460424744157"}],"id":"n0.5735294397612922"}],"shape":{"data":{"p":{"x":182.5171989578646,"y":232.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6584387665735523":{"id":"de6584387665735523","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.47807419727561884"}],"id":"n0.9207113995253955"}],"id":"n0.36444411269043075"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.27754890264373744"}],"id":"n0.9494594229882736"}],"shape":{"data":{"p":{"x":576.1657782593641,"y":185.6259652802052},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de012480490536642463":{"id":"de012480490536642463","lines":[{"blocks":[{"text":"Env of ","style":{"fontSize":"\\tiny"},"id":"n0.40909545976344974"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"i","id":"n0.35427989374640023"}],"id":"n0.6918224794336232"}],"id":"n0.6716473402196932"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.939569616596925"}],"style":{"align":"center"},"id":"n0.01145179328720447"}],"shape":{"data":{"p":{"x":0.0172119140625,"y":229.83665721496357},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de12292055506100197":{"id":"de12292055506100197","lines":[{"blocks":[{"text":"Envs","style":{"fontSize":"\\tiny"},"id":"n0.9459702196038209"}],"style":{"align":"center"},"id":"n0.7056217977509271"}],"shape":{"data":{"p":{"x":5.0172119140625,"y":146.83665721496357},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6435602377123977":{"id":"de6435602377123977","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.6970003767302986"}],"id":"n0.5950220408018525"}],"shape":{"data":{"p":{"x":42.0093994140625,"y":146},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9996999739406618":{"id":"de9996999739406618","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.5369596322341148"}],"id":"n0.26726632531312156"}],"shape":{"data":{"p":{"x":48.0093994140625,"y":230},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de45926917840285286":{"id":"de45926917840285286","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.33193660410626946"},{"id":"n0.05791779870879621","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.08047694735007327","lines":[{"id":"n0.7816226269678082","blocks":[{"id":"n0.2919634577615382","text":"i"}]}]}}},{"text":"|×|A","id":"n0.2065855154668208"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.02735575627040654","text":"i"}],"id":"n0.5841678693928647"}],"id":"n0.7970017989912566"}},"id":"n0.5110727722053909"},{"text":"|","id":"n0.27034545581103564"}],"id":"n0.8261875009076476"}],"id":"n0.5201323123537056"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4154985234933193"}],"style":{"align":"center"},"id":"n0.9504786860991157"}],"shape":{"data":{"p":{"x":90,"y":254.6290170380177},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9696621953343205":{"id":"de9696621953343205","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.9651143315377548"}],"id":"n0.638304223722447"}],"id":"n0.6627150763848109"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.733350121176997"}],"style":{"align":"center"},"id":"n0.037480843957762966"}],"shape":{"data":{"p":{"x":157.5752569651695,"y":328.3740652373729},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6152157786158032":{"id":"de6152157786158032","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.35880572400619837"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4362084347082764","text":"i"}],"id":"n0.2651270788247402"}],"id":"n0.5355411334500058"}},"id":"n0.2929620259609331"},{"text":"|","id":"n0.2764586619464937"}],"id":"n0.2801977747612696"}],"id":"n0.7073291188234092"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5683464147187822"}],"style":{"align":"center"},"id":"n0.3977797917887649"}],"shape":{"data":{"p":{"x":595,"y":113.41412353515625},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de37492081981477954":{"id":"de37492081981477954","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.06361873532402695"}],"id":"n0.794438943756369"}],"id":"n0.3742890977156048"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.29726610735971226"}],"style":{"align":"center"},"id":"n0.8524771677097138"}],"shape":{"data":{"p":{"x":231.5752569651695,"y":326.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de16483016651040594":{"id":"de16483016651040594","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.3307254272736544"}],"id":"n0.35570128805688106"}],"id":"n0.5843063118814504"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6800433846893965"}],"style":{"align":"center"},"id":"n0.1382199641670081"}],"shape":{"data":{"p":{"x":349.5752569651695,"y":286.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5858435209175927":{"id":"de5858435209175927","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.8630724159830749"}],"id":"n0.10997170062610095"}],"id":"n0.19884001565883946"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6946453596836426"}],"style":{"align":"center"},"id":"n0.5052580844707351"}],"shape":{"data":{"p":{"x":66.5752569651695,"y":191.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de739105016409006":{"id":"de739105016409006","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.8463427624385094"}],"id":"n0.8677445567741551"}],"id":"n0.9523563334968661"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5938522470819092"}],"style":{"align":"center"},"id":"n0.39782059849775453"}],"shape":{"data":{"p":{"x":593.5752569651695,"y":231.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de08038848791315778":{"id":"de08038848791315778","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.5637792325450797"}],"id":"n0.8153682870047718"}],"id":"n0.06429032264958878"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.12068162773028224"}],"style":{"align":"center"},"id":"n0.5359962618215615"}],"shape":{"data":{"p":{"x":469.5752569651695,"y":158.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de05131004919843152":{"id":"de05131004919843152","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.4601600173245559"}],"id":"n0.4702891312583537"}],"id":"n0.951802252792926"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.003195231366954765"}],"style":{"align":"center"},"id":"n0.9309387342842783"}],"shape":{"data":{"p":{"x":532.8988417911593,"y":158.83815680875063},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de540773596056596":{"id":"de540773596056596","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.2238645459187596"}],"id":"n0.272353911420099"}],"id":"n0.15126697453981852"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9917190814756962"}],"style":{"align":"center"},"id":"n0.7553146006612377"}],"shape":{"data":{"p":{"x":424.592468879232,"y":85.20226747242553},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9293029664421679":{"id":"de9293029664421679","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.3570916261199457"},{"id":"n0.12845562270225908","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.978783111912851","lines":[{"id":"n0.9922824075722854","blocks":[{"id":"n0.9781673696109443","text":"j"}]}]}}},{"text":"|","id":"n0.7968331349165683"}],"id":"n0.18387064331058434"}],"id":"n0.3497007107320673"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5747667428587113"}],"style":{"align":"center"},"id":"n0.19820451369007985"}],"shape":{"data":{"p":{"x":306.5752569651695,"y":85.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6039595436159426":{"id":"de6039595436159426","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.351398805520563"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.48442315345149445"}],"id":"n0.22172692899803725"}],"id":"n0.7109090021080886"}},"id":"n0.8245989377973624"},{"text":"|","id":"n0.9453516569619351"}],"id":"n0.8496850694621101"}],"id":"n0.4240221115956506"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9664372514825414"}],"style":{"align":"center"},"id":"n0.711141130846596"}],"shape":{"data":{"p":{"x":81,"y":80.41412353515625},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1822628181115682":{"id":"de1822628181115682","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.009072567688456878"}],"id":"n0.9987810547036093"}],"id":"n0.9056280993433128"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.10645997671208307"}],"style":{"align":"center"},"id":"n0.3764724270291231"}],"shape":{"data":{"p":{"x":157,"y":63.41412353515625},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de023526756442026064":{"id":"de023526756442026064","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.6169616174939561"}],"id":"n0.5542460624761409"}],"id":"n0.09762454449042579"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.09210366129022729"}],"style":{"align":"center"},"id":"n0.6764899055842895"}],"shape":{"data":{"p":{"x":-3.401122429361749,"y":64.14435383370333},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de018726185476633628":{"id":"de018726185476633628","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|×|S|","id":"n0.6493944792796353"}],"id":"n0.31216705932647026"}],"id":"n0.6077529724013804"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3531479305094207"}],"style":{"align":"center"},"id":"n0.60399643863951"}],"shape":{"data":{"p":{"x":146.08394629477812,"y":200.27918469789847},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6841190142781819":{"id":"de6841190142781819","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"T","id":"n0.7683100035109409"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.17581462020855665"}],"id":"n0.7885134808056073"}],"id":"n0.42320818106422853"}},"id":"n0.4859395402433364"},{"type":"single","text":"(","id":"n0.7342047706442416"},{"text":"s,a,s","id":"n0.9242146215609002"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"′","id":"n0.6976639139776573"}],"id":"n0.36649137880757676"}],"id":"n0.9077109131461794"}},"id":"n0.858637279194232"},{"type":"single","text":")","id":"n0.610314329815818"}],"id":"n0.9108959058111366"}],"id":"n0.8756710985439298"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.19642713448145832"}],"style":{"align":"center"},"id":"n0.5922218887012953"}],"shape":{"data":{"p":{"x":201.40112242936175,"y":149.27918469789847},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de04293699428649078":{"id":"de04293699428649078","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.6711516206867614"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.6293012772485833"}],"id":"n0.5099188220776707"}],"id":"n0.9515726342974276"}},"id":"n0.6397086361121886"}],"id":"n0.9016597190644242"}],"id":"n0.966922485547485"}},"id":"n0.7201687800889225"},{"type":"single","text":"(","id":"n0.19871584948867915"},{"text":"s","id":"n0.7082896529787819"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5336131573454217"}],"id":"n0.747649878480164"}],"id":"n0.906764969168768"}},"id":"n0.12002761346059354"},{"text":",a","id":"n0.46186803180346914"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.7591372230431157"}],"id":"n0.036654965525058314"}],"id":"n0.11558220844431832"}},"id":"n0.8274900593397492"},{"text":",s","id":"n0.33558272570819203"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.9182511567605076"}],"id":"n0.6823208742583062"}],"id":"n0.9715224083047242"},"powerValue":{"lines":[{"blocks":[{"text":"′","id":"n0.3099759867848324"}],"id":"n0.07252454170979417"}],"id":"n0.8433207561155169"}},"id":"n0.011563720551354795"},{"type":"single","text":")","id":"n0.14740387727406978"}],"id":"n0.364707453151766"}],"id":"n0.49009001515426154"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.1290575271160015"}],"style":{"align":"center"},"id":"n0.3646082883528139"}],"shape":{"data":{"p":{"x":236.610837007667,"y":90.439940578934},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de60646713842523":{"id":"de60646713842523","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.24591902022735268"}],"id":"n0.4565708745568702"}],"id":"n0.7236458004147461"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\scriptsize"},"id":"n0.5289197316272096"}],"id":"n0.29687791418063103"}],"shape":{"data":{"p":{"x":230.47431307477996,"y":61},"rotation":49.5},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de4411629295441355":{"id":"de4411629295441355","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.16870340820175111"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5279456732104058"}],"id":"n0.12907670911963076"}],"id":"n0.7822700061057228"}},"id":"n0.9377404542125218"}],"id":"n0.6706446933400576"}],"id":"n0.5656938308129515"}},"id":"n0.8013307877816385"},{"type":"single","text":"(","id":"n0.985266238712871"},{"text":"s","id":"n0.8271638019349599"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.06183936664223566"}],"id":"n0.13660785462172242"}],"id":"n0.12229695282215336"}},"id":"n0.6613803536952751"},{"text":",a","id":"n0.6015032396773592"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.46374276792931335"}],"id":"n0.7886303216702921"}],"id":"n0.5157308854738447"}},"id":"n0.22909248342684418"},{"text":",s","id":"n0.06235965186953618"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6566980955979471"}],"id":"n0.40280214465327213"}],"id":"n0.40557309953903786"},"powerValue":{"lines":[{"blocks":[{"text":"′","id":"n0.1289725219965525"}],"id":"n0.9746657310057514"}],"id":"n0.44363044936039064"}},"id":"n0.21824669956570997"},{"type":"single","text":")","id":"n0.07911624592295463"}],"id":"n0.09034195018334379"}],"id":"n0.37394730600376547"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.10719803903126146"}],"style":{"align":"center"},"id":"n0.034145748460466585"}],"shape":{"data":{"p":{"x":372.610837007667,"y":110.439940578934},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7010281499379019":{"id":"de7010281499379019","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.06144083114826682"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.596816246871475"}],"id":"n0.19270499103072902"}],"id":"n0.8765824185576179"}},"id":"n0.8940663977104886"},{"text":"|×|A","id":"n0.4445514206699219"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3255236756072324"}],"id":"n0.5545628363138091"}],"id":"n0.9438628177208579"}},"id":"n0.607005841235837"},{"text":"|×|S","id":"n0.7903939639174105"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.0903889441191188"}],"id":"n0.3812769088406949"}],"id":"n0.3831188775016634"}},"id":"n0.601211045335968"},{"text":"|","id":"n0.7474402100335875"}],"id":"n0.8416491680664595"}],"id":"n0.9767225469188732"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7795950076246325"}],"style":{"align":"center"},"id":"n0.38039104499447296"}],"shape":{"data":{"p":{"x":356.9753875732422,"y":129.96709218025205},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de04664323127911296":{"id":"de04664323127911296","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.49813709848875276"}],"id":"n0.9006780350873496"}],"id":"n0.08373904856088688"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\scriptsize"},"id":"n0.37196203298005615"}],"id":"n0.3491212219072135"}],"shape":{"data":{"p":{"x":366.47431307477996,"y":81},"rotation":49.5},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de16198272348575138":{"id":"de16198272348575138","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.5636079506241669"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.15201140972725113"}],"id":"n0.46390307381875373"}],"id":"n0.3033384222360125"}},"id":"n0.9640682618822976"},{"text":"|×|A","id":"n0.06376856138854725"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.4422875989040669"}],"id":"n0.2998811529747065"}],"id":"n0.9577409964156021"}},"id":"n0.25467665850738963"},{"text":"|×|S","id":"n0.8145614275243673"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8770746409066634"}],"id":"n0.39414625675950643"}],"id":"n0.8650993523594279"}},"id":"n0.8556409230193665"},{"text":"|","id":"n0.3813771503877965"}],"id":"n0.08228083687322618"}],"id":"n0.5587680319929698"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.06469661490070111"}],"style":{"align":"center"},"id":"n0.529015195049134"}],"shape":{"data":{"p":{"x":182.9753875732422,"y":93.96709218025205},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1255655849801256":{"id":"de1255655849801256","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.5775081849637576"}],"id":"n0.21811485831728739"}],"id":"n0.7666737289493661"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.24860653849838377"}],"id":"n0.4062273037250861"}],"shape":{"data":{"p":{"x":246.5171989578646,"y":44.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9161591960896418":{"id":"de9161591960896418","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.6318104962220974"}],"id":"n0.5925370726888699"}],"id":"n0.9498508894605631"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6701633702433445"}],"id":"n0.11559847239060783"}],"shape":{"data":{"p":{"x":242.5171989578646,"y":154.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8296046118428881":{"id":"de8296046118428881","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.6398689401106215"}],"id":"n0.4033876395448901"}],"id":"n0.28320581281574864"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.4349597993383858"}],"id":"n0.9448347503743157"}],"shape":{"data":{"p":{"x":274.398973109876,"y":154.85714149475098},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9797287230713403":{"id":"de9797287230713403","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.9505870200032105"}],"id":"n0.5894585729573776"}],"id":"n0.7671618023231281"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.31054545845421266"}],"id":"n0.5076526454333599"}],"shape":{"data":{"p":{"x":278.398973109876,"y":44.85714149475098},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de5739134075838137":{"id":"de5739134075838137","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.3944069710959337"}],"id":"n0.19451179227559212"}],"id":"n0.4663649957506413"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.10051684038523878"}],"id":"n0.9672525642765821"}],"shape":{"data":{"p":{"x":385.398973109876,"y":44.85714149475098},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de03130277592898212":{"id":"de03130277592898212","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.5534333454181448"}],"id":"n0.3072371727743546"}],"id":"n0.631865547408381"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.1458376395512646"}],"id":"n0.17811759237737768"}],"shape":{"data":{"p":{"x":352.5171989578646,"y":44.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6378018078330772":{"id":"de6378018078330772","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.7208760412987405"}],"id":"n0.2624712398833211"}],"shape":{"data":{"p":{"x":42.0093994140625,"y":86},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8481258525974809":{"id":"de8481258525974809","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.4863560218411527"}],"id":"n0.9159159238454151"}],"shape":{"data":{"p":{"x":42.0093994140625,"y":109},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8476603362025159":{"id":"de8476603362025159","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.4501116586327565"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.17091706834106257"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.025782905093796105"}],"id":"n0.4042546801411979"}],"id":"n0.022720621996522583"}},"id":"n0.22476328518358057"}],"id":"n0.3055198623290718"}],"id":"n0.4989652670930218"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6324025007844765"}],"style":{"align":"center"},"id":"n0.24964510519829197"}],"shape":{"data":{"p":{"x":273.6132065083135,"y":56.495030879974365},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8143133125744644":{"id":"de8143133125744644","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.9086075456708929"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.8370412454432139"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7703327140987262"}],"id":"n0.5389871057488758"}],"id":"n0.7381776497761259"}},"id":"n0.33824744641281645"}],"id":"n0.5481934605797949"}],"id":"n0.8829924132636315"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.36829213278754924"}],"style":{"align":"center"},"id":"n0.6450954768629698"}],"shape":{"data":{"p":{"x":381.6132065083135,"y":56.96521918264051},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3476499031597826":{"id":"de3476499031597826","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.30390839200015485"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.729990596735663"}],"id":"n0.7424364242976345"}],"id":"n0.6780372454725427"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.15414247250504576"}],"style":{"align":"center"},"id":"n0.7413564731553903"}],"shape":{"data":{"p":{"x":269.6132065083135,"y":167.49503087997437},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5306365077124713":{"id":"de5306365077124713","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"optionally dependent","id":"n0.8993394473941201"}],"id":"n0.7761974801344702"}],"shape":{"data":{"p":{"x":-6.990600585937493,"y":145.48763757301705},"rotation":270},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di12183456471916898","items":[],"style":{}},"shapes":[{"id":"dp5580500491360401","type":"doc-cube","data":{"p1":{"x":413.89243309975313,"y":45.5022752722482},"p2":{"x":451.9827880859375,"y":83.21222204612354},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp7412593590357124","type":"doc-cube","data":{"p1":{"x":413.89243309975313,"y":13.199859619140625},"p2":{"x":451.9827880859375,"y":50.90980639301608},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"da19200039013523407","data":[{"x":40.01719895786459,"y":57.34437565321065},{"x":51.206092622831534,"y":57.34437565321065}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp0239657809852718","type":"doc-cube","data":{"p1":{"x":1.5988775706382512,"y":37.84193818059583},"p2":{"x":39.68923255682262,"y":75.55188495447129},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp7194803427767733","type":"doc-cube","data":{"p1":{"x":83.17413453580775,"y":51.42721209483358},"p2":{"x":121.26448952199212,"y":89.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp8282129066226385","type":"doc-cube","data":{"p1":{"x":83.17413453580775,"y":19.42721209483358},"p2":{"x":121.26448952199212,"y":57.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da853407251837732","data":[{"x":121.26448952199212,"y":57.13715886870904},{"x":133.1304054661781,"y":57.13715886870904}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da8231681129714354","data":[{"x":152.66612152300183,"y":56.729627747941095},{"x":163.74979117488306,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp2827788892463312","type":"circle","data":{"p1":{"x":133.1304054661781,"y":47.30450264897962},"p2":{"x":152.66612152300183,"y":66.84021870580335}}},{"id":"dp532548436215186","type":"doc-cube","data":{"p1":{"x":163.59887757063825,"y":38.84193818059583},"p2":{"x":201.68923255682262,"y":76.55188495447129},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da308102308085787","data":[{"x":202.0093994140625,"y":56.729627747941095},{"x":248.7314323563021,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da6021732396444412","data":[{"x":297.14892256513724,"y":56.729627747941095},{"x":306.7314323563021,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4489210612652541","data":[{"x":404.14892256513724,"y":56.215249700218635},{"x":414.60827698470075,"y":56.215249700218635}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp5238821890873124","type":"doc-cube","data":{"p1":{"x":424.592468879232,"y":55.89985181931803},"p2":{"x":462.68282386541637,"y":93.60979859319349},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp7110419585223715","type":"doc-cube","data":{"p1":{"x":424.592468879232,"y":23.89985181931803},"p2":{"x":462.68282386541637,"y":61.60979859319349},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dg9204957316369451","entities":[{"id":"dp10499838332590139","type":"circle","data":{"p1":{"x":575.3800116578016,"y":188.44739167180677},"p2":{"x":594.9157277146253,"y":207.9831077286305}}},{"id":"dl1391479758821974","linkedId":"de6584387665735523"}]},{"id":"da2979160721047991","data":[{"x":509.2671484131258,"y":198.21524970021864},{"x":575.3800116578016,"y":198.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da27089434828529035","data":[{"x":585.1478696862134,"y":55.96521918264051},{"x":585.1478696862134,"y":188.44739167180677}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp6621931347037233","type":"doc-cube","data":{"p1":{"x":606.9096450138156,"y":198.12821003487528},"p2":{"x":645,"y":235.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp5776503678584604","type":"doc-cube","data":{"p1":{"x":606.9096450138156,"y":165.8257943817677},"p2":{"x":645,"y":203.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp22224605199990788","type":"doc-cube","data":{"p1":{"x":617.592468879232,"y":208.89985181931803},"p2":{"x":655.6828238654164,"y":246.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp8386984456762969","type":"doc-cube","data":{"p1":{"x":617.592468879232,"y":176.89985181931803},"p2":{"x":655.6828238654164,"y":214.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp5226002240201779","type":"doc-cube","data":{"p1":{"x":467.4913106703914,"y":119.12821003487528},"p2":{"x":505.58166565657575,"y":156.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp3137025663850519","type":"doc-cube","data":{"p1":{"x":467.4913106703914,"y":86.82579438176771},"p2":{"x":505.58166565657575,"y":124.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp6642259953317995","type":"doc-cube","data":{"p1":{"x":478.17413453580775,"y":129.42721209483358},"p2":{"x":516.2644895219921,"y":167.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp41047603791401865","type":"doc-cube","data":{"p1":{"x":478.17413453580775,"y":97.42721209483358},"p2":{"x":516.2644895219921,"y":135.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp2404545538889784","type":"doc-cube","data":{"p1":{"x":525.4913106703914,"y":119.12821003487528},"p2":{"x":563.5816656565758,"y":156.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp6064438594718595","type":"doc-cube","data":{"p1":{"x":525.4913106703914,"y":86.82579438176771},"p2":{"x":563.5816656565758,"y":124.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp5149951155315287","type":"doc-cube","data":{"p1":{"x":536.1741345358078,"y":129.89985181931803},"p2":{"x":574.2644895219921,"y":167.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp3108225276141863","type":"doc-cube","data":{"p1":{"x":536.1741345358078,"y":97.89985181931803},"p2":{"x":574.2644895219921,"y":135.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dg15563367846213083","entities":[{"id":"dp21043865271157292","type":"circle","data":{"p1":{"x":184.7314323563021,"y":235.19736115422864},"p2":{"x":204.26714841312582,"y":254.73307721105238}}},{"id":"dl12406206773144723","linkedId":"de8954529408852401"}]},{"id":"da5150116280603851","data":[{"x":462.60827698470075,"y":56.215249700218635},{"x":537.7314323563021,"y":56.215249700218635}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg954465914639369","entities":[{"id":"dp12510303758397479","type":"circle","data":{"p1":{"x":537.7314323563021,"y":46.197361154228645},"p2":{"x":557.2671484131258,"y":65.73307721105238}}},{"id":"dl6457629730029077","linkedId":"de9760449880962501"}]},{"id":"da6958538552085018","data":[{"x":547.499290384714,"y":65.73307721105238},{"x":547.499290384714,"y":86.21600341796875}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da7778825022864237","data":[{"x":404.0093994140625,"y":245.21524970021864},{"x":585.1478696862134,"y":245.21524970021864}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg41545057312416156","entities":[{"id":"dg8271149987198114","entities":[{"id":"dp31161403196624216","type":"rectangle","data":{"p1":{"x":8.99359130859375,"y":1.5402473973582005},"p2":{"x":21.650752040652606,"y":14.197408129417056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp6085656917177373","type":"rectangle","data":{"p1":{"x":10.57573640010105,"y":3.1223924888655574},"p2":{"x":23.232897132159906,"y":15.779553220924413}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp41813287093409257","type":"rectangle","data":{"p1":{"x":12.157881491608464,"y":4.704537580372914},"p2":{"x":24.81504222366732,"y":17.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl8322524008366461","linkedId":"de6035267197891458"}]},{"id":"dp942503727628808","type":"doc-cube","data":{"p1":{"x":306.5752569651695,"y":56.801277332206496},"p2":{"x":344.66561195135387,"y":94.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp8281586097067699","type":"doc-cube","data":{"p1":{"x":306.5752569651695,"y":24.801277332206496},"p2":{"x":344.66561195135387,"y":62.511224106081954},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da03822030711492408","data":[{"x":345.2671484131258,"y":56.96521918264051},{"x":355.0093994140625,"y":56.96521918264051}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da059191563599135355","data":[{"x":70.0093994140625,"y":57.13715886870904},{"x":83.0093994140625,"y":57.13715886870904}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da13306965166562712","data":[{"x":557.2671484131258,"y":55.96521918264051},{"x":585.1478696862134,"y":55.96521918264051}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg7539883759791381","entities":[{"id":"dp7497877315179022","type":"circle","data":{"p1":{"x":489.7314323563021,"y":188.19736115422864},"p2":{"x":509.2671484131258,"y":207.73307721105238}}},{"id":"dl6687676709899761","linkedId":"de26192952769719957"}]},{"id":"da9415792104793081","data":[{"x":499.49929038471396,"y":167.31321716308594},{"x":499.49929038471396,"y":189.19736115422864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp38660432328521854","type":"doc-cube","data":{"p1":{"x":304.89243309975313,"y":163.5022752722482},"p2":{"x":342.9827880859375,"y":201.21222204612354},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp7338164304551018","type":"doc-cube","data":{"p1":{"x":304.89243309975313,"y":131.19985961914062},"p2":{"x":342.9827880859375,"y":168.90980639301608},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp39348646886366523","type":"doc-cube","data":{"p1":{"x":315.592468879232,"y":173.89985181931803},"p2":{"x":353.68282386541637,"y":211.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp590233598124545","type":"doc-cube","data":{"p1":{"x":315.592468879232,"y":141.89985181931803},"p2":{"x":353.68282386541637,"y":179.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da05971979951523476","data":[{"x":293.14892256513724,"y":166.5022752722482},{"x":304.89243309975313,"y":166.5022752722482}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da42104124445416335","data":[{"x":375.0093994140625,"y":197.9652191826405},{"x":489.7314323563021,"y":197.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da8186217197536731","data":[{"x":354.0093994140625,"y":166.5022752722482},{"x":375.0093994140625,"y":166.5022752722482}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da05615183153668801","data":[{"x":375.0093994140625,"y":166.5022752722482},{"x":375.0093994140625,"y":197.9652191826405}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da673169699290058","data":[{"x":29.563405007743967,"y":160.9336164882478},{"x":41.42493473559304,"y":160.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da5645555795798565","data":[{"x":29.563405007743967,"y":244.9336164882478},{"x":46.42493473559304,"y":244.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da8738004703581135","data":[{"x":82.42493473559304,"y":244.9336164882478},{"x":99.0093994140625,"y":244.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da10460833736657693","data":[{"x":76.42493473559304,"y":160.9336164882478},{"x":87.0093994140625,"y":160.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"dp7869297321934083","type":"doc-cube","data":{"p1":{"x":85.90964501381563,"y":161.12821003487528},"p2":{"x":124,"y":198.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp13484715726844398","type":"doc-cube","data":{"p1":{"x":85.90964501381563,"y":128.8257943817677},"p2":{"x":124,"y":166.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp12477969564605385","type":"doc-cube","data":{"p1":{"x":96.592468879232,"y":171.89985181931803},"p2":{"x":134.68282386541637,"y":209.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp7903226572786035","type":"doc-cube","data":{"p1":{"x":96.592468879232,"y":139.89985181931803},"p2":{"x":134.68282386541637,"y":177.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp031755431326810024","type":"doc-cube","data":{"p1":{"x":176.49131067039139,"y":298.1282100348753},"p2":{"x":214.58166565657575,"y":335.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp3584813595344112","type":"doc-cube","data":{"p1":{"x":176.49131067039139,"y":265.8257943817677},"p2":{"x":214.58166565657575,"y":303.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp007099428310750833","type":"doc-cube","data":{"p1":{"x":187.17413453580775,"y":308.4272120948336},"p2":{"x":225.26448952199212,"y":346.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp22821526251270785","type":"doc-cube","data":{"p1":{"x":187.17413453580775,"y":276.4272120948336},"p2":{"x":225.26448952199212,"y":314.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp7185805497173068","type":"doc-cube","data":{"p1":{"x":249.49131067039139,"y":296.1282100348753},"p2":{"x":287.58166565657575,"y":333.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp018846218146621796","type":"doc-cube","data":{"p1":{"x":249.49131067039139,"y":263.8257943817677},"p2":{"x":287.58166565657575,"y":301.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp5690368574792177","type":"doc-cube","data":{"p1":{"x":260.17413453580775,"y":306.89985181931803},"p2":{"x":298.2644895219921,"y":344.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp38381778786212895","type":"doc-cube","data":{"p1":{"x":260.17413453580775,"y":274.89985181931803},"p2":{"x":298.2644895219921,"y":312.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da5658381447269285","data":[{"x":135.0093994140625,"y":244.9652191826405},{"x":184.7314323563021,"y":244.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da9995455804626399","data":[{"x":194.49929038471396,"y":254.73307721105238},{"x":194.49929038471396,"y":264.94285583496094}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da8640106553630609","data":[{"x":120.0093994140625,"y":209.5022752722482},{"x":120.0093994140625,"y":221.94285583496094}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da18632054957436273","data":[{"x":120.0093994140625,"y":221.94285583496094},{"x":255.7314323563021,"y":221.94285583496094}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"dg8055008932284284","entities":[{"id":"dp03367387182029269","type":"circle","data":{"p1":{"x":255.7314323563021,"y":212.19736115422864},"p2":{"x":275.2671484131258,"y":231.73307721105238}}},{"id":"dl20198523491621545","linkedId":"de4331374139554627"}]},{"id":"da8012264691401934","data":[{"x":265.49929038471396,"y":231.73307721105238},{"x":265.49929038471396,"y":264.21600341796875}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da7835806906210396","data":[{"x":204.26714841312582,"y":244.9652191826405},{"x":279.0093994140625,"y":244.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg7875487562730157","entities":[{"id":"dp578508923349293","type":"circle","data":{"p1":{"x":279.38001165780156,"y":235.44739167180677},"p2":{"x":298.9157277146253,"y":254.9831077286305}}},{"id":"dl1612850971509283","linkedId":"de8948224066984556"}]},{"id":"da9579582551601642","data":[{"x":289.1478696862134,"y":221.9652191826405},{"x":289.1478696862134,"y":235.44739167180677}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da59415295926599","data":[{"x":275.2671484131258,"y":221.9652191826405},{"x":289.1478696862134,"y":221.9652191826405}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp8939365025742361","type":"doc-cube","data":{"p1":{"x":354.90964501381563,"y":246.12821003487528},"p2":{"x":393,"y":283.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp048707061335577784","type":"doc-cube","data":{"p1":{"x":354.90964501381563,"y":213.8257943817677},"p2":{"x":393,"y":251.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp23688862660102084","type":"doc-cube","data":{"p1":{"x":365.592468879232,"y":256.89985181931803},"p2":{"x":403.68282386541637,"y":294.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp23160303178682695","type":"doc-cube","data":{"p1":{"x":365.592468879232,"y":224.89985181931803},"p2":{"x":403.68282386541637,"y":262.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da3866850608376675","data":[{"x":585.1478696862134,"y":207.9831077286305},{"x":585.1478696862134,"y":245.21524970021864}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da9337052957580414","data":[{"x":594.9157277146253,"y":198.21524970021864},{"x":606.9096450138156,"y":198.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp0349412583949118","type":"doc-cube","data":{"p1":{"x":608.1741345358078,"y":85.42721209483358},"p2":{"x":646.2644895219921,"y":123.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp9379059187709777","type":"doc-cube","data":{"p1":{"x":608.1741345358078,"y":53.42721209483358},"p2":{"x":646.2644895219921,"y":91.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da5343953893264877","data":[{"x":60.49929038471396,"y":8.21600341796875},{"x":60.49929038471396,"y":52.197361154228645}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9677469206122253","data":[{"x":24.81504222366732,"y":8.704537580372914},{"x":597.0093994140625,"y":8.704537580372914}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg6752644909371888","entities":[{"id":"dp43033051061531813","type":"circle","data":{"p1":{"x":617.7314323563021,"y":134.19736115422864},"p2":{"x":637.2671484131258,"y":153.73307721105238}}},{"id":"dl377456144583618","linkedId":"de4462760249275344"}]},{"id":"da17224206150215826","data":[{"x":627.499290384714,"y":153.73307721105238},{"x":627.499290384714,"y":165.94285583496094}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da9982300639182866","data":[{"x":627.499290384714,"y":123.21600341796875},{"x":627.499290384714,"y":134.19736115422864}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da7416010416599621","data":[{"x":597.0093994140625,"y":143.9652191826405},{"x":617.7314323563021,"y":143.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9022639564636132","data":[{"x":597.0093994140625,"y":8.704537580372914},{"x":597.0093994140625,"y":143.9652191826405}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp6501577681335067","type":"rectangle","data":{"p1":{"x":1.5361824061229754,"y":228.57503948597804},"p2":{"x":30.858642252069075,"y":257.8974993319241}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp6877052913645814","type":"rectangle","data":{"p1":{"x":1.5361824061229754,"y":145.57503948597804},"p2":{"x":30.858642252069075,"y":174.8974993319241}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"da4090530237206933","data":[{"x":16.49929038471396,"y":174.31321716308594},{"x":16.49929038471396,"y":228.21600341796875}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg6734392125901896","entities":[{"id":"dp2789239062719051","type":"rectangle","data":{"p1":{"x":48.0093994140625,"y":143},"p2":{"x":69.0093994140625,"y":178},"rotation":90}},{"id":"dl3628216806984257","linkedId":"de6435602377123977"}]},{"id":"dg22534662588403087","entities":[{"id":"dp13538335494399356","type":"rectangle","data":{"p1":{"x":54.0093994140625,"y":227},"p2":{"x":75.0093994140625,"y":262},"rotation":90}},{"id":"dl755351049022529","linkedId":"de9996999739406618"}]},{"id":"dg24449934841418952","entities":[{"id":"dp15533761819139724","type":"rectangle","data":{"p1":{"x":99.54648398243944,"y":227.63370702366495},"p2":{"x":128.9300421516284,"y":257.00945182101134}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp4643139166564427","type":"rectangle","data":{"p1":{"x":102.58616261365637,"y":230.67257737498306},"p2":{"x":131.96972078284546,"y":260.04832217232934}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp49163915811603554","type":"rectangle","data":{"p1":{"x":105.62584124487336,"y":233.71144772630112},"p2":{"x":135.0093994140625,"y":263.08719252364745}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{}},{"id":"da7872979366862605","data":[{"x":298.9157277146253,"y":245.21524970021864},{"x":354.0093994140625,"y":245.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp09732505074373066","type":"doc-cube","data":{"p1":{"x":184.31076744317738,"y":161.10001179268778},"p2":{"x":222.40112242936175,"y":198.80995856656313},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp18274731608286587","type":"doc-cube","data":{"p1":{"x":184.31076744317738,"y":128.7975961395802},"p2":{"x":222.40112242936175,"y":166.50754291345567},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp12130929956941183","type":"doc-cube","data":{"p1":{"x":194.99359130859375,"y":171.87165357713053},"p2":{"x":233.08394629477812,"y":209.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp028256799555335776","type":"doc-cube","data":{"p1":{"x":194.99359130859375,"y":139.87165357713053},"p2":{"x":233.08394629477812,"y":177.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5171751511814839","type":"doc-cube","data":{"p1":{"x":152.20960923433677,"y":161.10001179268778},"p2":{"x":190.29996422052113,"y":198.80995856656313},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp5608329832553007","type":"doc-cube","data":{"p1":{"x":152.20960923433677,"y":128.7975961395802},"p2":{"x":190.29996422052113,"y":166.50754291345567},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp7156234666550425","type":"doc-cube","data":{"p1":{"x":162.89243309975313,"y":171.87165357713053},"p2":{"x":200.9827880859375,"y":209.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp15378440916480773","type":"doc-cube","data":{"p1":{"x":162.89243309975313,"y":139.87165357713053},"p2":{"x":200.9827880859375,"y":177.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dg08929290825571146","entities":[{"id":"dp8942136593530361","type":"rectangle","data":{"p1":{"x":215.81933178116822,"y":67.40107022761589},"p2":{"x":247.89927876415908,"y":96.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp7590754257443322","type":"rectangle","data":{"p1":{"x":219.13794720457258,"y":70.439940578934},"p2":{"x":251.21789418756362,"y":99.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp6292476093797723","type":"rectangle","data":{"p1":{"x":222.456562627977,"y":73.47881093025205},"p2":{"x":254.5365096109681,"y":102.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"dg7711569844652904","entities":[{"id":"dp4908467651489763","type":"rectangle","data":{"p1":{"x":233.29222158426262,"y":83.40107022761589},"p2":{"x":266.20073998648286,"y":112.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp798959070951937","type":"rectangle","data":{"p1":{"x":236.69655129805233,"y":86.439940578934},"p2":{"x":269.6050697002727,"y":115.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp02317091301376495","type":"rectangle","data":{"p1":{"x":240.10088101184203,"y":89.47881093025205},"p2":{"x":273.0093994140625,"y":118.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{}},{"id":"dg19964813928951308","entities":[{"id":"dp034934788017860985","type":"rectangle","data":{"p1":{"x":351.8193317811682,"y":87.40107022761589},"p2":{"x":383.89927876415913,"y":116.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp900240286070412","type":"rectangle","data":{"p1":{"x":355.1379472045726,"y":90.439940578934},"p2":{"x":387.2178941875636,"y":119.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp3947392159799368","type":"rectangle","data":{"p1":{"x":358.45656262797706,"y":93.47881093025205},"p2":{"x":390.5365096109681,"y":122.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"dg19029399184522622","entities":[{"id":"dp4240042237526809","type":"rectangle","data":{"p1":{"x":369.2922215842626,"y":103.40107022761589},"p2":{"x":402.20073998648286,"y":132.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp24142162592296623","type":"rectangle","data":{"p1":{"x":372.6965512980523,"y":106.439940578934},"p2":{"x":405.6050697002727,"y":135.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp5443187775637572","type":"rectangle","data":{"p1":{"x":376.10088101184203,"y":109.47881093025205},"p2":{"x":409.0093994140625,"y":138.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{}},{"id":"da637809167456008","data":[{"x":258.49929038471396,"y":66.73307721105238},{"x":258.49929038471396,"y":83.21600341796875}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"dg006391677294819154","entities":[{"id":"dp7771922235587243","type":"circle","data":{"p1":{"x":248.7314323563021,"y":47.197361154228645},"p2":{"x":268.2671484131258,"y":66.73307721105238}}},{"id":"dl389019327591694","linkedId":"de1255655849801256"}]},{"id":"da5209013767862236","data":[{"x":16.49929038471396,"y":100.77681502496227},{"x":16.49929038471396,"y":145.31321716308594}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da7917530330246885","data":[{"x":76.0093994140625,"y":100.77681502496227},{"x":217.81933178116822,"y":100.77681502496227}],"head":"fh>","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da38135419526097825","data":[{"x":76.0093994140625,"y":122.77681502496227},{"x":358.45656262797706,"y":122.77681502496227}],"head":"fh>","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da09903958236513599","data":[{"x":183.4779265063455,"y":76.24041288683861},{"x":183.4779265063455,"y":117.21600341796875}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4673472459214669","data":[{"x":183.4779265063455,"y":117.21600341796875},{"x":236.0093994140625,"y":117.21600341796875}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da3357191226606715","data":[{"x":236.0093994140625,"y":117.21600341796875},{"x":236.0093994140625,"y":137.21600341796875}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da7674599403021374","data":[{"x":236.0093994140625,"y":137.21600341796875},{"x":254.49929038471396,"y":137.21600341796875}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg3111258413323337","entities":[{"id":"dp527895228022196","type":"circle","data":{"p1":{"x":244.7314323563021,"y":157.19736115422864},"p2":{"x":264.2671484131258,"y":176.73307721105238}}},{"id":"dl34043414874577427","linkedId":"de9161591960896418"}]},{"id":"dg6145165827194954","entities":[{"id":"dp261344319135447","type":"circle","data":{"p1":{"x":273.6132065083135,"y":156.67856788635257},"p2":{"x":293.14892256513724,"y":176.2142839431763}}},{"id":"dl21460496321325784","linkedId":"de8296046118428881"}],"data":{"rotation":0}},{"id":"da6657225238385869","data":[{"x":232.9879218216862,"y":166.9652191826405},{"x":244.7314323563021,"y":166.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da36307604254714243","data":[{"x":264.2671484131258,"y":166.9652191826405},{"x":273.6132065083135,"y":166.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da07983334347477489","data":[{"x":254.49929038471396,"y":137.21600341796875},{"x":254.49929038471396,"y":157.19736115422864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da2811500562982141","data":[{"x":140.49929038471396,"y":122.77681502496227},{"x":140.49929038471396,"y":167.31321716308594}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da35308780946559915","data":[{"x":140.49929038471396,"y":167.31321716308594},{"x":152.0093994140625,"y":167.31321716308594}],"head":"fh>","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"dg6474901284015173","entities":[{"id":"dp23763267875478333","type":"circle","data":{"p1":{"x":277.6132065083135,"y":46.67856788635257},"p2":{"x":297.14892256513724,"y":66.2142839431763}}},{"id":"dl023538663551297745","linkedId":"de9797287230713403"}],"data":{"rotation":0}},{"id":"da38022140950114736","data":[{"x":268.2671484131258,"y":56.96521918264051},{"x":277.6132065083135,"y":56.96521918264051}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg27597926385049165","entities":[{"id":"dp10151926770216746","type":"circle","data":{"p1":{"x":354.7314323563021,"y":47.197361154228645},"p2":{"x":374.2671484131258,"y":66.73307721105238}}},{"id":"dl7669813038971061","linkedId":"de03130277592898212"}]},{"id":"dg5771720689263735","entities":[{"id":"dp3859604845475457","type":"circle","data":{"p1":{"x":384.6132065083135,"y":46.67856788635257},"p2":{"x":404.14892256513724,"y":66.2142839431763}}},{"id":"dl6079264183911899","linkedId":"de5739134075838137"}],"data":{"rotation":0}},{"id":"da3886363031679785","data":[{"x":374.2671484131258,"y":56.96521918264051},{"x":384.6132065083135,"y":56.96521918264051}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg12964984834139792","entities":[{"id":"dp5857498755316624","type":"rectangle","data":{"p1":{"x":48.0093994140625,"y":83},"p2":{"x":69.0093994140625,"y":118},"rotation":90}},{"id":"dl7825586801032587","linkedId":"de6378018078330772"}]},{"id":"dg8834776660883104","entities":[{"id":"dp3330655612344646","type":"rectangle","data":{"p1":{"x":48.0093994140625,"y":106},"p2":{"x":69.0093994140625,"y":141},"rotation":90}},{"id":"dl4102774702186407","linkedId":"de8481258525974809"}]},{"id":"da8265208003206985","data":[{"x":16.49929038471396,"y":100.77681502496227},{"x":41.0093994140625,"y":100.77681502496227}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da60878731726692","data":[{"x":16.49929038471396,"y":122.77681502496227},{"x":41.0093994140625,"y":122.77681502496227}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da034831188233359844","data":[{"x":364.49929038471396,"y":66.73307721105238},{"x":364.49929038471396,"y":87.21600341796875}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}}],"settings":{"grid":true,"diagramHeight":347.94146728515625}}]},{"id":"n0.3042139671924857","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":1347,"delayRenderCache":{"av":1347,"map":{"n0.10534765439253158":{"n0.19818936353891803":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.5201323123537056":{"n0.8261875009076476":{"w":28.1756,"h":8.4545,"bl":0.8214}},"n0.6627150763848109":{"n0.638304223722447":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.7073291188234092":{"n0.2801977747612696":{"w":26.2496,"h":8.4545,"bl":0.8214}},"n0.3742890977156048":{"n0.794438943756369":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.5843063118814504":{"n0.35570128805688106":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.19884001565883946":{"n0.10997170062610095":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.9523563334968661":{"n0.8677445567741551":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.89449632340263":{"n0.9283375581593811":{"w":15.625,"h":9.1146,"bl":0.7619}},"n0.5585144594769098":{"n0.8011604082776529":{"w":24.2151,"h":9.4491,"bl":0.8402}},"n0.03458318572511776":{"n0.0860315124689226":{"w":29.6766,"h":9.1146,"bl":0.7619}},"n0.6358514931961325":{"n0.9225802517691526":{"w":7.0349,"h":8.4545,"bl":0.8214}},"n0.5587516503235763":{"n0.6037200504114792":{"w":21.6743,"h":9.1146,"bl":0.7619}},"n0.7264028620765699":{"n0.8042656885336161":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.04583797116036181":{"n0.49246669600141635":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.5175725534760129":{"n0.25330121363332925":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.8764715381876009":{"n0.5159037234950323":{"w":20.7972,"h":9.9736,"bl":0.6963}},"n0.7324353081628885":{"n0.3821079040693218":{"w":24.6672,"h":9.1146,"bl":0.7619}},"n0.7820935964803029":{"n0.8353405095841582":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.43208464797421753":{"n0.8957631635704928":{"w":19.694,"h":8.4545,"bl":0.8214}},"n0.2601044691611345":{"n0.16188097070730345":{"w":23.9981,"h":9.9736,"bl":0.6963}},"n0.1395073386628325":{"n0.14935564515850985":{"w":20.9871,"h":9.9736,"bl":0.6963}},"n0.8840114401506087":{"n0.8304290040433637":{"w":19.694,"h":8.4545,"bl":0.8214}},"n0.6997469764205988":{"n0.14721663159612897":{"w":24.4231,"h":9.1146,"bl":0.7619}},"n0.976576704540332":{"n0.6768200944743077":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.06429032264958878":{"n0.8153682870047718":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.951802252792926":{"n0.4702891312583537":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.15126697453981852":{"n0.272353911420099":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.3497007107320673":{"n0.18387064331058434":{"w":26.4938,"h":8.4545,"bl":0.8214}},"n0.4240221115956506":{"n0.8496850694621101":{"w":26.2496,"h":8.4545,"bl":0.8214}},"n0.8756710985439298":{"n0.9108959058111366":{"w":28.9804,"h":11.348,"bl":0.6717}},"n0.9767225469188732":{"n0.8416491680664595":{"w":45.2293,"h":8.4545,"bl":0.8214}},"n0.5587680319929698":{"n0.08228083687322618":{"w":45.9617,"h":8.4545,"bl":0.8214}},"n0.49009001515426154":{"n0.364707453151766":{"w":34.2972,"h":12.6682,"bl":0.6267}},"n0.37394730600376547":{"n0.09034195018334379":{"w":33.5015,"h":12.6682,"bl":0.6267}},"n0.6077529724013804":{"n0.31216705932647026":{"w":39.4513,"h":8.1019,"bl":0.8571}},"n0.4989652670930218":{"n0.3055198623290718":{"w":5.9498,"h":8.4545,"bl":0.8214}},"n0.8829924132636315":{"n0.5481934605797949":{"w":5.7057,"h":8.4545,"bl":0.8214}}}}}

==> plots/docs/59fdd8c4-a9f1-485d-b49e-4c7bfbd03d27 <==
{"id":"n0.7456383844689902","lines":[{"id":"n0.8763064465791919","blocks":[]},{"id":"n0.44711846644901","blocks":[{"id":"n0.9288385843406479","text":"\\diagram","type":"composite","elements":{"de7404139643581418":{"id":"de7404139643581418","lines":[{"blocks":[{"text":"Value iteration solver","style":{"fontSize":"\\tiny"},"id":"n0.19770521534247454"}],"style":{"align":"center"},"id":"n0.0030156944848367395"}],"shape":{"data":{"p":{"x":234.49359130859375,"y":16.635022970635077},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de949941888849803":{"id":"de949941888849803","lines":[{"blocks":[{"text":"Value iteration solver","style":{"fontSize":"\\tiny"},"id":"n0.4593913524176294"}],"style":{"align":"center"},"id":"n0.443496815967684"}],"shape":{"data":{"p":{"x":234.49359130859375,"y":104.63502297063508},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de32130721406148366":{"id":"de32130721406148366","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.8797025232152835"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"L-2,K","id":"n0.7574525922899173"}],"id":"n0.6792864006937782"}],"id":"n0.4871679788236192"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3983774231491659"}],"id":"n0.17604683573999136"}],"id":"n0.7520448645232582"}},"id":"n0.6169344591193611"},{"type":"single","text":"(","id":"n0.247693808610445"},{"text":"s,a","id":"n0.4968446333492895"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6906023085940054"}],"id":"n0.33010937497493464"}],"id":"n0.1641173131260556"}},"id":"n0.7238556114449535"},{"type":"single","text":")","id":"n0.982544451005702"}],"id":"n0.8091899817257213"}],"id":"n0.49121514402082456"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.22186047312577228"}],"style":{"align":"center"},"id":"n0.797204439117494"}],"shape":{"data":{"p":{"x":332.4011224293617,"y":97.72752972042764},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de9910374172859537":{"id":"de9910374172859537","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.005737793719555517"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8383320490845296"}],"id":"n0.7977828385970613"}],"id":"n0.8416031365428731"}},"id":"n0.8044300209222583"},{"text":"|","id":"n0.30338364897354686"}],"id":"n0.6479673560913659"}],"id":"n0.878034595656866"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.009638223477540953"}],"style":{"align":"center"},"id":"n0.04633807084968611"}],"shape":{"data":{"p":{"x":298.99359130859375,"y":141.42014678034167},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9448075050931994":{"id":"de9448075050931994","lines":[{"blocks":[{"text":"Softmax","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.3881871005493689"}],"style":{"align":"center"},"id":"n0.9932399499088576"}],"shape":{"data":{"p":{"x":399.9827880859375,"y":105.47110766449265},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7963858066415856":{"id":"de7963858066415856","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.3905984278663106"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"L-1,K","id":"n0.7986457472156983"}],"id":"n0.5996773595196319"}],"id":"n0.5085266219885212"},"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.3863209742516749"}],"id":"n0.6152400257446515"}],"id":"n0.0400742394500917"}},"id":"n0.5473655481704303"},{"type":"single","text":"(","id":"n0.19500742768663515"},{"text":"s,a","id":"n0.21247214621856103"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.7358306889430006"}],"id":"n0.5656120957983657"}],"id":"n0.9216699336648997"}},"id":"n0.8566877677939349"},{"type":"single","text":")","id":"n0.15889176983574416"}],"id":"n0.624454071858985"}],"id":"n0.5762378149466976"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5245830463600181"}],"style":{"align":"center"},"id":"n0.0717754399241497"}],"shape":{"data":{"p":{"x":332.4011224293617,"y":9.72752972042764},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de030313905425286558":{"id":"de030313905425286558","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.2240811407333707"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.0676601920612836"}],"id":"n0.13277312603126212"}],"id":"n0.7545877627634885"}},"id":"n0.04813229485411008"},{"text":"|","id":"n0.5427307784547795"}],"id":"n0.564695130185312"}],"id":"n0.7620427428820304"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6477223589534982"}],"style":{"align":"center"},"id":"n0.42293417942939726"}],"shape":{"data":{"p":{"x":298.99359130859375,"y":53.42014678034167},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5663753911346638":{"id":"de5663753911346638","lines":[{"blocks":[{"text":"Softmax","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.6609290096212981"}],"style":{"align":"center"},"id":"n0.3977909836140512"}],"shape":{"data":{"p":{"x":399.9827880859375,"y":17.47110766449265},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de0550914994150582":{"id":"de0550914994150582","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.5140039025205387"}],"id":"n0.3709058944946262"}],"id":"n0.47706945579402205"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9035451130987506"}],"id":"n0.38722324292532817"}],"shape":{"data":{"p":{"x":285.5,"y":174.54608154296875},"rotation":90},"anchor":"left-top"},"isTextMode":true},"de9740250816234686":{"id":"de9740250816234686","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.4016400439397185"}],"id":"n0.3934814190940734"}],"id":"n0.5457109854785729"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7604199860398932"}],"id":"n0.5009673578426002"}],"shape":{"data":{"p":{"x":363.5,"y":174.54608154296875},"rotation":90},"anchor":"left-top"},"isTextMode":true},"de9385566531380667":{"id":"de9385566531380667","lines":[{"blocks":[{"text":"Value iteration solver","style":{"fontSize":"\\tiny"},"id":"n0.7217592392524406"}],"style":{"align":"center"},"id":"n0.7213343873567817"}],"shape":{"data":{"p":{"x":235.49359130859375,"y":242.63502297063508},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9230782278135958":{"id":"de9230782278135958","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.1380841457076989"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"0,K","id":"n0.5116599012581777"}],"id":"n0.07456673727038288"}],"id":"n0.742823387835992"},"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5193821290096721"}],"id":"n0.04841632932536677"}],"id":"n0.9650646770652205"}},"id":"n0.9039984150883122"},{"type":"single","text":"(","id":"n0.8842144191413104"},{"text":"s,a","id":"n0.822359185523424"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.05419841640105538"}],"id":"n0.4594820213704369"}],"id":"n0.5705112118491114"}},"id":"n0.6090589366914465"},{"type":"single","text":")","id":"n0.26344848149904343"}],"id":"n0.16312157425304696"}],"id":"n0.5421621652642399"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.11454114241444535"}],"style":{"align":"center"},"id":"n0.034864380703128584"}],"shape":{"data":{"p":{"x":335.4011224293617,"y":235.72752972042764},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de13776807857324536":{"id":"de13776807857324536","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.9813758713228182"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.25818223492049186"}],"id":"n0.08476983469556298"}],"id":"n0.5732016289079991"}},"id":"n0.7340773131771539"},{"text":"|","id":"n0.7212270463159804"}],"id":"n0.4521066476362081"}],"id":"n0.021551824456943036"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7877763209738127"}],"style":{"align":"center"},"id":"n0.047020047972589296"}],"shape":{"data":{"p":{"x":300.99359130859375,"y":279.42014678034167},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9826326892666628":{"id":"de9826326892666628","lines":[{"blocks":[{"text":"Softmax","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.3123466420650318"}],"style":{"align":"center"},"id":"n0.8430356477283305"}],"shape":{"data":{"p":{"x":397.9827880859375,"y":243.47110766449265},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6123916227603201":{"id":"de6123916227603201","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.7284304063632188"}],"id":"n0.9893739898342253"}],"id":"n0.09492127571336417"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6928984319873144"}],"id":"n0.16728586144452362"}],"shape":{"data":{"p":{"x":434.5,"y":174.54608154296875},"rotation":90},"anchor":"left-top"},"isTextMode":true},"de39438104803862406":{"id":"de39438104803862406","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\hat","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"𝜋","id":"n0.7586939751845192"}],"id":"n0.8019077953128695"}],"id":"n0.16274775883676695"}},"id":"n0.6354860275022087"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4097985681310048"}],"id":"n0.5576389802155606"}],"id":"n0.46948006831709677"},"powerValue":{"lines":[{"blocks":[{"text":"0","id":"n0.3771778972134905"}],"id":"n0.3491918701529553"}],"id":"n0.6804177236712141"}},"id":"n0.8564787329672008"},{"type":"single","text":"(","id":"n0.07632820792608874"},{"text":"s,a","id":"n0.37648471103085024"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.775601513941599"}],"id":"n0.40374530105673934"}],"id":"n0.12508214063133827"}},"id":"n0.2606369486644555"},{"type":"single","text":")","id":"n0.8835602704953642"}],"id":"n0.43201992570641323"}],"id":"n0.6639940912465938"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.016141386358724086"}],"style":{"align":"center"},"id":"n0.6607706569816483"}],"shape":{"data":{"p":{"x":460,"y":279.6975843468925},"rotation":0},"anchor":"left-top","style":{"fillColor":[80,227,194,1]}},"isTextMode":true,"isInGroup":false},"de2579719695378768":{"id":"de2579719695378768","lines":[{"blocks":[{"text":"Level ","style":{"fontSize":"\\tiny"},"id":"n0.3632367527785749"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"L-1","id":"n0.20846838892596553"}],"id":"n0.5835614246651424"}],"id":"n0.4508209020473879"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.6120189070802013"}],"style":{"align":"center"},"id":"n0.8349679808894037"}],"shape":{"data":{"p":{"x":182.49359130859375,"y":17.635022970635077},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6314113770356831":{"id":"de6314113770356831","lines":[{"blocks":[{"text":"Level ","style":{"fontSize":"\\tiny"},"id":"n0.21504016787584845"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"L-2","id":"n0.21266299444689585"}],"id":"n0.6814644698850401"}],"id":"n0.20834096396169643"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.09669984625424677"}],"style":{"align":"center"},"id":"n0.9433971486576183"}],"shape":{"data":{"p":{"x":183,"y":105.63502297063508},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de19675038100118147":{"id":"de19675038100118147","lines":[{"blocks":[{"text":"Level ","style":{"fontSize":"\\tiny"},"id":"n0.4665094201284141"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"0","id":"n0.4041203922664638"}],"id":"n0.35536501373177276"}],"id":"n0.542136158452516"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.7350935049092755"}],"style":{"align":"center"},"id":"n0.018888212550350003"}],"shape":{"data":{"p":{"x":183,"y":241.63502297063508},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3793798924569056":{"id":"de3793798924569056","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.8934204249110584"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.8340023940541792","text":"i"}],"id":"n0.990519759646665"}],"id":"n0.6266561818284284"}},"id":"n0.7459659549277033"},{"text":"|","id":"n0.02530197623617303"}],"id":"n0.6296807647435203"}],"id":"n0.8814959856119453"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6089052983923968"}],"style":{"align":"center"},"id":"n0.3309086780043087"}],"shape":{"data":{"p":{"x":402,"y":306.4255789092479},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de02539145642801577":{"id":"de02539145642801577","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.056371739255644204"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.13174007075183192"}],"id":"n0.248403283253676"}],"id":"n0.3661469535821704"}},"id":"n0.9569596830675164"},{"text":"|","id":"n0.2533120784434968"}],"id":"n0.593332307309044"}],"id":"n0.3838513742554275"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.18568227913067625"}],"style":{"align":"center"},"id":"n0.06428877903424657"}],"shape":{"data":{"p":{"x":402,"y":253.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de05168791060859412":{"id":"de05168791060859412","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.6582585624233113"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.788965801871945"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.12614605121514644","text":"i"}],"id":"n0.021324803176446805"}],"id":"n0.10482432157327626"}},"id":"n0.04797838599969828"}],"id":"n0.8901422202213247"}],"id":"n0.8788180716067089"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.3044316332222887"}],"id":"n0.6868342941933696"}],"id":"n0.25994957128260676"}},"id":"n0.8499402048082008"}],"id":"n0.47796249916056044"}],"id":"n0.6748794387292034"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.14765023594948823"}],"id":"n0.4677300447181276"}],"shape":{"data":{"p":{"x":414.99359130859375,"y":296}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de33489281180821995":{"id":"de33489281180821995","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.09407891212168473"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.34600370469723996"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.22683942594424145"}],"id":"n0.010431547090191229"}],"id":"n0.1709610314528911"}},"id":"n0.9697516612181147"}],"id":"n0.37307691542753463"}],"id":"n0.15252746660662364"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.63917899335727"}],"id":"n0.6436412748391367"}],"id":"n0.1347447194698812"}},"id":"n0.3152914544875969"}],"id":"n0.772350973034134"}],"id":"n0.20568306821556503"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4577189107404238"}],"id":"n0.5423432343479035"}],"shape":{"data":{"p":{"x":414.99359130859375,"y":243.55827729192396}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de599100908346867":{"id":"de599100908346867","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.4866774580992028"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9967038337399736"}],"id":"n0.8694528209142025"}],"id":"n0.7855968366770971"}},"id":"n0.6221054991623272"},{"text":"|","id":"n0.23801682853525774"}],"id":"n0.9293510086231909"}],"id":"n0.34935182724472136"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5628668240365013"}],"style":{"align":"center"},"id":"n0.7885752919089821"}],"shape":{"data":{"p":{"x":402,"y":114.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7808512405889996":{"id":"de7808512405889996","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.7362026767584469"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.8163758712340334"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8725591332626943"}],"id":"n0.892491453782452"}],"id":"n0.11958147842711542"}},"id":"n0.8848331183670357"}],"id":"n0.6007899845556632"}],"id":"n0.6118672296885168"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.7993776462627542"}],"id":"n0.025512495977708438"}],"id":"n0.5357554047434483"}},"id":"n0.9984456052965838"}],"id":"n0.6102202981030778"}],"id":"n0.7990525584386923"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6148671870434375"}],"id":"n0.6565569611219635"}],"shape":{"data":{"p":{"x":414.99359130859375,"y":104.55827729192396}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de6183527944901863":{"id":"de6183527944901863","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.6147068921960703"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7066805573624653"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4942985658276202"}],"id":"n0.7086286483486222"}],"id":"n0.17496155535778413"}},"id":"n0.3122931531715807"}],"id":"n0.9201585131605319"}],"id":"n0.07909149458138565"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.19903607225869724"}],"id":"n0.67779796803327"}],"id":"n0.680415402902476"}},"id":"n0.4640400734380665"}],"id":"n0.8325561577006042"}],"id":"n0.6833550991018396"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.960391229975732"}],"id":"n0.3488295089348885"}],"shape":{"data":{"p":{"x":414.99359130859375,"y":17.558277291923957}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de10775284719956923":{"id":"de10775284719956923","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.25871157002202505"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9276959523680952","text":"j"}],"id":"n0.9479672303757438"}],"id":"n0.26069607650483806"}},"id":"n0.906468976536928"},{"text":"|","id":"n0.6566745052972824"}],"id":"n0.6389208899453975"}],"id":"n0.37277273316714243"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4332897151220161"}],"style":{"align":"center"},"id":"n0.06291855946151559"}],"shape":{"data":{"p":{"x":404.08829782270914,"y":28.1858628361133},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di41729058265448593","items":[],"style":{}},"shapes":[{"id":"dp47833610138437277","type":"doc-rounded-rect","data":{"p1":{"x":229.3642310148602,"y":17.810200449549598},"p2":{"x":312.91291638898514,"y":41.7005827509488},"rotation":0},"style":{"fillColor":[140,200,240,1]}},{"id":"dp7252990734982117","type":"doc-rounded-rect","data":{"p1":{"x":229.3642310148602,"y":105.8102004495496},"p2":{"x":312.91291638898514,"y":129.7005827509488},"rotation":0},"style":{"fillColor":[140,200,240,1]}},{"id":"dp5238403623954342","type":"doc-cube","data":{"p1":{"x":326.5752569651695,"y":120.84735887517525},"p2":{"x":369.92608642578125,"y":158.5573056490507},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp3426937152560734","type":"doc-cube","data":{"p1":{"x":326.5752569651695,"y":88.84735887517525},"p2":{"x":369.92608642578125,"y":126.5573056490507},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da3764417224670913","data":[{"x":313.0093994140625,"y":118.1858628361133},{"x":325.93050100541586,"y":118.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9225803741722312","data":[{"x":370.93050100541586,"y":118.1858628361133},{"x":382.0093994140625,"y":118.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp8261396135456109","type":"rectangle","data":{"p1":{"x":382.54710037167024,"y":94.04608154296875},"p2":{"x":390.1573101697012,"y":141.04608154296875}}},{"id":"da06700100677924525","data":[{"x":391.0093994140625,"y":118.1858628361133},{"x":413.08829782270914,"y":118.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp8553147868712787","type":"doc-cube","data":{"p1":{"x":326.5752569651695,"y":32.847358875175246},"p2":{"x":369.92608642578125,"y":70.5573056490507},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp2137631360458554","type":"doc-cube","data":{"p1":{"x":326.5752569651695,"y":0.8473588751752459},"p2":{"x":369.92608642578125,"y":38.557305649050704},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da15943921980254028","data":[{"x":313.0672439523636,"y":30.1858628361133},{"x":325.93050100541586,"y":30.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da8049389990280313","data":[{"x":369.93050100541586,"y":30.1858628361133},{"x":383.0093994140625,"y":30.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp8184268731954947","type":"rectangle","data":{"p1":{"x":382.54710037167024,"y":6.04608154296875},"p2":{"x":390.1573101697012,"y":53.04608154296875}}},{"id":"da45763509473825215","data":[{"x":390.0093994140625,"y":30.1858628361133},{"x":412.08829782270914,"y":30.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da23976988799793553","data":[{"x":271.9004128140757,"y":82.1858628361133},{"x":420.0093994140625,"y":82.1858628361133}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9389736317801487","data":[{"x":420.0093994140625,"y":109.5402473973582},{"x":420.0093994140625,"y":82.1858628361133}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp7423675029202152","type":"doc-rounded-rect","data":{"p1":{"x":230.3642310148602,"y":243.8102004495496},"p2":{"x":313.91291638898514,"y":267.7005827509488},"rotation":0},"style":{"fillColor":[140,200,240,1]}},{"id":"da9790415098060559","data":[{"x":272.9004128140757,"y":308.1858628361133},{"x":272.9004128140757,"y":268.14283514022827}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp7435646245202219","type":"doc-cube","data":{"p1":{"x":328.5752569651695,"y":258.84735887517525},"p2":{"x":366.66561195135387,"y":296.5573056490507},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp08033017088121319","type":"doc-cube","data":{"p1":{"x":328.5752569651695,"y":226.84735887517525},"p2":{"x":366.66561195135387,"y":264.5573056490507},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da8713163721465647","data":[{"x":314.0672439523636,"y":256.1858628361133},{"x":327.93050100541586,"y":256.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da2411252945849418","data":[{"x":366.93050100541586,"y":256.1858628361133},{"x":381.0093994140625,"y":256.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp9011794347447228","type":"rectangle","data":{"p1":{"x":380.54710037167024,"y":232.04608154296875},"p2":{"x":388.1573101697012,"y":279.04608154296875}}},{"id":"da20364951303761303","data":[{"x":388.0093994140625,"y":256.1858628361133},{"x":412.99359130859375,"y":256.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9481886775137895","data":[{"x":273.9004128140757,"y":219.02993774414062},{"x":273.9004128140757,"y":204.1324462890625}],"head":"fh>","tail":"no","shaft":"--","middle":"no","headScale":0.6},{"id":"da16940211400592764","data":[{"x":273.9004128140757,"y":219.02993774414062},{"x":421.0093994140625,"y":219.02993774414062}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6},{"id":"da3473100070999804","data":[{"x":421.0093994140625,"y":248.5402473973582},{"x":421.0093994140625,"y":219.1858628361133}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6},{"id":"dp12319438729391963","type":"right-arrow","data":{"p1":{"x":436.68282386541637,"y":24.471092435162753},"p2":{"x":449.68282386541637,"y":36.97583639268228},"arrowPercentage":0.4}},{"id":"dp7125078369975848","type":"doc-cube","data":{"p1":{"x":453.592468879232,"y":303.29005322612454},"p2":{"x":491.68282386541637,"y":341},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp9152516441590235","type":"doc-cube","data":{"p1":{"x":453.592468879232,"y":271.29005322612454},"p2":{"x":491.68282386541637,"y":309},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da909845752930831","data":[{"x":272.9004128140757,"y":176.1324462890625},{"x":420.0093994140625,"y":176.1324462890625}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6},{"id":"da09205056674657586","data":[{"x":271.9004128140757,"y":82.1858628361133},{"x":271.9004128140757,"y":41.15322399139404}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da44421738044179104","data":[{"x":272.9004128140757,"y":176.1324462890625},{"x":272.9004128140757,"y":130.15322399139404}],"head":"fh>","tail":"no","shaft":"--","middle":"no","headScale":0.6},{"id":"da9378807022106552","data":[{"x":272.9004128140757,"y":308.1858628361133},{"x":413.0093994140625,"y":308.1858628361133}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg5752425887968442","entities":[{"id":"dg8348766324290573","entities":[{"id":"dp9208284147887935","type":"rectangle","data":{"p1":{"x":412.99359130859375,"y":300.98197010543424},"p2":{"x":425.6507520406526,"y":313.6391308374931}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp008477122704914297","type":"rectangle","data":{"p1":{"x":414.57573640010105,"y":302.5641151969416},"p2":{"x":427.2328971321599,"y":315.22127592900046}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp3642009145930136","type":"rectangle","data":{"p1":{"x":416.15788149160846,"y":304.14626028844896},"p2":{"x":428.8150422236673,"y":316.8034210205078}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl04460893008583788","linkedId":"de05168791060859412"}]},{"id":"da7912672485721097","data":[{"x":428.99359130859375,"y":308.1858628361133},{"x":453.0093994140625,"y":308.1858628361133}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"dg9035236793094654","entities":[{"id":"dg5023454242459575","entities":[{"id":"dp4101738498195575","type":"rectangle","data":{"p1":{"x":412.99359130859375,"y":248.5402473973582},"p2":{"x":425.6507520406526,"y":261.19740812941706}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp5331236483757704","type":"rectangle","data":{"p1":{"x":414.57573640010105,"y":250.12239248886556},"p2":{"x":427.2328971321599,"y":262.7795532209244}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp9471391528134872","type":"rectangle","data":{"p1":{"x":416.15788149160846,"y":251.70453758037291},"p2":{"x":428.8150422236673,"y":264.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl2659154614400385","linkedId":"de33489281180821995"}]},{"id":"dg45923819168090696","entities":[{"id":"dg390100338337527","entities":[{"id":"dp6129333426434289","type":"rectangle","data":{"p1":{"x":412.99359130859375,"y":109.5402473973582},"p2":{"x":425.6507520406526,"y":122.19740812941706}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp32210977992707734","type":"rectangle","data":{"p1":{"x":414.57573640010105,"y":111.12239248886556},"p2":{"x":427.2328971321599,"y":123.77955322092441}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp7088279109032376","type":"rectangle","data":{"p1":{"x":416.15788149160846,"y":112.70453758037291},"p2":{"x":428.8150422236673,"y":125.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl8128743428252136","linkedId":"de7808512405889996"}]},{"id":"dg8422714549228933","entities":[{"id":"dg8749080403551495","entities":[{"id":"dp04357528838072988","type":"rectangle","data":{"p1":{"x":412.99359130859375,"y":22.5402473973582},"p2":{"x":425.6507520406526,"y":35.197408129417056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp7977411862931905","type":"rectangle","data":{"p1":{"x":414.57573640010105,"y":24.122392488865557},"p2":{"x":427.2328971321599,"y":36.77955322092441}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp013304563458476082","type":"rectangle","data":{"p1":{"x":416.15788149160846,"y":25.704537580372914},"p2":{"x":428.8150422236673,"y":38.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl4309794460639673","linkedId":"de6183527944901863"}]},{"id":"dp10615464469127711","type":"right-arrow","data":{"p1":{"x":436.68282386541637,"y":111.97583639268228},"p2":{"x":449.68282386541637,"y":124.48058035020182},"arrowPercentage":0.4}},{"id":"dp11234244974403396","type":"right-arrow","data":{"p1":{"x":436.68282386541637,"y":250.48058035020182},"p2":{"x":449.68282386541637,"y":262.9853243077214},"arrowPercentage":0.4}}],"settings":{"grid":true,"diagramHeight":341.9701232910156}}]},{"id":"n0.5773724414561772","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":1699,"delayRenderCache":{"av":1699,"map":{"n0.878034595656866":{"n0.6479673560913659":{"w":26.2496,"h":8.4545,"bl":0.8214}},"n0.7620427428820304":{"n0.564695130185312":{"w":26.4938,"h":8.4545,"bl":0.8214}},"n0.021551824456943036":{"n0.4521066476362081":{"w":26.4938,"h":8.4545,"bl":0.8214}},"n0.49121514402082456":{"n0.8091899817257213":{"w":33.5015,"h":9.1146,"bl":0.7619}},"n0.5762378149466976":{"n0.624454071858985":{"w":33.7457,"h":9.1146,"bl":0.7619}},"n0.5421621652642399":{"n0.16312157425304696":{"w":28.2208,"h":9.1146,"bl":0.7619}},"n0.6639940912465938":{"n0.43201992570641323":{"w":28.465,"h":15.4984,"bl":0.7264}},"n0.8814959856119453":{"n0.6296807647435203":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.3838513742554275":{"n0.593332307309044":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.6748794387292034":{"n0.47796249916056044":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.34935182724472136":{"n0.9293510086231909":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.7990525584386923":{"n0.6102202981030778":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.6833550991018396":{"n0.8325561577006042":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.37277273316714243":{"n0.6389208899453975":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.20568306821556503":{"n0.772350973034134":{"w":7.4599,"h":9.6481,"bl":0.7198}}}}}

==> plots/docs/5ff3344f-e3ef-49c3-9fc8-e6006ee92bde <==
{"id":"n0.9735571899555475","lines":[{"id":"n0.09626705958257009","blocks":[]},{"id":"n0.2918628718558065","blocks":[{"id":"n0.37860086508951385","text":"\\diagram","type":"composite","elements":{"de0634562876505389":{"id":"de0634562876505389","lines":[{"blocks":[{"text":"Value iteration solver","style":{"fontSize":"\\tiny"},"id":"n0.2393113020621569"}],"style":{"align":"center"},"id":"n0.7036002702805659"}],"shape":{"data":{"p":{"x":190,"y":39.248550073937906},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7452464315882257":{"id":"de7452464315882257","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.8293342112764326"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6364811329040743"}],"id":"n0.09795120049062156"}],"id":"n0.328815333454892"}},"id":"n0.6905435550237693"},{"text":"|","id":"n0.6451205917090073"}],"id":"n0.1154698172732449"}],"id":"n0.4639640815729844"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9594496036142959"}],"style":{"align":"center"},"id":"n0.3990772838906833"}],"shape":{"data":{"p":{"x":281.5752569651695,"y":83.90358032942736},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de30539217550006503":{"id":"de30539217550006503","lines":[{"blocks":[{"text":"Softmax","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.5380915526612213"}],"style":{"align":"center"},"id":"n0.9635321019519416"}],"shape":{"data":{"p":{"x":443.48919677734375,"y":12.084634767795478},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6158175282739142":{"id":"de6158175282739142","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.6454358308840946"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"L,K","id":"n0.7684800122204358"}],"id":"n0.7190303345779496"}],"id":"n0.5721805846990413"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5245745158244517"}],"id":"n0.7086308650615849"}],"id":"n0.283793262999148"}},"id":"n0.172266758285198"},{"type":"single","text":"(","id":"n0.9033436097145575"},{"text":"s,a","id":"n0.10996256372674273"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8067534064680955"}],"id":"n0.30546746033830807"}],"id":"n0.779788527208449"}},"id":"n0.18425677171769483"},{"type":"single","text":")","id":"n0.1760959765402652"}],"id":"n0.1781866772261569"}],"id":"n0.45802729846083956"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6479475484287407"}],"style":{"align":"center"},"id":"n0.34957141144569714"}],"shape":{"data":{"p":{"x":287.4011224293617,"y":31.481335521572248},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7578803692968976":{"id":"de7578803692968976","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.6735115506100067"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8910240050030935"}],"id":"n0.492933483487094"}],"id":"n0.5543595260820138"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.025605870710162293"}],"id":"n0.2899697062197255"}],"id":"n0.250689808273159"}},"id":"n0.35261412989877283"},{"type":"single","text":"(","id":"n0.8513162358432065"},{"text":"s","id":"n0.040384118441435746"},{"type":"single","text":")","id":"n0.616977251271351"}],"id":"n0.5361220979168753"}],"id":"n0.16920259577024832"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.32636677561643945"}],"style":{"align":"center"},"id":"n0.09078805888162278"}],"shape":{"data":{"p":{"x":333.9827880859375,"y":86.934645988932},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6802701882630025":{"id":"de6802701882630025","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.1346456291087723"}],"id":"n0.04427435903979493"}],"id":"n0.24530697980996785"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.05328824754854278"}],"style":{"align":"center"},"id":"n0.4266733370356186"}],"shape":{"data":{"p":{"x":316.5752569651695,"y":100.82953052127158},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de45675243102562924":{"id":"de45675243102562924","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.8342108437915399"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.5616116446250121"}],"id":"n0.28707750677524335"}],"id":"n0.3709395641010995"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5291916187896755"}],"style":{"align":"center"},"id":"n0.8710600789821672"}],"shape":{"data":{"p":{"x":360.0379365869461,"y":53.79938993941613},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de29561144923861726":{"id":"de29561144923861726","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"q","id":"n0.7861428367417931"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"L,K","id":"n0.8357121406402748"}],"id":"n0.5227598617191422"}],"id":"n0.3628902113797876"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.712903964628566"}],"id":"n0.31475679751150354"}],"id":"n0.7407370441747998"}},"id":"n0.1391651580626443"},{"type":"single","text":"(","id":"n0.2635047033354987"},{"text":"a","id":"n0.36959698716328204"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.24175630353672606"}],"id":"n0.30304596472597756"}],"id":"n0.6422484908790382"}},"id":"n0.34631958848430067"},{"type":"single","text":")","id":"n0.19016959825871682"}],"id":"n0.17101577099144838"}],"id":"n0.8479159783897559"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.06257449221844236"}],"style":{"align":"center"},"id":"n0.8975266426892756"}],"shape":{"data":{"p":{"x":392.9593927759736,"y":37.245461431688},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de15477765764642415":{"id":"de15477765764642415","lines":[{"blocks":[{"text":"Argmax","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.5927037459254869"}],"style":{"align":"center"},"id":"n0.18987849489526099"}],"shape":{"data":{"p":{"x":443.9827880859375,"y":66.73613757171921},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de22048441519143336":{"id":"de22048441519143336","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7153442312137162"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6821186587904562"}],"id":"n0.544484029247013"}],"id":"n0.14612408706422375"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.20960450932884633"}],"id":"n0.747255326029669"}],"id":"n0.7712424245331346"}},"id":"n0.346101542372347"}],"id":"n0.7253550691720647"}],"id":"n0.07047354575524611"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3540147473589985"}],"id":"n0.6466078670383382"}],"shape":{"data":{"p":{"x":446,"y":64.56357350349424}},"anchor":"left-top"},"isTextMode":true},"de6172859081567905":{"id":"de6172859081567905","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.29745597199177953"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.600571084112483"}],"id":"n0.996951432460681"}],"id":"n0.22174708464338644"}},"id":"n0.16095678407547664"},{"text":"|","id":"n0.12931111642842286"}],"id":"n0.4249884359941296"}],"id":"n0.18027727489244993"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.758609235691853"}],"style":{"align":"center"},"id":"n0.578764375406543"}],"shape":{"data":{"p":{"x":437.4827880859375,"y":22.311111450195312},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de029769300904883833":{"id":"de029769300904883833","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.16059604139512107"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.14509492759894793"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9295753376642859"}],"id":"n0.27376384560424927"}],"id":"n0.10688134315026021"}},"id":"n0.23859632174727086"}],"id":"n0.4708863947241193"}],"id":"n0.06716223629911067"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.6027299015914285"}],"id":"n0.15347978730734502"}],"id":"n0.019425296462810104"}},"id":"n0.9321418717828704"}],"id":"n0.3935658500937744"}],"id":"n0.9992338966947969"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5355528677259982"}],"id":"n0.7623875181255182"}],"shape":{"data":{"p":{"x":448.9827880859375,"y":12}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de1929515620516158":{"id":"de1929515620516158","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.15411396745112516"}],"id":"n0.06625770994633151"}],"id":"n0.16559125385250617"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7008248018013283"}],"id":"n0.3962088806452788"}],"shape":{"data":{"p":{"x":363.8237031885086,"y":41.210105519402646},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9533855630629304":{"id":"de9533855630629304","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.803168905710903"}],"id":"n0.595609449097565"}],"id":"n0.6114877208310152"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3396408939754496"}],"id":"n0.3955509286506018"}],"shape":{"data":{"p":{"x":329.4247300786326,"y":40.40960864627158}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true}},"connections":[],"intersections":{"id":"di37777461296401205","items":[],"style":{}},"shapes":[{"id":"dp003544426753230079","type":"doc-rounded-rect","data":{"p1":{"x":184.87063970626645,"y":40.42372755285243},"p2":{"x":268.4193250803914,"y":64.31410985425163},"rotation":0},"style":{"fillColor":[140,200,240,1]}},{"id":"da5945521334690271","data":[{"x":268.57365264376983,"y":52.79938993941613},{"x":280.4369096968221,"y":52.79938993941613}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da3960110458681976","data":[{"x":406.40682150548196,"y":24.79938993941613},{"x":426.51580810546875,"y":24.79938993941613}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp6988907231690673","type":"rectangle","data":{"p1":{"x":426.0535090630765,"y":0.6596086462715789},"p2":{"x":433.66371886110744,"y":47.65960864627158}}},{"id":"da3908323885544205","data":[{"x":433.51580810546875,"y":24.79938993941613},{"x":445.5947065141154,"y":24.79938993941613}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp4210477301545459","type":"doc-cube","data":{"p1":{"x":281.5752569651695,"y":54.601164676319854},"p2":{"x":319.66561195135387,"y":92.31111145019531},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp5009696529486707","type":"doc-cube","data":{"p1":{"x":281.5752569651695,"y":22.601164676319854},"p2":{"x":319.66561195135387,"y":60.31111145019531},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp10826384287995405","type":"doc-cube","data":{"p1":{"x":324.5752569651695,"y":77.52711486816406},"p2":{"x":362.66561195135387,"y":115.23706164203952},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da01663430025434587","data":[{"x":319.4369096968221,"y":52.79938993941613},{"x":331.6389634770701,"y":52.79938993941613}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg5248469829845708","entities":[{"id":"dp14571626825558615","type":"circle","data":{"p1":{"x":331.6389634770701,"y":43.23103503787314},"p2":{"x":351.1746795338938,"y":62.76675109469687}}},{"id":"dl4804558576697693","linkedId":"de9533855630629304"}]},{"id":"da979653912349423","data":[{"x":341.40682150548196,"y":77.52711486816406},{"x":341.40682150548196,"y":62.76675109469687}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da7884999857903685","data":[{"x":351.1746795338938,"y":52.99889306628501},{"x":363.3767333141418,"y":52.99889306628501}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg2725140409654083","entities":[{"id":"dp07794459160541112","type":"circle","data":{"p1":{"x":363.0379365869461,"y":43.031531911004265},"p2":{"x":382.57365264376983,"y":62.567247967827996}}},{"id":"dl6796094159610477","linkedId":"de1929515620516158"}],"data":{"rotation":0}},{"id":"da9333930392682195","data":[{"x":382.57365264376983,"y":52.79938993941613},{"x":394.7757064240178,"y":52.79938993941613}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp718863484943477","type":"rectangle","data":{"p1":{"x":395.0093994140625,"y":37.245461431688},"p2":{"x":418.0093994140625,"y":66.56792127763404}},"style":{"fillColor":[245,166,35,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp8753097908953678","type":"rectangle","data":{"p1":{"x":426.0535090630765,"y":55.65960864627158},"p2":{"x":433.66371886110744,"y":102.65960864627158}}},{"id":"dp6584784912429689","type":"square","data":{"p1":{"x":446,"y":72.56357350349424},"p2":{"x":458.5,"y":85.06357350349424}},"style":{"fillColor":[248,231,28,1]}},{"id":"da1725587121521539","data":[{"x":406.5093994140625,"y":78.90669135466102},{"x":406.5093994140625,"y":66.14632758119383}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da8991990548373658","data":[{"x":406.40682150548196,"y":36.52711486816406},{"x":406.40682150548196,"y":24.527114868164062}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4919998310196001","data":[{"x":406.5093994140625,"y":78.90669135466102},{"x":426.6183860140493,"y":78.90669135466102}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9029528484206584","data":[{"x":433.6183860140493,"y":78.90669135466102},{"x":445.69728442269593,"y":78.90669135466102}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg5700695566556591","entities":[{"id":"dg8570720766417066","entities":[{"id":"dp6218468945744007","type":"rectangle","data":{"p1":{"x":445.9827880859375,"y":16.981970105434243},"p2":{"x":458.63994881799636,"y":29.6391308374931}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp289772994101404","type":"rectangle","data":{"p1":{"x":447.5649331774448,"y":18.5641151969416},"p2":{"x":460.22209390950366,"y":31.221275929000456}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp6286541772730896","type":"rectangle","data":{"p1":{"x":449.1470782689522,"y":20.146260288448957},"p2":{"x":461.80423900101107,"y":32.80342102050781}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl9671172040205072","linkedId":"de029769300904883833"}]}],"settings":{"grid":true,"diagramHeight":122.98385620117188}}]},{"id":"n0.0733441201018945","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":321,"delayRenderCache":{"av":321,"map":{"n0.4639640815729844":{"n0.1154698172732449":{"w":26.2496,"h":8.4545,"bl":0.8214}},"n0.18027727489244993":{"n0.4249884359941296":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.45802729846083956":{"n0.1781866772261569":{"w":28.248,"h":9.1146,"bl":0.7619}},"n0.16920259577024832":{"n0.5361220979168753":{"w":22.4157,"h":12.5054,"bl":0.7021}},"n0.8479159783897559":{"n0.17101577099144838":{"w":20.4083,"h":9.1146,"bl":0.7619}},"n0.07047354575524611":{"n0.7253550691720647":{"w":5.3982,"h":9.1146,"bl":0.7619}},"n0.9992338966947969":{"n0.3935658500937744":{"w":7.4599,"h":9.6481,"bl":0.7198}}}}}

==> plots/docs/8d120bbf-8ed1-48f8-be65-4a481f7a1e35 <==
{"id":"n0.28715960587730205","lines":[{"id":"n0.29452044693609114","blocks":[]},{"id":"n0.20454292606745117","blocks":[{"id":"n0.6840725551755149","text":"\\diagram","type":"composite","elements":{"de830133496527524":{"id":"de830133496527524","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.888716145367255"},{"id":"n0.15104764783136782","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.36671146661237697","lines":[{"id":"n0.8179473477339385","blocks":[{"id":"n0.9550966687339157","text":"i"}]}]}}},{"text":"×W","id":"n0.5599012392663407"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.41671340239262555"}],"id":"n0.7908228230325796"}],"id":"n0.46363745184185046"}},"id":"n0.678323976462252"},{"text":"×H","id":"n0.16969816635029078"},{"id":"n0.039609500242658635","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.17353734365161166","lines":[{"id":"n0.038406751864820565","blocks":[{"id":"n0.39762182261952717","text":"j"}]}]}}},{"text":"×W","id":"n0.3008060942961859"},{"id":"n0.3607380716179993","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7303295250166091","lines":[{"id":"n0.9959625119092972","blocks":[{"id":"n0.24721289861843165","text":"j"}]}]}}},{"text":"×|A","id":"n0.7472395874987383"},{"id":"n0.3920680333441362","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.8195620441773821","lines":[{"id":"n0.580356851690097","blocks":[{"id":"n0.019039025036673207","text":"i"}]}]}}},{"text":"|×|𝛺","id":"n0.5911674285490001"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3521376731337347"}],"id":"n0.12198891662407862"}],"id":"n0.6303078999133256"}},"id":"n0.8010527248379509"},{"text":"|","id":"n0.09645521585780603"}],"id":"n0.22684036926304696"}],"id":"n0.12264719501879284"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8934350916238187"}],"style":{"align":"center"},"id":"n0.26840922209508244"}],"shape":{"data":{"p":{"x":274,"y":71.05827729192396},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de31428410007153573":{"id":"de31428410007153573","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"2D convolutional layer","id":"n0.16885513588950096"}],"id":"n0.06845146326372276"}],"shape":{"data":{"p":{"x":139.7593994140625,"y":11.070138759285399},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5068466687657365":{"id":"de5068466687657365","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.6485921189478068"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×200×|A","id":"n0.09462604923524598"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7357774409027493"}],"id":"n0.8321220245420999"}],"id":"n0.056047845178978095"}},"id":"n0.34039756771574803"},{"text":"×𝛺","id":"n0.10022572740377522"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.018645629099951266"}],"id":"n0.2507497419973437"}],"id":"n0.5522533401755028"}},"id":"n0.6223560424619412"},{"text":"|","id":"n0.14742117445867353"}],"id":"n0.9045013624179807"}],"id":"n0.28195840591444044"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.27517338485264564"}],"id":"n0.11799573819626064"}],"shape":{"data":{"p":{"x":132.7593994140625,"y":0.07013875928538482},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de546742242883713":{"id":"de546742242883713","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.872383021644545"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1","id":"n0.7272182565354888"}],"id":"n0.9042131022522326"}],"id":"n0.038708607070670586"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7164403655705867"}],"id":"n0.31004931376728595"}],"shape":{"data":{"p":{"x":125.75939941406247,"y":24.0701387592854},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5705596917101636":{"id":"de5705596917101636","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"2D convolutional layer","id":"n0.5472261254339543"}],"id":"n0.08300183269532035"}],"shape":{"data":{"p":{"x":113.2593994140625,"y":10.570138759285385},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6002399326791896":{"id":"de6002399326791896","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.5163073951096822"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3×3×1×200","id":"n0.03293938249114303"}],"id":"n0.8635446728446938"}],"id":"n0.00554654937310417"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.09854121342956024"}],"id":"n0.4855904436457106"}],"shape":{"data":{"p":{"x":105.2593994140625,"y":10.570138759285392},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9263864201631913":{"id":"de9263864201631913","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.020891449239466064"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1","id":"n0.7882173865781894"}],"id":"n0.956542045504768"}],"id":"n0.8597594355492408"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9753627930496795"}],"id":"n0.867659227440186"}],"shape":{"data":{"p":{"x":98.2593994140625,"y":23.570138759285385},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de30334807816745935":{"id":"de30334807816745935","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Activation: sigmoid","id":"n0.3095276842699177"}],"id":"n0.6203656270879352"}],"shape":{"data":{"p":{"x":151.7593994140625,"y":15.070138759285399},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7476602457265411":{"id":"de7476602457265411","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.6928414408579382"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7696527085094487"}],"id":"n0.9249682609169809"}],"id":"n0.6033597829383572"}},"id":"n0.796271880879913"},{"text":"×W","id":"n0.8124065052244716"},{"id":"n0.5558073109510935","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.26051854782853656","lines":[{"id":"n0.9510684309087385","blocks":[{"id":"n0.021780209106427417","text":"i"}]}]}}},{"text":"×|A","id":"n0.7399565040359255"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.15565566038690504"}],"id":"n0.9036242193532307"}],"id":"n0.5163854680637376"}},"id":"n0.19101800992060047"},{"text":"×𝛺","id":"n0.6221485586612392"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.91989118239133"}],"id":"n0.1277352944004988"}],"id":"n0.8165743475653806"}},"id":"n0.958018226031242"},{"text":"|","id":"n0.6820777378036293"}],"id":"n0.7635730023714855"}],"id":"n0.7636721946274969"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.026328566609607806"}],"style":{"align":"center"},"id":"n0.7961220810897758"}],"shape":{"data":{"p":{"x":157.9753875732422,"y":48.560739345222885},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2201987216315624":{"id":"de2201987216315624","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.7132498602809136"}],"id":"n0.3466031727800791"}],"id":"n0.27484400963508127"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\scriptsize"},"id":"n0.6677785758317261"}],"id":"n0.08446180503343959"}],"shape":{"data":{"p":{"x":172.49811067557866,"y":-0.4063528350291712},"rotation":49.5},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8364529015502058":{"id":"de8364529015502058","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.8599819514151139"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5284243819925398"}],"id":"n0.43397894302458195"}],"id":"n0.5203002474914415"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.7093998630382501"}],"id":"n0.8794057646934292"}],"id":"n0.13734081724066582"}},"id":"n0.9586627531781591"},{"type":"single","text":"(","id":"n0.2277236073298805"},{"text":"s","id":"n0.7235534741127996"},{"type":"single","text":")","id":"n0.5423795029927823"}],"id":"n0.008391880325343104"}],"id":"n0.8068253129909273"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.7783573921404539"}],"style":{"align":"center"},"id":"n0.4805870590674932"}],"shape":{"data":{"p":{"x":54.31714561700551,"y":172.21718170370752},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7069425642293998":{"id":"de7069425642293998","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.005083172132470448"},{"id":"n0.6011201773360508","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2905804311605169","lines":[{"id":"n0.9714403353577845","blocks":[{"id":"n0.9660014246304194","text":"i"}]}]}}},{"id":"n0.8703022194174608","text":"×W"},{"id":"n0.7524534765602964","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.08243965341437276","lines":[{"id":"n0.8151768469634642","blocks":[{"id":"n0.5103346716209716","text":"i"}]}]}}}],"id":"n0.9115976780097668"}],"id":"n0.2742966032445735"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8503622370030484"}],"style":{"align":"center"},"id":"n0.7049519028495159"}],"shape":{"data":{"p":{"x":20.909614496237566,"y":184.1120662360471},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de09279253696072942":{"id":"de09279253696072942","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.4910014458934293"},{"id":"n0.8615066548897736","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9575001423927905","lines":[{"id":"n0.27052359880341914","blocks":[{"id":"n0.8845606799651806","text":"i"}]}]}}},{"text":"×W","id":"n0.659142267370771"},{"id":"n0.6083060945162448","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7126463045547087","lines":[{"id":"n0.8733096058843968","blocks":[{"id":"n0.015992116033920034","text":"i"}]}]}}},{"text":"×H","id":"n0.32992532734899993"},{"id":"n0.33587015564662304","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.11277231313626235","lines":[{"id":"n0.4319993442378911","blocks":[{"id":"n0.3045815083089889","text":"j"}]}]}}},{"text":"×W","id":"n0.06804613915010371"},{"id":"n0.38530347794077335","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.06629092672006331","lines":[{"id":"n0.30582049305888703","blocks":[{"id":"n0.6796539873208021","text":"j"}]}]}}},{"text":"×|A","id":"n0.795047829499475"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.30683837280018733"}],"id":"n0.05876238109896281"}],"id":"n0.8536749608131902"}},"id":"n0.12748157878062338"},{"text":"×A","id":"n0.7742199666318177"},{"id":"n0.6456645765287621","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7418617950362201","lines":[{"id":"n0.3239890683037132","blocks":[{"id":"n0.1956380655810923","text":"j"}]}]}}},{"text":"|","id":"n0.5271039502302577"}],"id":"n0.27881606013744675"}],"id":"n0.3566822829252332"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.02033497072142687"}],"style":{"align":"center"},"id":"n0.07737509054617053"}],"shape":{"data":{"p":{"x":281.29996422052113,"y":305.8058692110944},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5724928845451427":{"id":"de5724928845451427","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.6209544034078567"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9240656630032333"}],"id":"n0.6953438142929429"}],"id":"n0.40078647540400847"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.9680237366661995"}],"id":"n0.19941693119236126"}],"id":"n0.9183308773255874"}},"id":"n0.749968146026206"},{"type":"single","text":"(","id":"n0.36590915762485476"},{"text":"s","id":"n0.8817001599358769"},{"type":"single","text":")","id":"n0.7877088141325723"}],"id":"n0.15906262428338502"}],"id":"n0.10589766223614272"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.05246689859301301"}],"style":{"align":"center"},"id":"n0.3289653371420669"}],"shape":{"data":{"p":{"x":563.407531120768,"y":31.217181703707524},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8862399825472123":{"id":"de8862399825472123","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜂","id":"n0.08841301020629855"}],"id":"n0.9389266420440985"}],"id":"n0.838979028267915"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6644917188788857"}],"id":"n0.7384985395864783"}],"shape":{"data":{"p":{"x":517.398973109876,"y":26.45078865972181},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de5631212479888772":{"id":"de5631212479888772","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.9525486490876891"}],"id":"n0.2317967537056933"}],"id":"n0.8247411379987435"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.47255320127532596"}],"id":"n0.08230385127998541"}],"shape":{"data":{"p":{"x":627,"y":170.34364716497083}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de943353730681556":{"id":"de943353730681556","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.5584175853313227"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.6259426616056865"}],"id":"n0.4664845985318422"}],"id":"n0.7533964028274516"}},"id":"n0.3603030527412392"}],"id":"n0.7886272795362079"}],"id":"n0.5054452515819241"}},"id":"n0.8511512956512159"}],"id":"n0.30799020377446107"}],"id":"n0.5973717047898972"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9046484463074862"}],"id":"n0.8574308925216818"}],"shape":{"data":{"p":{"x":201,"y":227.6290170380177}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de7017196159240964":{"id":"de7017196159240964","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.8419303604558264"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8744834530110013"}],"id":"n0.9787111276864338"}],"id":"n0.9250652536355461"}},"id":"n0.8370633037128976"}],"id":"n0.9804800724410077"}],"id":"n0.5276168185965409"}},"id":"n0.16378716658177073"}],"id":"n0.13534933903798363"}],"id":"n0.04010641624309197"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.871833201414649"}],"id":"n0.4971954423167957"}],"shape":{"data":{"p":{"x":438,"y":197.39167897191663}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de8939303688783218":{"id":"de8939303688783218","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⊤","id":"n0.051813233084192944"}],"id":"n0.960716301838975"}],"id":"n0.2991346959721153"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.10743327573701134"}],"id":"n0.4445115508842854"}],"shape":{"data":{"p":{"x":314.31729449710235,"y":171.1441440381019},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de42671147127769893":{"id":"de42671147127769893","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.2105991058479868"}],"id":"n0.6898669597151807"}],"id":"n0.8636088782949856"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.17690363562700084"}],"id":"n0.6977511955253459"}],"shape":{"data":{"p":{"x":104,"y":170.34364716497083}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de0077756148427987615":{"id":"de0077756148427987615","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.7808842253596036"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.8412023551991661"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.2392245969950375"}],"id":"n0.6702209885816119"}],"id":"n0.6981445718985935"}},"id":"n0.18404916440608687"}],"id":"n0.6311475456865279"}],"id":"n0.49059051491697736"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.23131975052950882"}],"id":"n0.7578890736339061"}],"id":"n0.07250555470401698"}},"id":"n0.010866027179482707"}],"id":"n0.22137403373846753"}],"id":"n0.8554662319877668"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.39843064903810554"}],"id":"n0.40498540954485573"}],"shape":{"data":{"p":{"x":64.99359130859375,"y":104.55827729192396}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de9839075823404071":{"id":"de9839075823404071","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.46107283295633916"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.07797177132489064"}],"id":"n0.8192352865137036"}],"id":"n0.8533218395760711"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.2784785651723245"}],"id":"n0.9599880442014379"}],"id":"n0.8570434995157119"}},"id":"n0.4243079250467019"},{"id":"n0.2933130695804871","type":"single","text":"("},{"id":"n0.5444368383855107","text":"s,a"},{"id":"n0.5854650558170484","type":"single","text":")"}],"id":"n0.4664481726460583"}],"id":"n0.3223836254719801"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.5308587113556174"}],"style":{"align":"center"},"id":"n0.7266358655856826"}],"shape":{"data":{"p":{"x":169.9827880859375,"y":162.80245561794527},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1090782511171895":{"id":"de1090782511171895","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.7707876775405613"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.12008251905162615","text":"i"}],"id":"n0.4973178642373326"}],"id":"n0.24065984544285235"}},"id":"n0.20692698822685096"},{"text":"|×H","id":"n0.13077721782901275"},{"id":"n0.6298403962112051","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.1684123085518181","lines":[{"id":"n0.607684858931526","blocks":[{"id":"n0.7642240954984785","text":"j"}]}]}}}],"id":"n0.48014294592380113"}],"id":"n0.12142712283211354"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7113835606186685"}],"style":{"align":"center"},"id":"n0.9140171115099107"}],"shape":{"data":{"p":{"x":146.29996422052108,"y":212.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de27818778541908484":{"id":"de27818778541908484","lines":[{"blocks":[{"id":"n0.19811593342069855","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.27303294008700485","lines":[{"id":"n0.20807316996563263","blocks":[{"id":"n0.8476450789047942","text":"⟨s,a⟩∈"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}}}],"id":"n0.315154072876368"}],"shape":{"data":{"p":{"x":172.2593994140625,"y":188.57013875928538},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5665977907448196":{"id":"de5665977907448196","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"P","id":"n0.307663362192103"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.10623070241454569"}],"id":"n0.8827687096036736"}],"id":"n0.5503718734749985"},"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.8967256030802724"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.46344775539216965"}],"id":"n0.0910101533328953"}],"id":"n0.3890398752134623"}},"id":"n0.7392678537130051"}],"id":"n0.8408046439029846"}],"id":"n0.24075512889589712"}},"id":"n0.24299648297894794"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"∁","id":"n0.9559161988759053"}],"id":"n0.0614877672214893"}],"id":"n0.08636211467259147"}},"id":"n0.8633596343116492"}],"id":"n0.13555213879565464"}],"id":"n0.8868465557438261"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6149708464894408"}],"id":"n0.8085337507563177"}],"shape":{"data":{"p":{"x":173.2593994140625,"y":200.57013875928538},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de30843334298970215":{"id":"de30843334298970215","lines":[{"blocks":[{"id":"n0.32033707080720686","text":"reshape","style":{"fontSize":{"value":0.4}}}],"style":{"align":"center"},"id":"n0.3735752378184525"}],"shape":{"data":{"p":{"x":124.29996422052108,"y":160.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9248573790762489":{"id":"de9248573790762489","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.7603334384584806"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.3217610877936177"},{"id":"n0.21383482447251523","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9825801512442374","lines":[{"id":"n0.07189415363336216","blocks":[{"id":"n0.04384100305856253","text":"j"}]}]}}}],"id":"n0.16362173088793375"}],"id":"n0.16619311131198167"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.6632166449495389"}],"id":"n0.3737897722083008"}],"id":"n0.7585584777622782"}},"id":"n0.2518456284544879"}],"id":"n0.9369673044431397"}],"id":"n0.1167764301657912"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.23477981152773864"}],"id":"n0.6641020234620718"}],"shape":{"data":{"p":{"x":64.99359130859375,"y":125.55827729192396}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de4498440874344303":{"id":"de4498440874344303","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.8588232679304955"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.18868339216376362","text":"j"}],"id":"n0.4414432983578507"}],"id":"n0.08884608357346835"}},"id":"n0.5391030170731603"},{"text":"|","id":"n0.6639977883797332"}],"id":"n0.5903833754603707"}],"id":"n0.33986799877509544"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4046521967791459"}],"style":{"align":"center"},"id":"n0.6302171432238233"}],"shape":{"data":{"p":{"x":51,"y":131.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de19860656186876802":{"id":"de19860656186876802","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.9728792456619699"}],"id":"n0.3614715090637004"}],"id":"n0.31851350704837644"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6103450736207618"}],"id":"n0.22301542229688098"}],"shape":{"data":{"p":{"x":276,"y":170.34364716497083}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de17895393746656385":{"id":"de17895393746656385","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.2225457776491735"}],"style":{"align":"center"},"id":"n0.48149747604985205"}],"shape":{"data":{"p":{"x":342.2999642205211,"y":160.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de0956511130065969":{"id":"de0956511130065969","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.21684088306783855"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8810173732013185"}],"id":"n0.09244370019065884"}],"id":"n0.9908347680288985"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.2171008019923657"}],"id":"n0.7344164383742948"}],"id":"n0.10489682643546083"}},"id":"n0.7092440768028014"},{"type":"single","text":"(","id":"n0.1630181873482086"},{"text":"s,a","id":"n0.32282624326485454"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.45678412884730646","text":"i"}],"id":"n0.0872462204668929"}],"id":"n0.0441292851971995"}},"id":"n0.37481095126090547"},{"type":"single","text":")","id":"n0.029012923234883692"}],"id":"n0.25774265518288164"}],"id":"n0.1846677557628713"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.8537851218944812"}],"style":{"align":"center"},"id":"n0.7254641411995377"}],"shape":{"data":{"p":{"x":390.9827880859375,"y":157.80245561794527},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9168744279554575":{"id":"de9168744279554575","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.8973834832800198"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.08165736455520789","text":"j"}],"id":"n0.19048861557441343"}],"id":"n0.11691188405925867"}},"id":"n0.23522145637931424"},{"text":"|×H","id":"n0.13561582343082956"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4348102888760459","text":"i"}],"id":"n0.9816122324013963"}],"id":"n0.645012438850548"}},"id":"n0.47560350934855466"},{"text":"×W","id":"n0.13212722290639367"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.8609083576254704","text":"i"}],"id":"n0.8165011523965076"}],"id":"n0.7742212388926979"}},"id":"n0.9032057221818466"},{"text":"×|A","id":"n0.05523285678774892"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.6954448285145305","text":"i"}],"id":"n0.9349445110858419"}],"id":"n0.3074719355739637"}},"id":"n0.23130510103780288"},{"text":"|","id":"n0.907281144214686"}],"id":"n0.5592823458575049"}],"id":"n0.8891057395138631"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.03796355660326678"}],"style":{"align":"center"},"id":"n0.87548864355613"}],"shape":{"data":{"p":{"x":373.2999642205211,"y":208.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3279148366297122":{"id":"de3279148366297122","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.9764923833878913"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"o","id":"n0.8545723140790371"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.656088695208134"}],"id":"n0.9423376863555075"}],"id":"n0.05268244245386278"}},"id":"n0.13117074509106152"}],"id":"n0.8149136508863273"}],"id":"n0.5320387796314341"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.6071295041600127"}],"id":"n0.8125459681939333"}],"id":"n0.6267102920693011"}},"id":"n0.12500792441251707"}],"id":"n0.20304082800058465"}],"id":"n0.009969838646760376"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3074931501193965"}],"id":"n0.09711639066157196"}],"shape":{"data":{"p":{"x":66.99359130859375,"y":83.2140237518849}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de37592669576036997":{"id":"de37592669576036997","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.37140121002635285"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.8222042970629553","text":"i"}],"id":"n0.8532041137459934"}],"id":"n0.6723412507106035"}},"id":"n0.43193967528583666"},{"text":"|","id":"n0.29947608577971097"}],"id":"n0.08150258236245111"}],"id":"n0.4797470730986"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5563251825052116"}],"style":{"align":"center"},"id":"n0.256507361805991"}],"shape":{"data":{"p":{"x":51,"y":111.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de21007012170022854":{"id":"de21007012170022854","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|𝛺","id":"n0.36016219737294297"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4393028134718642"}],"id":"n0.6659609798693562"}],"id":"n0.5437564035996625"}},"id":"n0.10133264164423617"},{"text":"|","id":"n0.7224327312760754"}],"id":"n0.4032393424919807"}],"id":"n0.8679679641366074"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7382787493809047"}],"style":{"align":"center"},"id":"n0.3534678316598481"}],"shape":{"data":{"p":{"x":51,"y":90.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4170855423696589":{"id":"de4170855423696589","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.8667350681769705"}],"id":"n0.45712645502986815"}],"id":"n0.6457390848865447"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9794651469988409"}],"id":"n0.5564923070041499"}],"shape":{"data":{"p":{"x":495,"y":170.34364716497083}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8293020670412787":{"id":"de8293020670412787","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⊤","id":"n0.6140443696320139"}],"id":"n0.7432367586553266"}],"id":"n0.07659008397190314"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.868990594364446"}],"id":"n0.9922236445990658"}],"shape":{"data":{"p":{"x":528.3172944971024,"y":171.1441440381019},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de669945869924045":{"id":"de669945869924045","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.34518448981183725"}],"style":{"align":"center"},"id":"n0.8690897824719104"}],"shape":{"data":{"p":{"x":544.2999642205211,"y":160.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8145527982242438":{"id":"de8145527982242438","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.4267226079420261"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.2937109514143881"}],"id":"n0.19683042376548032"}],"id":"n0.5952520400922403"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.062236602762587356"}],"id":"n0.5664962141458856"}],"id":"n0.3577607064246804"}},"id":"n0.09695746678638462"},{"type":"single","text":"(","id":"n0.6281659403480571"},{"text":"s","id":"n0.7022231872432894"},{"type":"single","text":")","id":"n0.185653476301755"}],"id":"n0.12698408810015294"}],"id":"n0.8024924706930465"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.32891985484141095"}],"style":{"align":"center"},"id":"n0.8824838961846289"}],"shape":{"data":{"p":{"x":583.407531120768,"y":172.21718170370752},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6553654751023015":{"id":"de6553654751023015","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.394426262818969"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.23499173389848416"}],"id":"n0.005625112307531932"}],"id":"n0.796539540727877"}},"id":"n0.12271738779981445"},{"text":"×W","id":"n0.34614302360500226"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7421539385815077"}],"id":"n0.35134270037528714"}],"id":"n0.7583559929329973"}},"id":"n0.5521611919047027"},{"text":"×H","id":"n0.36205238542179075"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5906657040606391"}],"id":"n0.2317659176249558"}],"id":"n0.49004230698462936"}},"id":"n0.7758571018564613"},{"text":"×W","id":"n0.24293871410295753"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.005343589685217642"}],"id":"n0.3650620138975105"}],"id":"n0.45390929658934875"}},"id":"n0.5378082324788938"}],"id":"n0.864399840513006"}],"id":"n0.4464515627733918"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6578105722546257"}],"style":{"align":"center"},"id":"n0.40036281772086113"}],"shape":{"data":{"p":{"x":560,"y":193.1120662360471},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4773866742381614":{"id":"de4773866742381614","lines":[{"blocks":[{"text":"Expand along dimensions ","style":{"fontSize":{"value":0.4}},"id":"n0.4777894131524951"},{"id":"n0.8336835840112506","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.766638339102051","lines":[{"id":"n0.7058263596247902","blocks":[{"id":"n0.766599551830595","text":"H"},{"id":"n0.06466344616431674","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.0037084846037074293","lines":[{"id":"n0.18954123602279727","blocks":[{"id":"n0.7103732797925326","text":"j"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}}},{"id":"n0.12596522527849463","text":",","style":{"fontSize":{"value":0.4}}},{"id":"n0.810974683227552","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.47147723642626493","lines":[{"id":"n0.6254596818194615","blocks":[{"id":"n0.516270729737571","text":"W"},{"id":"n0.6497664086249271","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6505778140428289","lines":[{"id":"n0.42528586649288136","blocks":[{"id":"n0.10351850513902994","text":"j"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}}}],"style":{"align":"center"},"id":"n0.675126439532246"}],"shape":{"data":{"p":{"x":214.29996422052108,"y":19.805869211094375},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de39442010604872957":{"id":"de39442010604872957","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.14714877240293278"}],"id":"n0.13157685618989423"}],"id":"n0.23581435920432314"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6573834073407789"}],"id":"n0.5823267703072419"}],"shape":{"data":{"p":{"x":395.99359130859375,"y":28.905746459960938}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de0411298464122003":{"id":"de0411298464122003","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.980927202048494"}],"id":"n0.974705051418195"}],"id":"n0.47526699081088797"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5398708628961781"}],"id":"n0.2768969188858561"}],"shape":{"data":{"p":{"x":363.99359130859375,"y":28.870376586914062}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de7388266462341742":{"id":"de7388266462341742","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.5071050351318276"}],"style":{"align":"center"},"id":"n0.13105491006599146"}],"shape":{"data":{"p":{"x":247.29996422052108,"y":32.805869211094375},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de0830381032376537":{"id":"de0830381032376537","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.8965425373877725","type":"composite","text":"\\Pr","elements":{}},{"id":"n0.3442353613415672","type":"single","text":"("},{"id":"n0.0845208498103871","text":"o"},{"id":"n0.31676876570778445","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.4690998683411016","lines":[{"id":"n0.1330729774493402","blocks":[{"id":"n0.5730378908635343","text":"i"}]}]}}},{"id":"n0.5475042978382414","text":"|s,a"},{"id":"n0.35289670728570566","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5110242207761153","lines":[{"id":"n0.7948905322565856","blocks":[{"id":"n0.30612191359910423","text":"i"}]}]}}},{"id":"n0.3831480288091813","type":"single","text":")"}],"id":"n0.18446577248835783"}],"id":"n0.7503090051164691"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6385329125259112"}],"style":{"align":"center"},"id":"n0.6832618478377599"}],"shape":{"data":{"p":{"x":436.6178159936692,"y":31.565967721611457},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7458997970769539":{"id":"de7458997970769539","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.0718166669177347"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3168480525463271"}],"id":"n0.12648840840709297"}],"id":"n0.15890614400874914"}},"id":"n0.7519119373679519"},{"text":"×W","id":"n0.5920452203425906"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.1776212629466427"}],"id":"n0.14108349465921566"}],"id":"n0.03706276421585164"}},"id":"n0.21062676702879468"},{"text":"×H","id":"n0.05552562153997176"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.06280782700699583"}],"id":"n0.9425552972309041"}],"id":"n0.2761944122243878"}},"id":"n0.2635350789248214"},{"text":"×W","id":"n0.13676684268811634"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.319378960058051"}],"id":"n0.3927870336843269"}],"id":"n0.908260687161133"}},"id":"n0.26239027238645707"}],"id":"n0.7568409456873406"}],"id":"n0.24506231822248026"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7432260243774154"}],"style":{"align":"center"},"id":"n0.007628739367402604"}],"shape":{"data":{"p":{"x":418.9756827354431,"y":51.26288890838623},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2003253275462542":{"id":"de2003253275462542","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.05993666967703404"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9042661943311023"}],"id":"n0.9386350158346954"}],"id":"n0.3995965561196029"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.4199011904587484"}],"id":"n0.8247882463362652"}],"id":"n0.3247054696277607"}},"id":"n0.8299140372309248"},{"type":"single","text":"(","id":"n0.6623530921690994"},{"text":"s","id":"n0.43889332452392593"},{"type":"single","text":")","id":"n0.08122931977256154"}],"id":"n0.14447215791313917"}],"id":"n0.8685308613044107"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.9383609344299102"}],"style":{"align":"center"},"id":"n0.42613163751687644"}],"shape":{"data":{"p":{"x":583.407531120768,"y":273.2171817037075},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7565797893523323":{"id":"de7565797893523323","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.8002262262900506"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.24564655302018923"}],"id":"n0.3088543549628897"}],"id":"n0.8515017815217956"}},"id":"n0.3413536317663919"},{"text":"×W","id":"n0.016568973436302148"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5749350813051146"}],"id":"n0.8332324771261821"}],"id":"n0.4520368826794676"}},"id":"n0.7656998147065233"},{"text":"×H","id":"n0.584135691491046"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.4105217232748377"}],"id":"n0.7144078818603381"}],"id":"n0.5926601031321859"}},"id":"n0.8384180698480208"},{"text":"×W","id":"n0.5376518715799503"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.6088208828591788"}],"id":"n0.526078288818403"}],"id":"n0.33542278812265924"}},"id":"n0.8176488346950643"}],"id":"n0.5064483700922966"}],"id":"n0.6615254849573731"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.1349214364108775"}],"style":{"align":"center"},"id":"n0.7067476805507515"}],"shape":{"data":{"p":{"x":561,"y":294.1120662360471},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5290652384541861":{"id":"de5290652384541861","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.46027237797742626"}],"id":"n0.7177733724273605"}],"id":"n0.6097892962585569"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5473614520072723"}],"id":"n0.9341008659211252"}],"shape":{"data":{"p":{"x":479.9827880859375,"y":28.49939362493177}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de46277186945107696":{"id":"de46277186945107696","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.46771412146034685"}],"style":{"align":"center"},"id":"n0.8110806422154855"}],"shape":{"data":{"p":{"x":352.00939941406244,"y":260.80245561794527},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8463101795697547":{"id":"de8463101795697547","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.2602801313897891"}],"id":"n0.38287986979292277"}],"id":"n0.9651448539051894"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.1141182818123545"}],"id":"n0.8571368685375644"}],"shape":{"data":{"p":{"x":412.99359130859375,"y":270.90574645996094}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de857602324837198":{"id":"de857602324837198","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.1568773903181273"}],"id":"n0.8420086078291884"}],"id":"n0.4282342875453744"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.2084298801907456"}],"id":"n0.7275271279585349"}],"shape":{"data":{"p":{"x":380.99359130859375,"y":270.87037658691406}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9277590802208895":{"id":"de9277590802208895","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.14144761073521783"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6978940101307265"}],"id":"n0.9882271030569612"}],"id":"n0.7190211040442582"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.05348292174395319"}],"id":"n0.6020659708555867"}],"id":"n0.07516815562681134"}},"id":"n0.4392028187363797"},{"type":"single","text":"(","id":"n0.32049668130328013"},{"text":"s,a","id":"n0.8665530680262943"},{"type":"single","text":")","id":"n0.9212341774477784"}],"id":"n0.8414305306060739"}],"id":"n0.2339738641536926"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.4325019727590309"}],"style":{"align":"center"},"id":"n0.7391255984161547"}],"shape":{"data":{"p":{"x":318.15324163402437,"y":254.80245561794527},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6680758227104713":{"id":"de6680758227104713","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.38809881048380124"}],"id":"n0.03754649801948018"}],"id":"n0.9286164676290005"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7589032828734961"}],"id":"n0.3501760318677496"}],"shape":{"data":{"p":{"x":53,"y":208.34364716497083}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de33451906419634647":{"id":"de33451906419634647","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"id":"n0.8372553384111951","text":"X"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.5872417922678372"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.03830798375830846"}],"id":"n0.17834281279956343"}],"id":"n0.235315821971545"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.6277978845181515"}],"id":"n0.94137873539362"}],"id":"n0.5946312346390881"}},"id":"n0.7000175404116691"}],"id":"n0.1963309157355273"}],"id":"n0.4401800566575105"}},"id":"n0.9516233886005141"},{"type":"single","text":"(","id":"n0.5407370816987096"},{"text":"s,a","id":"n0.6564324879943835"},{"type":"single","text":")","id":"n0.48642615921601484"}],"id":"n0.4237285521604277"}],"id":"n0.20649554028200523"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5481037893136345"}],"style":{"align":"center"},"id":"n0.012275783186388889"}],"shape":{"data":{"p":{"x":57.40112242936175,"y":260.20880845297444},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de23024235703851592":{"id":"de23024235703851592","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.9291547683556114"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.5163815412944552","text":"i"}],"id":"n0.18972846315785996"}],"id":"n0.5700081006974362"}},"id":"n0.9827207480147806"},{"text":"×W","id":"n0.2084825202211329"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4251312613811131","text":"i"}],"id":"n0.40357285884537597"}],"id":"n0.08454621183956479"}},"id":"n0.006496406810263533"},{"text":"×H","id":"n0.5574819716886936"},{"id":"n0.8461517982433133","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.32111423845020015","lines":[{"id":"n0.2699080480690079","blocks":[{"id":"n0.8186288242446029","text":"j"}]}]}}}],"id":"n0.8072900678294179"}],"id":"n0.8962696595786119"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.794439420444337"}],"style":{"align":"center"},"id":"n0.06738415328718728"}],"shape":{"data":{"p":{"x":10,"y":302.6290170380177},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de39900376536250404":{"id":"de39900376536250404","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.2723198198313941"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9591550340193618"}],"id":"n0.5964767574562275"}],"id":"n0.6551061619768701"}},"id":"n0.07094054403522487"},{"text":"×W","id":"n0.4674033076598587"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.30931752182513406"}],"id":"n0.5516107555819181"}],"id":"n0.2408426998855402"}},"id":"n0.9568216286077658"},{"text":"×H","id":"n0.2782871445677946"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.18382258695628395"}],"id":"n0.5935551549083624"}],"id":"n0.5186587852573017"}},"id":"n0.6780650757034818"},{"text":"×W","id":"n0.13629958420015487"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.19496263696955318"}],"id":"n0.2519479940241587"}],"id":"n0.24152246688556933"}},"id":"n0.38140606080332695"}],"id":"n0.08267215938659933"}],"id":"n0.7023420069695498"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.16188461314545588"}],"style":{"align":"center"},"id":"n0.38597499972620275"}],"shape":{"data":{"p":{"x":540.3810645367254,"y":50.80793110814713},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1403991638934048":{"id":"de1403991638934048","lines":[{"blocks":[{"text":"Env map for agent ","style":{"fontSize":{"value":0.4}},"id":"n0.9712413089337955"},{"id":"n0.20032978619065522","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.04625616876755467","lines":[{"id":"n0.2585342501714727","blocks":[{"id":"n0.867836739311739","text":"i"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}}}],"style":{"align":"center"},"id":"n0.3435864613679471"}],"shape":{"data":{"p":{"x":18.107566900246866,"y":48.65347228287732},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de21276987906964906":{"id":"de21276987906964906","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.4093467247683491","text":"O"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8166139838940352"}],"id":"n0.043042421802454545"}],"id":"n0.3127550529781269"}},"id":"n0.4603781322459519"},{"type":"single","text":"(","id":"n0.7321504678612816"},{"text":"s,a","id":"n0.005065657196590356"},{"id":"n0.6976724784573709","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.25955722025508643","lines":[{"id":"n0.009544485526986168","blocks":[{"id":"n0.11863656857749305","text":"i"}]}]}}},{"text":",o","id":"n0.2549026018291045"},{"id":"n0.8588600373699287","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.3178461024367669","lines":[{"id":"n0.4778072763325152","blocks":[{"id":"n0.0016428669114334493","text":"i"}]}]}}},{"type":"single","text":")","id":"n0.8624895098210799"}],"id":"n0.8847247660066546"}],"id":"n0.23124838131896186"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5728168841051675"}],"style":{"align":"center"},"id":"n0.16039627818252766"}],"shape":{"data":{"p":{"x":318.4011224293617,"y":17.681440548064366},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de6967035079120742":{"id":"de6967035079120742","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"O","id":"n0.7663962241632654"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7473083347132004"}],"id":"n0.2703144490961966"}],"id":"n0.1991865376500357"}},"id":"n0.5882428150387884"},{"type":"single","text":"(","id":"n0.03746013119834379"},{"text":"s","id":"n0.1985457752930604"},{"id":"n0.5376262985786864","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9078990163736704","lines":[{"id":"n0.5338368310554413","blocks":[{"id":"n0.20146336820493738","text":"i"}]}]}}},{"text":",a","id":"n0.15356174462514338"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4917042302820358"}],"id":"n0.3646442975237121"}],"id":"n0.8832778644999733"}},"id":"n0.6012821954948677"},{"text":",o","id":"n0.292345748241547"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.883382721516984"}],"id":"n0.5450711900828653"}],"id":"n0.191353720293008"}},"id":"n0.44608469355529423"},{"type":"single","text":")","id":"n0.12310447143393777"}],"id":"n0.8935425919742013"}],"id":"n0.5653478407878947"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6368133830903722"}],"style":{"align":"center"},"id":"n0.5620708150660785"}],"shape":{"data":{"p":{"x":178.94530465440607,"y":29.072458095222885},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de41779621283020885":{"id":"de41779621283020885","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.31808763908175397","text":"T"},{"id":"n0.7811607469746116","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9934384487042336","lines":[{"id":"n0.8249034781604134","blocks":[{"id":"n0.38552263098111217","text":"i"}]}]}}}],"id":"n0.5966198281161046"}],"id":"n0.03826225597296773"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7099380664464363"}],"id":"n0.4556250393584236"}],"shape":{"data":{"p":{"x":223,"y":256.6290170380177}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de34251506853038727":{"id":"de34251506853038727","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"3D channel-wise conv layer","id":"n0.45099606085613075"}],"id":"n0.9168304829570921"}],"shape":{"data":{"p":{"x":492.5,"y":158.59364716497083},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de0897703378860828":{"id":"de0897703378860828","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.7713406074602509"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×3×3×|A","id":"n0.8795321550721087"},{"id":"n0.23366925302629848","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2933669962193266","lines":[{"id":"n0.5282555781020577","blocks":[{"id":"n0.15873731962818005","text":"i"}]}]}}},{"text":"|×|A","id":"n0.6430833826318751"},{"id":"n0.4466440054019756","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6784456112344799","lines":[{"id":"n0.481923060795445","blocks":[{"id":"n0.16599295159904703","text":"i"}]}]}}},{"text":"|","id":"n0.8858597521722005"}],"id":"n0.27010289520160713"}],"id":"n0.4916509212070379"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7014747910320709"}],"id":"n0.6812788064366586"}],"shape":{"data":{"p":{"x":485.5,"y":155.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de660336245025593":{"id":"de660336245025593","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.9199440943311219"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1","id":"n0.5215522760989746"}],"id":"n0.7509404326875604"}],"id":"n0.2816604439341721"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5875591290851307"}],"id":"n0.5860391761773773"}],"shape":{"data":{"p":{"x":479.5,"y":174.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9591453651554063":{"id":"de9591453651554063","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"3D channel-wise conv layer","id":"n0.05191440829554517"}],"id":"n0.17237313422475875"}],"shape":{"data":{"p":{"x":252.5,"y":159.59364716497083},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de45735341519520456":{"id":"de45735341519520456","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.3314400328996967"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×3×3×|A","id":"n0.2917759348473479"},{"id":"n0.3609113348534887","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9335465805122038","lines":[{"id":"n0.8435857768293036","blocks":[{"id":"n0.6881939329826796","text":"j"}]}]}}},{"text":"|×|A","id":"n0.5101759115117066"},{"id":"n0.18745062227453024","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.42588280166580916","lines":[{"id":"n0.7479203928049911","blocks":[{"id":"n0.12498090824807195","text":"j"}]}]}}},{"text":"|","id":"n0.9622768332023766"}],"id":"n0.19712993762208386"}],"id":"n0.8920883669508386"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.08525903771344989"}],"id":"n0.5251548027051971"}],"shape":{"data":{"p":{"x":245.5,"y":156.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de52514505709446":{"id":"de52514505709446","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.21377116286758535"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1","id":"n0.8243123237640093"}],"id":"n0.29355940165675376"}],"id":"n0.004686903710433121"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.027630590179415826"}],"id":"n0.7395885647252762"}],"shape":{"data":{"p":{"x":239.5,"y":175.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de117272111129469":{"id":"de117272111129469","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"4D channel-wise conv layer","id":"n0.9306252205114571"}],"id":"n0.39657295829914774"}],"shape":{"data":{"p":{"x":277.5,"y":236.59364716497083},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de7615362257186091":{"id":"de7615362257186091","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.4130287381629909"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3×3×3×3×|A|×|A|","id":"n0.36715312468569916"}],"id":"n0.3200974499624347"}],"id":"n0.08237313594205076"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3510258372240125"}],"id":"n0.6116826147621695"}],"shape":{"data":{"p":{"x":270.5,"y":230.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6516545387625636":{"id":"de6516545387625636","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.500807289500258"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1×1","id":"n0.8113093053356222"}],"id":"n0.35291789532253914"}],"id":"n0.8258704275455162"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6295809682720299"}],"id":"n0.17484403301633678"}],"shape":{"data":{"p":{"x":264.5,"y":246.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de10870917208802044":{"id":"de10870917208802044","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.6447790487623963"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.6169936476655333"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.045612797957085505"}],"id":"n0.22292745515142354"}],"id":"n0.8415070752340081"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.8563935651909795"}],"id":"n0.9684488874652912"}],"id":"n0.5774917245565432"}},"id":"n0.7034740122979639"}],"id":"n0.07669296594331176"}],"id":"n0.0994922811168637"}},"id":"n0.8242576641109514"},{"type":"single","text":"(","id":"n0.5749209994620474"},{"text":"s,a","id":"n0.5092861365050867"},{"type":"single","text":")","id":"n0.5051619485545153"}],"id":"n0.16051818902884407"}],"id":"n0.3114158995400982"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.14258793098244626"}],"style":{"align":"center"},"id":"n0.9960370761185398"}],"shape":{"data":{"p":{"x":116.40112242936175,"y":222.53370987198798},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3162967005585082":{"id":"de3162967005585082","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×H","id":"n0.5084690952694362"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.82135938647904"}],"id":"n0.35478653377661695"}],"id":"n0.23011811938807103"}},"id":"n0.4848196183730935"},{"text":"×W","id":"n0.40299386914870117"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.03503589739992141"}],"id":"n0.9852695233050719"}],"id":"n0.5841533398669001"}},"id":"n0.7007170507377265"}],"id":"n0.2738713707452638"}],"id":"n0.832831636206383"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9604007485113473"}],"style":{"align":"center"},"id":"n0.6776359740492512"}],"shape":{"data":{"p":{"x":20,"y":192.1120662360471},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2104159824026235":{"id":"de2104159824026235","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.7876280219507019"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6290273553863923"}],"id":"n0.07730342401283585"}],"id":"n0.09106588172363139"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.13182050895445974"}],"id":"n0.8009488580250363"}],"id":"n0.28390283275685135"}},"id":"n0.7189470474140787"},{"type":"single","text":"(","id":"n0.9200273278034197"},{"text":"s,a","id":"n0.646388645726921"},{"type":"single","text":")","id":"n0.9214108582392662"}],"id":"n0.19072972727490445"}],"id":"n0.44294341390001013"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.9221759651055457"}],"style":{"align":"center"},"id":"n0.8601035183982335"}],"shape":{"data":{"p":{"x":171.9827880859375,"y":261.80245561794527},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8990960063160915":{"id":"de8990960063160915","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⟨s,a⟩∈P","id":"n0.39889804243963156"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.11906623756041412"}],"id":"n0.2572134513703166"}],"id":"n0.12924158531451835"},"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.6116493305333659"}],"id":"n0.4929970812996085"}],"id":"n0.9343545064639578"}},"id":"n0.8359040854265134"}],"id":"n0.2555656084479139"}],"id":"n0.8001658363143611"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.19978794391158705"}],"id":"n0.578648975033156"}],"shape":{"data":{"p":{"x":171.2593994140625,"y":293.5701387592854},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8745360752140423":{"id":"de8745360752140423","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×W","id":"n0.14771945004597176"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8206652003562014"}],"id":"n0.3071335603483367"}],"id":"n0.0070596474573974"}},"id":"n0.2986233368509299"},{"text":"×|A","id":"n0.6465069551089713"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6825004675603832"}],"id":"n0.029569346878788982"}],"id":"n0.2641187807105312"}},"id":"n0.16309711346390343"},{"text":"|×|A","id":"n0.13113792884500786"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.150293276858394"}],"id":"n0.9495867001768996"}],"id":"n0.3505805194696199"}},"id":"n0.9680356977111231"},{"text":"|","id":"n0.4968696429602695"}],"id":"n0.960824309431972"}],"id":"n0.7546823378521905"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8550027525837427"}],"style":{"align":"center"},"id":"n0.3285386933870884"}],"shape":{"data":{"p":{"x":9,"y":309.95391845703125},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9681358751947411":{"id":"de9681358751947411","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.6735155867197911"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.822951003368392"}],"id":"n0.3875169435950563"}],"id":"n0.5393744984404478"}},"id":"n0.015158075214938282"},{"text":"×W","id":"n0.9328996247353945"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.23811111870702528"}],"id":"n0.7304818694832187"}],"id":"n0.71047928281358"}},"id":"n0.19056974257318737"},{"text":"×H","id":"n0.3445684342557569"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.022240047955429443"}],"id":"n0.09543772425738717"}],"id":"n0.5356780984386695"}},"id":"n0.7251456758815455"}],"id":"n0.7675969773404887"}],"id":"n0.7185940494962384"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.26479353790136995"}],"style":{"align":"center"},"id":"n0.07069884526832615"}],"shape":{"data":{"p":{"x":115,"y":299.6290170380177},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6804744066955923":{"id":"de6804744066955923","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×W","id":"n0.7254971108419839"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8556966236175492"}],"id":"n0.6256926549735815"}],"id":"n0.7314977349612517"}},"id":"n0.9220443438229273"},{"text":"×|A","id":"n0.5642899003657063"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3047713439072508"}],"id":"n0.2869302910733671"}],"id":"n0.2632708866522573"}},"id":"n0.4425430359350071"},{"text":"×A","id":"n0.5442896384796381"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.9472826684666635"}],"id":"n0.7388989824221315"}],"id":"n0.8540986958813741"}},"id":"n0.8917579792144881"},{"text":"|","id":"n0.174251111004877"}],"id":"n0.15127848760257478"}],"id":"n0.934508072726157"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9783427957246185"}],"style":{"align":"center"},"id":"n0.330671341117847"}],"shape":{"data":{"p":{"x":114,"y":306.95391845703125},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5301995220615792":{"id":"de5301995220615792","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×W","id":"n0.6117308415951288"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.40483598555446476"}],"id":"n0.6840556074512587"}],"id":"n0.6126873023620558"}},"id":"n0.063179090824099"},{"text":"×|A","id":"n0.9336298325406398"},{"id":"n0.5162968033203927","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.3059733431069611","lines":[{"id":"n0.6706970193389152","blocks":[{"id":"n0.5994754649617351","text":"i"}]}]}}},{"text":"×A","id":"n0.4450143072946269"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.49680642770751104"}],"id":"n0.32082172568795664"}],"id":"n0.960799079841429"}},"id":"n0.164921740577342"},{"text":"|","id":"n0.541991390065071"}],"id":"n0.8705964676783371"}],"id":"n0.7840692535254685"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6362533217886697"}],"style":{"align":"center"},"id":"n0.8382510826015033"}],"shape":{"data":{"p":{"x":145.29996422052108,"y":220.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de45379357826059574":{"id":"de45379357826059574","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.863071493418518"}],"style":{"align":"center"},"id":"n0.8446101747497616"}],"shape":{"data":{"p":{"x":108.00939941406244,"y":283.80245561794527},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di5159292854007935","items":[],"style":{}},"shapes":[{"id":"dp6622237718632957","type":"doc-cube","data":{"p1":{"x":152.89243309975313,"y":175.09592243721903},"p2":{"x":195.15612200055915,"y":212.80586921109438},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp7977048112572978","type":"doc-cube","data":{"p1":{"x":152.89243309975313,"y":142.79350678411146},"p2":{"x":195.15612200055915,"y":180.50345355798692},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dg8483270993201228","entities":[{"id":"dp7384638156337533","type":"rectangle","data":{"p1":{"x":157.85418515207553,"y":5.994717392586722},"p2":{"x":189.90884998009108,"y":35.37046218993311}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp2742804657475568","type":"rectangle","data":{"p1":{"x":161.1701851799656,"y":9.033587743904832},"p2":{"x":193.22485000798127,"y":38.4093325412511}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp8917185552111246","type":"rectangle","data":{"p1":{"x":164.4861852078557,"y":12.072458095222885},"p2":{"x":196.54085003587147,"y":41.44820289256921}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"dg22710741968910475","entities":[{"id":"dg1612353785263314","entities":[{"id":"dp8411049564449569","type":"rectangle","data":{"p1":{"x":63.99359130859375,"y":109.5402473973582},"p2":{"x":76.6507520406526,"y":122.19740812941706}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp639236493824461","type":"rectangle","data":{"p1":{"x":65.57573640010105,"y":111.12239248886556},"p2":{"x":78.2328971321599,"y":123.77955322092441}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp7897895271166255","type":"rectangle","data":{"p1":{"x":67.15788149160846,"y":112.70453758037291},"p2":{"x":79.81504222366732,"y":125.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl9317274722545805","linkedId":"de0077756148427987615"}]},{"id":"dg5022281278414338","entities":[{"id":"dp6584292212823948","type":"rectangle","data":{"p1":{"x":46.76515712043911,"y":40.457077960817855},"p2":{"x":48.87080794747369,"y":42.56272878785251}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7634301089799995","type":"rectangle","data":{"p1":{"x":32.86592987226048,"y":26.557850712639492},"p2":{"x":62.770035195652184,"y":56.461956036031125}},"style":{"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp941185546601065","type":"rectangle","data":{"p1":{"x":60.74970508255704,"y":42.60671136364056},"p2":{"x":62.855355909591694,"y":44.71236219067538}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp12518955187598535","type":"rectangle","data":{"p1":{"x":44.529110485308124,"y":51.82566063705568},"p2":{"x":46.61544341484719,"y":53.911993566594646}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9425702251933581","type":"rectangle","data":{"p1":{"x":53.78238338576345,"y":40.502153054974656},"p2":{"x":55.88803421279809,"y":42.60780388200919}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp15268933323188394","type":"rectangle","data":{"p1":{"x":51.44491778877999,"y":54.40459995273574},"p2":{"x":53.55056861581458,"y":56.510250779770445}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7349145908262524","type":"rectangle","data":{"p1":{"x":35.20629315386839,"y":49.476155713122694},"p2":{"x":37.31194398090304,"y":51.58180654015723}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp018307640963909133","type":"rectangle","data":{"p1":{"x":51.45135708794521,"y":42.794543557801376},"p2":{"x":53.55700791497986,"y":44.900194384836}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9798505615248356","type":"rectangle","data":{"p1":{"x":37.51027439519254,"y":42.5616362694839},"p2":{"x":39.615925222227204,"y":44.66728709651858}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp054134720767317956","type":"rectangle","data":{"p1":{"x":32.97056848369576,"y":47.24300676261623},"p2":{"x":35.0053870199127,"y":49.277825298833136}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp24121436979654787","type":"rectangle","data":{"p1":{"x":53.78238338576338,"y":52.06713435575227},"p2":{"x":55.888034212797976,"y":54.17278518278687}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5483749790467487","type":"rectangle","data":{"p1":{"x":33.07359727033966,"y":30.958019173714746},"p2":{"x":35.0053870199127,"y":35.41401419606339}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7224264188314182","type":"rectangle","data":{"p1":{"x":33.07359727033966,"y":51.827787768269644},"p2":{"x":37.323534719400456,"y":53.88192420198243}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5887727300494723","type":"rectangle","data":{"p1":{"x":35.2372017898615,"y":42.794543557801376},"p2":{"x":41.959830118376004,"y":44.85511929067934}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp16641140208384075","type":"rectangle","data":{"p1":{"x":39.873497188836936,"y":45.05473756480188},"p2":{"x":48.9335911143348,"y":47.131411545592925}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9404293655527154","type":"rectangle","data":{"p1":{"x":39.873497188836936,"y":47.131411545592925},"p2":{"x":44.29729571535945,"y":49.50751293756787}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5790284043711376","type":"rectangle","data":{"p1":{"x":42.191644888324674,"y":49.739327707516736},"p2":{"x":46.61544341484719,"y":51.82566063705568}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp14115968377148302","type":"rectangle","data":{"p1":{"x":56.04257739276399,"y":28.87599841212699},"p2":{"x":60.46637591928632,"y":30.962331341666015}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9911215666839048","type":"rectangle","data":{"p1":{"x":53.78238338576338,"y":31.13619241912761},"p2":{"x":58.20618191228584,"y":33.222525348666636}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9229359877586667","type":"rectangle","data":{"p1":{"x":60.71750858673076,"y":33.334120565689716},"p2":{"x":62.64929833630396,"y":37.69674575014224}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp03975774153187217","type":"rectangle","data":{"p1":{"x":58.45731457973022,"y":33.43824187070231},"p2":{"x":60.52432961177354,"y":37.91677444012913}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp2688864035259695","type":"rectangle","data":{"p1":{"x":60.71750858673076,"y":47.185053070128816},"p2":{"x":62.784523618774045,"y":51.66358563955592}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp49434807172942263","type":"rectangle","data":{"p1":{"x":56.06189529025964,"y":54.433576798979345},"p2":{"x":60.46637591928632,"y":56.40400234354394}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp3547941895884805","type":"rectangle","data":{"p1":{"x":49.146087986787904,"y":38.148589210078086},"p2":{"x":53.569886513310294,"y":40.23492213961691}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp6149100927668762","type":"rectangle","data":{"p1":{"x":42.18681541395077,"y":31.184487162866958},"p2":{"x":44.29246624098542,"y":33.29013798990161}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp6236361675538047","type":"rectangle","data":{"p1":{"x":49.141258512413984,"y":33.50263486235468},"p2":{"x":51.246909339448706,"y":35.608285689389334}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp33083943579870945","type":"rectangle","data":{"p1":{"x":53.777553911389475,"y":47.46947475176819},"p2":{"x":55.883204738424055,"y":49.57512557880307}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp4059609980214478","type":"rectangle","data":{"p1":{"x":56.09570161087714,"y":45.03541966730623},"p2":{"x":58.201352437911794,"y":47.141070494340795}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7983374591042727","type":"rectangle","data":{"p1":{"x":49.141258512413984,"y":28.92429315586645},"p2":{"x":51.246909339448706,"y":31.02994398290113}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp458619221511277","type":"rectangle","data":{"p1":{"x":39.868667714463015,"y":35.82078256184241},"p2":{"x":41.97431854149774,"y":37.92643338887703}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp760537205040309","type":"rectangle","data":{"p1":{"x":51.45940621190172,"y":26.548191763891396},"p2":{"x":53.565057038936374,"y":28.65384259092619}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}}],"data":{"rotation":0}},{"id":"dp491477702765458","type":"rectangle","data":{"p1":{"x":48.78095245361328,"y":31.495927638679916},"p2":{"x":134.78095245361328,"y":55.62555105176587},"rotation":270}},{"id":"dp30550026210942716","type":"rectangle","data":{"p1":{"x":75.91057586669922,"y":31.495927638679916},"p2":{"x":161.91057586669922,"y":55.625551051765896},"rotation":270}},{"id":"dp205081585511121","type":"rectangle","data":{"p1":{"x":133.9753875732422,"y":0.5607393452228777},"p2":{"x":141.9753875732422,"y":86.5607393452229}}},{"id":"da6255417888001278","data":[{"x":62.85535590959171,"y":42.60671136364056},{"x":80.0093994140625,"y":42.60671136364056}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg4057455004606121","entities":[{"id":"dp8829635558448385","type":"rectangle","data":{"p1":{"x":175.3133045986259,"y":21.994717392586722},"p2":{"x":207.36796942664145,"y":51.37046218993311}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp4576128651121294","type":"rectangle","data":{"p1":{"x":178.629304626516,"y":25.03358774390483},"p2":{"x":210.68396945453168,"y":54.4093325412511}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp9782337459077366","type":"rectangle","data":{"p1":{"x":181.94530465440607,"y":28.072458095222885},"p2":{"x":213.99996948242188,"y":57.44820289256921}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"da5095274510017072","data":[{"x":142.0093994140625,"y":42.60671136364056},{"x":163.0093994140625,"y":42.60671136364056}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da7452683182568292","data":[{"x":213.62422468507543,"y":41.44820289256921},{"x":312.0093994140625,"y":41.44820289256921}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp9101006504208546","type":"doc-cube","data":{"p1":{"x":44.909614496237566,"y":162.80965058293958},"p2":{"x":82.99996948242193,"y":200.51959735681504},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da5647146191766867","data":[{"x":82.98209142684937,"y":182.93293158498426},{"x":106.2142333984375,"y":182.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg9521102190475543","entities":[{"id":"dp19818381292907983","type":"circle","data":{"p1":{"x":106.2142333984375,"y":173.1650735565724},"p2":{"x":125.74994945526123,"y":192.70078961339613}}},{"id":"dl5336932286757903","linkedId":"de42671147127769893"}]},{"id":"da8298169380593463","data":[{"x":205.0093994140625,"y":182.93293158498426},{"x":222.0093994140625,"y":182.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg949991068622825","entities":[{"id":"dp019087905739112232","type":"rectangle","data":{"p1":{"x":222.00640869140625,"y":158.80965058293958},"p2":{"x":243.00640869140625,"y":238.80965058293953}}},{"id":"dl6010164519079402","linkedId":"de9591453651554063"},{"id":"dl9415606179860345","linkedId":"de45735341519520456"},{"id":"dl6861227487454671","linkedId":"de52514505709446"}]},{"id":"da2635283354670219","data":[{"x":207.98209142684937,"y":210.55038849797864},{"x":222.0093994140625,"y":210.55038849797864}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da7988329293723304","data":[{"x":297.74994945526123,"y":182.93293158498426},{"x":313.53152789553985,"y":182.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6451961657470695","entities":[{"id":"dp8738376037206987","type":"circle","data":{"p1":{"x":313.53152789553985,"y":172.96557042970352},"p2":{"x":333.0672439523636,"y":192.50128648652725}}},{"id":"dl07766096735198125","linkedId":"de8939303688783218"}]},{"id":"da48869933214538896","data":[{"x":427.0672439523636,"y":182.73342845811538},{"x":462.0093994140625,"y":182.73342845811538}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg9004625109246001","entities":[{"id":"dg3748164866414456","entities":[{"id":"dp5509037023859227","type":"rectangle","data":{"p1":{"x":436,"y":202.37364907735088},"p2":{"x":448.65716073205886,"y":215.03080980940973}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp2177725905865473","type":"rectangle","data":{"p1":{"x":437.58214509150736,"y":203.95579416885823},"p2":{"x":450.2393058235662,"y":216.6129549009171}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp2982156234219324","type":"rectangle","data":{"p1":{"x":439.1642901830147,"y":205.5379392603656},"p2":{"x":451.82145091507357,"y":218.19509999242445}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}}],"data":{}},{"id":"dl04261871052164312","linkedId":"de7017196159240964"}]},{"id":"dg7770051742104693","entities":[{"id":"dg6879742697168143","entities":[{"id":"dp733881807495532","type":"rectangle","data":{"p1":{"x":199,"y":232.61098714345195},"p2":{"x":211.65716073205886,"y":245.2681478755108}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp9571343654651887","type":"rectangle","data":{"p1":{"x":200.58214509150736,"y":234.1931322349593},"p2":{"x":213.2393058235662,"y":246.85029296701816}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp4276722835541409","type":"rectangle","data":{"p1":{"x":202.1642901830147,"y":235.77527732646666},"p2":{"x":214.82145091507357,"y":248.43243805852552}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}}],"data":{}},{"id":"dl3016453782434083","linkedId":"de943353730681556"}]},{"id":"dg8757060045119001","entities":[{"id":"dp4296214797357958","type":"rectangle","data":{"p1":{"x":462.00640869140625,"y":157.80965058293958},"p2":{"x":483.00640869140625,"y":237.80965058293953}}},{"id":"dl3744631857488627","linkedId":"de34251506853038727"},{"id":"dl19816395846600354","linkedId":"de0897703378860828"},{"id":"dl717557293755684","linkedId":"de660336245025593"}]},{"id":"da4096156558091564","data":[{"x":483.0093994140625,"y":182.73342845811538},{"x":497.2142333984375,"y":182.73342845811538}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp19126358492857554","type":"doc-cube","data":{"p1":{"x":297.89243309975313,"y":267.09592243721903},"p2":{"x":340.15612200055915,"y":304.8058692110944},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp7816021932988355","type":"doc-cube","data":{"p1":{"x":297.89243309975313,"y":234.79350678411146},"p2":{"x":340.15612200055915,"y":272.5034535579869},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp5604777893071713","type":"doc-cube","data":{"p1":{"x":308.7457105132565,"y":277.3949244971773},"p2":{"x":351.0093994140625,"y":315.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp7934318242807215","type":"doc-cube","data":{"p1":{"x":308.7457105132565,"y":245.39492449717733},"p2":{"x":351.0093994140625,"y":283.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da5886723440129011","data":[{"x":610.0093994140625,"y":182.73342845811538},{"x":626.2142333984375,"y":182.73342845811538}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg2711048233910618","entities":[{"id":"dp9744063565275916","type":"circle","data":{"p1":{"x":626.2142333984375,"y":173.1650735565724},"p2":{"x":645.7499494552612,"y":192.70078961339613}}},{"id":"dl8909188918888535","linkedId":"de5631212479888772"}]},{"id":"dp6166308761367747","type":"doc-cube","data":{"p1":{"x":550,"y":21.809650582939582},"p2":{"x":588.0903549861844,"y":59.51959735681504},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"dp35984004071735387","type":"right-arrow","data":{"p1":{"x":591.6828238654164,"y":37.01865805716483},"p2":{"x":604.6828238654164,"y":49.523402014684365},"arrowPercentage":0.4}},{"id":"dp20135056334796086","type":"right-arrow","data":{"p1":{"x":27.682823865416367,"y":175.01865805716483},"p2":{"x":40.68282386541637,"y":187.52340201468436},"arrowPercentage":0.4}},{"id":"dg9794871144668333","entities":[{"id":"dp30648019613019284","type":"circle","data":{"p1":{"x":515.6132065083135,"y":31.2722150513234},"p2":{"x":535.1489225651372,"y":50.80793110814713}}},{"id":"dl9290812430313644","linkedId":"de8862399825472123"}]},{"id":"da874563705382023","data":[{"x":207.98209142684937,"y":232.61098714345195},{"x":207.98209142684937,"y":210.55038849797864}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da060468175387625056","data":[{"x":451.98209142684937,"y":210.55038849797864},{"x":462.0093994140625,"y":210.55038849797864}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg9769168345695671","entities":[{"id":"dg7049738960854695","entities":[{"id":"dp6476120928270528","type":"rectangle","data":{"p1":{"x":63.99359130859375,"y":130.5402473973582},"p2":{"x":76.6507520406526,"y":143.19740812941706}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp140945334013155","type":"rectangle","data":{"p1":{"x":65.57573640010105,"y":132.12239248886556},"p2":{"x":78.2328971321599,"y":144.7795532209244}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp6967821362141615","type":"rectangle","data":{"p1":{"x":67.15788149160846,"y":133.70453758037291},"p2":{"x":79.81504222366732,"y":146.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl2867078864360555","linkedId":"de9248573790762489"}]},{"id":"dp2535340361018632","type":"doc-cube","data":{"p1":{"x":163.5752569651695,"y":185.39492449717733},"p2":{"x":205.0093994140625,"y":223.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp9677376167535234","type":"doc-cube","data":{"p1":{"x":163.5752569651695,"y":153.39492449717733},"p2":{"x":205.0093994140625,"y":191.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da816214625717876","data":[{"x":125.74994945526123,"y":182.93293158498426},{"x":153.0093994140625,"y":183.08636474609375}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6055197197769788","entities":[{"id":"dp3484523225939222","type":"circle","data":{"p1":{"x":278.2142333984375,"y":173.1650735565724},"p2":{"x":297.74994945526123,"y":192.70078961339613}}},{"id":"dl7429748158984153","linkedId":"de19860656186876802"}]},{"id":"da2811811086482159","data":[{"x":243.0093994140625,"y":182.93293158498426},{"x":278.2142333984375,"y":182.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9822177726400323","data":[{"x":287.98209142684937,"y":173.1650735565724},{"x":287.98209142684937,"y":139.08636474609375}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da8248729303496711","data":[{"x":80.0093994140625,"y":139.08636474609375},{"x":287.98209142684937,"y":139.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da5594349890606285","data":[{"x":333.0672439523636,"y":182.73342845811538},{"x":385.5752569651695,"y":182.73342845811538}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp1404845983163685","type":"doc-cube","data":{"p1":{"x":385.5752569651695,"y":180.39492449717733},"p2":{"x":427.0093994140625,"y":218.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp10524773268557919","type":"doc-cube","data":{"p1":{"x":385.5752569651695,"y":148.39492449717733},"p2":{"x":427.0093994140625,"y":186.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"dg8484742129714533","entities":[{"id":"dg9038736138675647","entities":[{"id":"dp9996305414061866","type":"rectangle","data":{"p1":{"x":63.99359130859375,"y":88.19599385731914},"p2":{"x":76.6507520406526,"y":100.853154589378}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp21860303704643136","type":"rectangle","data":{"p1":{"x":65.57573640010105,"y":89.7781389488265},"p2":{"x":78.2328971321599,"y":102.43529968088535}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp8561186880022829","type":"rectangle","data":{"p1":{"x":67.15788149160846,"y":91.36028404033385},"p2":{"x":79.81504222366732,"y":104.01744477239271}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl23537597833849233","linkedId":"de3279148366297122"}]},{"id":"da5893669933322039","data":[{"x":79.81504222366732,"y":118.08636474609375},{"x":507.0093994140625,"y":118.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg5470884334023867","entities":[{"id":"dp7943579170689357","type":"circle","data":{"p1":{"x":497.2142333984375,"y":173.1650735565724},"p2":{"x":516.7499494552612,"y":192.70078961339613}}},{"id":"dl41378762513915945","linkedId":"de4170855423696589"}]},{"id":"da6067276147750311","data":[{"x":506.98209142684937,"y":173.1650735565724},{"x":506.98209142684937,"y":118.08636474609375}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da3658460936994632","data":[{"x":516.7499494552612,"y":182.93293158498426},{"x":527.5315278955399,"y":182.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg8290168484072875","entities":[{"id":"dp43094216648041606","type":"circle","data":{"p1":{"x":527.5315278955399,"y":172.96557042970352},"p2":{"x":547.0672439523636,"y":192.50128648652725}}},{"id":"dl37666879315892676","linkedId":"de8293020670412787"}]},{"id":"da9124292323903822","data":[{"x":547.0672439523636,"y":182.73342845811538},{"x":571.0093994140625,"y":182.73342845811538}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp8563869802684876","type":"doc-cube","data":{"p1":{"x":572,"y":162.80965058293958},"p2":{"x":610.0903549861844,"y":200.51959735681504},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da8350532175954528","data":[{"x":635.9820914268494,"y":283.1048712710528},{"x":635.9820914268494,"y":192.70078961339613}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da14438530859309862","data":[{"x":434.743540763855,"y":283.1048712710528},{"x":572.0093994140625,"y":283.1048712710528}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6552341923862859","entities":[{"id":"dp4114310463952291","type":"circle","data":{"p1":{"x":366.20782470703125,"y":31.691802978515625},"p2":{"x":385.743540763855,"y":51.227519035339355}}},{"id":"dl8524192395429857","linkedId":"de0411298464122003"}]},{"id":"da9857160005357748","data":[{"x":352.0093994140625,"y":41.45966100692749},{"x":366.20782470703125,"y":41.45966100692749}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg5361109596292808","entities":[{"id":"dp3737490376357602","type":"circle","data":{"p1":{"x":398.20782470703125,"y":31.7271728515625},"p2":{"x":417.743540763855,"y":51.26288890838623}}},{"id":"dl06797239555156298","linkedId":"de39442010604872957"}]},{"id":"da4043032123170953","data":[{"x":385.743540763855,"y":41.495030879974365},{"x":398.20782470703125,"y":41.495030879974365}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9273551234543298","data":[{"x":417.743540763855,"y":41.495030879974365},{"x":430.0093994140625,"y":41.495030879974365}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da5120502812969023","data":[{"x":375.9756827354431,"y":96.36028404033385},{"x":375.9756827354431,"y":51.227519035339355}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da41002029497127945","data":[{"x":407.9756827354431,"y":118.21600341796875},{"x":407.9756827354431,"y":51.26288890838623}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da027839575910060255","data":[{"x":79.81504222366732,"y":96.36028404033385},{"x":375.9756827354431,"y":96.36028404033385}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp29147501886307037","type":"doc-cube","data":{"p1":{"x":312.99359130859375,"y":41.27390942729642},"p2":{"x":352.0093994140625,"y":78.98385620117188},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp18465950721045088","type":"doc-cube","data":{"p1":{"x":312.99359130859375,"y":9.273909427296417},"p2":{"x":352.0093994140625,"y":46.983856201171875},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp7293007378919645","type":"doc-cube","data":{"p1":{"x":430.99359130859375,"y":22.273909427296417},"p2":{"x":469.0839462947781,"y":59.983856201171875},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp29862627321028845","type":"doc-cube","data":{"p1":{"x":572,"y":263.8096505829396},"p2":{"x":610.0903549861844,"y":301.51959735681504},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da881050927661438","data":[{"x":610.0093994140625,"y":283.1048712710528},{"x":635.9820914268494,"y":283.1048712710528}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da536505232054884","data":[{"x":351.32182448864523,"y":283.1048712710528},{"x":383.20782470703125,"y":283.1048712710528}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg9352496300077404","entities":[{"id":"dp8381260328807054","type":"circle","data":{"p1":{"x":482.197021484375,"y":31.320820016533332},"p2":{"x":501.73273754119873,"y":50.85653607335706}}},{"id":"dl04218115805922773","linkedId":"de5290652384541861"}]},{"id":"da1671169067994731","data":[{"x":469.0093994140625,"y":41.495030879974365},{"x":482.197021484375,"y":41.495030879974365}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da4434413038574352","data":[{"x":491.96487951278687,"y":95.21600341796875},{"x":491.96487951278687,"y":50.85653607335706}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9824275673759653","data":[{"x":491.96487951278687,"y":95.21600341796875},{"x":635.9820914268494,"y":95.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8315863874944149","data":[{"x":635.9820914268494,"y":173.1650735565724},{"x":635.9820914268494,"y":95.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8675175182676189","data":[{"x":501.73273754119873,"y":41.0886780449452},{"x":515.6132065083135,"y":41.0886780449452}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da1706452397478937","data":[{"x":535.1489225651372,"y":41.040073079735265},{"x":549.029391532252,"y":41.040073079735265}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg8999168748503741","entities":[{"id":"dp7767797686105347","type":"circle","data":{"p1":{"x":383.20782470703125,"y":273.6918029785156},"p2":{"x":402.743540763855,"y":293.22751903533936}}},{"id":"dl6027413285167649","linkedId":"de857602324837198"}]},{"id":"dg6669031335846896","entities":[{"id":"dp8030836569988877","type":"circle","data":{"p1":{"x":415.20782470703125,"y":273.7271728515625},"p2":{"x":434.743540763855,"y":293.26288890838623}}},{"id":"dl9104054636494301","linkedId":"de8463101795697547"}]},{"id":"da007300751910995107","data":[{"x":402.743540763855,"y":283.49503087997437},{"x":415.20782470703125,"y":283.49503087997437}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da10649370567532523","data":[{"x":392.9756827354431,"y":330.08636474609375},{"x":392.9756827354431,"y":293.22751903533936}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da4284726936260912","data":[{"x":424.9756827354431,"y":334.08636474609375},{"x":424.9756827354431,"y":293.26288890838623}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da819754312498066","data":[{"x":6.0093994140625,"y":118.08636474609375},{"x":63.81504222366732,"y":118.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da6859220166447162","data":[{"x":10.982091426849365,"y":139.08636474609375},{"x":64.0093994140625,"y":139.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da16116560471307007","data":[{"x":10.982091426849365,"y":330.08636474609375},{"x":392.9756827354431,"y":330.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da4402995226506323","data":[{"x":10.982091426849365,"y":330.08636474609375},{"x":10.982091426849365,"y":139.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da07365458199363362","data":[{"x":6.0093994140625,"y":334.08636474609375},{"x":6.0093994140625,"y":118.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8609599008450401","data":[{"x":6.0093994140625,"y":334.08636474609375},{"x":424.9756827354431,"y":334.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg18633038966604198","entities":[{"id":"dp23789513342027635","type":"rectangle","data":{"p1":{"x":247.00640869140625,"y":231.08636474609375},"p2":{"x":268.00640869140625,"y":321.08636474609375}}},{"id":"dl5964117034027434","linkedId":"de117272111129469"},{"id":"dl43136719617667074","linkedId":"de7615362257186091"},{"id":"dl848449371733256","linkedId":"de6516545387625636"}]},{"id":"da8132116984781697","data":[{"x":235.98209142684937,"y":269.55038849797864},{"x":247.0093994140625,"y":269.55038849797864}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da2679111615406278","data":[{"x":268.0093994140625,"y":267.09592243721903},{"x":297.8924330997532,"y":267.09592243721903}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg2436496973924449","entities":[{"id":"dp8472658757800087","type":"circle","data":{"p1":{"x":55.2142333984375,"y":211.1650735565724},"p2":{"x":74.74994945526123,"y":230.70078961339613}}},{"id":"dl6546463077814686","linkedId":"de6680758227104713"}]},{"id":"da7870207852415669","data":[{"x":64.98209142684937,"y":211.1650735565724},{"x":64.98209142684937,"y":200.55038849797864}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"dp19398203200317687","type":"doc-cube","data":{"p1":{"x":39.31076744317738,"y":273.5022752722482},"p2":{"x":77.40112242936175,"y":311.21222204612354},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp09881308613683815","type":"doc-cube","data":{"p1":{"x":39.31076744317738,"y":241.19985961914062},"p2":{"x":77.40112242936175,"y":278.9098063930161},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp45325200116230313","type":"doc-cube","data":{"p1":{"x":49.99359130859375,"y":283.8012773322065},"p2":{"x":88.08394629477812,"y":321.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp7083211951380533","type":"doc-cube","data":{"p1":{"x":49.99359130859375,"y":251.8012773322065},"p2":{"x":88.08394629477812,"y":289.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da6699254290055761","data":[{"x":93.0093994140625,"y":290.93293158498426},{"x":154.0093994140625,"y":290.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da5597155529763433","data":[{"x":64.98209142684937,"y":241.51122410608195},{"x":64.98209142684937,"y":230.70078961339613}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg299842150815365","entities":[{"id":"dp8541761199432887","type":"doc-cube","data":{"p1":{"x":219.62434362521276,"y":261.21600341796875},"p2":{"x":236.08394629477812,"y":277.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dl3981580537257483","linkedId":"de41779621283020885"}]},{"id":"dp1231293400345943","type":"doc-cube","data":{"p1":{"x":98.31076744317738,"y":235.82717669126174},"p2":{"x":136.40112242936175,"y":273.5371234651371},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp9189534433042095","type":"doc-cube","data":{"p1":{"x":98.31076744317738,"y":203.52476103815417},"p2":{"x":136.40112242936175,"y":241.23470781202963},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp07285677194005613","type":"doc-cube","data":{"p1":{"x":108.99359130859375,"y":246.12617875122004},"p2":{"x":147.08394629477812,"y":283.8361255250955},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp5541115348388084","type":"doc-cube","data":{"p1":{"x":108.99359130859375,"y":214.12617875122004},"p2":{"x":147.08394629477812,"y":251.8361255250955},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da7225287201552757","data":[{"x":115.98209142684937,"y":203.51122410608195},{"x":115.98209142684937,"y":192.70078961339613}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da1495707413591436","data":[{"x":74.74994945526123,"y":220.93293158498426},{"x":93.0093994140625,"y":220.93293158498426}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9737361179617816","data":[{"x":93.0093994140625,"y":290.93293158498426},{"x":93.0093994140625,"y":220.93293158498426}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp47773940152606587","type":"doc-cube","data":{"p1":{"x":153.89243309975313,"y":274.09592243721903},"p2":{"x":196.15612200055915,"y":311.8058692110944},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp6190514455540355","type":"doc-cube","data":{"p1":{"x":153.89243309975313,"y":241.79350678411146},"p2":{"x":196.15612200055915,"y":279.5034535579869},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp39046556118951337","type":"doc-cube","data":{"p1":{"x":164.5752569651695,"y":284.3949244971773},"p2":{"x":206.0093994140625,"y":322.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp9887279274745566","type":"doc-cube","data":{"p1":{"x":164.5752569651695,"y":252.39492449717733},"p2":{"x":206.0093994140625,"y":290.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da9292084301369448","data":[{"x":206.0093994140625,"y":290.93293158498426},{"x":247.0093994140625,"y":290.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6}],"settings":{"grid":true,"diagramHeight":337.95391845703125}}]},{"id":"n0.8643197968059031","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":5643,"delayRenderCache":{"av":5643,"map":{"n0.12264719501879284":{"n0.22684036926304696":{"w":90.6576,"h":8.4545,"bl":0.8214}},"n0.28195840591444044":{"n0.9045013624179807":{"w":64.6792,"h":8.4545,"bl":0.8214}},"n0.00554654937310417":{"n0.8635446728446938":{"w":42.164,"h":8.1019,"bl":0.8571}},"n0.7636721946274969":{"n0.7635730023714855":{"w":55.9986,"h":8.4545,"bl":0.8214}},"n0.3566822829252332":{"n0.27881606013744675":{"w":86.3173,"h":8.4545,"bl":0.8214}},"n0.4916509212070379":{"n0.27010289520160713":{"w":61.4873,"h":8.4545,"bl":0.8214}},"n0.2816604439341721":{"n0.7509404326875604":{"w":24.7215,"h":8.1019,"bl":0.8571}},"n0.004686903710433121":{"n0.29355940165675376":{"w":24.7215,"h":8.1019,"bl":0.8571}},"n0.8920883669508386":{"n0.19712993762208386":{"w":61.9755,"h":8.4545,"bl":0.8214}},"n0.8068253129909273":{"n0.008391880325343104":{"w":22.4157,"h":12.5054,"bl":0.7021}},"n0.10589766223614272":{"n0.15906262428338502":{"w":15.8511,"h":12.5054,"bl":0.7021}},"n0.5973717047898972":{"n0.30799020377446107":{"w":6.9897,"h":9.4491,"bl":0.8402}},"n0.04010641624309197":{"n0.13534933903798363":{"w":6.7455,"h":9.4491,"bl":0.8402}},"n0.8554662319877668":{"n0.22137403373846753":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.2742966032445735":{"n0.9115976780097668":{"w":22.8226,"h":8.4545,"bl":0.8214}},"n0.12142712283211354":{"n0.48014294592380113":{"w":24.5135,"h":8.4545,"bl":0.8214}},"n0.3223836254719801":{"n0.4664481726460583":{"w":30.0022,"h":12.5054,"bl":0.7021}},"n0.27303294008700485":{"n0.20807316996563263":{"w":21.8099,"h":8.1019,"bl":0.8571}},"n0.8868465557438261":{"n0.13555213879565464":{"w":12.424,"h":12.5326,"bl":0.8268}},"n0.33986799877509544":{"n0.5903833754603707":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.8891057395138631":{"n0.5592823458575049":{"w":58.5033,"h":8.4545,"bl":0.8214}},"n0.1846677557628713":{"n0.25774265518288164":{"w":32.4165,"h":12.5054,"bl":0.7021}},"n0.009969838646760376":{"n0.20304082800058465":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.4797470730986":{"n0.08150258236245111":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.8679679641366074":{"n0.4032393424919807":{"w":11.6193,"h":8.4545,"bl":0.8214}},"n0.4464515627733918":{"n0.864399840513006":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.8024924706930465":{"n0.12698408810015294":{"w":18.1297,"h":12.5054,"bl":0.7021}},"n0.766638339102051":{"n0.7058263596247902":{"w":7.4599,"h":8.4545,"bl":0.8214}},"n0.47147723642626493":{"n0.6254596818194615":{"w":8.5901,"h":8.4545,"bl":0.8214}},"n0.1167764301657912":{"n0.9369673044431397":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.7503090051164691":{"n0.18446577248835783":{"w":28.9352,"h":8.4545,"bl":0.8214}},"n0.24506231822248026":{"n0.7568409456873406":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.6615254849573731":{"n0.5064483700922966":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.8685308613044107":{"n0.14447215791313917":{"w":18.1297,"h":12.5054,"bl":0.7021}},"n0.8258704275455162":{"n0.35291789532253914":{"w":35.3823,"h":8.1019,"bl":0.8571}},"n0.08237313594205076":{"n0.3200974499624347":{"w":68.2961,"h":8.1019,"bl":0.8571}},"n0.2339738641536926":{"n0.8414305306060739":{"w":25.7161,"h":12.5054,"bl":0.7021}},"n0.20649554028200523":{"n0.4237285521604277":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.7023420069695498":{"n0.08267215938659933":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.23124838131896186":{"n0.8847247660066546":{"w":30.3819,"h":8.4545,"bl":0.8214}},"n0.5653478407878947":{"n0.8935425919742013":{"w":32.3079,"h":8.4545,"bl":0.8214}},"n0.03826225597296773":{"n0.5966198281161046":{"w":6.0764,"h":8.4545,"bl":0.8214}},"n0.3114158995400982":{"n0.16051818902884407":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.832831636206383":{"n0.2738713707452638":{"w":30.5718,"h":8.4545,"bl":0.8214}},"n0.44294341390001013":{"n0.19072972727490445":{"w":30.0022,"h":12.5054,"bl":0.7021}},"n0.8001658363143611":{"n0.2555656084479139":{"w":29.4687,"h":9.1146,"bl":0.7619}},"n0.8962696595786119":{"n0.8072900678294179":{"w":37.5434,"h":8.4545,"bl":0.8214}},"n0.7546823378521905":{"n0.960824309431972":{"w":52.861,"h":8.4545,"bl":0.8214}},"n0.7185940494962384":{"n0.7675969773404887":{"w":37.5434,"h":8.4545,"bl":0.8214}},"n0.934508072726157":{"n0.15127848760257478":{"w":48.7739,"h":8.4545,"bl":0.8214}},"n0.7840692535254685":{"n0.8705964676783371":{"w":48.7739,"h":8.4545,"bl":0.8214}}}}}

==> plots/docs/b89772eb-8011-46b7-a78f-95fb2bd8066b <==
{"id":"n0.8628316918407355","lines":[{"id":"n0.562747597967387","blocks":[]},{"id":"n0.5273559793818359","blocks":[{"id":"n0.8236255645064039","text":"\\diagram","type":"composite","elements":{"de49825060737485827":{"id":"de49825060737485827","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.49455426490344423"}],"id":"n0.3700714401035192"}],"id":"n0.507439450247194"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.05259571325594736"}],"id":"n0.03200298763200937"}],"shape":{"data":{"p":{"x":43.51719895786459,"y":44.62593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8392772638175428":{"id":"de8392772638175428","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"K","id":"n0.3280016587529575"}],"id":"n0.16000872253933585"}],"id":"n0.8754298217202812"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.24308943320830023"},{"text":"-recurrence","style":{"fontSize":{"value":0.4}},"id":"n0.21761928944529574"}],"style":{"align":"center"},"id":"n0.6188698522177833"}],"shape":{"data":{"p":{"x":40.48858574589599,"y":50.62593476262708},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7341561404291017":{"id":"de7341561404291017","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"U","id":"n0.14414333629632226"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"0","id":"n0.5905869300100071"}],"id":"n0.4959477743407148"}],"id":"n0.8219514388463278"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.26550122080025473"}],"id":"n0.9834551544666157"}],"id":"n0.027947209104751458"}},"id":"n0.860745668223655"},{"type":"single","text":"(","id":"n0.32172556728556234"},{"text":"s","id":"n0.23871287102752237"},{"type":"single","text":")","id":"n0.32322946097667593"}],"id":"n0.13909617635472848"}],"id":"n0.3405674873132667"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6065860912160819"}],"style":{"align":"center"},"id":"n0.9330200118644694"}],"shape":{"data":{"p":{"x":15.006408691406207,"y":47.249469301363774},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de878652079817785":{"id":"de878652079817785","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.9958750569996075","text":"\\overline","type":"composite","elements":{"value":{"id":"n0.8274210037083352","lines":[{"id":"n0.7895789030039244","blocks":[{"id":"n0.43073904367060356","text":"R"},{"id":"n0.9535602388338378","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.536952360116205","lines":[{"id":"n0.5762810627605497","blocks":[{"id":"n0.3884757344320906","text":"i"}]}]}}}]}]}}},{"type":"single","text":"(","id":"n0.15628260744819755"},{"text":"s,a","id":"n0.1681254651066575"},{"type":"single","text":")","id":"n0.8467666474282782"}],"id":"n0.960706236887447"}],"id":"n0.019004960502556623"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7380032901435976"}],"style":{"align":"center"},"id":"n0.5577433365257503"}],"shape":{"data":{"p":{"x":182.99999999999994,"y":219.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7882416035892696":{"id":"de7882416035892696","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.8070505170474311"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K-1","id":"n0.7820588648858702"}],"id":"n0.05204179071363346"}],"id":"n0.7461165093705924"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6797434591650722"}],"id":"n0.9780683932837613"}],"id":"n0.20405798469217795"}},"id":"n0.6767929484781436"},{"type":"single","text":"(","id":"n0.2979368193140759"},{"text":"s,a","id":"n0.6780472158337372"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.16812272379692583"}],"id":"n0.48746411688136204"}],"id":"n0.8678109095937245"}},"id":"n0.8473536042680254"},{"type":"single","text":")","id":"n0.4158045198032194"}],"id":"n0.6959331038941989"}],"id":"n0.4540862647774402"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8650872834849428"}],"style":{"align":"center"},"id":"n0.7460705152308109"}],"shape":{"data":{"p":{"x":97.99999999999994,"y":28.307382940085972},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8829192640173664":{"id":"de8829192640173664","lines":[{"blocks":[{"style":{"fontSize":"\\tiny"},"text":"max","id":"n0.09150222951303144"}],"id":"n0.41006002604551295"}],"shape":{"data":{"p":{"x":141.9161720677406,"y":43.48307625737806},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6212929260153228":{"id":"de6212929260153228","lines":[{"blocks":[{"text":"over ","style":{"fontSize":{"value":0.4}},"id":"n0.3759199150140131"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.8115277575240654"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7678858912569642"}],"id":"n0.27427660411047583"}],"id":"n0.7064297452925781"}},"id":"n0.5252128827500564"}],"id":"n0.4306183045431822"}],"id":"n0.7517415472449318"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.09107955876747975"}],"style":{"align":"center"},"id":"n0.1754719445147397"}],"shape":{"data":{"p":{"x":139.02611356688283,"y":57.07236067739149},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6961368095322311":{"id":"de6961368095322311","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"U","id":"n0.7420053721935991"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K-1","id":"n0.8374766026964253"}],"id":"n0.9292519201634248"}],"id":"n0.678570655622885"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.20744229043569407"}],"id":"n0.6341865633801596"}],"id":"n0.13966502816369797"}},"id":"n0.451547018102906"},{"type":"single","text":"(","id":"n0.83564795344481"},{"text":"s","id":"n0.9551868824980847"},{"type":"single","text":")","id":"n0.05549337685606481"}],"id":"n0.04906427405686231"}],"id":"n0.408476759756512"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5547124045533918"}],"style":{"align":"center"},"id":"n0.8132906214521824"}],"shape":{"data":{"p":{"x":182.0064086914062,"y":48.249469301363774},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de04836713429619688":{"id":"de04836713429619688","lines":[{"blocks":[{"text":"3D convolutional layer","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.9255886619942555"}],"style":{"align":"center"},"id":"n0.5044981362680492"}],"shape":{"data":{"p":{"x":400.7522976254404,"y":20.737859009608997},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4304294819132035":{"id":"de4304294819132035","lines":[{"blocks":[{"text":"Filter: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.7411218868021072"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×3×3×1×|A","style":{"mathModeType":"\\displaystyle"},"id":"n0.7439831288651368"},{"id":"n0.20038780616676166","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5273071114603862","lines":[{"id":"n0.2630313592514699","blocks":[{"id":"n0.9486521416434981","text":"i"}]}]}},"style":{"mathModeType":"\\displaystyle"}},{"text":"|","id":"n0.4331918560462156","style":{"mathModeType":"\\displaystyle"}}],"id":"n0.24224066795434895"}],"id":"n0.4948186869059896"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8823231620659291"}],"style":{"align":"center"},"id":"n0.063711797895871"}],"shape":{"data":{"p":{"x":392.51716844028647,"y":13.625934762627082},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1540081823410162":{"id":"de1540081823410162","lines":[{"blocks":[{"text":"Stride: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.04887852559195127"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1","id":"n0.0006046228652674124"}],"id":"n0.8114851563395926"}],"id":"n0.03631791790874783"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.37639896831524444"}],"style":{"align":"center"},"id":"n0.08980327572054025"}],"shape":{"data":{"p":{"x":385.52020640099363,"y":25.813468264617768},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6418911130447893":{"id":"de6418911130447893","lines":[{"blocks":[{"text":"3D convolutional layer","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.5579558575718451"}],"style":{"align":"center"},"id":"n0.9240321464139629"}],"shape":{"data":{"p":{"x":269.7522976254404,"y":23.737859009608997},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4386358202714504":{"id":"de4386358202714504","lines":[{"blocks":[{"text":"Filter: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.9095064291184971"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×3×3×1×|A","style":{"mathModeType":"\\displaystyle"},"id":"n0.805560192272305"},{"id":"n0.1918696226589085","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.4184995246269638","lines":[{"id":"n0.20172986713473895","blocks":[{"id":"n0.2338179798265101","text":"j"}]}]}},"style":{"mathModeType":"\\displaystyle"}},{"text":"|","id":"n0.6775938225632441","style":{"mathModeType":"\\displaystyle"}}],"id":"n0.10192837968410129"}],"id":"n0.10368321027700222"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6585904782524061"}],"style":{"align":"center"},"id":"n0.2141492919151311"}],"shape":{"data":{"p":{"x":261.51716844028647,"y":16.625934762627082},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9007883307111533":{"id":"de9007883307111533","lines":[{"blocks":[{"text":"Stride: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.24564546709807833"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1","id":"n0.788064759206107"}],"id":"n0.1471848314421922"}],"id":"n0.6113778876903095"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.542137284137528"}],"style":{"align":"center"},"id":"n0.15125705242321952"}],"shape":{"data":{"p":{"x":254.52020640099363,"y":28.813468264617768},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5541208246815192":{"id":"de5541208246815192","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.5041178283729908"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.9002246682459194"}],"id":"n0.5324681959368309"}],"id":"n0.5467348900570257"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5764000405107381"}],"id":"n0.7042306286918925"}],"id":"n0.8276904729959691"}},"id":"n0.24336808018267586"},{"type":"single","text":"(","id":"n0.8353469868189909"},{"text":"s,a","id":"n0.26468356341896015"},{"type":"single","text":")","id":"n0.30937765220020563"}],"id":"n0.25329414575928455"}],"id":"n0.8174948536978763"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5628238923487163"}],"style":{"align":"center"},"id":"n0.2604262847326111"}],"shape":{"data":{"p":{"x":424,"y":32.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de6127666039309161":{"id":"de6127666039309161","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.27594370866893114"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.3189564528479387"}],"id":"n0.8008403275771725"}],"id":"n0.16008272810937152"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5568189705645645"}],"id":"n0.9004139476633783"}],"id":"n0.9550466807690905"}},"id":"n0.38090799160040656"},{"type":"single","text":"(","id":"n0.3822111221954114"},{"text":"s,a","id":"n0.2356453221454542"},{"type":"single","text":")","id":"n0.8604232677303914"}],"id":"n0.7081331412186238"}],"id":"n0.6850706070771972"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.028734220868174454"}],"style":{"align":"center"},"id":"n0.43185577108968776"}],"shape":{"data":{"p":{"x":627,"y":185.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de28435527997219756":{"id":"de28435527997219756","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.08705093799143793"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.5891023591185407"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.9745168370340724"}],"id":"n0.958791673039098"}],"id":"n0.5039758522513191"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.5077092681029911"}],"id":"n0.864499051948938"}],"id":"n0.8320198695658971"}},"id":"n0.33459736015383257"}],"id":"n0.7615972764891554"}],"id":"n0.7244497752506611"}},"id":"n0.9720753771004256"},{"type":"single","text":"(","id":"n0.8591747481643697"},{"text":"s,a","id":"n0.17031193184549975"},{"type":"single","text":")","id":"n0.26795896373366945"}],"id":"n0.36970927642703466"}],"id":"n0.9153175281526549"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.30265450177445663"}],"style":{"align":"center"},"id":"n0.13500136400373175"}],"shape":{"data":{"p":{"x":477.58166565657575,"y":105.83474321560152},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de23402032048605892":{"id":"de23402032048605892","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1-","id":"n0.9148565968805094"},{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.06176305597570009"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.9604509141810909"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.6769009588768056"}],"id":"n0.8034744293145191"}],"id":"n0.06201144688230409"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.18625086752317932"}],"id":"n0.5951331231125816"}],"id":"n0.394072288365348"}},"id":"n0.20412815548829943"}],"id":"n0.7549304966285213"}],"id":"n0.4586129786426738"}},"id":"n0.7666961378815713"}],"id":"n0.31354421293919166"}],"id":"n0.047463607109459405"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.06354871958030639"}],"style":{"align":"center"},"id":"n0.8712918476355476"}],"shape":{"data":{"p":{"x":545.5816656565758,"y":106.30738294008597},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5414059609216073":{"id":"de5414059609216073","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⊤","id":"n0.3037765506455372"}],"id":"n0.3258322941087266"}],"id":"n0.38197129936659513"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7703953942288464"}],"id":"n0.5926678419513765"}],"shape":{"data":{"p":{"x":483.9161720677406,"y":44.17643163575815},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de5279245661967291":{"id":"de5279245661967291","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.1348097845975078"}],"id":"n0.09263916432355268"}],"id":"n0.4522059294213938"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.40620553658268865"}],"id":"n0.5650827310011799"}],"shape":{"data":{"p":{"x":535.5171989578646,"y":43.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de3842459334625856":{"id":"de3842459334625856","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.09128646721982836"}],"id":"n0.1645121089452033"}],"id":"n0.30112295613345186"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9229260139686721"}],"id":"n0.9912310077698254"}],"shape":{"data":{"p":{"x":230.5171989578646,"y":220.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6724674073740904":{"id":"de6724674073740904","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.6536524566939939"}],"id":"n0.8208839175415283"}],"id":"n0.07669072170856572"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5594436296680694"}],"id":"n0.77373365802956"}],"shape":{"data":{"p":{"x":576.1657782593641,"y":185.6259652802052},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de16664139451638227":{"id":"de16664139451638227","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⊤","id":"n0.2968545073165423"}],"id":"n0.3700267897409688"}],"id":"n0.687359062348055"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.29203876646287985"}],"id":"n0.5391793768832565"}],"shape":{"data":{"p":{"x":323.9161720677406,"y":45.17643163575815},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8268699887031468":{"id":"de8268699887031468","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.3915984754793784"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.3417202940877271"}],"id":"n0.7534884352237681"}],"id":"n0.7440048651355136"}},"id":"n0.05589435437227719"}],"id":"n0.4447440037807877"}],"id":"n0.7100476968630136"}},"id":"n0.4846887253442911"}],"id":"n0.7635891487221897"}],"id":"n0.6377335918019102"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.09659427055567638"}],"id":"n0.19349664935775568"}],"shape":{"data":{"p":{"x":209.59887757063825,"y":13.661304635673957}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de8705375563265205":{"id":"de8705375563265205","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.9552801703362863"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.34683177399551446"}],"id":"n0.30677207232372883"}],"id":"n0.355649984111561"}},"id":"n0.14589399605715192"}],"id":"n0.07548818109930044"}],"id":"n0.8021436907932609"}},"id":"n0.7115273960748678"}],"id":"n0.773475139164786"}],"id":"n0.769201243672291"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.00392747107489777"}],"id":"n0.8926299965974056"}],"shape":{"data":{"p":{"x":326.59887757063825,"y":12.625934762627082}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de23681891905315045":{"id":"de23681891905315045","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.8953639408865319"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.4149842063285205"}],"id":"n0.19796433252479173"}],"id":"n0.7872800310627679"}},"id":"n0.7339670170784438"},{"text":"|","id":"n0.6835423634317954"}],"id":"n0.9774562041920496"}],"id":"n0.04103796103922863"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.020117516451057416"}],"style":{"align":"center"},"id":"n0.34896747346457"}],"shape":{"data":{"p":{"x":-4,"y":2.983856201171875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de48398552182920707":{"id":"de48398552182920707","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.9266641391509445"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.5568862477146572"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.33934474488506416"}],"id":"n0.931750154936541"}],"id":"n0.057924422351373295"}},"id":"n0.8902100788558625"}],"id":"n0.4967429723445542"}],"id":"n0.36540566276141506"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.38746857642979204"}],"id":"n0.8869775529225605"}],"id":"n0.526142623353475"}},"id":"n0.5603748434152191"}],"id":"n0.6524612630217288"}],"id":"n0.8651163527017454"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7428763826954485"}],"id":"n0.5887641859815747"}],"shape":{"data":{"p":{"x":9.99359130859375,"y":-3.4417227080760426}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de48673237968752736":{"id":"de48673237968752736","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.23292943631388763"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.3016682683679175"}],"id":"n0.025440374297824198"}],"id":"n0.6127761903648783"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4666539713796616"}],"id":"n0.668351275345753"}],"id":"n0.2767409612998937"}},"id":"n0.724881061692201"},{"type":"single","text":"(","id":"n0.31414876243208134"},{"text":"s,a","id":"n0.9864117007105992"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.1248712269325194"}],"id":"n0.06525388807431942"}],"id":"n0.5646104364600255"}},"id":"n0.07435533398861138"},{"type":"single","text":")","id":"n0.5624481888687876"}],"id":"n0.4248082564228923"}],"id":"n0.6138080945790303"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.10695921374173234"}],"style":{"align":"center"},"id":"n0.7097339872021309"}],"shape":{"data":{"p":{"x":278.4011224293617,"y":33.68144817745889},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8846298562061499":{"id":"de8846298562061499","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.9240098393557779"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.15499462180864287"}],"id":"n0.4318738583219519"}],"id":"n0.5324136919490754"}},"id":"n0.03725379254995542"},{"text":"×W","id":"n0.5377241879080408"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.006083119336494969"}],"id":"n0.7914171866983244"}],"id":"n0.09591925744493657"}},"id":"n0.3132651821130823"},{"text":"×H","id":"n0.5004129826576436"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.7914725656335135"}],"id":"n0.1666645969839271"}],"id":"n0.21297786696722532"}},"id":"n0.8885724783469957"},{"text":"×W","id":"n0.6576475851357684"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.811406949344728"}],"id":"n0.3269255955473507"}],"id":"n0.9914809921042727"}},"id":"n0.649669996204548"},{"text":"×|A","id":"n0.3569691578905021"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.0812859212449546"}],"id":"n0.44980866937891073"}],"id":"n0.9576709953840956"}},"id":"n0.5893869902083619"},{"text":"|×|A","id":"n0.9021067821601803"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8935952646673961"}],"id":"n0.16896322121170715"}],"id":"n0.5754560664408199"}},"id":"n0.3914541099875819"},{"text":"|","id":"n0.8576312480942625"}],"id":"n0.15286703063243756"}],"id":"n0.9346331450716716"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7420023035191288"}],"style":{"align":"center"},"id":"n0.28601838441576555"}],"shape":{"data":{"p":{"x":354,"y":281.9838562011719},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9056851396423851":{"id":"de9056851396423851","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.3975583049207363"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.06300427758300442"}],"id":"n0.20985140923926293"}],"id":"n0.7920020741174281"}},"id":"n0.6124542089220948"},{"text":"×W","id":"n0.52786224995756"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6476996367412975"}],"id":"n0.19763128347540593"}],"id":"n0.5508098725003492"}},"id":"n0.1896532976045786"},{"text":"×H","id":"n0.6288155425985547"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.007222502636268002"}],"id":"n0.054198563577345205"}],"id":"n0.6690767590448217"}},"id":"n0.43593740460130137"},{"text":"×W","id":"n0.5201671469445934"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.828782969496656"}],"id":"n0.11314837801358313"}],"id":"n0.7490363675695493"}},"id":"n0.8263341454929529"}],"id":"n0.522341707304876"}],"id":"n0.4658812440199587"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5435050101233148"}],"style":{"align":"center"},"id":"n0.9664266160818378"}],"shape":{"data":{"p":{"x":-2,"y":66.80793110814716},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de17725590586649997":{"id":"de17725590586649997","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.7697015924694854"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9255487288302668","text":"i"}],"id":"n0.7188220392736842"}],"id":"n0.6556097098409805"}},"id":"n0.9550082434015339"},{"text":"×W","id":"n0.22086728083849638"},{"id":"n0.10686891860923686","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7950620791776775","lines":[{"id":"n0.9773869714200802","blocks":[{"id":"n0.7852054377104776","text":"i"}]}]}}},{"text":"×H","id":"n0.17503155648954793"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.2236222367379872"}],"id":"n0.015536579478339307"}],"id":"n0.4474869123314231"}},"id":"n0.7683706952890572"},{"text":"×W","id":"n0.37544184562018157"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.26205685100766263"}],"id":"n0.8192353100200187"}],"id":"n0.9808450237463693"}},"id":"n0.7732845998155922"}],"id":"n0.7037197434395268"}],"id":"n0.6779540611266668"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.832519388159987"}],"style":{"align":"center"},"id":"n0.7153854145196572"}],"shape":{"data":{"p":{"x":139,"y":68.80793110814716},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8020780160490844":{"id":"de8020780160490844","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.19254118440377188"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.026708629040808507"}],"id":"n0.09432173819124712"}],"id":"n0.8686400357039945"}},"id":"n0.4802286381463339"},{"text":"×W","id":"n0.17312173914197304"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.2786013489390031"}],"id":"n0.16553076516208476"}],"id":"n0.0593824842978008"}},"id":"n0.882010426100716"},{"text":"×H","id":"n0.41778977561438135"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.08879210981933316"}],"id":"n0.52338464392984"}],"id":"n0.7557619000986653"}},"id":"n0.0884478826117927"},{"text":"×W","id":"n0.27385964723967615"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.1339468242647479"}],"id":"n0.7932762094562638"}],"id":"n0.7933576266650011"}},"id":"n0.10511854772275031"},{"text":"×|A","id":"n0.992631034430089"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.21675636965666656"}],"id":"n0.7762497937584696"}],"id":"n0.42825336586871243"}},"id":"n0.5203396537118956"},{"text":"|","id":"n0.9659200368612286"}],"id":"n0.3315585301606032"}],"id":"n0.2594341695196014"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.42799371253152896"}],"style":{"align":"center"},"id":"n0.6841868762211407"}],"shape":{"data":{"p":{"x":81.49929038471396,"y":80.21600341796875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de35837508646930627":{"id":"de35837508646930627","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.6752105647865525"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.5421777995235713","text":"i"}],"id":"n0.6673260548869122"}],"id":"n0.9149894207372442"}},"id":"n0.4884171265223254"},{"text":"|×H","id":"n0.31802552971937215"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8552332406632621"}],"id":"n0.0023972541780015177"}],"id":"n0.9653179998027317"}},"id":"n0.10300070602660427"},{"text":"×W","id":"n0.8554204348452248"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8818196953034094"}],"id":"n0.6501696933127412"}],"id":"n0.8035121608949127"}},"id":"n0.24019777675753962"},{"text":"×|A","id":"n0.9243501476649474"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.6066945677921896","text":"j"}],"id":"n0.0752357949125324"}],"id":"n0.005099696887602478"}},"id":"n0.3694483709039966"},{"text":"|","id":"n0.22700339936023584"}],"id":"n0.035945705013095575"}],"id":"n0.8035966151360414"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9934441125242666"}],"style":{"align":"center"},"id":"n0.7339952625586599"}],"shape":{"data":{"p":{"x":254.49929038471396,"y":86.21600341796875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de44431680897613113":{"id":"de44431680897613113","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.30503785226816715"},{"id":"n0.12058067480096524","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.14472103467257824","lines":[{"id":"n0.47748592585873983","blocks":[{"id":"n0.017744946456977884","text":"j"}]}]}}},{"text":"×A","id":"n0.8678266411174607"},{"id":"n0.3546478795143535","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9368869249435956","lines":[{"id":"n0.706322193982863","blocks":[{"id":"n0.7336895096776936","text":"j"}]}]}}},{"text":"|×H","id":"n0.09055987566643942"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4715056720982993","text":"i"}],"id":"n0.010659160438502013"}],"id":"n0.4276082222151729"}},"id":"n0.468399590720896"},{"text":"×W","id":"n0.8798716378432485"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7710942261178746","text":"i"}],"id":"n0.750499963069041"}],"id":"n0.2905758440450652"}},"id":"n0.5549385663006416"},{"text":"×|A","id":"n0.06074146956194504"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9280595346450058","text":"i"}],"id":"n0.7785574871342951"}],"id":"n0.4945902397594186"}},"id":"n0.6548284470302579"},{"text":"|","id":"n0.20016963550019895"}],"id":"n0.9974246527053048"}],"id":"n0.8652985179455455"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9486350789859588"}],"style":{"align":"center"},"id":"n0.041652101070513536"}],"shape":{"data":{"p":{"x":380.49929038471396,"y":86.21600341796875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de11129279367613587":{"id":"de11129279367613587","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.43190907136130297"}],"style":{"align":"center"},"id":"n0.9233886406772411"}],"shape":{"data":{"p":{"x":209.59887757063825,"y":34.300435473167056},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4390051875579064":{"id":"de4390051875579064","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.28249310277124473"}],"style":{"align":"center"},"id":"n0.33436862044616644"}],"shape":{"data":{"p":{"x":339.76316775365297,"y":34.429355783134895},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1507135434759932":{"id":"de1507135434759932","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.4872662421724989"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.1096318083339114","text":"j"}],"id":"n0.08828378784498514"}],"id":"n0.4313687052503603"}},"id":"n0.602195369768934"},{"text":"×A","id":"n0.9082697695415494"},{"id":"n0.2835671734457961","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6971546230925536","lines":[{"id":"n0.7992977157443393","blocks":[{"id":"n0.8876145669787254","text":"j"}]}]}}},{"text":"|×H","id":"n0.716329668428678"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9107067680455683","text":"i"}],"id":"n0.5384319111418014"}],"id":"n0.3603334496393018"}},"id":"n0.2766257768924789"},{"text":"×W","id":"n0.5241081903205831"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.46252002726247676","text":"i"}],"id":"n0.35424214207291405"}],"id":"n0.7505731487542968"}},"id":"n0.8393193586503307"}],"id":"n0.4120157811821672"}],"id":"n0.40235662659270877"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.07942332055987467"}],"style":{"align":"center"},"id":"n0.8941317310966974"}],"shape":{"data":{"p":{"x":306.2671484131258,"y":57.96521918264051},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de522171948209275":{"id":"de522171948209275","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.07347982487587168"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6943621769917845"}],"id":"n0.8538407585486798"}],"id":"n0.23779598982390726"}},"id":"n0.9994533451097276"},{"text":"×W","id":"n0.5641323880399061"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7655910428307564"}],"id":"n0.0744036343268597"}],"id":"n0.8624241408950293"}},"id":"n0.5632405278854995"},{"text":"×H","id":"n0.38042025325061846"},{"id":"n0.6900959648010496","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.11219020746017283","lines":[{"id":"n0.03178520695856757","blocks":[{"id":"n0.5553908242528094","text":"j"}]}]}}},{"text":"×W","id":"n0.454434201497254"},{"id":"n0.5384307991107282","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7520327457247449","lines":[{"id":"n0.7277586400121654","blocks":[{"id":"n0.7354762063033926","text":"j"}]}]}}},{"text":"×|A","id":"n0.22485390461849852"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.408823091251288"}],"id":"n0.16585619659351103"}],"id":"n0.2924015559398825"}},"id":"n0.9146328100298982"},{"text":"|×|A","id":"n0.6720662299968945"},{"id":"n0.2227552496632479","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5039818588024179","lines":[{"id":"n0.9567124009660033","blocks":[{"id":"n0.758271073863773","text":"j"}]}]}}},{"text":"|","id":"n0.4681849489955767"}],"id":"n0.8672176115946004"}],"id":"n0.5663416250436877"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7955583954820513"}],"style":{"align":"center"},"id":"n0.524381383059356"}],"shape":{"data":{"p":{"x":450.60827698470075,"y":57.215249700218635},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de04941809146159737":{"id":"de04941809146159737","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.916266029563227"}],"style":{"align":"center"},"id":"n0.0991665152370298"}],"shape":{"data":{"p":{"x":452.68282386541637,"y":34.30738294008598},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6620171831553086":{"id":"de6620171831553086","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.06644675650866261"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5812713175375215"}],"id":"n0.9600611837462389"}],"id":"n0.08529489713954752"}},"id":"n0.8646489637780295"},{"text":"×W","id":"n0.8089785591043599"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.07684623624518028"}],"id":"n0.29565576360943635"}],"id":"n0.35672593270715947"}},"id":"n0.6798175258010559"},{"text":"×H","id":"n0.5071816299008141"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5787419699083496"}],"id":"n0.844131361406786"}],"id":"n0.6818487507936537"}},"id":"n0.15833282812438276"},{"text":"×W","id":"n0.9130348269297166"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.3777307375122563"}],"id":"n0.24573635349157308"}],"id":"n0.10589104972322194"}},"id":"n0.07698402670484605"},{"text":"×|A","id":"n0.8504775928759356"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7788587289830557"}],"id":"n0.22215615429686775"}],"id":"n0.20835969360451156"}},"id":"n0.4127374457395061"},{"text":"|×|A","id":"n0.028993692012068584"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.6303562730740266"}],"id":"n0.12768825363388836"}],"id":"n0.9790385343606987"}},"id":"n0.46668316132436494"},{"text":"|","id":"n0.837018209659206"}],"id":"n0.4139531593661605"}],"id":"n0.2688194492057001"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7634823240114856"}],"style":{"align":"center"},"id":"n0.7873382932403481"}],"shape":{"data":{"p":{"x":490.60827698470075,"y":159.21524970021864},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de11098522098733432":{"id":"de11098522098733432","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.30690009171114196"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5919306379608547"}],"id":"n0.7979906207756955"}],"id":"n0.3081021407237814"}},"id":"n0.8316015393846763"},{"text":"×W","id":"n0.8769431682553834"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.40798222036222587"}],"id":"n0.7503499867028827"}],"id":"n0.3148845401510407"}},"id":"n0.8642976180964292"},{"text":"×H","id":"n0.2519436465858962"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.03898210518009182"}],"id":"n0.7871624906068271"}],"id":"n0.787894730359483"}},"id":"n0.9967576722087257"},{"text":"×W","id":"n0.16617853467699106"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.6465546664341582"}],"id":"n0.0544832208057191"}],"id":"n0.34225070472881414"}},"id":"n0.8689876849907643"},{"text":"×|A","id":"n0.738367115137506"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7432839740810651"}],"id":"n0.2521045996472795"}],"id":"n0.3590950542783178"}},"id":"n0.8911538754232573"},{"text":"|×|A","id":"n0.33713830235063225"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.1799236854589148"}],"id":"n0.09029960826674222"}],"id":"n0.7852857038869694"}},"id":"n0.40885625536349934"},{"text":"|","id":"n0.7311220792156645"}],"id":"n0.3127101080275474"}],"id":"n0.8434406802059295"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6334771093928775"}],"style":{"align":"center"},"id":"n0.24022153427204107"}],"shape":{"data":{"p":{"x":376.60827698470075,"y":149.21524970021864},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9498932232987138":{"id":"de9498932232987138","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.05817662287806291"}],"id":"n0.8226545479203107"}],"id":"n0.14671194271672894"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.16502998636958033"}],"id":"n0.24002220610340408"}],"shape":{"data":{"p":{"x":479.5171989578646,"y":185.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de21836601327672356":{"id":"de21836601327672356","lines":[{"blocks":[{"text":"4D convolutional layer","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.5581912545269967"}],"style":{"align":"center"},"id":"n0.2222051032077259"}],"shape":{"data":{"p":{"x":260.7522976254404,"y":113.11192424698191},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5046958092324985":{"id":"de5046958092324985","lines":[{"blocks":[{"text":"Filter: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.808913255521164"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3×3×3×3×1×|A|","style":{"mathModeType":"\\displaystyle"},"id":"n0.614441534176204"}],"id":"n0.2070918756904696"}],"id":"n0.8084507466865571"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.06910730168479695"}],"style":{"align":"center"},"id":"n0.9327962624050163"}],"shape":{"data":{"p":{"x":252.51716844028647,"y":101},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de20876449516190876":{"id":"de20876449516190876","lines":[{"blocks":[{"text":"Stride: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.6171687124432887"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1×1","id":"n0.5768882542983327"}],"id":"n0.5764231602461787"}],"id":"n0.4078630694843064"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.18145225750901695"}],"style":{"align":"center"},"id":"n0.981925283009887"}],"shape":{"data":{"p":{"x":245.52020640099363,"y":115.18753350199069},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5418541516011492":{"id":"de5418541516011492","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"T","id":"n0.7688004359587917"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3796404679311245"}],"id":"n0.2753147448993347"}],"id":"n0.9936634121326251"}},"id":"n0.49998465427461736"}],"id":"n0.29351627084059895"}],"id":"n0.1325705150031895"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5881905538269003"}],"id":"n0.05491706422767484"}],"shape":{"data":{"p":{"x":195,"y":141.6290170380177}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de593748394392474":{"id":"de593748394392474","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.2024513439070299"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.6079080211235881"}],"id":"n0.039372446555006935"}],"id":"n0.17424852726676154"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.27754197573671946"}],"id":"n0.9898910152004727"}],"id":"n0.9131833576629502"}},"id":"n0.06928870624904726"},{"type":"single","text":"(","id":"n0.36341506215089003"},{"text":"s,a","id":"n0.34063805430204086"},{"type":"single","text":")","id":"n0.0880183115160802"}],"id":"n0.011029513288379977"}],"id":"n0.5354735391707355"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3680450720683681"}],"style":{"align":"center"},"id":"n0.3056060788524073"}],"shape":{"data":{"p":{"x":287,"y":126.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8913158837985631":{"id":"de8913158837985631","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Activation: ReLU","id":"n0.05693186723663479"}],"id":"n0.7546118539131947"}],"shape":{"data":{"p":{"x":100.5172119140625,"y":204.4443130493164},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de49845263097063075":{"id":"de49845263097063075","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.3561453397862475"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1","id":"n0.4691350123111182"}],"id":"n0.5771846971278596"}],"id":"n0.42747229650193197"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5927800692205678"}],"id":"n0.8453167772585206"}],"shape":{"data":{"p":{"x":74.5172119140625,"y":208.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de19958885418575512":{"id":"de19958885418575512","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.8237715942731867"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3×3×4×200","id":"n0.14754586405517744"}],"id":"n0.3382643066492892"}],"id":"n0.0671748381274353"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5746527989732806"}],"id":"n0.8533482083801416"}],"shape":{"data":{"p":{"x":81.5172119140625,"y":196.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9991017222779492":{"id":"de9991017222779492","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"2D convolutional layer","id":"n0.3305531879713304"}],"id":"n0.796093615307945"}],"shape":{"data":{"p":{"x":89.5172119140625,"y":196.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de7794946484826855":{"id":"de7794946484826855","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.24491485485523845"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1","id":"n0.34253594693251954"}],"id":"n0.8201033238122026"}],"id":"n0.35431681432038165"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.1461140221830728"}],"id":"n0.21950866463284258"}],"shape":{"data":{"p":{"x":112.0172119140625,"y":209.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9437130437561829":{"id":"de9437130437561829","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.5979703033955528"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×200×|A","id":"n0.9453268524544269"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.630998937819023"}],"id":"n0.8083322454877857"}],"id":"n0.3487417949962308"}},"id":"n0.7879825099348208"},{"text":"|","id":"n0.35092453772066623"}],"id":"n0.9924403943583895"}],"id":"n0.12323602675056611"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3716906131006634"}],"id":"n0.8408340296938122"}],"shape":{"data":{"p":{"x":119.0172119140625,"y":192.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de3957690388394757":{"id":"de3957690388394757","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"2D convolutional layer","id":"n0.2831710279467221"}],"id":"n0.13269695582335794"}],"shape":{"data":{"p":{"x":127.0172119140625,"y":196.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de5805238498780745":{"id":"de5805238498780745","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Activation: ReLU","id":"n0.9772703803458971"}],"id":"n0.6842961852820442"}],"shape":{"data":{"p":{"x":100.5172119140625,"y":119.4443130493164},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4297722923504397":{"id":"de4297722923504397","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"4D convolutional layer","id":"n0.6128428799527574"}],"id":"n0.1863077684458414"}],"shape":{"data":{"p":{"x":89.5172119140625,"y":113.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9970137941515702":{"id":"de9970137941515702","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.8551779072921222"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3×3×3×3×2×100","id":"n0.5894255189656732"}],"id":"n0.7063629133230427"}],"id":"n0.3210884854241822"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3397182068614162"}],"id":"n0.3961409225340591"}],"shape":{"data":{"p":{"x":81.5172119140625,"y":101.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de618679292194954":{"id":"de618679292194954","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.9710282475795413"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1×1","id":"n0.7066017249082943"}],"id":"n0.5611562227899454"}],"id":"n0.14206887739882257"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7443737249209761"}],"id":"n0.7181779079849848"}],"shape":{"data":{"p":{"x":74.5172119140625,"y":115.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4392674425233447":{"id":"de4392674425233447","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"4D convolutional layer","id":"n0.5301660593230821"}],"id":"n0.3958610824559792"}],"shape":{"data":{"p":{"x":127.0172119140625,"y":112.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de04204407547054956":{"id":"de04204407547054956","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.10551866878206084"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1×1×100×|A|","id":"n0.8656058523394414"}],"id":"n0.02722195288173035"}],"id":"n0.633784928341107"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.16890997532945828"}],"id":"n0.5765982436223782"}],"shape":{"data":{"p":{"x":119.0172119140625,"y":98.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8792070875119302":{"id":"de8792070875119302","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.8513302607064426"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1×1","id":"n0.32634089926763865"}],"id":"n0.31301881936258424"}],"id":"n0.36024324575911404"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.07486874930869836"}],"id":"n0.5385064198666598"}],"shape":{"data":{"p":{"x":112.0172119140625,"y":116.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7209237783119844":{"id":"de7209237783119844","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.9729776412783562","text":"R"},{"id":"n0.2835126069111431","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.08389011410193059","lines":[{"id":"n0.9819171012848007","blocks":[{"id":"n0.047536987371397776","text":"i"}]}]}}},{"type":"single","text":"(","id":"n0.8691568773847549"},{"text":"s,a","id":"n0.5889567509171811"},{"type":"single","text":")","id":"n0.5276003849362187"}],"id":"n0.2095657756783389"}],"id":"n0.2982039446388105"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.015031633040377246"}],"style":{"align":"center"},"id":"n0.25864148778868534"}],"shape":{"data":{"p":{"x":151.99999999999994,"y":125.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de038275511556437936":{"id":"de038275511556437936","lines":[{"blocks":[{"text":"expand along","style":{"fontSize":{"value":0.4}},"id":"n0.7377298173475393"}],"style":{"align":"center"},"id":"n0.9617942479760144"}],"shape":{"data":{"p":{"x":117.29996422052108,"y":198.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9771146900240346":{"id":"de9771146900240346","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.6399812305379686"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.7507470953748117"}],"id":"n0.6350793290242283"}],"id":"n0.6673921088194974"}},"id":"n0.8403559765691839"}],"id":"n0.6655942045909249"}],"id":"n0.39382613896308327"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.68068017586931"},{"text":",","style":{"fontSize":{"value":0.4}},"id":"n0.6656502821413655"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"W","id":"n0.13463231949855103"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.3824123960513046"}],"id":"n0.9272158036074829"}],"id":"n0.06135171794311067"}},"id":"n0.8809286095868312"},{"id":"n0.22244046571993925","text":",A"},{"id":"n0.004709735571196472","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5915201252700317","lines":[{"id":"n0.9228932234027902","blocks":[{"id":"n0.13351951205842272","text":"j"}]}]}}}],"id":"n0.9862134259506325"}],"id":"n0.7869443691048681"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8476247623710638"}],"style":{"align":"center"},"id":"n0.22591749357595425"}],"shape":{"data":{"p":{"x":120.29996422052108,"y":214},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9138085967477212":{"id":"de9138085967477212","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.5246867276122629"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.44468150511900717"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.28346165577162274"}],"id":"n0.13986293163761343"}],"id":"n0.2918402784940872"},"indexValue":{"lines":[{"blocks":[{"id":"n0.8675891867791983","text":"R"}],"id":"n0.5950250442193212"}],"id":"n0.9362693118359131"}},"id":"n0.1802718268590522"}],"id":"n0.9060303829634953"}],"id":"n0.6254132286642293"}},"id":"n0.6166884885015271"},{"type":"single","text":"(","id":"n0.8913429643789912"},{"text":"s,a","id":"n0.039437228771850075"},{"type":"single","text":")","id":"n0.12396919054212252"}],"id":"n0.1563681651083162"}],"id":"n0.3888587151739875"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.2655067483208675"}],"style":{"align":"center"},"id":"n0.590575319588402"}],"shape":{"data":{"p":{"x":308.58166565657575,"y":271.8347432156015},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de20514259198876084":{"id":"de20514259198876084","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1-","id":"n0.668198392710996"},{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.7571321692537014"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.5272197079611174"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.8937534642238385"}],"id":"n0.4214733950927938"}],"id":"n0.7177250752548958"},"indexValue":{"lines":[{"blocks":[{"id":"n0.7474702890391776","text":"R"}],"id":"n0.5319220509984435"}],"id":"n0.2693561890123892"}},"id":"n0.8118552033966404"}],"id":"n0.7837346203169866"}],"id":"n0.009197237518780765"}},"id":"n0.3760909778409871"}],"id":"n0.2830138817581649"}],"id":"n0.4091118874775652"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.904834482548242"}],"style":{"align":"center"},"id":"n0.08067293266874409"}],"shape":{"data":{"p":{"x":245.5816656565757,"y":273.8347432156015},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7312818138853312":{"id":"de7312818138853312","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.129410645790617"}],"id":"n0.0932584376979364"}],"id":"n0.6176372360853613"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7572352029835652"}],"id":"n0.013809604713022283"}],"shape":{"data":{"p":{"x":294.5171989578646,"y":200.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de18788604977197143":{"id":"de18788604977197143","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.7208189660776849"}],"id":"n0.6520254498093123"}],"id":"n0.4440631194786806"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.818256381077096"}],"id":"n0.5427659946248642"}],"shape":{"data":{"p":{"x":337.16577825936406,"y":220.6259652802052},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4165371666675024":{"id":"de4165371666675024","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"R","id":"n0.0853109433397754"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9419594729096477"}],"id":"n0.968664482499086"}],"id":"n0.9296545885225689"}},"id":"n0.8016860732170108"},{"type":"single","text":"(","id":"n0.013403756317966753"},{"text":"s,a","id":"n0.6226098915614835"},{"type":"single","text":")","id":"n0.6431540514618153"}],"id":"n0.9579442511261114"}],"id":"n0.747319571117421"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8339656140112792"}],"style":{"align":"center"},"id":"n0.7419316581247017"}],"shape":{"data":{"p":{"x":391.99999999999994,"y":228.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de4583001414534833":{"id":"de4583001414534833","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.921779451769565"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8518855671786338"}],"id":"n0.11299044556288429"}],"id":"n0.7604477425721416"}},"id":"n0.9296973827163246"},{"text":"×W","id":"n0.1538161200467536"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8171545339012034"}],"id":"n0.9385952818455519"}],"id":"n0.1867963143872604"}},"id":"n0.587800547063406"},{"text":"×H","id":"n0.46918365779553817"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.008491500153849252"}],"id":"n0.02332069353328614"}],"id":"n0.828953364810201"}},"id":"n0.340743747243319"},{"text":"×W","id":"n0.7074877741896182"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.7296990462222239"}],"id":"n0.8203240114425976"}],"id":"n0.8593990452589579"}},"id":"n0.4786005730910594"},{"text":"×|A","id":"n0.7863315375672915"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3876218112318073"}],"id":"n0.11576612414543375"}],"id":"n0.4475959595518957"}},"id":"n0.20566171753843232"},{"text":"|×|A","id":"n0.5637944255714951"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.9738597378483855"}],"id":"n0.45027017249932344"}],"id":"n0.8867471707265016"}},"id":"n0.3206198173113135"},{"text":"|","id":"n0.06621334827614778"}],"id":"n0.3805910514369335"}],"id":"n0.7089762412406253"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8667210386776814"}],"style":{"align":"center"},"id":"n0.5745830515114823"}],"shape":{"data":{"p":{"x":565,"y":238.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1583966116698592":{"id":"de1583966116698592","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.25051324056472835"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5104485528147293"}],"id":"n0.7119266041364181"}],"id":"n0.6720067974614112"}},"id":"n0.22417906398881216"},{"text":"×W","id":"n0.38694565250942947"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.11308467701634828"}],"id":"n0.2561855248327065"}],"id":"n0.8964395188293126"}},"id":"n0.873709845049295"},{"text":"×H","id":"n0.07805176795000945"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5261696737053156"}],"id":"n0.9217072167579223"}],"id":"n0.508954517101174"}},"id":"n0.9127868590808386"},{"text":"×W","id":"n0.4359191161625884"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8355586213743413"}],"id":"n0.28414560810793055"}],"id":"n0.02678663819435756"}},"id":"n0.7433295513012017"},{"text":"×|A","id":"n0.7044446941084268"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.13006501606547882"}],"id":"n0.0153861215235791"}],"id":"n0.4633317385584048"}},"id":"n0.7469097027384985"},{"text":"|×|A","id":"n0.6972895534173722"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.2138797359882061"}],"id":"n0.17566364102152088"}],"id":"n0.2007068588156009"}},"id":"n0.35156909735178665"},{"text":"|","id":"n0.11037384940026396"}],"id":"n0.08339218194311648"}],"id":"n0.4177074897863875"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.32265772539243165"}],"style":{"align":"center"},"id":"n0.43506864788632593"}],"shape":{"data":{"p":{"x":286,"y":324.9838562011719},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7104577832050005":{"id":"de7104577832050005","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.8075229294190343"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.22083786699300711"}],"id":"n0.5255935204300768"}],"id":"n0.4311607854420607"}},"id":"n0.0914520644866017"},{"text":"×W","id":"n0.2652626755745493"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.16552874564810538"}],"id":"n0.8782516293388296"}],"id":"n0.85421562944347"}},"id":"n0.4873403498265405"},{"text":"×H","id":"n0.8038175045166087"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.08554711175121255"}],"id":"n0.6725093589093312"}],"id":"n0.5375129209530072"}},"id":"n0.6141587701812863"},{"text":"×W","id":"n0.01933840850697721"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.020443097004659405"}],"id":"n0.522494558892066"}],"id":"n0.21268471635124353"}},"id":"n0.8246463885708728"},{"text":"×|A","id":"n0.4801458926047433"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.21798914880275522"}],"id":"n0.7652275275201048"}],"id":"n0.9870166818264658"}},"id":"n0.06268927174621086"},{"text":"|×|A","id":"n0.1087166598051661"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.1336164611793449"}],"id":"n0.8600008500233927"}],"id":"n0.362784223053767"}},"id":"n0.05402756018969823"},{"text":"|","id":"n0.6466916443560289"}],"id":"n0.9209111051638239"}],"id":"n0.26785386114980914"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7785792835100691"}],"style":{"align":"center"},"id":"n0.6668498709114434"}],"shape":{"data":{"p":{"x":189,"y":324.9838562011719},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5557732641915689":{"id":"de5557732641915689","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.9221364007242416"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8708924348985256"}],"id":"n0.4361484756663945"}],"id":"n0.44176253688535194"}},"id":"n0.04716332947140223"},{"text":"×W","id":"n0.712883274296817"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6132920401588458"}],"id":"n0.7616430739518658"}],"id":"n0.2696234113493192"}},"id":"n0.013541307813835557"},{"text":"×H","id":"n0.7340685198492256"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.20818575598044387"}],"id":"n0.10504536827258204"}],"id":"n0.6062678939699782"}},"id":"n0.111041145839339"},{"text":"×W","id":"n0.45675239871196416"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8037406560355145"}],"id":"n0.2762161569037047"}],"id":"n0.2607323870924354"}},"id":"n0.35059931187490756"},{"text":"×|A","id":"n0.9153432582945753"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5041720294833045"}],"id":"n0.04667625220583438"}],"id":"n0.9892646631408653"}},"id":"n0.6319894876092336"},{"text":"|×|A","id":"n0.7986057437532796"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.0712045303235258"}],"id":"n0.4180675169846606"}],"id":"n0.3078710101191444"}},"id":"n0.3499893192850838"},{"text":"|","id":"n0.8972496317508627"}],"id":"n0.4931140849769742"}],"id":"n0.9409319662631248"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6201032476437982"}],"style":{"align":"center"},"id":"n0.1098735865660323"}],"shape":{"data":{"p":{"x":129,"y":271.9838562011719},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5375910533835289":{"id":"de5375910533835289","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.3818972620683758"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.6936000842560022"}],"id":"n0.8834480079197842"}],"id":"n0.47579159718552"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.0161172559129108"}],"id":"n0.3091250253697164"}],"id":"n0.04860701906399467"}},"id":"n0.5280536840296086"},{"type":"single","text":"(","id":"n0.3717890650866613"},{"text":"s,a","id":"n0.8688828975071476"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6224899193762006"}],"id":"n0.6917619864650839"}],"id":"n0.7395427912098691"}},"id":"n0.2917797323041105"},{"type":"single","text":")","id":"n0.14063453808692916"}],"id":"n0.19153155965893243"}],"id":"n0.7764373811879"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7429848061739557"}],"style":{"align":"center"},"id":"n0.33650805746857215"}],"shape":{"data":{"p":{"x":616,"y":62.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de9514175999666843":{"id":"de9514175999666843","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.5850924357739005"}],"id":"n0.5376003386086392"}],"id":"n0.0762310102206607"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6456319389028695"}],"id":"n0.11134966197085183"}],"shape":{"data":{"p":{"x":615.5171989578646,"y":131.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true}},"connections":[],"intersections":{"id":"di2780349073832271","items":[],"style":{}},"shapes":[{"id":"dp14990224151474485","type":"doc-cube","data":{"p1":{"x":403.89243309975313,"y":45.5022752722482},"p2":{"x":441.9827880859375,"y":83.21222204612354},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp24405884183873572","type":"doc-cube","data":{"p1":{"x":403.89243309975313,"y":13.199859619140625},"p2":{"x":441.9827880859375,"y":50.90980639301608},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"da6949805193558927","data":[{"x":40.01719895786459,"y":57.34437565321065},{"x":51.206092622831534,"y":57.34437565321065}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp7751921556432406","type":"doc-cube","data":{"p1":{"x":1.5988775706382512,"y":37.84193818059583},"p2":{"x":39.68923255682262,"y":75.55188495447129},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp8785182138928569","type":"doc-cube","data":{"p1":{"x":92.17413453580775,"y":51.42721209483358},"p2":{"x":130.26448952199212,"y":89.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp844065271006349","type":"doc-cube","data":{"p1":{"x":92.17413453580775,"y":19.42721209483358},"p2":{"x":130.26448952199212,"y":57.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp8899522848110837","type":"doc-cube","data":{"p1":{"x":162.90964501381563,"y":231.12821003487528},"p2":{"x":201,"y":268.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp6103754823685426","type":"doc-cube","data":{"p1":{"x":162.90964501381563,"y":198.8257943817677},"p2":{"x":201,"y":236.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp5314894875590921","type":"doc-cube","data":{"p1":{"x":173.592468879232,"y":241.89985181931803},"p2":{"x":211.68282386541637,"y":279.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp7433023052420107","type":"doc-cube","data":{"p1":{"x":173.592468879232,"y":209.89985181931803},"p2":{"x":211.68282386541637,"y":247.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da9197567997449922","data":[{"x":130.26448952199212,"y":57.13715886870904},{"x":142.1304054661781,"y":57.13715886870904}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4367992055092309","data":[{"x":161.66612152300183,"y":56.729627747941095},{"x":172.74979117488306,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp49796068475762456","type":"circle","data":{"p1":{"x":142.1304054661781,"y":47.30450264897962},"p2":{"x":161.66612152300183,"y":66.84021870580335}}},{"id":"dp12323737849555427","type":"doc-cube","data":{"p1":{"x":172.59887757063825,"y":38.84193818059583},"p2":{"x":210.68923255682262,"y":76.55188495447129},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp9747833728278197","type":"rectangle","data":{"p1":{"x":366.57731762375033,"y":11.841938180595832},"p2":{"x":391.60827698470075,"y":88.84193818059583}}},{"id":"dg48705751945207343","entities":[{"id":"dg5483839555055041","entities":[{"id":"dp575668142911451","type":"rectangle","data":{"p1":{"x":324.59887757063825,"y":17.607904868061325},"p2":{"x":337.2560383026971,"y":30.26506560012018}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp08016503403204545","type":"rectangle","data":{"p1":{"x":326.18102266214555,"y":19.190049959568682},"p2":{"x":338.8381833942044,"y":31.847210691627538}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp2892912392670768","type":"rectangle","data":{"p1":{"x":327.76316775365297,"y":20.77219505107604},"p2":{"x":340.4203284857118,"y":33.429355783134895}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}}],"data":{}},{"id":"dl476644294595165","linkedId":"de8705375563265205"}]},{"id":"dp21090197840764624","type":"rectangle","data":{"p1":{"x":235.57731762375033,"y":14.841938180595832},"p2":{"x":260.60827698470075,"y":91.84193818059583}}},{"id":"da5090470079597946","data":[{"x":210.63773467215037,"y":56.729627747941095},{"x":235.60827698470075,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da16305663881483423","data":[{"x":260.8334608267643,"y":56.729627747941095},{"x":270.7314323563021,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg5268113431064796","entities":[{"id":"dg34625322291609306","entities":[{"id":"dp4907438325901321","type":"rectangle","data":{"p1":{"x":207.59887757063825,"y":18.6432747411082},"p2":{"x":220.2560383026971,"y":31.300435473167056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp9607763071254807","type":"rectangle","data":{"p1":{"x":209.1810226621456,"y":20.225419832615557},"p2":{"x":221.83818339420446,"y":32.88258056467441}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp9702120349022043","type":"rectangle","data":{"p1":{"x":210.76316775365297,"y":21.807564924122914},"p2":{"x":223.42032848571182,"y":34.46472565618177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}}],"data":{}},{"id":"dl22840323663350937","linkedId":"de8268699887031468"}]},{"id":"dg5119081581839389","entities":[{"id":"dp5997815318584838","type":"circle","data":{"p1":{"x":323.1304054661781,"y":46.99785802735977},"p2":{"x":342.66612152300183,"y":66.5335740841835}}},{"id":"dl051729928572972206","linkedId":"de16664139451638227"}]},{"id":"da41753940725179994","data":[{"x":342.66612152300183,"y":56.765716055771634},{"x":366.60827698470075,"y":56.765716055771634}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4665736284321893","data":[{"x":392.0861485032234,"y":56.215249700218635},{"x":403.60827698470075,"y":56.215249700218635}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp28495266948125453","type":"doc-cube","data":{"p1":{"x":414.592468879232,"y":55.89985181931803},"p2":{"x":452.68282386541637,"y":93.60979859319349},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp8552058952329378","type":"doc-cube","data":{"p1":{"x":414.592468879232,"y":23.89985181931803},"p2":{"x":452.68282386541637,"y":61.60979859319349},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dg17309319634559373","entities":[{"id":"dp015239561323907358","type":"circle","data":{"p1":{"x":575.3800116578016,"y":188.44739167180677},"p2":{"x":594.9157277146253,"y":207.9831077286305}}},{"id":"dl29152123864399115","linkedId":"de6724674073740904"}]},{"id":"da6983784416503829","data":[{"x":501.2671484131258,"y":198.21524970021864},{"x":575.3800116578016,"y":198.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da3283043273032493","data":[{"x":585.1478696862134,"y":55.96521918264051},{"x":585.1478696862134,"y":188.44739167180677}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp13376537653618326","type":"doc-cube","data":{"p1":{"x":606.9096450138156,"y":198.12821003487528},"p2":{"x":645,"y":235.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp3054749720417138","type":"doc-cube","data":{"p1":{"x":606.9096450138156,"y":165.8257943817677},"p2":{"x":645,"y":203.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp41034984821714504","type":"doc-cube","data":{"p1":{"x":617.592468879232,"y":208.89985181931803},"p2":{"x":655.6828238654164,"y":246.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp8886673172247268","type":"doc-cube","data":{"p1":{"x":617.592468879232,"y":176.89985181931803},"p2":{"x":655.6828238654164,"y":214.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da9953024180193935","data":[{"x":340.2560383026971,"y":26.26506560012018},{"x":366.0093994140625,"y":26.26506560012018}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da449948342434481","data":[{"x":223.42032848571182,"y":28.807564924122914},{"x":235.94245696718917,"y":28.807564924122914}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp19338476574456598","type":"doc-cube","data":{"p1":{"x":459.4913106703914,"y":119.12821003487528},"p2":{"x":497.58166565657575,"y":156.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp8030024715026778","type":"doc-cube","data":{"p1":{"x":459.4913106703914,"y":86.82579438176771},"p2":{"x":497.58166565657575,"y":124.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp125416381304714","type":"doc-cube","data":{"p1":{"x":470.17413453580775,"y":129.42721209483358},"p2":{"x":508.2644895219921,"y":167.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp6916795208149304","type":"doc-cube","data":{"p1":{"x":470.17413453580775,"y":97.42721209483358},"p2":{"x":508.2644895219921,"y":135.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp2468627412531159","type":"doc-cube","data":{"p1":{"x":525.4913106703914,"y":119.12821003487528},"p2":{"x":563.5816656565758,"y":156.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp22016459532661758","type":"doc-cube","data":{"p1":{"x":525.4913106703914,"y":86.82579438176771},"p2":{"x":563.5816656565758,"y":124.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp8150954059179112","type":"doc-cube","data":{"p1":{"x":536.1741345358078,"y":129.89985181931803},"p2":{"x":574.2644895219921,"y":167.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp05758749241223038","type":"doc-cube","data":{"p1":{"x":536.1741345358078,"y":97.89985181931803},"p2":{"x":574.2644895219921,"y":135.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dg7864340864191153","entities":[{"id":"dp18345955570639116","type":"circle","data":{"p1":{"x":232.7314323563021,"y":223.19736115422864},"p2":{"x":252.26714841312582,"y":242.73307721105238}}},{"id":"dl9306573912534319","linkedId":"de3842459334625856"}]},{"id":"da8891685749627016","data":[{"x":452.60827698470075,"y":56.215249700218635},{"x":483.1304054661781,"y":56.215249700218635}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg5666011018312356","entities":[{"id":"dp9124936588147989","type":"circle","data":{"p1":{"x":537.7314323563021,"y":46.197361154228645},"p2":{"x":557.2671484131258,"y":65.73307721105238}}},{"id":"dl7867532605259782","linkedId":"de5279245661967291"}]},{"id":"da8790688520118102","data":[{"x":547.499290384714,"y":65.73307721105238},{"x":547.499290384714,"y":86.21600341796875}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"dg8772277223546896","entities":[{"id":"dp9608104972311906","type":"circle","data":{"p1":{"x":483.1304054661781,"y":45.99785802735977},"p2":{"x":502.66612152300183,"y":65.5335740841835}}},{"id":"dl860205744073318","linkedId":"de5414059609216073"}],"data":{}},{"id":"da4537344221289057","data":[{"x":502.66612152300183,"y":55.96521918264051},{"x":537.7314323563021,"y":55.96521918264051}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da6439031813379001","data":[{"x":419.7987614003159,"y":233.21524970021864},{"x":585.1478696862134,"y":233.21524970021864}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg6839742550484962","entities":[{"id":"dg5310372500915896","entities":[{"id":"dp6417093932066409","type":"rectangle","data":{"p1":{"x":8.99359130859375,"y":1.5402473973582005},"p2":{"x":21.650752040652606,"y":14.197408129417056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp8266435787880344","type":"rectangle","data":{"p1":{"x":10.57573640010105,"y":3.1223924888655574},"p2":{"x":23.232897132159906,"y":15.779553220924413}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp5776532759061219","type":"rectangle","data":{"p1":{"x":12.157881491608464,"y":4.704537580372914},"p2":{"x":24.81504222366732,"y":17.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl7562753566974094","linkedId":"de48398552182920707"}]},{"id":"dp7209277368997147","type":"doc-cube","data":{"p1":{"x":270.5752569651695,"y":56.801277332206496},"p2":{"x":308.66561195135387,"y":94.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp3734636867943475","type":"doc-cube","data":{"p1":{"x":270.5752569651695,"y":24.801277332206496},"p2":{"x":308.66561195135387,"y":62.511224106081954},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da4212914548171849","data":[{"x":309.2671484131258,"y":56.96521918264051},{"x":323.0093994140625,"y":56.96521918264051}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da8328460715812909","data":[{"x":70.0093994140625,"y":57.13715886870904},{"x":92.26448952199212,"y":57.13715886870904}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da5204873677507988","data":[{"x":557.2671484131258,"y":55.96521918264051},{"x":585.1478696862134,"y":55.96521918264051}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg34712524270343836","entities":[{"id":"dp37922344119144635","type":"circle","data":{"p1":{"x":481.7314323563021,"y":188.19736115422864},"p2":{"x":501.2671484131258,"y":207.73307721105238}}},{"id":"dl5441292163557927","linkedId":"de9498932232987138"}]},{"id":"da9848201611653264","data":[{"x":491.49929038471396,"y":167.31321716308594},{"x":491.49929038471396,"y":189.19736115422864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9356199515291648","data":[{"x":198.14786968621343,"y":76.96521918264051},{"x":198.14786968621343,"y":130.21600341796875}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp36614154743620286","type":"rectangle","data":{"p1":{"x":226.57731762375033,"y":101.21600341796875},"p2":{"x":251.60827698470075,"y":185.21600341796875}}},{"id":"dg6506031910909329","entities":[{"id":"dp6523267676928928","type":"doc-cube","data":{"p1":{"x":191.62434362521276,"y":146.21600341796875},"p2":{"x":208.08394629477812,"y":162.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dl7345083637550276","linkedId":"de5418541516011492"}]},{"id":"da7801880500008729","data":[{"x":208.42032848571182,"y":154.80756492412291},{"x":226.0093994140625,"y":154.80756492412291}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da045930330977075995","data":[{"x":198.14786968621343,"y":130.21600341796875},{"x":226.0093994140625,"y":130.21600341796875}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp1009362638384308","type":"doc-cube","data":{"p1":{"x":266.89243309975313,"y":139.5022752722482},"p2":{"x":304.9827880859375,"y":177.21222204612354},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp8845379047524937","type":"doc-cube","data":{"p1":{"x":266.89243309975313,"y":107.19985961914062},"p2":{"x":304.9827880859375,"y":144.90980639301608},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp5398496350087281","type":"doc-cube","data":{"p1":{"x":277.592468879232,"y":149.89985181931803},"p2":{"x":315.68282386541637,"y":187.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp17001763161707162","type":"doc-cube","data":{"p1":{"x":277.592468879232,"y":117.89985181931803},"p2":{"x":315.68282386541637,"y":155.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da6755513325025082","data":[{"x":252.0093994140625,"y":142.5022752722482},{"x":266.89243309975313,"y":142.5022752722482}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da5839508455852414","data":[{"x":375.0093994140625,"y":197.9652191826405},{"x":481.7314323563021,"y":197.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da6520536481094008","data":[{"x":315.89243309975313,"y":142.5022752722482},{"x":375.0093994140625,"y":142.5022752722482}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da6223170250390233","data":[{"x":375.0093994140625,"y":142.5022752722482},{"x":375.0093994140625,"y":197.9652191826405}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg4876687212389459","entities":[{"id":"dp46454992351115565","type":"rectangle","data":{"p1":{"x":6.743766507919418,"y":101.63121309108607},"p2":{"x":36.79161019925965,"y":130.95367293703205}},"style":{"strokeColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dg8343682138407165","entities":[{"id":"dp776531624489611","type":"rectangle","data":{"p1":{"x":23.558526932530896,"y":118.92873841303452},"p2":{"x":25.66417775956546,"y":121.03438924006917}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp09636319241084101","type":"rectangle","data":{"p1":{"x":9.659299684352277,"y":105.02951116485616},"p2":{"x":39.56340500774397,"y":134.9336164882478}},"style":{"boxShadow":{"fill":[155,155,155,1]},"fillColor":[255,255,255,1]}},{"id":"dp4542673426534998","type":"rectangle","data":{"p1":{"x":37.54307489464884,"y":121.07837181585722},"p2":{"x":39.64872572168349,"y":123.18402264289205}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7517531721738098","type":"rectangle","data":{"p1":{"x":21.32248029739992,"y":130.29732108927234},"p2":{"x":23.408813226938975,"y":132.3836540188113}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7424285459413666","type":"rectangle","data":{"p1":{"x":30.57575319785525,"y":118.97381350719132},"p2":{"x":32.68140402488987,"y":121.07946433422586}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp2187897295217227","type":"rectangle","data":{"p1":{"x":28.238287600871786,"y":132.8762604049524},"p2":{"x":30.34393842790638,"y":134.9819112319871}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp591011055398821","type":"rectangle","data":{"p1":{"x":11.99966296596017,"y":127.94781616533936},"p2":{"x":14.10531379299482,"y":130.0534669923739}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp10549255661273271","type":"rectangle","data":{"p1":{"x":28.244726900036994,"y":121.26620401001804},"p2":{"x":30.350377727071645,"y":123.37185483705267}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp48315751179595523","type":"rectangle","data":{"p1":{"x":14.303644207284322,"y":121.03329672170057},"p2":{"x":16.409295034318973,"y":123.13894754873525}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp09228914560259338","type":"rectangle","data":{"p1":{"x":9.76393829578754,"y":125.7146672148329},"p2":{"x":11.798756832004472,"y":127.7494857510498}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp07696527225880301","type":"rectangle","data":{"p1":{"x":30.575753197855164,"y":130.53879480796894},"p2":{"x":32.68140402488976,"y":132.64444563500354}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5046873712573121","type":"rectangle","data":{"p1":{"x":9.866967082431444,"y":109.42967962593141},"p2":{"x":11.798756832004472,"y":113.88567464828006}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp10639888501546224","type":"rectangle","data":{"p1":{"x":9.866967082431444,"y":130.2994482204863},"p2":{"x":14.116904531492253,"y":132.3535846541991}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp03655512040885056","type":"rectangle","data":{"p1":{"x":12.030571601953284,"y":121.26620401001804},"p2":{"x":18.753199930467787,"y":123.32677974289601}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp10827553729293315","type":"rectangle","data":{"p1":{"x":16.666867000928733,"y":123.52639801701855},"p2":{"x":25.726960926426585,"y":125.6030719978096}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp23537435320969347","type":"rectangle","data":{"p1":{"x":16.666867000928733,"y":125.6030719978096},"p2":{"x":21.090665527451222,"y":127.97917338978453}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp798566212688985","type":"rectangle","data":{"p1":{"x":18.985014700416457,"y":128.2109881597334},"p2":{"x":23.408813226938975,"y":130.29732108927234}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5762405859628885","type":"rectangle","data":{"p1":{"x":32.835947204855756,"y":107.34765886434366},"p2":{"x":37.2597457313781,"y":109.43399179388268}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp52394507536378","type":"rectangle","data":{"p1":{"x":30.575753197855164,"y":109.60785287134428},"p2":{"x":34.999551724377625,"y":111.6941858008833}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp08281576660854384","type":"rectangle","data":{"p1":{"x":37.51087839882254,"y":111.80578101790638},"p2":{"x":39.44266814839574,"y":116.16840620235891}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5577979226831644","type":"rectangle","data":{"p1":{"x":35.250684391822006,"y":111.90990232291898},"p2":{"x":37.31769942386532,"y":116.3884348923458}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5057205085433467","type":"rectangle","data":{"p1":{"x":37.51087839882254,"y":125.65671352234548},"p2":{"x":39.57789343086583,"y":130.1352460917726}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp4512706381415301","type":"rectangle","data":{"p1":{"x":32.85526510235144,"y":132.905237251196},"p2":{"x":37.2597457313781,"y":134.8756627957606}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9794822969993058","type":"rectangle","data":{"p1":{"x":25.939457798879687,"y":116.62024966229475},"p2":{"x":30.363256325402062,"y":118.70658259183358}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp044264019666153454","type":"rectangle","data":{"p1":{"x":18.98018522604255,"y":109.65614761508363},"p2":{"x":21.0858360530772,"y":111.76179844211828}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp1466883217919721","type":"rectangle","data":{"p1":{"x":25.934628324505752,"y":111.97429531457135},"p2":{"x":28.04027915154049,"y":114.079946141606}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp650343481751867","type":"rectangle","data":{"p1":{"x":30.570923723481258,"y":125.94113520398486},"p2":{"x":32.67657455051585,"y":128.04678603101974}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9510716723900396","type":"rectangle","data":{"p1":{"x":32.889071422968925,"y":123.5070801195229},"p2":{"x":34.994722250003576,"y":125.61273094655746}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp49548771039898365","type":"rectangle","data":{"p1":{"x":25.934628324505752,"y":107.39595360808312},"p2":{"x":28.04027915154049,"y":109.5016044351178}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp28752193051771213","type":"rectangle","data":{"p1":{"x":16.662037526554798,"y":114.29244301405907},"p2":{"x":18.767688353589506,"y":116.3980938410937}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp42681388277735866","type":"rectangle","data":{"p1":{"x":28.252776023993505,"y":105.01985221610806},"p2":{"x":30.358426851028156,"y":107.12550304314286}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}}]}]},{"id":"dg7947812146816244","entities":[{"id":"dg42402985072836286","entities":[{"id":"dp5366672673986501","type":"rectangle","data":{"p1":{"x":6.754925534814049,"y":138.60033347539206},"p2":{"x":36.80276922615428,"y":167.92279332133808}},"style":{"strokeColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp01476874744542922","type":"rectangle","data":{"p1":{"x":9.75492553481405,"y":141.60033347539206},"p2":{"x":39.80276922615428,"y":170.92279332133808}},"style":{"strokeColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]},"fillColor":[255,255,255,1]}}]},{"id":"dp6630803563195715","type":"rectangle","data":{"p1":{"x":32.93896497293281,"y":154.25366925943968},"p2":{"x":35.022598812787294,"y":156.33730309929422}},"style":{"fillColor":[245,166,35,1],"strokeColor":[245,166,35,1],"boxShadow":{"fill":[155,155,155,1]}}}]},{"id":"dp2657910889604185","type":"rectangle","data":{"p1":{"x":83.026611328125,"y":100.21600341796875},"p2":{"x":91.0093994140625,"y":189.21600341796875}}},{"id":"dp08631295206854994","type":"rectangle","data":{"p1":{"x":94.026611328125,"y":100.21600341796875},"p2":{"x":118.026611328125,"y":189.21600341796875}}},{"id":"dp5015713956466579","type":"rectangle","data":{"p1":{"x":56.026611328125,"y":100.21600341796875},"p2":{"x":80.026611328125,"y":189.21600341796875}}},{"id":"da2316879304074464","data":[{"x":38.56340500774397,"y":136.9336164882478},{"x":55.42493473559304,"y":136.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da7603240354022516","data":[{"x":24.49929038471396,"y":171.31321716308594},{"x":24.49929038471396,"y":188.19736115422864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg1092150889775978","entities":[{"id":"dp9954113311031296","type":"rectangle","data":{"p1":{"x":23.558526932530896,"y":202.92873841303452},"p2":{"x":25.66417775956546,"y":205.03438924006917}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp13339104191848405","type":"rectangle","data":{"p1":{"x":9.659299684352277,"y":189.02951116485616},"p2":{"x":39.56340500774397,"y":218.9336164882478}},"style":{"boxShadow":{"fill":[155,155,155,1]},"fillColor":[255,255,255,1]}},{"id":"dp9215697306740127","type":"rectangle","data":{"p1":{"x":37.54307489464884,"y":205.07837181585722},"p2":{"x":39.64872572168349,"y":207.18402264289205}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9893460518428052","type":"rectangle","data":{"p1":{"x":21.32248029739992,"y":214.29732108927234},"p2":{"x":23.408813226938975,"y":216.3836540188113}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp8627106894066896","type":"rectangle","data":{"p1":{"x":30.57575319785525,"y":202.97381350719132},"p2":{"x":32.68140402488987,"y":205.07946433422586}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5575418095764657","type":"rectangle","data":{"p1":{"x":28.238287600871786,"y":216.8762604049524},"p2":{"x":30.34393842790638,"y":218.9819112319871}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp1290207446549887","type":"rectangle","data":{"p1":{"x":11.99966296596017,"y":211.94781616533936},"p2":{"x":14.10531379299482,"y":214.0534669923739}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9442750653267553","type":"rectangle","data":{"p1":{"x":28.244726900036994,"y":205.26620401001804},"p2":{"x":30.350377727071645,"y":207.37185483705267}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp4802362519752237","type":"rectangle","data":{"p1":{"x":14.303644207284322,"y":205.03329672170057},"p2":{"x":16.409295034318973,"y":207.13894754873525}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp2723767529078016","type":"rectangle","data":{"p1":{"x":9.76393829578754,"y":209.7146672148329},"p2":{"x":11.798756832004472,"y":211.7494857510498}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7569028132398223","type":"rectangle","data":{"p1":{"x":30.575753197855164,"y":214.53879480796894},"p2":{"x":32.68140402488976,"y":216.64444563500354}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9970278121826268","type":"rectangle","data":{"p1":{"x":9.866967082431444,"y":193.4296796259314},"p2":{"x":11.798756832004472,"y":197.88567464828006}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp4036610544119197","type":"rectangle","data":{"p1":{"x":9.866967082431444,"y":214.2994482204863},"p2":{"x":14.116904531492253,"y":216.3535846541991}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp8968742480258425","type":"rectangle","data":{"p1":{"x":12.030571601953284,"y":205.26620401001804},"p2":{"x":18.753199930467787,"y":207.326779742896}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp1899883385859371","type":"rectangle","data":{"p1":{"x":16.666867000928733,"y":207.52639801701855},"p2":{"x":25.726960926426585,"y":209.6030719978096}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp8509824335979563","type":"rectangle","data":{"p1":{"x":16.666867000928733,"y":209.6030719978096},"p2":{"x":21.090665527451222,"y":211.97917338978453}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp6477753281033174","type":"rectangle","data":{"p1":{"x":18.985014700416457,"y":212.2109881597334},"p2":{"x":23.408813226938975,"y":214.29732108927234}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp33687450466130264","type":"rectangle","data":{"p1":{"x":32.835947204855756,"y":191.34765886434366},"p2":{"x":37.2597457313781,"y":193.43399179388268}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp6422861029956799","type":"rectangle","data":{"p1":{"x":30.575753197855164,"y":193.60785287134428},"p2":{"x":34.999551724377625,"y":195.6941858008833}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp16854570501165456","type":"rectangle","data":{"p1":{"x":37.51087839882254,"y":195.80578101790638},"p2":{"x":39.44266814839574,"y":200.1684062023589}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7190945406323468","type":"rectangle","data":{"p1":{"x":35.250684391822006,"y":195.90990232291898},"p2":{"x":37.31769942386532,"y":200.3884348923458}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp8201804471978769","type":"rectangle","data":{"p1":{"x":37.51087839882254,"y":209.65671352234548},"p2":{"x":39.57789343086583,"y":214.1352460917726}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp0978748132177627","type":"rectangle","data":{"p1":{"x":32.85526510235144,"y":216.905237251196},"p2":{"x":37.2597457313781,"y":218.8756627957606}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp17876075451600437","type":"rectangle","data":{"p1":{"x":25.939457798879687,"y":200.62024966229475},"p2":{"x":30.363256325402062,"y":202.70658259183358}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9290422019998839","type":"rectangle","data":{"p1":{"x":18.98018522604255,"y":193.65614761508363},"p2":{"x":21.0858360530772,"y":195.76179844211828}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp12588320681146237","type":"rectangle","data":{"p1":{"x":25.934628324505752,"y":195.97429531457135},"p2":{"x":28.04027915154049,"y":198.079946141606}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp6519377730025322","type":"rectangle","data":{"p1":{"x":30.570923723481258,"y":209.94113520398486},"p2":{"x":32.67657455051585,"y":212.04678603101974}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp22105976859820342","type":"rectangle","data":{"p1":{"x":32.889071422968925,"y":207.5070801195229},"p2":{"x":34.994722250003576,"y":209.61273094655746}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp1855997675757235","type":"rectangle","data":{"p1":{"x":25.934628324505752,"y":191.39595360808312},"p2":{"x":28.04027915154049,"y":193.5016044351178}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp09107112896950009","type":"rectangle","data":{"p1":{"x":16.662037526554798,"y":198.29244301405907},"p2":{"x":18.767688353589506,"y":200.3980938410937}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp410629668178655","type":"rectangle","data":{"p1":{"x":28.252776023993505,"y":189.01985221610806},"p2":{"x":30.358426851028156,"y":191.12550304314286}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}}]},{"id":"dg2423948431923939","entities":[{"id":"dp10443581611316621","type":"rectangle","data":{"p1":{"x":9.75492553481405,"y":222.60033347539206},"p2":{"x":39.80276922615428,"y":251.92279332133808}},"style":{"strokeColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]},"fillColor":[255,255,255,1]}},{"id":"dp46357080878324264","type":"rectangle","data":{"p1":{"x":32.93896497293281,"y":236.25366925943968},"p2":{"x":35.022598812787294,"y":238.33730309929422}},"style":{"fillColor":[245,166,35,1],"strokeColor":[245,166,35,1],"boxShadow":{"fill":[155,155,155,1]}}}]},{"id":"dg2629691174216253","entities":[{"id":"dg41920582080262037","entities":[{"id":"dl2645106817182066","linkedId":"de3957690388394757"},{"id":"dl8307616693404456","linkedId":"de9437130437561829"},{"id":"dl5381812000928694","linkedId":"de7794946484826855"}],"data":{"rotation":90}},{"id":"dg9374920961374769","entities":[{"id":"dl3584575941687689","linkedId":"de9991017222779492"},{"id":"dl9100732043267474","linkedId":"de19958885418575512"},{"id":"dl6432441582775346","linkedId":"de49845263097063075"}],"data":{"rotation":90}},{"id":"dp9677582662226305","type":"rectangle","data":{"p1":{"x":83.026611328125,"y":193.1030216217041},"p2":{"x":91.026611328125,"y":264.1030216217041}}},{"id":"dp5483405438508648","type":"rectangle","data":{"p1":{"x":94.026611328125,"y":193.1030216217041},"p2":{"x":118.026611328125,"y":264.1030216217041}}},{"id":"dp6739538718666911","type":"rectangle","data":{"p1":{"x":56.026611328125,"y":193.1030216217041},"p2":{"x":80.026611328125,"y":264.1030216217041}}},{"id":"dl8054083505541851","linkedId":"de8913158837985631"}]},{"id":"da7987444022977732","data":[{"x":38.56340500774397,"y":220.9336164882478},{"x":55.42493473559304,"y":220.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4833872206251586","data":[{"x":118.42493473559304,"y":220.9336164882478},{"x":162.0093994140625,"y":220.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da28774511274180226","data":[{"x":117.42493473559304,"y":136.9336164882478},{"x":131.0093994140625,"y":136.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp032300108571785335","type":"doc-cube","data":{"p1":{"x":130.90964501381563,"y":137.12821003487528},"p2":{"x":169,"y":174.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp8689638891930163","type":"doc-cube","data":{"p1":{"x":130.90964501381563,"y":104.82579438176771},"p2":{"x":169,"y":142.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp46796818169982624","type":"doc-cube","data":{"p1":{"x":141.592468879232,"y":147.89985181931803},"p2":{"x":179.68282386541637,"y":185.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp18654960695364986","type":"doc-cube","data":{"p1":{"x":141.592468879232,"y":115.89985181931803},"p2":{"x":179.68282386541637,"y":153.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5796097857133129","type":"doc-cube","data":{"p1":{"x":224.49131067039139,"y":286.1282100348753},"p2":{"x":262.58166565657575,"y":323.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp8905943944570951","type":"doc-cube","data":{"p1":{"x":224.49131067039139,"y":253.8257943817677},"p2":{"x":262.58166565657575,"y":291.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp07475380820616206","type":"doc-cube","data":{"p1":{"x":235.17413453580775,"y":296.4272120948336},"p2":{"x":273.2644895219921,"y":334.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp04076385251012349","type":"doc-cube","data":{"p1":{"x":235.17413453580775,"y":264.4272120948336},"p2":{"x":273.2644895219921,"y":302.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp256726783214128","type":"doc-cube","data":{"p1":{"x":290.4913106703914,"y":284.1282100348753},"p2":{"x":328.58166565657575,"y":321.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp02970722890567945","type":"doc-cube","data":{"p1":{"x":290.4913106703914,"y":251.8257943817677},"p2":{"x":328.58166565657575,"y":289.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp15340142017396352","type":"doc-cube","data":{"p1":{"x":301.17413453580775,"y":294.89985181931803},"p2":{"x":339.2644895219921,"y":332.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp3371339396431723","type":"doc-cube","data":{"p1":{"x":301.17413453580775,"y":262.89985181931803},"p2":{"x":339.2644895219921,"y":300.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da1936716116269368","data":[{"x":211.68282386541637,"y":232.9652191826405},{"x":232.7314323563021,"y":232.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da09652295103309871","data":[{"x":242.49929038471396,"y":242.73307721105238},{"x":242.49929038471396,"y":253.38780212402344}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da05570659084657903","data":[{"x":165.0093994140625,"y":185.5022752722482},{"x":165.0093994140625,"y":192.94285583496094}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da503179763891904","data":[{"x":165.0093994140625,"y":192.94285583496094},{"x":306.49929038471396,"y":192.94285583496094}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg8303076532667495","entities":[{"id":"dp9919009890132662","type":"circle","data":{"p1":{"x":296.7314323563021,"y":203.19736115422864},"p2":{"x":316.2671484131258,"y":222.73307721105238}}},{"id":"dl3281941997823845","linkedId":"de7312818138853312"}]},{"id":"da012760867966330913","data":[{"x":306.49929038471396,"y":192.94285583496094},{"x":306.49929038471396,"y":203.19736115422864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da17610889282896403","data":[{"x":306.49929038471396,"y":222.73307721105238},{"x":306.49929038471396,"y":251.94285583496094}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da7954537709950458","data":[{"x":252.26714841312582,"y":232.9652191826405},{"x":336.38001165780156,"y":232.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg022188156504345358","entities":[{"id":"dp882701495807743","type":"circle","data":{"p1":{"x":336.38001165780156,"y":223.44739167180677},"p2":{"x":355.9157277146253,"y":242.9831077286305}}},{"id":"dl5767208896380549","linkedId":"de18788604977197143"}]},{"id":"da007392881901756132","data":[{"x":346.1478696862134,"y":213.19288635253906},{"x":346.1478696862134,"y":223.44739167180677}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da5608151902147727","data":[{"x":316.2671484131258,"y":212.9652191826405},{"x":346.1478696862134,"y":213.19288635253906}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9982419724932328","data":[{"x":355.9157277146253,"y":233.21524970021864},{"x":370.7987614003159,"y":233.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp5494387577736761","type":"doc-cube","data":{"p1":{"x":371.90964501381563,"y":240.12821003487528},"p2":{"x":410,"y":277.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp9840299030242623","type":"doc-cube","data":{"p1":{"x":371.90964501381563,"y":207.8257943817677},"p2":{"x":410,"y":245.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp0700905801207472","type":"doc-cube","data":{"p1":{"x":382.592468879232,"y":250.89985181931803},"p2":{"x":420.68282386541637,"y":288.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp7358646795505828","type":"doc-cube","data":{"p1":{"x":382.592468879232,"y":218.89985181931803},"p2":{"x":420.68282386541637,"y":256.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da35931337732752766","data":[{"x":585.1478696862134,"y":207.9831077286305},{"x":585.1478696862134,"y":233.21524970021864}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da4465892145796957","data":[{"x":594.9157277146253,"y":198.21524970021864},{"x":606.9096450138156,"y":198.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp43037807676417295","type":"doc-cube","data":{"p1":{"x":608.1741345358078,"y":85.42721209483358},"p2":{"x":646.2644895219921,"y":123.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp46356129901525867","type":"doc-cube","data":{"p1":{"x":608.1741345358078,"y":53.42721209483358},"p2":{"x":646.2644895219921,"y":91.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da4033821799514925","data":[{"x":60.49929038471396,"y":8.21600341796875},{"x":60.49929038471396,"y":52.197361154228645}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da31513085646614347","data":[{"x":24.81504222366732,"y":8.704537580372914},{"x":597.0093994140625,"y":8.704537580372914}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg400068704729871","entities":[{"id":"dp09758932003963472","type":"circle","data":{"p1":{"x":617.7314323563021,"y":134.19736115422864},"p2":{"x":637.2671484131258,"y":153.73307721105238}}},{"id":"dl3052853572706562","linkedId":"de9514175999666843"}]},{"id":"da7860029488436255","data":[{"x":627.499290384714,"y":153.73307721105238},{"x":627.499290384714,"y":165.94285583496094}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da8378432600870507","data":[{"x":627.499290384714,"y":123.21600341796875},{"x":627.499290384714,"y":134.19736115422864}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da10865471188678466","data":[{"x":597.0093994140625,"y":143.9652191826405},{"x":617.7314323563021,"y":143.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da43058112228638956","data":[{"x":597.0093994140625,"y":8.704537580372914},{"x":597.0093994140625,"y":143.9652191826405}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6}],"settings":{"grid":true,"diagramHeight":347.9201354980469}}]},{"id":"n0.3370407539120146","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":3860,"delayRenderCache":{"av":3860,"map":{"n0.4948186869059896":{"n0.24224066795434895":{"w":53.7652,"h":8.4545,"bl":0.8214}},"n0.03631791790874783":{"n0.8114851563395926":{"w":24.7215,"h":8.1019,"bl":0.8571}},"n0.10368321027700222":{"n0.10192837968410129":{"w":54.0093,"h":8.4545,"bl":0.8214}},"n0.6113778876903095":{"n0.1471848314421922":{"w":24.7215,"h":8.1019,"bl":0.8571}},"n0.04103796103922863":{"n0.9774562041920496":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.9346331450716716":{"n0.15286703063243756":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.4658812440199587":{"n0.522341707304876":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.6779540611266668":{"n0.7037197434395268":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.2594341695196014":{"n0.3315585301606032":{"w":71.7773,"h":8.4545,"bl":0.8214}},"n0.8035966151360414":{"n0.035945705013095575":{"w":58.9916,"h":8.4545,"bl":0.8214}},"n0.8652985179455455":{"n0.9974246527053048":{"w":73.0433,"h":8.4545,"bl":0.8214}},"n0.3405674873132667":{"n0.13909617635472848":{"w":15.625,"h":9.1146,"bl":0.7619}},"n0.019004960502556623":{"n0.960706236887447":{"w":20.3631,"h":9.4491,"bl":0.8402}},"n0.4540862647774402":{"n0.6959331038941989":{"w":29.6766,"h":9.1146,"bl":0.7619}},"n0.7517415472449318":{"n0.4306183045431822":{"w":7.0349,"h":8.4545,"bl":0.8214}},"n0.408476759756512":{"n0.04906427405686231":{"w":21.6743,"h":9.1146,"bl":0.7619}},"n0.8174948536978763":{"n0.25329414575928455":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.6850706070771972":{"n0.7081331412186238":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.9153175281526549":{"n0.36970927642703466":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.047463607109459405":{"n0.31354421293919166":{"w":20.7972,"h":9.9736,"bl":0.6963}},"n0.6377335918019102":{"n0.7635891487221897":{"w":6.9897,"h":9.4491,"bl":0.8402}},"n0.769201243672291":{"n0.773475139164786":{"w":6.7455,"h":9.4491,"bl":0.8402}},"n0.8651163527017454":{"n0.6524612630217288":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.6138080945790303":{"n0.4248082564228923":{"w":24.6672,"h":9.1146,"bl":0.7619}},"n0.40235662659270877":{"n0.4120157811821672":{"w":54.6604,"h":8.4545,"bl":0.8214}},"n0.5663416250436877":{"n0.8672176115946004":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.2688194492057001":{"n0.4139531593661605":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.8434406802059295":{"n0.3127101080275474":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.8084507466865571":{"n0.2070918756904696":{"w":62.5,"h":8.1019,"bl":0.8571}},"n0.4078630694843064":{"n0.5764231602461787":{"w":35.3823,"h":8.1019,"bl":0.8571}},"n0.1325705150031895":{"n0.29351627084059895":{"w":6.0764,"h":8.4545,"bl":0.8214}},"n0.5354735391707355":{"n0.011029513288379977":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.3210884854241822":{"n0.7063629133230427":{"w":63.4856,"h":8.1019,"bl":0.8571}},"n0.633784928341107":{"n0.02722195288173035":{"w":69.2817,"h":8.1019,"bl":0.8571}},"n0.0671748381274353":{"n0.3382643066492892":{"w":42.164,"h":8.1019,"bl":0.8571}},"n0.12323602675056611":{"n0.9924403943583895":{"w":49.8861,"h":8.4545,"bl":0.8214}},"n0.14206887739882257":{"n0.5611562227899454":{"w":35.3823,"h":8.1019,"bl":0.8571}},"n0.36024324575911404":{"n0.31301881936258424":{"w":35.3823,"h":8.1019,"bl":0.8571}},"n0.2982039446388105":{"n0.2095657756783389":{"w":19.694,"h":8.4545,"bl":0.8214}},"n0.39382613896308327":{"n0.6655942045909249":{"w":7.4599,"h":8.4545,"bl":0.8214}},"n0.7869443691048681":{"n0.9862134259506325":{"w":18.9254,"h":8.4545,"bl":0.8214}},"n0.3888587151739875":{"n0.1563681651083162":{"w":23.9981,"h":9.9736,"bl":0.6963}},"n0.4091118874775652":{"n0.2830138817581649":{"w":20.9871,"h":9.9736,"bl":0.6963}},"n0.747319571117421":{"n0.9579442511261114":{"w":19.694,"h":8.4545,"bl":0.8214}},"n0.7089762412406253":{"n0.3805910514369335":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.4177074897863875":{"n0.08339218194311648":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.26785386114980914":{"n0.9209111051638239":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.9409319662631248":{"n0.4931140849769742":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.7764373811879":{"n0.19153155965893243":{"w":24.4231,"h":9.1146,"bl":0.7619}}}}}

==> plots/docs/d31f12dc-761f-4b2e-977d-e46e77d677c6 <==
{"id":"n0.25338045829944633","lines":[{"id":"n0.7943069201579043","blocks":[]},{"id":"n0.8548540010333312","blocks":[{"id":"n0.28855487568557425","text":"\\diagram","type":"composite","elements":{"de5520970398776124":{"id":"de5520970398776124","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.27151433873504516"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4636885140653977"}],"id":"n0.1117015472631393"}],"id":"n0.7622507405737542"}},"id":"n0.1394569138907935"},{"text":"|×|𝛺","id":"n0.2675884865558562"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.2315164678700763"}],"id":"n0.2749069621900577"}],"id":"n0.34863616730742186"}},"id":"n0.14457479221384584"},{"text":"|","id":"n0.047235420711965403"}],"id":"n0.8622852515762334"}],"id":"n0.6538694462700769"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8783443695980817"}],"style":{"align":"center"},"id":"n0.07846061311474695"}],"shape":{"data":{"p":{"x":189.09038550376243,"y":63.23626428200146},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de828983001736362":{"id":"de828983001736362","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.14179019025753226"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5749151404407025"}],"id":"n0.2143796473185655"}],"id":"n0.09084256075912345"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.4641599294522796"}],"id":"n0.7513396748046104"}],"id":"n0.37517258111186624"}},"id":"n0.3889504856587369"},{"type":"single","text":"(","id":"n0.4153840753872462"},{"text":"s","id":"n0.27379039666989824"},{"type":"single","text":")","id":"n0.4721169865752184"}],"id":"n0.6615510692663404"}],"id":"n0.0967657311158161"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.4013948251365338"}],"style":{"align":"center"},"id":"n0.441050774848742"}],"shape":{"data":{"p":{"x":113.40753112076794,"y":164.39516869378502},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de07208453170872553":{"id":"de07208453170872553","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.9495180972961037"}],"id":"n0.43859045338187364"}],"id":"n0.006608013145942282"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.493594653748731"}],"style":{"align":"center"},"id":"n0.6349481183113024"}],"shape":{"data":{"p":{"x":96,"y":179.2900532261246},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8834167216713067":{"id":"de8834167216713067","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.22364208655963358"}],"id":"n0.08847662245070831"}],"id":"n0.5562758659701175"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6771809112206673"}],"style":{"align":"center"},"id":"n0.19983733450358176"}],"shape":{"data":{"p":{"x":203.39034972428357,"y":297.9838562011719},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de04997776156109879":{"id":"de04997776156109879","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.897803963229926"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.08874136617804429"}],"id":"n0.34502941267511034"}],"id":"n0.4261746236899189"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.94840773762354"}],"id":"n0.2666371980940394"}],"id":"n0.042645947864674794"}},"id":"n0.3816973634716303"},{"type":"single","text":"(","id":"n0.48950838725563806"},{"text":"s","id":"n0.5769828033292839"},{"type":"single","text":")","id":"n0.10888111089770058"}],"id":"n0.9817385017994846"}],"id":"n0.5955230560954696"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.06144290259826923"}],"style":{"align":"center"},"id":"n0.046256853314367685"}],"shape":{"data":{"p":{"x":446.4979166245305,"y":23.395168693785024},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1263861426676729":{"id":"de1263861426676729","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.5579350812384536"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3478954273203627"}],"id":"n0.19435338820378134"}],"id":"n0.6165632336495481"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.48810065734612507"}],"id":"n0.6527594226319431"}],"id":"n0.9927622996794807"}},"id":"n0.3310870136335953"},{"type":"single","text":"(","id":"n0.24733232207573397"},{"text":"s,a","id":"n0.2640130706228947"},{"type":"single","text":")","id":"n0.320797152671904"}],"id":"n0.12385914641248141"}],"id":"n0.10292510313515457"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.8792233341240645"}],"style":{"align":"center"},"id":"n0.581431440814911"}],"shape":{"data":{"p":{"x":225.07317358969993,"y":153.98044260802277},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7586505332283031":{"id":"de7586505332283031","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.4927180768830606"}],"id":"n0.7049969082472012"}],"id":"n0.5491990457901264"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8331730280336691"}],"style":{"align":"center"},"id":"n0.4908615520610786"}],"shape":{"data":{"p":{"x":217.66564246893194,"y":205.87532714036234},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de769876825831503":{"id":"de769876825831503","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.2476163548834478"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.05289691975208344"}],"id":"n0.9475595525928506"}],"id":"n0.26913830451602294"}},"id":"n0.3823787096886917"},{"text":"|","id":"n0.3572567729085736"}],"id":"n0.6437754419605293"}],"id":"n0.801448369692964"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8248570835206583"}],"style":{"align":"center"},"id":"n0.33378938373308187"}],"shape":{"data":{"p":{"x":125.09038550376243,"y":124.16184319124937},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9878510090899617":{"id":"de9878510090899617","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.26474967983170705"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8971092040815121"}],"id":"n0.589078373381241"}],"id":"n0.6144261277188128"}},"id":"n0.6252549284208646"},{"text":"|","id":"n0.012925371806804309"}],"id":"n0.9645001095314869"}],"id":"n0.16824565767494604"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.36432594095690884"}],"style":{"align":"center"},"id":"n0.9517376011612726"}],"shape":{"data":{"p":{"x":125.09038550376243,"y":104.16184319124937},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de040532016393358905":{"id":"de040532016393358905","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|𝛺","id":"n0.017627045438355138"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.567640267774302"}],"id":"n0.5876253790254438"}],"id":"n0.8016798244873558"}},"id":"n0.29881555110954827"},{"text":"|","id":"n0.5141272299841424"}],"id":"n0.8320770388847725"}],"id":"n0.5233019382756188"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3876548054566744"}],"style":{"align":"center"},"id":"n0.7670897406456516"}],"shape":{"data":{"p":{"x":125.09038550376243,"y":83.16184319124937},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4342493044242768":{"id":"de4342493044242768","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.9688909438345801"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.11465109772496085"}],"id":"n0.805198393901633"}],"id":"n0.9860014414794123"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.3365944052709"}],"id":"n0.24308677305968152"}],"id":"n0.33971423872499673"}},"id":"n0.4481408429704987"},{"type":"single","text":"(","id":"n0.48292648096903945"},{"text":"s","id":"n0.09419811564487834"},{"type":"single","text":")","id":"n0.1532926878468186"}],"id":"n0.9863990264272267"}],"id":"n0.39686664852335385"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.47318647813400827"}],"style":{"align":"center"},"id":"n0.4561115989782121"}],"shape":{"data":{"p":{"x":569.4979166245305,"y":164.39516869378502},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1069292797428456":{"id":"de1069292797428456","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"composite","text":"\\Pr","elements":{},"id":"n0.893109935736548"},{"type":"single","text":"(","id":"n0.9543708301694047"},{"text":"o","id":"n0.9304630750587284"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7951549406875484"}],"id":"n0.3259176389383067"}],"id":"n0.3838815664172657"}},"id":"n0.012190115400921409"},{"text":"|s,a","id":"n0.6633100830421328"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4796694870508367"}],"id":"n0.08360553435830642"}],"id":"n0.8402381803414027"}},"id":"n0.22742123199036857"},{"type":"single","text":")","id":"n0.9526418894946047"}],"id":"n0.21882807550247785"}],"id":"n0.7414166285458648"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.15957685423588397"}],"style":{"align":"center"},"id":"n0.8382613973508035"}],"shape":{"data":{"p":{"x":319.7082014974316,"y":23.743954711688957},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7272921803134598":{"id":"de7272921803134598","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.6169228088745604"}],"id":"n0.8192075369172236"}],"id":"n0.5053983715856316"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.49323858999303005"}],"style":{"align":"center"},"id":"n0.22946509979998075"}],"shape":{"data":{"p":{"x":308.06606823920555,"y":39.44087589846373},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3762499993351762":{"id":"de3762499993351762","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.07320753465653862"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.46024205589598743"}],"id":"n0.9452681236751148"}],"id":"n0.6955125721326587"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.5312255638734711"}],"id":"n0.39967597290956625"}],"id":"n0.9341639557260559"}},"id":"n0.4175368060735638"},{"type":"single","text":"(","id":"n0.8125475236978077"},{"text":"s","id":"n0.351545201203727"},{"type":"single","text":")","id":"n0.7249340044377426"}],"id":"n0.5234834432647619"}],"id":"n0.8204346809622691"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.1835526429852079"}],"style":{"align":"center"},"id":"n0.36577372130072083"}],"shape":{"data":{"p":{"x":569.4979166245305,"y":265.395168693785},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5537469412531904":{"id":"de5537469412531904","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.3444215796140062"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6732995066259508"}],"id":"n0.2317602136179413"}],"id":"n0.04477763558765413"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.24421246794559215"}],"id":"n0.24136736621281973"}],"id":"n0.802362797715338"}},"id":"n0.036129547494320846"},{"type":"single","text":"(","id":"n0.1905873277459469"},{"text":"s,a","id":"n0.7504823179517286"},{"type":"single","text":")","id":"n0.9556456824948709"}],"id":"n0.4968593472306042"}],"id":"n0.6329778626633036"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.5871582382398293"}],"style":{"align":"center"},"id":"n0.031214142057099936"}],"shape":{"data":{"p":{"x":240.2436271377868,"y":254.98044260802277},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de38487360283742666":{"id":"de38487360283742666","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⟨s,a⟩∈P","id":"n0.9493257460171807"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.0637310156548887"}],"id":"n0.6215067546401203"}],"id":"n0.19531961549334165"},"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.010474151883645755"}],"id":"n0.5030753749829053"}],"id":"n0.301602005952047"}},"id":"n0.8037365022814322"}],"id":"n0.7795957295841542"}],"id":"n0.8476611167760499"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6221849330837028"}],"id":"n0.26477504035527244"}],"shape":{"data":{"p":{"x":238.34978491782493,"y":286.7481257493629},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9715702645442834":{"id":"de9715702645442834","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.6249619007940019"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.7804181971152868"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.5010191634308674"}],"id":"n0.09833512951191548"}],"id":"n0.7775190735055468"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.6356951276867575"}],"id":"n0.8668797493357865"}],"id":"n0.32877103183081413"}},"id":"n0.4500177953582223"}],"id":"n0.83712498968937"}],"id":"n0.04838708755876753"}},"id":"n0.7587963723902582"},{"type":"single","text":"(","id":"n0.9035787260749824"},{"text":"s,a","id":"n0.9119426963835975"},{"type":"single","text":")","id":"n0.8996281514045852"}],"id":"n0.44456487845322856"}],"id":"n0.37357327720965383"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3415234652411294"}],"style":{"align":"center"},"id":"n0.08209456400124648"}],"shape":{"data":{"p":{"x":117.49150793312418,"y":254.38679544305194},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de777519150267751":{"id":"de777519150267751","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.708169864947874"}],"id":"n0.4600841538833922"}],"id":"n0.803624317973094"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.15327389506075506"}],"style":{"align":"center"},"id":"n0.13008437109947923"}],"shape":{"data":{"p":{"x":80.09038550376243,"y":295.8070040280952},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2938177892970333":{"id":"de2938177892970333","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.41806308068322995"}],"id":"n0.08978729943238095"}],"id":"n0.2483893817822127"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7966415745224384"}],"style":{"align":"center"},"id":"n0.22000167342181998"}],"shape":{"data":{"p":{"x":426.47145004048775,"y":38.98591809822463},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de49606201729253674":{"id":"de49606201729253674","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.4662020816813366"}],"id":"n0.9923703182999024"}],"id":"n0.10744352025325266"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.24604688373448957"}],"id":"n0.8519992825477789"}],"shape":{"data":{"p":{"x":111.09038550376243,"y":201.52163415504833}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de23325305718254907":{"id":"de23325305718254907","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.7979787517676606"}],"id":"n0.5573311515059192"}],"id":"n0.7963742656758848"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9131254761902869"}],"id":"n0.6855452719069914"}],"shape":{"data":{"p":{"x":481.0839768123562,"y":263.08373345003844}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9752351203905827":{"id":"de9752351203905827","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.5411448237521672"}],"id":"n0.42940441151394837"}],"id":"n0.6249678696487018"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5251141136924362"}],"id":"n0.6205838356665792"}],"shape":{"data":{"p":{"x":451.0839768123562,"y":263.04836357699156}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4427510142690705":{"id":"de4427510142690705","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.6473788903274942"}],"id":"n0.28172712935215594"}],"id":"n0.49565357867421134"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5717228225550308"}],"id":"n0.38989133361763373"}],"shape":{"data":{"p":{"x":363.07317358969993,"y":20.67738061500927}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de21516737336846048":{"id":"de21516737336846048","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.6552982732289234"}],"id":"n0.01837465200897337"}],"id":"n0.03166421290171506"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6980806282271741"}],"id":"n0.700129871063206"}],"shape":{"data":{"p":{"x":279.0839768123562,"y":21.083733450038437}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de66011368422189":{"id":"de66011368422189","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.4181417722821359"}],"id":"n0.2901340212969634"}],"id":"n0.9377912065800365"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7114358006326251"}],"id":"n0.9572312474456759"}],"shape":{"data":{"p":{"x":247.08397681235618,"y":21.048363576991562}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de17339897452830244":{"id":"de17339897452830244","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.32011581099575515"}],"id":"n0.48032552796931505"}],"id":"n0.6098667043946604"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.1918989233501993"}],"id":"n0.1123475664115372"}],"shape":{"data":{"p":{"x":492.09038550376243,"y":162.52163415504833}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6658095144342686":{"id":"de6658095144342686","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.04566694455289677"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"o","id":"n0.4690478936906626"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.26568131608860956"}],"id":"n0.4181611779164287"}],"id":"n0.9796608489781882"}},"id":"n0.19874676327498553"}],"id":"n0.17563860398529862"}],"id":"n0.518107722756628"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.030613434388105487"}],"id":"n0.0857132965788101"}],"id":"n0.5927140745037591"}},"id":"n0.44439756021995347"}],"id":"n0.7050310140621812"}],"id":"n0.5206787888668472"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9436715546247578"}],"id":"n0.8866638644305771"}],"shape":{"data":{"p":{"x":141.08397681235618,"y":75.3920107419624}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de7522212595218865":{"id":"de7522212595218865","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.9201805558857985"}],"id":"n0.4150342211710165"}],"id":"n0.9756851757003704"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.24536760764214205"}],"id":"n0.3505649113359728"}],"shape":{"data":{"p":{"x":299.09038550376243,"y":162.52163415504833}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de41418421309961495":{"id":"de41418421309961495","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.017504874173464913"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.4824121787239064"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.4089467599378185"}],"id":"n0.6951856021652583"}],"id":"n0.3903696214115149"}},"id":"n0.7157059533793924"}],"id":"n0.1548520232970234"}],"id":"n0.4634946863213816"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.44582937785428833"}],"id":"n0.24721055235684797"}],"id":"n0.9602180403860188"}},"id":"n0.6160427835409938"}],"id":"n0.5660597128568199"}],"id":"n0.1301789488913847"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.07306106530879108"}],"id":"n0.5756709131973967"}],"shape":{"data":{"p":{"x":139.08397681235618,"y":117.73626428200146}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de4746109038062831":{"id":"de4746109038062831","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜂","id":"n0.6466061046461433"}],"id":"n0.7302807030126197"}],"id":"n0.7891280452896823"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8189562118218683"}],"id":"n0.5711161538928315"}],"shape":{"data":{"p":{"x":400.4893586136384,"y":18.62877564979931},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de14515593214146394":{"id":"de14515593214146394","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.3993967946976933"}],"id":"n0.8513486599475975"}],"id":"n0.7635312661181304"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3389140722650501"}],"id":"n0.014183471947202264"}],"shape":{"data":{"p":{"x":613.0903855037625,"y":162.52163415504833}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de31945308578801956":{"id":"de31945308578801956","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.6761337058482566"}],"id":"n0.8322914479919379"}],"id":"n0.4975080524356512"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7533020277434055"}],"id":"n0.04571303176510533"}],"shape":{"data":{"p":{"x":172.09038550376243,"y":162.52163415504833}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de3437232299036792":{"id":"de3437232299036792","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.7836336026147002"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.8669790981921077"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.45006927492141435"}],"id":"n0.8432470184549252"}],"id":"n0.7760493020829007"}},"id":"n0.8510052871461884"}],"id":"n0.6085925846811548"}],"id":"n0.7845320934138384"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.7598083618016642"}],"id":"n0.2333118184252101"}],"id":"n0.10901128152382666"}},"id":"n0.22888754770276676"}],"id":"n0.6781410424131757"}],"id":"n0.6933598697700811"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9928222755901932"}],"id":"n0.4175433094163179"}],"shape":{"data":{"p":{"x":139.08397681235618,"y":96.73626428200146}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de7044486226873938":{"id":"de7044486226873938","lines":[{"blocks":[{"text":"Env of ","style":{"fontSize":"\\tiny"},"id":"n0.5099793436595266"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4672407192966339"}],"id":"n0.7945254040989973"}],"id":"n0.5184897446323622"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.3030723685580643"}],"style":{"align":"center"},"id":"n0.6399406701300896"}],"shape":{"data":{"p":{"x":71.0172119140625,"y":19.836657214963566},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de12233133224262716":{"id":"de12233133224262716","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.6066601636292384"}],"id":"n0.17172801310522656"}],"shape":{"data":{"p":{"x":146.0093994140625,"y":18.487637573017054},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de46179107522947693":{"id":"de46179107522947693","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.013630509284332293","text":"\\overline","type":"composite","elements":{"value":{"id":"n0.1758891244744567","lines":[{"id":"n0.5764298561436061","blocks":[{"id":"n0.6936611013083895","text":"T"},{"id":"n0.38120918513713975","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2740917218026975","lines":[{"id":"n0.2623134127841795","blocks":[{"id":"n0.1398397090605179","text":"j"}]}]}}}]}]}}},{"id":"n0.8637212773995331","type":"single","text":"("},{"id":"n0.1184595306083227","text":"s"},{"id":"n0.7995764123716085","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.22694177844776497","lines":[{"id":"n0.9719713993739867","blocks":[{"id":"n0.36678450979810284","text":"j"}]}]}}},{"id":"n0.44743090344259095","text":",a"},{"id":"n0.9732165628501099","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9740311565942015","lines":[{"id":"n0.5282287035504141","blocks":[{"id":"n0.8611731955874364","text":"j"}]}]}}},{"id":"n0.4518938002610928","text":",s"},{"id":"n0.33445895890955124","text":"\\power-index","type":"composite","elements":{"indexValue":{"id":"n0.19409567144365947","lines":[{"id":"n0.21874968140141626","blocks":[{"id":"n0.8869740525148799","text":"j"}]}]},"powerValue":{"id":"n0.9581713259022835","lines":[{"id":"n0.33154237150314714","blocks":[{"id":"n0.5128302910455178","text":"′"}]}]}}},{"id":"n0.5208916699492883","type":"single","text":")"}],"id":"n0.3168167494404379"}],"id":"n0.4767325958984765"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.2627541312577786"}],"style":{"align":"center"},"id":"n0.1063418548762598"}],"shape":{"data":{"p":{"x":285.610837007667,"y":211.439940578934},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7780578807104204":{"id":"de7780578807104204","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.3511778113409634"}],"id":"n0.6791373232583222"}],"id":"n0.9190651324944978"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\scriptsize"},"id":"n0.5102771242337476"}],"id":"n0.727761724805509"}],"shape":{"data":{"p":{"x":279.47431307477996,"y":182},"rotation":49.5},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7949056139072763":{"id":"de7949056139072763","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.7323452707351161"}],"id":"n0.9998912548605183"}],"id":"n0.2695926434935332"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.06716032875908473"}],"id":"n0.3041700245436336"}],"shape":{"data":{"p":{"x":393.398973109876,"y":163.85714149475098},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de18751418875508108":{"id":"de18751418875508108","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.6657655635791759"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.6988767036565222","text":"S"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.9918120171219929"}],"id":"n0.4639519314559222"}],"id":"n0.9002291473294042"}},"id":"n0.3696878338976073"}],"id":"n0.7807554544460695"}],"id":"n0.22070928010431268"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.03709216209504618"}],"style":{"align":"center"},"id":"n0.24756927622662173"}],"shape":{"data":{"p":{"x":387.6132065083135,"y":176.49503087997437},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4732927849438495":{"id":"de4732927849438495","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.6690562907245137"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.8251746388397112","text":"i"}],"id":"n0.7872000785640887"}],"id":"n0.5671193837451141"}},"id":"n0.6653553919120421"}],"id":"n0.8743865335203924"}],"id":"n0.7369081718594115"}},"id":"n0.8307042719014721"},{"type":"single","text":"(","id":"n0.8161136531935869"},{"text":"s","id":"n0.6317085800446827"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.863245780817153","text":"i"}],"id":"n0.19411642848546928"}],"id":"n0.15499224249872112"}},"id":"n0.07263915415971667"},{"text":",a","id":"n0.35331379313221434"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.19072136140105989","text":"i"}],"id":"n0.28789446170314803"}],"id":"n0.7535370809803013"}},"id":"n0.5786958769021082"},{"text":",s","id":"n0.8729865630953615"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.27671413047786286","text":"i"}],"id":"n0.0658217758732682"}],"id":"n0.8357421006926671"},"powerValue":{"lines":[{"blocks":[{"text":"′","id":"n0.38218768799271197"}],"id":"n0.4181362511671829"}],"id":"n0.5053937731298157"}},"id":"n0.35834813904867335"},{"type":"single","text":")","id":"n0.9331666725428862"}],"id":"n0.6269908053119784"}],"id":"n0.8307652002174195"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.2505705598926036"}],"style":{"align":"center"},"id":"n0.6554982900972093"}],"shape":{"data":{"p":{"x":480.610837007667,"y":210.439940578934},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de050079977272444065":{"id":"de050079977272444065","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.1738546458892547"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5114629739047636"}],"id":"n0.2614889628337296"}],"id":"n0.48558053202701057"}},"id":"n0.031390229467598285"},{"text":"|×|A","id":"n0.44019166576794566"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4637563564016487"}],"id":"n0.8669426250713395"}],"id":"n0.22756702503613369"}},"id":"n0.9448409720070239"},{"text":"|×|S","id":"n0.6901681656015859"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9829367529890434"}],"id":"n0.14589201133848984"}],"id":"n0.4412492132056076"}},"id":"n0.15350060445090596"},{"text":"|","id":"n0.6097945030746335"}],"id":"n0.359211311045716"}],"id":"n0.5307342112945057"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.960813422623283"}],"style":{"align":"center"},"id":"n0.9181020972926659"}],"shape":{"data":{"p":{"x":444.9753875732422,"y":229.96709218025205},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6309121644461761":{"id":"de6309121644461761","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.7226923294314347"}],"id":"n0.18588346131724376"}],"id":"n0.771851697492894"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\scriptsize"},"id":"n0.8944203923289638"}],"id":"n0.22539485656992042"}],"shape":{"data":{"p":{"x":474.47431307477996,"y":181},"rotation":49.5},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de9901244604061572":{"id":"de9901244604061572","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.6103673174997359"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.983002655974881"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7018351678973132","text":"i"}],"id":"n0.7010329296925055"}],"id":"n0.7244476972754041"}},"id":"n0.17542069322933473"}],"id":"n0.19976495412619033"}],"id":"n0.9154711282656824"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.21271815915282222"}],"style":{"align":"center"},"id":"n0.5686213055828779"}],"shape":{"data":{"p":{"x":520.6132065083135,"y":176.49503087997437},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4468797854678037":{"id":"de4468797854678037","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.9747497283041866"}],"id":"n0.08076912011418358"}],"id":"n0.5883148292773521"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.866124436049301"}],"id":"n0.8475282880647284"}],"shape":{"data":{"p":{"x":526.398973109876,"y":163.85714149475098},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6963008676951739":{"id":"de6963008676951739","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.9467432607928974"}],"id":"n0.38641848532049905"}],"id":"n0.5349620693643276"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7052032195921623"}],"style":{"align":"center"},"id":"n0.006805448686313831"}],"shape":{"data":{"p":{"x":551.4714500404878,"y":179.98591809822463},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5307733598657904":{"id":"de5307733598657904","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.07306710235810865"}],"id":"n0.37648057370659616"}],"id":"n0.10130076633391227"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7743980585092951"}],"style":{"align":"center"},"id":"n0.9014467266778325"}],"shape":{"data":{"p":{"x":549.4714500404878,"y":279.9859180982246},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de35702312713851314":{"id":"de35702312713851314","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|×|S|","id":"n0.9098320743091413"}],"id":"n0.28064584064339515"}],"id":"n0.31823182025495567"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8374452296648147"}],"style":{"align":"center"},"id":"n0.9010594346309162"}],"shape":{"data":{"p":{"x":301.99359130859375,"y":278.9718017578125},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9284763344198799":{"id":"de9284763344198799","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.3777097004849297","text":"T"},{"id":"n0.6035946850133376","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6458733035771684","lines":[{"id":"n0.8996133625620213","blocks":[{"id":"n0.04865555559290735","text":"i"}]}]}}},{"type":"single","text":"(","id":"n0.9430238294952795"},{"text":"s,a,s","id":"n0.5718031955471183"},{"id":"n0.2761454214500738","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.7897967364936616","lines":[{"id":"n0.9758438418244391","blocks":[{"id":"n0.4895623117809469","text":"′"}]}]}}},{"type":"single","text":")","id":"n0.47133613654659334"}],"id":"n0.45421291588955426"}],"id":"n0.803263754257443"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.24979216144084027"}],"style":{"align":"center"},"id":"n0.8280339397799843"}],"shape":{"data":{"p":{"x":379.40112242936175,"y":233.27918469789847},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8341143779891083":{"id":"de8341143779891083","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.919589422656347"}],"id":"n0.507537421036887"}],"id":"n0.25074793897328806"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.04248175548225519"}],"id":"n0.32866920481796"}],"shape":{"data":{"p":{"x":420.0839768123562,"y":263.04836357699156}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de40063125596160476":{"id":"de40063125596160476","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.30820532932014166"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.33575061932716554"}],"id":"n0.22267003548064213"}],"id":"n0.7776956814282687"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4572670445753324"}],"style":{"align":"center"},"id":"n0.22331571707557485"}],"shape":{"data":{"p":{"x":513.6132065083135,"y":276.49503087997437},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de24456460257009915":{"id":"de24456460257009915","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.537723752459317"}],"id":"n0.36660980309716384"}],"id":"n0.013381938972016005"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.14629858535251006"}],"id":"n0.8005719086749645"}],"shape":{"data":{"p":{"x":517.398973109876,"y":263.857141494751},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de1363233054056363":{"id":"de1363233054056363","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.2640899370100982"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7957312675333303","text":"j"}],"id":"n0.4289763060352012"}],"id":"n0.5636851996964858"}},"id":"n0.6200066969093145"},{"text":"|×|A","id":"n0.24931989747100292"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7061769676734742","text":"j"}],"id":"n0.8338566948931943"}],"id":"n0.6497095558154655"}},"id":"n0.6467263721354128"},{"text":"|×|S","id":"n0.681059980774184"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4234643670864695","text":"j"}],"id":"n0.2839239830649629"}],"id":"n0.9936617197736568"}},"id":"n0.10945988810950902"},{"text":"|","id":"n0.2779183338745703"}],"id":"n0.06478265473108147"}],"id":"n0.5747157058513406"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.07143623474426697"}],"style":{"align":"center"},"id":"n0.9594258614626692"}],"shape":{"data":{"p":{"x":231.9753875732422,"y":214.96709218025205},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8164181201179905":{"id":"de8164181201179905","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.36909629287933576"}],"id":"n0.23203813653136018"}],"shape":{"data":{"p":{"x":69.5093994140625,"y":86.98763757301705},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de917768460299415":{"id":"de917768460299415","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.810206964359198"}],"id":"n0.987302506030517"}],"shape":{"data":{"p":{"x":54.5093994140625,"y":161.98763757301705},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de577878045869977":{"id":"de577878045869977","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.4064584503096027"}],"id":"n0.6168405228893412"}],"shape":{"data":{"p":{"x":39.5093994140625,"y":238.98763757301705},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de25110577288426494":{"id":"de25110577288426494","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"optionally dependent","id":"n0.4294657609427419"}],"id":"n0.2075778433860329"}],"shape":{"data":{"p":{"x":26.0093994140625,"y":44.487637573017054},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9499061837025173":{"id":"de9499061837025173","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"O","id":"n0.03930271760983639"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9011877772769519"}],"id":"n0.2388782643341718"}],"id":"n0.7468827239368123"}},"id":"n0.6953668642779995"},{"type":"single","text":"(","id":"n0.867129969382012"},{"text":"s,a","id":"n0.14021984306407043"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7655408689436833"}],"id":"n0.6550037690461015"}],"id":"n0.40458429035569443"}},"id":"n0.12811158542692813"},{"text":",o","id":"n0.04109526130856023"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9264905662614205"}],"id":"n0.6836812671851038"}],"id":"n0.696923725427885"}},"id":"n0.13306711535718385"},{"type":"single","text":")","id":"n0.06019184064626515"}],"id":"n0.4699397483891101"}],"id":"n0.7532302997838924"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9532813190383616"}],"style":{"align":"center"},"id":"n0.6075074297187724"}],"shape":{"data":{"p":{"x":201.41693053483044,"y":10.859427538141873},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de5622973739907038":{"id":"de5622973739907038","lines":[{"blocks":[{"text":"Envs","style":{"fontSize":"\\tiny"},"id":"n0.21323080848364517"}],"style":{"align":"center"},"id":"n0.5256645226151633"}],"shape":{"data":{"p":{"x":14.0172119140625,"y":19.836657214963566},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6571793473371186":{"id":"de6571793473371186","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.5029636989508328","text":"1-"},{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.5923570668684544"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.4834162458318534"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.32720262256835997"}],"id":"n0.48124815737646"}],"id":"n0.6927750915470068"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.5237791160596883"}],"id":"n0.6078049422868859"}],"id":"n0.6621310130027627"}},"id":"n0.2934739111828135"}],"id":"n0.01844241672470992"}],"id":"n0.6640143275241097"}},"id":"n0.10774757238169008"}],"id":"n0.5698678369589656"}],"id":"n0.9213915518587037"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6941094154964307"}],"style":{"align":"center"},"id":"n0.5991071178838041"}],"shape":{"data":{"p":{"x":183.49150793312418,"y":214.5206788661286},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8759589275482531":{"id":"de8759589275482531","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⟨s,a⟩∈","id":"n0.07936266846190287"}],"id":"n0.8149341385306228"}],"id":"n0.13020470631706216"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5524560793549289"}],"id":"n0.4859903828788752"}],"shape":{"data":{"p":{"x":229.07317358969988,"y":180.2828582611303},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de027912896577368507":{"id":"de027912896577368507","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"P","id":"n0.8348951616133002"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.294027956435992"}],"id":"n0.9879948918298702"}],"id":"n0.7322371853995608"},"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.8647546073343904"}],"id":"n0.8126379184044228"}],"id":"n0.462874068420569"}},"id":"n0.19183621734909861"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"∁","id":"n0.8307733655110068"}],"id":"n0.8500675537164684"}],"id":"n0.21676817271064475"}},"id":"n0.5730612827824997"}],"id":"n0.10160514417398603"}],"id":"n0.8721596412132258"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5086512898297695"}],"id":"n0.8667644861112345"}],"shape":{"data":{"p":{"x":235.07317358969988,"y":191.2828582611303},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di11968482578171047","items":[],"style":{}},"shapes":[{"id":"dp736494545583406","type":"doc-cube","data":{"p1":{"x":206.98281860351562,"y":166.27390942729653},"p2":{"x":249.24650750432158,"y":203.98385620117188},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp3937974403007931","type":"doc-cube","data":{"p1":{"x":206.98281860351562,"y":133.97149377418896},"p2":{"x":249.24650750432158,"y":171.68144054806442},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dg4857174382127132","entities":[{"id":"dg3449782978264446","entities":[{"id":"dp06947519900625876","type":"rectangle","data":{"p1":{"x":138.08397681235618,"y":101.7182343874357},"p2":{"x":150.74113754441504,"y":114.37539511949456}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp20987111150207616","type":"rectangle","data":{"p1":{"x":139.66612190386348,"y":103.30037947894306},"p2":{"x":152.32328263592234,"y":115.95754021100191}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp49462251128848367","type":"rectangle","data":{"p1":{"x":141.2482669953709,"y":104.88252457045041},"p2":{"x":153.90542772742975,"y":117.53968530250927}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl42310251642970464","linkedId":"de3437232299036792"}]},{"id":"da8512811121136399","data":[{"x":179.9299333078854,"y":33.451896417373916},{"x":195.08397681235618,"y":33.451896417373916}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dp9164171276212354","type":"doc-cube","data":{"p1":{"x":104,"y":154.98763757301708},"p2":{"x":142.09035498618437,"y":192.69758434689254},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da36194738276189287","data":[{"x":142.0724769306118,"y":175.26897912575146},{"x":174.30461890219993,"y":175.26897912575146}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6925834452262651","entities":[{"id":"dp7122737596261504","type":"circle","data":{"p1":{"x":174.30461890219993,"y":165.3430605466499},"p2":{"x":193.84033495902366,"y":184.87877660347363}}},{"id":"dl21082570538075251","linkedId":"de31945308578801956"}]},{"id":"da9781576713698847","data":[{"x":184.0724769306118,"y":195.5987463529243},{"x":184.0724769306118,"y":184.87877660347363}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9130259516533765","data":[{"x":259.09978491782493,"y":175.11091857506176},{"x":301.30461890219993,"y":175.11091857506176}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da8078770409643174","data":[{"x":320.84033495902366,"y":175.44642591476443},{"x":392.6132065083135,"y":175.44642591476443}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da5717337911460176","data":[{"x":412.14892256513724,"y":174.91141544819288},{"x":494.30461890219993,"y":174.91141544819288}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp015528813822181187","type":"doc-cube","data":{"p1":{"x":219.98281860351557,"y":267.27390942729653},"p2":{"x":262.2465075043216,"y":304.9838562011719},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp10757977244525407","type":"doc-cube","data":{"p1":{"x":219.98281860351557,"y":234.97149377418896},"p2":{"x":262.2465075043216,"y":272.6814405480644},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp8961558328475161","type":"doc-cube","data":{"p1":{"x":230.83609601701892,"y":277.5729114872548},"p2":{"x":273.09978491782493,"y":315.2828582611303},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp6167927249451948","type":"doc-cube","data":{"p1":{"x":230.83609601701892,"y":245.57291148725483},"p2":{"x":273.09978491782493,"y":283.2828582611303},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da5541931341066593","data":[{"x":596.099784917825,"y":174.91141544819288},{"x":612.3046189022,"y":174.91141544819288}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg5507586732404957","entities":[{"id":"dp2474566988972675","type":"circle","data":{"p1":{"x":612.3046189022,"y":165.3430605466499},"p2":{"x":631.8403349590237,"y":184.87877660347363}}},{"id":"dl9309649904975439","linkedId":"de14515593214146394"}]},{"id":"dp25197333914514775","type":"doc-cube","data":{"p1":{"x":433.0903855037625,"y":13.987637573017082},"p2":{"x":471.18074048994686,"y":51.69758434689254},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"dp37574443914210653","type":"right-arrow","data":{"p1":{"x":474.77320936917886,"y":29.196645047242328},"p2":{"x":487.77320936917886,"y":41.701389004761864},"arrowPercentage":0.4}},{"id":"dp08763935736717032","type":"right-arrow","data":{"p1":{"x":86.7732093691788,"y":167.19664504724233},"p2":{"x":99.7732093691788,"y":179.70138900476186},"arrowPercentage":0.4}},{"id":"dg13119570528477054","entities":[{"id":"dp646631666663311","type":"circle","data":{"p1":{"x":398.7035920120759,"y":23.4502020414009},"p2":{"x":418.2393080688996,"y":42.98591809822463}}},{"id":"dl6858481371533711","linkedId":"de4746109038062831"}]},{"id":"dg7135466245084179","entities":[{"id":"dg8432308452604242","entities":[{"id":"dp8942514088023354","type":"rectangle","data":{"p1":{"x":138.08397681235618,"y":122.7182343874357},"p2":{"x":150.74113754441504,"y":135.37539511949456}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp35227720864097356","type":"rectangle","data":{"p1":{"x":139.66612190386348,"y":124.30037947894306},"p2":{"x":152.32328263592234,"y":136.9575402110019}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp32821010554962604","type":"rectangle","data":{"p1":{"x":141.2482669953709,"y":125.88252457045041},"p2":{"x":153.90542772742975,"y":138.53968530250927}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl31480972409938146","linkedId":"de41418421309961495"}]},{"id":"dp1387905064421593","type":"doc-cube","data":{"p1":{"x":217.66564246893194,"y":176.57291148725483},"p2":{"x":259.09978491782493,"y":214.2828582611303},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp19759085845352287","type":"doc-cube","data":{"p1":{"x":217.66564246893194,"y":144.57291148725483},"p2":{"x":259.09978491782493,"y":182.2828582611303},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da3810595798413534","data":[{"x":193.84033495902366,"y":175.11091857506176},{"x":206.0093994140625,"y":175.11091857506176}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg14935737342636268","entities":[{"id":"dp7130874326641121","type":"circle","data":{"p1":{"x":301.30461890219993,"y":165.3430605466499},"p2":{"x":320.84033495902366,"y":184.87877660347363}}},{"id":"dl3679786690104043","linkedId":"de7522212595218865"}]},{"id":"da6732502125459128","data":[{"x":311.0724769306118,"y":165.3430605466499},{"x":311.0724769306118,"y":131.26435173617125}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da6645842690011527","data":[{"x":154.09978491782493,"y":131.26435173617125},{"x":311.0724769306118,"y":131.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg034018568564376794","entities":[{"id":"dg010410268580065107","entities":[{"id":"dp2671548493581788","type":"rectangle","data":{"p1":{"x":138.08397681235618,"y":80.37398084739664},"p2":{"x":150.74113754441504,"y":93.0311415794555}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp39155139166343367","type":"rectangle","data":{"p1":{"x":139.66612190386348,"y":81.956125938904},"p2":{"x":152.32328263592234,"y":94.61328667096285}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp9534721276938438","type":"rectangle","data":{"p1":{"x":141.2482669953709,"y":83.53827103041135},"p2":{"x":153.90542772742975,"y":96.1954317624702}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl8828715697007943","linkedId":"de6658095144342686"}]},{"id":"da5686891709937563","data":[{"x":153.90542772742975,"y":110.26435173617125},{"x":504.07247693061186,"y":110.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg22020581913434567","entities":[{"id":"dp1786034723960801","type":"circle","data":{"p1":{"x":494.30461890219993,"y":165.3430605466499},"p2":{"x":513.8403349590237,"y":184.87877660347363}}},{"id":"dl5377592576205668","linkedId":"de17339897452830244"}]},{"id":"da6626157824412076","data":[{"x":504.07247693061186,"y":165.3430605466499},{"x":504.07247693061186,"y":110.26435173617125}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da007611409748998321","data":[{"x":513.8403349590237,"y":175.11091857506176},{"x":525.6132065083135,"y":175.11091857506176}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp23841769197210172","type":"doc-cube","data":{"p1":{"x":558.0903855037625,"y":154.98763757301708},"p2":{"x":596.1807404899469,"y":192.69758434689254},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da014232816717384411","data":[{"x":622.0724769306119,"y":275.2828582611303},{"x":622.0724769306119,"y":184.87877660347363}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da3514202122360184","data":[{"x":536.1489225651372,"y":275.4464259147644},{"x":557.0093994140625,"y":275.4464259147644}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg42312302720444395","entities":[{"id":"dp4114507869592985","type":"circle","data":{"p1":{"x":249.29821021079368,"y":23.869789968593125},"p2":{"x":268.8339262676174,"y":43.405506025416855}}},{"id":"dl8024629095656042","linkedId":"de66011368422189"}]},{"id":"da12461802170632863","data":[{"x":235.09978491782493,"y":33.63764799700499},{"x":249.29821021079368,"y":33.63764799700499}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg22448264621035063","entities":[{"id":"dp1224597961569569","type":"circle","data":{"p1":{"x":281.2982102107937,"y":23.90515984164},"p2":{"x":300.8339262676174,"y":43.44087589846373}}},{"id":"dl4891615338121085","linkedId":"de21516737336846048"}]},{"id":"da038265993665470566","data":[{"x":268.8339262676174,"y":33.673017870051865},{"x":281.2982102107937,"y":33.673017870051865}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da4303535348042271","data":[{"x":300.8339262676174,"y":33.673017870051865},{"x":313.09978491782493,"y":33.673017870051865}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da12991360138833485","data":[{"x":259.06606823920555,"y":88.53827103041135},{"x":259.06606823920555,"y":43.405506025416855}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da8630138130538123","data":[{"x":291.06606823920555,"y":110.39399040804625},{"x":291.06606823920555,"y":43.44087589846373}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da4687117982275335","data":[{"x":153.90542772742975,"y":88.53827103041135},{"x":259.06606823920555,"y":88.53827103041135}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp2833493815756354","type":"doc-cube","data":{"p1":{"x":195.0093994140625,"y":33.451896417373916},"p2":{"x":235.17433179854055,"y":71.16184319124937},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp7211172021631458","type":"doc-cube","data":{"p1":{"x":195.0093994140625,"y":1.4518964173739164},"p2":{"x":235.17433179854055,"y":39.161843191249375},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp28182991976211436","type":"doc-cube","data":{"p1":{"x":314.0839768123562,"y":14.451896417373916},"p2":{"x":352.17433179854055,"y":52.161843191249375},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp41233534794370286","type":"doc-cube","data":{"p1":{"x":558.0903855037625,"y":255.98763757301708},"p2":{"x":596.1807404899469,"y":293.69758434689254},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da3578566881853964","data":[{"x":596.099784917825,"y":275.2828582611303},{"x":622.0724769306119,"y":275.2828582611303}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da22910905289663774","data":[{"x":441.8339262676174,"y":275.2828582611303},{"x":453.2982102107937,"y":275.2828582611303}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6119160641031665","entities":[{"id":"dp6940299382763646","type":"circle","data":{"p1":{"x":365.28740698813743,"y":23.498807006610832},"p2":{"x":384.8231230449612,"y":43.03452306343456}}},{"id":"dl8194607481224132","linkedId":"de4427510142690705"}]},{"id":"da06170766786087989","data":[{"x":352.09978491782493,"y":33.673017870051865},{"x":365.28740698813743,"y":33.673017870051865}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da7661767127582952","data":[{"x":375.0552650165493,"y":87.39399040804625},{"x":375.0552650165493,"y":43.03452306343456}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da5904324486887984","data":[{"x":375.0552650165493,"y":87.39399040804625},{"x":622.0724769306119,"y":87.39399040804625}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da39666738665513357","data":[{"x":622.0724769306119,"y":165.3430605466499},{"x":622.0724769306119,"y":87.39399040804625}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8621241068926349","data":[{"x":384.8231230449612,"y":33.2666650350227},{"x":398.7035920120759,"y":33.2666650350227}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da15883595570438813","data":[{"x":418.2393080688996,"y":33.218060069812765},{"x":432.1197770360145,"y":33.218060069812765}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg5665293210572151","entities":[{"id":"dp5223536771260155","type":"circle","data":{"p1":{"x":453.2982102107937,"y":265.8697899685931},"p2":{"x":472.8339262676174,"y":285.40550602541686}}},{"id":"dl9856755625912192","linkedId":"de9752351203905827"}]},{"id":"dg2859204043050667","entities":[{"id":"dp27442180512290504","type":"circle","data":{"p1":{"x":483.2982102107937,"y":265.90515984164},"p2":{"x":502.8339262676174,"y":285.44087589846373}}},{"id":"dl09600199380841445","linkedId":"de23325305718254907"}]},{"id":"da8204967439508815","data":[{"x":472.8339262676174,"y":275.67301787005186},{"x":483.2982102107937,"y":275.67301787005186}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da6400775207512097","data":[{"x":463.06606823920555,"y":319.26435173617125},{"x":463.06606823920555,"y":285.40550602541686}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9515171657668875","data":[{"x":493.06606823920555,"y":326.26435173617125},{"x":493.06606823920555,"y":285.44087589846373}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da10613409214611624","data":[{"x":72.09978491782493,"y":110.26435173617125},{"x":137.90542772742975,"y":110.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da2953123613930908","data":[{"x":77.0724769306118,"y":131.26435173617125},{"x":138.09978491782493,"y":131.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da4221174999797901","data":[{"x":77.0724769306118,"y":319.26435173617125},{"x":463.06606823920555,"y":319.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da2519721272826567","data":[{"x":77.0724769306118,"y":319.26435173617125},{"x":77.0724769306118,"y":131.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da32642060477246626","data":[{"x":72.09978491782493,"y":326.26435173617125},{"x":72.09978491782493,"y":110.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da6097416351721896","data":[{"x":72.09978491782493,"y":326.26435173617125},{"x":493.06606823920555,"y":326.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg28288844823488657","entities":[{"id":"dp21529388042290099","type":"circle","data":{"p1":{"x":113.30461890219993,"y":204.3430605466499},"p2":{"x":132.84033495902366,"y":223.87877660347363}}},{"id":"dl2703305754153198","linkedId":"de49606201729253674"}]},{"id":"da19119945301524477","data":[{"x":123.0724769306118,"y":204.3430605466499},{"x":123.0724769306118,"y":193.08636474609375}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"dp7751841189826612","type":"doc-cube","data":{"p1":{"x":99.40115294693982,"y":267.6802622623257},"p2":{"x":137.49150793312418,"y":305.39020903620104},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp09191320884543552","type":"doc-cube","data":{"p1":{"x":99.40115294693982,"y":235.37784660921812},"p2":{"x":137.49150793312418,"y":273.0877933830936},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp3598762218995919","type":"doc-cube","data":{"p1":{"x":110.08397681235618,"y":277.979264322284},"p2":{"x":148.17433179854055,"y":315.68921109615945},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp9971546776994589","type":"doc-cube","data":{"p1":{"x":110.08397681235618,"y":245.979264322284},"p2":{"x":148.17433179854055,"y":283.68921109615945},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp678013530603216","type":"rectangle","data":{"p1":{"x":72.53618240612298,"y":18.57503948597804},"p2":{"x":101.85864225206907,"y":47.89749933192411}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"da12399125708023151","data":[{"x":101.92993330788539,"y":33.451896417373916},{"x":144.0093994140625,"y":33.451896417373916}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dg03257418016404867","entities":[{"id":"dp3152110579077312","type":"rectangle","data":{"p1":{"x":152.0093994140625,"y":15.487637573017054},"p2":{"x":173.0093994140625,"y":50.487637573017054},"rotation":90}},{"id":"dl06335489444716114","linkedId":"de12233133224262716"}]},{"id":"dg022598253553454573","entities":[{"id":"dp7162741970895288","type":"rectangle","data":{"p1":{"x":264.8193317811682,"y":188.4010702276159},"p2":{"x":296.8992787641591,"y":217.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp7166353491492305","type":"rectangle","data":{"p1":{"x":268.1379472045726,"y":191.439940578934},"p2":{"x":300.2178941875636,"y":220.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp45092874176182973","type":"rectangle","data":{"p1":{"x":271.456562627977,"y":194.47881093025205},"p2":{"x":303.5365096109681,"y":223.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"dg9063844885927825","entities":[{"id":"dp3324864871780777","type":"rectangle","data":{"p1":{"x":282.2922215842626,"y":204.4010702276159},"p2":{"x":315.20073998648286,"y":233.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp16290898091617434","type":"rectangle","data":{"p1":{"x":285.6965512980523,"y":207.439940578934},"p2":{"x":318.6050697002727,"y":236.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp45688045414785683","type":"rectangle","data":{"p1":{"x":289.10088101184203,"y":210.47881093025205},"p2":{"x":322.0093994140625,"y":239.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{}},{"id":"da16784612594529036","data":[{"x":311.0724769306118,"y":204.21600341796875},{"x":311.0724769306118,"y":184.87877660347363}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dg18184788905852511","entities":[{"id":"dp8646170164656934","type":"circle","data":{"p1":{"x":392.6132065083135,"y":165.67856788635257},"p2":{"x":412.14892256513724,"y":185.2142839431763}}},{"id":"dl6828844980552891","linkedId":"de7949056139072763"}],"data":{"rotation":0}},{"id":"dg6537970351311602","entities":[{"id":"dp40893869773660274","type":"rectangle","data":{"p1":{"x":459.8193317811682,"y":187.4010702276159},"p2":{"x":491.8992787641591,"y":216.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp48003443565701986","type":"rectangle","data":{"p1":{"x":463.1379472045726,"y":190.439940578934},"p2":{"x":495.2178941875636,"y":219.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp7658880754652924","type":"rectangle","data":{"p1":{"x":466.456562627977,"y":193.47881093025205},"p2":{"x":498.5365096109681,"y":222.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"dg8118707468459647","entities":[{"id":"dp5740912673943488","type":"rectangle","data":{"p1":{"x":477.2922215842626,"y":203.4010702276159},"p2":{"x":510.20073998648286,"y":232.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp35219300120680974","type":"rectangle","data":{"p1":{"x":480.6965512980523,"y":206.439940578934},"p2":{"x":513.6050697002727,"y":235.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp6242015767297737","type":"rectangle","data":{"p1":{"x":484.10088101184203,"y":209.47881093025205},"p2":{"x":517.0093994140625,"y":238.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{}},{"id":"da7178618526318812","data":[{"x":504.07247693061186,"y":203.4010702276159},{"x":504.07247693061186,"y":184.87877660347363}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dg21946987099562154","entities":[{"id":"dp08167676563876336","type":"circle","data":{"p1":{"x":525.6132065083135,"y":165.67856788635257},"p2":{"x":545.1489225651372,"y":185.2142839431763}}},{"id":"dl9823479464918712","linkedId":"de4468797854678037"}],"data":{"rotation":0}},{"id":"da7528501861897603","data":[{"x":545.1489225651372,"y":175.44642591476443},{"x":558.0093994140625,"y":175.44642591476443}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da06891007608653754","data":[{"x":273.0093994140625,"y":285.2828582611303},{"x":291.0093994140625,"y":285.2828582611303}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp36222220506471525","type":"doc-cube","data":{"p1":{"x":362.3107674431774,"y":245.10001179268778},"p2":{"x":400.40112242936175,"y":282.8099585665631},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp49160010269192633","type":"doc-cube","data":{"p1":{"x":362.3107674431774,"y":212.7975961395802},"p2":{"x":400.40112242936175,"y":250.50754291345567},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp028345364209015234","type":"doc-cube","data":{"p1":{"x":372.99359130859375,"y":255.87165357713053},"p2":{"x":411.0839462947781,"y":293.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp08300142719153847","type":"doc-cube","data":{"p1":{"x":372.99359130859375,"y":223.87165357713053},"p2":{"x":411.0839462947781,"y":261.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp20157966704302677","type":"doc-cube","data":{"p1":{"x":330.20960923433677,"y":245.10001179268778},"p2":{"x":368.29996422052113,"y":282.8099585665631},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp840449126725197","type":"doc-cube","data":{"p1":{"x":330.20960923433677,"y":212.7975961395802},"p2":{"x":368.29996422052113,"y":250.50754291345567},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp5184103697755356","type":"doc-cube","data":{"p1":{"x":340.89243309975313,"y":255.87165357713053},"p2":{"x":378.9827880859375,"y":293.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp38152875855088375","type":"doc-cube","data":{"p1":{"x":340.89243309975313,"y":223.87165357713053},"p2":{"x":378.9827880859375,"y":261.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"da9346851626995165","data":[{"x":411.0093994140625,"y":275.2828582611303},{"x":422.2982102107937,"y":275.2828582611303}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dg5680346096153936","entities":[{"id":"dp20902577586770232","type":"circle","data":{"p1":{"x":422.2982102107937,"y":265.8697899685931},"p2":{"x":441.8339262676174,"y":285.40550602541686}}},{"id":"dl8017040983907677","linkedId":"de8341143779891083"}]},{"id":"da7586293919208427","data":[{"x":291.0093994140625,"y":303.39399040804625},{"x":432.06606823920555,"y":303.39399040804625}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7560479291363291","data":[{"x":291.0093994140625,"y":303.39399040804625},{"x":291.0093994140625,"y":285.2828582611303}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8899836517412827","data":[{"x":432.06606823920555,"y":303.39399040804625},{"x":432.06606823920555,"y":285.40550602541686}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da6017064760040944","data":[{"x":502.8339262676174,"y":275.4464259147644},{"x":516.6132065083135,"y":275.4464259147644}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg7716441606617934","entities":[{"id":"dp5518051175170133","type":"circle","data":{"p1":{"x":516.6132065083135,"y":265.67856788635254},"p2":{"x":536.1489225651372,"y":285.21428394317627}}},{"id":"dl7634889538117462","linkedId":"de24456460257009915"}],"data":{"rotation":0}},{"id":"da6913802546127341","data":[{"x":507.06606823920555,"y":338.08636474609375},{"x":507.06606823920555,"y":239.44087589846373}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da41338346233577594","data":[{"x":381.4011224293617,"y":344.08636474609375},{"x":381.4011224293617,"y":293.581600351006}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da8829406212403315","data":[{"x":301.4011224293617,"y":332.08636474609375},{"x":301.4011224293617,"y":240.08636474609375}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da6357185847481888","data":[{"x":40.92993330788539,"y":68.45189641737392},{"x":88.06606823920555,"y":68.45189641737392}],"head":"no","tail":"no","shaft":"--","headScale":0.6,"style":{"thickness":2}},{"id":"dg6791254461787495","entities":[{"id":"dp7486564023570643","type":"rectangle","data":{"p1":{"x":45.5093994140625,"y":85.98763757301705},"p2":{"x":66.5093994140625,"y":120.98763757301705},"rotation":180}},{"id":"dl35265567380820073","linkedId":"de8164181201179905"}]},{"id":"da15242885145344998","data":[{"x":88.06606823920555,"y":68.45189641737392},{"x":88.06606823920555,"y":48.8064075697439}],"head":"no","tail":"no","shaft":"--","headScale":0.6,"style":{"thickness":2}},{"id":"dg042014731349737655","entities":[{"id":"dp42646116629358155","type":"rectangle","data":{"p1":{"x":30.5093994140625,"y":160.98763757301705},"p2":{"x":51.5093994140625,"y":195.98763757301705},"rotation":180}},{"id":"dl05036021293983439","linkedId":"de917768460299415"}]},{"id":"dg5545058864855459","entities":[{"id":"dp6893988467776901","type":"rectangle","data":{"p1":{"x":15.5093994140625,"y":237.98763757301705},"p2":{"x":36.5093994140625,"y":272.9876375730171},"rotation":180}},{"id":"dl885283454862652","linkedId":"de577878045869977"}]},{"id":"da856743504473545","data":[{"x":56.92993330788539,"y":86.08636474609375},{"x":56.92993330788539,"y":68.45189641737392}],"head":"no","tail":"fh<","shaft":"--","headScale":0.6,"style":{"thickness":2}},{"id":"da8995970177679058","data":[{"x":40.92993330788539,"y":161.08636474609375},{"x":40.92993330788539,"y":68.08636474609375}],"head":"no","tail":"fh<","shaft":"--","headScale":0.6,"style":{"thickness":2}},{"id":"da6768359987484875","data":[{"x":25.929933307885392,"y":238.08636474609375},{"x":25.929933307885392,"y":47.21600341796875}],"head":"no","tail":"fh<","shaft":"--","headScale":0.6,"style":{"thickness":2}},{"id":"da38251931450937326","data":[{"x":56.92993330788545,"y":332.08636474609375},{"x":301.4011224293617,"y":332.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da7899027626513784","data":[{"x":40.92993330788539,"y":338.08636474609375},{"x":507.06606823920555,"y":338.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da13412493721590724","data":[{"x":25.929933307885392,"y":344.08636474609375},{"x":381.4011224293617,"y":344.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da997526913950449","data":[{"x":56.92993330788545,"y":332.08636474609375},{"x":56.92993330788545,"y":121.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da9611237820087917","data":[{"x":40.92993330788539,"y":338.08636474609375},{"x":40.92993330788539,"y":196.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da5383501755569913","data":[{"x":25.929933307885392,"y":344.08636474609375},{"x":25.929933307885392,"y":273.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dp1794917753730061","type":"rectangle","data":{"p1":{"x":10.536182406122975,"y":18.57503948597804},"p2":{"x":39.858642252069075,"y":47.89749933192408}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"da1035032699410634","data":[{"x":40.0093994140625,"y":33.451896417373916},{"x":71.92993330788539,"y":33.451896417373916}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da656704405537178","data":[{"x":123.0724769306118,"y":235.5987463529243},{"x":123.0724769306118,"y":223.87877660347363}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp1508235303229002","type":"doc-cube","data":{"p1":{"x":163.40115294693982,"y":227.81414568540237},"p2":{"x":201.49150793312418,"y":265.5240924592777},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp9992749909706351","type":"doc-cube","data":{"p1":{"x":163.40115294693982,"y":195.5117300322948},"p2":{"x":201.49150793312418,"y":233.22167680617025},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp7034960302191771","type":"doc-cube","data":{"p1":{"x":174.08397681235618,"y":238.11314774536066},"p2":{"x":212.17433179854055,"y":275.8230945192361},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp49521555987026833","type":"doc-cube","data":{"p1":{"x":174.08397681235618,"y":206.11314774536066},"p2":{"x":212.17433179854055,"y":243.82309451923612},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da8544942580045773","data":[{"x":132.84033495902366,"y":214.11091857506176},{"x":155.0093994140625,"y":214.11091857506176}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8231745533625754","data":[{"x":155.0093994140625,"y":285.2828582611303},{"x":155.0093994140625,"y":214.11091857506176}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9346291681395247","data":[{"x":155.0093994140625,"y":285.2828582611303},{"x":220.0093994140625,"y":285.2828582611303}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6}],"settings":{"grid":true,"diagramHeight":345.9408874511719}}]},{"id":"n0.8469391538169186","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":3261,"delayRenderCache":{"av":3261,"map":{"n0.5562758659701175":{"n0.08847662245070831":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.5491990457901264":{"n0.7049969082472012":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.801448369692964":{"n0.6437754419605293":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.16824565767494604":{"n0.9645001095314869":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.5233019382756188":{"n0.8320770388847725":{"w":11.6193,"h":8.4545,"bl":0.8214}},"n0.803624317973094":{"n0.4600841538833922":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.0967657311158161":{"n0.6615510692663404":{"w":22.4157,"h":12.5054,"bl":0.7021}},"n0.5955230560954696":{"n0.9817385017994846":{"w":15.8511,"h":12.5054,"bl":0.7021}},"n0.10292510313515457":{"n0.12385914641248141":{"w":30.0022,"h":12.5054,"bl":0.7021}},"n0.39686664852335385":{"n0.9863990264272267":{"w":18.1297,"h":12.5054,"bl":0.7021}},"n0.7414166285458648":{"n0.21882807550247785":{"w":28.9352,"h":8.4545,"bl":0.8214}},"n0.8204346809622691":{"n0.5234834432647619":{"w":18.1297,"h":12.5054,"bl":0.7021}},"n0.6329778626633036":{"n0.4968593472306042":{"w":25.7161,"h":12.5054,"bl":0.7021}},"n0.8476611167760499":{"n0.7795957295841542":{"w":29.4687,"h":9.1146,"bl":0.7619}},"n0.37357327720965383":{"n0.44456487845322856":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.5206787888668472":{"n0.7050310140621812":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.1301789488913847":{"n0.5660597128568199":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.6933598697700811":{"n0.6781410424131757":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.6538694462700769":{"n0.8622852515762334":{"w":45.1298,"h":8.4545,"bl":0.8214}},"n0.4767325958984765":{"n0.3168167494404379":{"w":34.2972,"h":12.6682,"bl":0.6267}},"n0.22070928010431268":{"n0.7807554544460695":{"w":5.9498,"h":8.4545,"bl":0.8214}},"n0.5307342112945057":{"n0.359211311045716":{"w":45.2293,"h":8.4545,"bl":0.8214}},"n0.8307652002174195":{"n0.6269908053119784":{"w":33.5015,"h":12.6682,"bl":0.6267}},"n0.9154711282656824":{"n0.19976495412619033":{"w":5.7057,"h":8.4545,"bl":0.8214}},"n0.31823182025495567":{"n0.28064584064339515":{"w":39.4513,"h":8.1019,"bl":0.8571}},"n0.803263754257443":{"n0.45421291588955426":{"w":28.9804,"h":11.348,"bl":0.6717}},"n0.5747157058513406":{"n0.06478265473108147":{"w":45.9617,"h":8.4545,"bl":0.8214}},"n0.7532302997838924":{"n0.4699397483891101":{"w":30.3819,"h":8.4545,"bl":0.8214}},"n0.9213915518587037":{"n0.5698678369589656":{"w":20.7972,"h":9.9736,"bl":0.6963}},"n0.13020470631706216":{"n0.8149341385306228":{"w":21.8099,"h":8.1019,"bl":0.8571}},"n0.8721596412132258":{"n0.10160514417398603":{"w":12.0443,"h":11.0044,"bl":0.8028}}}}}

==> plots/docs/f2c8181d-ae2e-4c8a-84e1-5fea8033fe03 <==
{"id":"n0.18805762998880904","lines":[{"id":"n0.10628078590158863","blocks":[]},{"id":"n0.04419106341594836","blocks":[{"id":"n0.8838103512889588","text":"\\diagram","type":"composite","elements":{"de6103756180794349":{"id":"de6103756180794349","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜃","style":{"mathType":"\\mathbf"},"id":"n0.22674499425613304"}],"id":"n0.8251165182411753"}],"id":"n0.34276351265372096"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.3104246612387036"}],"style":{"align":"center"},"id":"n0.28170482108071027"}],"shape":{"data":{"p":{"x":39.97359713596575,"y":178.63632516949775},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4921345059974387":{"id":"de4921345059974387","lines":[{"blocks":[{"text":"Envs","style":{"fontSize":"\\tiny"},"id":"n0.7886006601830433"}],"style":{"align":"center"},"id":"n0.2652218053583968"}],"shape":{"data":{"p":{"x":182.0172119140625,"y":178.83665721496357},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de09648216086759942":{"id":"de09648216086759942","lines":[{"blocks":[{"text":"MAQMDP planning module","style":{"fontSize":"\\tiny"},"id":"n0.1692246054674058"}],"style":{"align":"center"},"id":"n0.4574645504738164"}],"shape":{"data":{"p":{"x":277.026611328125,"y":167.7467308044433},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6319421349768997":{"id":"de6319421349768997","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.15166061834504974"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.759422983008895"}],"id":"n0.9918347669429193"}],"id":"n0.7606601194513969"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.09962989669326383"}],"id":"n0.2931944948632237"}],"id":"n0.6156082247263208"}},"id":"n0.31326272255816034"}],"id":"n0.8796898714453854"}],"id":"n0.9805767880860297"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3371603844651063"}],"id":"n0.30306266283677585"}],"shape":{"data":{"p":{"x":60.0172119140625,"y":37.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de9909381176935796":{"id":"de9909381176935796","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.7770745399973855"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.279482495896181","text":"j"}],"id":"n0.049294457730357566"}],"id":"n0.47502194828777755"}},"id":"n0.3104698583774652"},{"text":"|","id":"n0.8069761130046857"}],"id":"n0.8584969463576833"}],"id":"n0.2798165469167486"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6562813764434903"}],"style":{"align":"center"},"id":"n0.363983952699487"}],"shape":{"data":{"p":{"x":154.5172119140625,"y":85.09351124763486},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7940121895808216":{"id":"de7940121895808216","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|𝛺","id":"n0.8392268213222378"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.45931023392974546"}],"id":"n0.4386172708809295"}],"id":"n0.4584664630282278"}},"id":"n0.4763352696187795"},{"text":"|","id":"n0.14967209541319826"}],"id":"n0.35156619811075585"}],"id":"n0.0956182946294597"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9708121693643827"}],"style":{"align":"center"},"id":"n0.35881694925462093"}],"shape":{"data":{"p":{"x":192.02362060546875,"y":103.28239979743955},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3438066760605898":{"id":"de3438066760605898","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.6185751205939924"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7630019635107705"}],"id":"n0.18231221574247525"}],"id":"n0.6089119962955543"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.8931427045562066"}],"id":"n0.45448693554527053"}],"id":"n0.19216976991918355"}},"id":"n0.7171050426488565"}],"id":"n0.4046619303284873"}],"id":"n0.8192672737499627"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5089895969159941"}],"id":"n0.43765832669474447"}],"shape":{"data":{"p":{"x":77.0172119140625,"y":37.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de02563280881487806":{"id":"de02563280881487806","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.48393696995564994"}],"id":"n0.7670471443345628"}],"id":"n0.8865234094211434"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.11082735422175616"}],"style":{"align":"center"},"id":"n0.9320416525991655"}],"shape":{"data":{"p":{"x":51.0172119140625,"y":38.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2952691414875843":{"id":"de2952691414875843","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"}","id":"n0.6356927531194121"}],"id":"n0.36904407403017525"}],"id":"n0.9553225079236318"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8271860448504322"}],"style":{"align":"center"},"id":"n0.6542691589207725"}],"shape":{"data":{"p":{"x":115.0172119140625,"y":38.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2137567380595542":{"id":"de2137567380595542","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.008045371016361047"}],"id":"n0.056940874031297994"}],"id":"n0.4727756332635742"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.9381759798707874"}],"id":"n0.4639351367653197"}],"shape":{"data":{"p":{"x":83.0172119140625,"y":39.30042969200531}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4411703412746728":{"id":"de4411703412746728","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.5673059339913724"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.061383121218202774"}],"id":"n0.6367317616117458"}],"id":"n0.11324966217388632"},"powerValue":{"lines":[{"blocks":[{"text":"T","id":"n0.3556798658020468"}],"id":"n0.25916704271678803"}],"id":"n0.5837359185292408"}},"id":"n0.7818593738823849"}],"id":"n0.21276920260652177"}],"id":"n0.07663451775769459"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6650778724083672"}],"id":"n0.6330050359540009"}],"shape":{"data":{"p":{"x":107.0172119140625,"y":37.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de035400546782350384":{"id":"de035400546782350384","lines":[{"blocks":[{"text":"step size","style":{"fontSize":"\\tiny"},"id":"n0.9764453106149684"}],"style":{"align":"center"},"id":"n0.17208796365792245"}],"shape":{"data":{"p":{"x":80.2672119140625,"y":13.532399797439552},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de011428175050699707":{"id":"de011428175050699707","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.8415160191222524"}],"id":"n0.6764598294619883"}],"id":"n0.4915964638796144"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\huge"},"id":"n0.04242692615873578"}],"style":{"align":"center"},"id":"n0.7062294202886628"}],"shape":{"data":{"p":{"x":123.0172119140625,"y":31.282399797439552},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6537304728518818":{"id":"de6537304728518818","lines":[{"blocks":[{"text":"sIPOMDPLite-net belief update module","style":{"fontSize":"\\tiny"},"id":"n0.7546254988855303"}],"style":{"align":"center"},"id":"n0.8691198432839606"}],"shape":{"data":{"p":{"x":239.0172119140625,"y":72.387485023934},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7705556078782059":{"id":"de7705556078782059","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.008293039797159674"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5216747967197923"}],"id":"n0.35693243297690636"}],"id":"n0.41737925849133406"},"powerValue":{"lines":[{"blocks":[{"text":"0","id":"n0.6979465989849813"}],"id":"n0.14420185103029626"}],"id":"n0.40474595580324424"}},"id":"n0.3277983918828431"},{"type":"single","text":"(","id":"n0.8809554206446106"},{"text":"s","id":"n0.7858656026709734"},{"type":"single","text":")","id":"n0.6124441271549628"}],"id":"n0.6634858829152157"}],"id":"n0.05892219861296333"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.7774372556191349"}],"style":{"align":"center"},"id":"n0.2595929551888332"}],"shape":{"data":{"p":{"x":78.42474303483044,"y":147.65347228287732},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de17319207116005386":{"id":"de17319207116005386","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.780829103006283"}],"id":"n0.6355606499794044"}],"id":"n0.966917583179874"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9759693950963464"}],"style":{"align":"center"},"id":"n0.9848921236101413"}],"shape":{"data":{"p":{"x":58.0172119140625,"y":160.5483568152169},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5959307484371226":{"id":"de5959307484371226","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.6726140179660547"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.762679550225982"}],"id":"n0.8397633926464323"}],"id":"n0.7290894455779042"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.17320945559767842"}],"id":"n0.09662066496380262"}],"id":"n0.25944338759843943"}},"id":"n0.7583015172184857"},{"type":"single","text":"(","id":"n0.3786770174641547"},{"text":"s","id":"n0.7625989177777934"},{"type":"single","text":")","id":"n0.5639546157732511"}],"id":"n0.6922443966909593"}],"id":"n0.8095639861826163"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.3649388247074752"}],"style":{"align":"center"},"id":"n0.5687985959786279"}],"shape":{"data":{"p":{"x":423.42474303483044,"y":74.65347228287732},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de07073982375164545":{"id":"de07073982375164545","lines":[{"blocks":[{"text":"Sparse softmax cross entropy","style":{"fontSize":"\\tiny"},"id":"n0.27095514986534974"}],"style":{"align":"center"},"id":"n0.31120224083679693"}],"shape":{"data":{"p":{"x":352.3273048400878,"y":26.79249272346499},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6830611398030915":{"id":"de6830611398030915","lines":[{"blocks":[{"text":"RMSProp Optimizer","style":{"fontSize":"\\tiny"},"id":"n0.10517431055464077"}],"style":{"align":"center"},"id":"n0.297970068178369"}],"shape":{"data":{"p":{"x":469.3273048400878,"y":0.7924927234649886},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6104984434949119":{"id":"de6104984434949119","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.34613872236485066"}],"id":"n0.15018417810138507"}],"id":"n0.24973157094907705"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.5489273765608476"}],"id":"n0.07614620034088282"}],"shape":{"data":{"p":{"x":500.63994881799636,"y":36.42916718304414}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8090494859670556":{"id":"de8090494859670556","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"}","id":"n0.16533359404242964"}],"id":"n0.6042093799923687"}],"id":"n0.7620537820832181"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5331785463618879"}],"style":{"align":"center"},"id":"n0.3358850621573517"}],"shape":{"data":{"p":{"x":536,"y":35.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de15916424799553974":{"id":"de15916424799553974","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.16381382403266276"}],"id":"n0.31153597860941096"}],"id":"n0.9087874361013744"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.014338093252062256"}],"style":{"align":"center"},"id":"n0.8352763945462958"}],"shape":{"data":{"p":{"x":482,"y":35.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5571887982091397":{"id":"de5571887982091397","lines":[{"blocks":[{"text":"step size","style":{"fontSize":"\\tiny"},"id":"n0.8485972952380658"}],"style":{"align":"center"},"id":"n0.14538206619684813"}],"shape":{"data":{"p":{"x":497.5649331774448,"y":47.94894342945699},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6104151282223247":{"id":"de6104151282223247","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.5426573890919397"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9965857282116861"}],"id":"n0.676222141387296"}],"id":"n0.21237977565877797"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.7246782685259634"}],"id":"n0.12791338011177222"}],"id":"n0.629879321844137"}},"id":"n0.23433173455375367"}],"id":"n0.07297285074437698"}],"id":"n0.678448619782392"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5031310617013929"}],"id":"n0.6304535325735754"}],"shape":{"data":{"p":{"x":529,"y":186.0137939453125}},"anchor":"left-top"},"isTextMode":true},"de7214680511204863":{"id":"de7214680511204863","lines":[{"blocks":[{"text":"Evaluation","style":{"fontSize":"\\tiny"},"id":"n0.3229327737426322"}],"style":{"align":"center"},"id":"n0.015974279420830406"}],"shape":{"data":{"p":{"x":381.39875726699825,"y":178.76184458732604},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7549900886099203":{"id":"de7549900886099203","lines":[{"blocks":[{"text":"Training","style":{"fontSize":"\\tiny"},"id":"n0.803890300664885"}],"style":{"align":"center"},"id":"n0.03181144687105686"}],"shape":{"data":{"p":{"x":404.0760807037352,"y":159.0441082000733},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5046710934384864":{"id":"de5046710934384864","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.24609779131871923"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.22706401339330085"}],"id":"n0.33524231977662367"}],"id":"n0.5487085448306963"}},"id":"n0.9534120892256168"},{"text":"|","id":"n0.7717020579670113"}],"id":"n0.19455039516198558"}],"id":"n0.44181901465933904"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.11344735225385527"}],"style":{"align":"center"},"id":"n0.19566480723516833"}],"shape":{"data":{"p":{"x":448.5,"y":177.8249053955078},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6139659569366251":{"id":"de6139659569366251","lines":[{"blocks":[{"text":"Recurrent belief update","style":{"fontSize":"\\tiny"},"id":"n0.9792646145620199"}],"style":{"align":"center"},"id":"n0.300225697394062"}],"shape":{"data":{"p":{"x":265.0172119140625,"y":38.35211515088713},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5190732616850979":{"id":"de5190732616850979","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.03595251541093991"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5555799269653077"}],"id":"n0.7826657345235788"}],"id":"n0.20729284139918103"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.18543534405426731"}],"id":"n0.4732846757636109"}],"id":"n0.6985821718961494"}},"id":"n0.3199206488286901"},{"type":"single","text":"(","id":"n0.12285033223688102"},{"text":"s","id":"n0.09153978246159955"},{"type":"single","text":")","id":"n0.8513960623698407"}],"id":"n0.4675833849066542"}],"id":"n0.2860407715183735"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.31907694747023063"}],"style":{"align":"center"},"id":"n0.6745466833125002"}],"shape":{"data":{"p":{"x":184.42474303483044,"y":144.65347228287732},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9578891903894824":{"id":"de9578891903894824","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.15860019140094073"}],"id":"n0.526338816874079"}],"id":"n0.14877766752441013"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.02063639735628442"}],"id":"n0.46798948411037133"}],"shape":{"data":{"p":{"x":132.0172119140625,"y":143.04796763870638}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6727368075661122":{"id":"de6727368075661122","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.27279228036029113"}],"id":"n0.7808913629699232"}],"id":"n0.3813400136477225"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6236698896964832"}],"style":{"align":"center"},"id":"n0.362718419602585"}],"shape":{"data":{"p":{"x":163.0172119140625,"y":153.5483568152169},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de12018452445458294":{"id":"de12018452445458294","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.4304601760832991"}],"id":"n0.7197864701343688"}],"id":"n0.3232354544137075"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.46162195355427316"}],"style":{"align":"center"},"id":"n0.15662968742916283"}],"shape":{"data":{"p":{"x":402.0172119140625,"y":87.28239979743955},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9279013124591611":{"id":"de9279013124591611","lines":[{"blocks":[{"text":"Interaction indicators","style":{"fontSize":{"value":0.4}},"id":"n0.41359606004965843"}],"style":{"align":"center"},"id":"n0.9861904073319885"}],"shape":{"data":{"p":{"x":103.80276922615428,"y":270.28239979743955},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de03535318107247609":{"id":"de03535318107247609","lines":[{"blocks":[{"text":"value","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.1285566936690723"}],"style":{"align":"center"},"id":"n0.9484429575143738"}],"shape":{"data":{"p":{"x":250,"y":284.96759033203125},"rotation":0},"anchor":"left-top","style":{"fillColor":[245,166,35,1]}},"isTextMode":true,"isInGroup":true},"de6581424833173313":{"id":"de6581424833173313","lines":[{"blocks":[{"text":"indexing vector","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.014119603541997483"}],"style":{"align":"center"},"id":"n0.11737167060362119"}],"shape":{"data":{"p":{"x":430.00000000000006,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de6830316854968421":{"id":"de6830316854968421","lines":[{"blocks":[{"text":"sub-module","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.6161909700312669"}],"style":{"align":"center"},"id":"n0.5050592436335899"}],"shape":{"data":{"p":{"x":565,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[74,144,226,0.5]}},"isTextMode":true,"isInGroup":true},"de6916130444344799":{"id":"de6916130444344799","lines":[{"blocks":[{"text":"training algorithm","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.08509839011126474"}],"style":{"align":"center"},"id":"n0.8553495772556003"}],"shape":{"data":{"p":{"x":491,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[255,100,100,1]}},"isTextMode":true,"isInGroup":true},"de7846039342937636":{"id":"de7846039342937636","lines":[{"blocks":[{"text":"model","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.5182017439975346"}],"style":{"align":"center"},"id":"n0.8576427129423225"}],"shape":{"data":{"p":{"x":378,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de38901163369922753":{"id":"de38901163369922753","lines":[{"blocks":[{"text":"trainable variable","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.16199844627080617"}],"style":{"align":"center"},"id":"n0.7231446857744572"}],"shape":{"data":{"p":{"x":296.00000000000006,"y":284.9838562011719},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9474792898469997":{"id":"de9474792898469997","lines":[{"blocks":[{"text":"belief/probability","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.7950880955069464"}],"style":{"align":"center"},"id":"n0.051025330855066775"}],"shape":{"data":{"p":{"x":167.00000000000006,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[80,227,194,1]}},"isTextMode":true,"isInGroup":true},"de157530155636616":{"id":"de157530155636616","lines":[{"blocks":[{"text":"input/output","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.2070151504513611"}],"style":{"align":"center"},"id":"n0.7316417110811024"}],"shape":{"data":{"p":{"x":110.00000000000006,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de5551324285345347":{"id":"de5551324285345347","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.10112709389658225"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.15719802354624712"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.230433667689528"}],"id":"n0.6000958793716686"}],"id":"n0.15896386458891132"}},"id":"n0.5010451678163392"}],"id":"n0.36143427726355126"}],"id":"n0.6079979627375813"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.9283315301145045"}],"id":"n0.8944995803110658"}],"id":"n0.057705097653189874"}},"id":"n0.967172965753176"}],"id":"n0.7129346546594733"}],"id":"n0.8842098281055866"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.15550535315998992"}],"id":"n0.8290424429158296"}],"shape":{"data":{"p":{"x":460,"y":167.5137939453125}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de11067232215210976":{"id":"de11067232215210976","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.6278015293063248"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.11467269437820349"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.30987021170003315"}],"id":"n0.8111485637648763"}],"id":"n0.605238568977055"}},"id":"n0.44655036459612485"}],"id":"n0.6280076279345186"}],"id":"n0.8328557278802435"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.8653763603017739"}],"id":"n0.1893791319877034"}],"id":"n0.6088615053213609"}},"id":"n0.06539787902914118"}],"id":"n0.8820827388445249"}],"id":"n0.6926625074118744"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.002378739463359425"}],"id":"n0.001579009779701046"}],"shape":{"data":{"p":{"x":494.9827880859375,"y":35.57558217048643},"rotation":0},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de7333755688576151":{"id":"de7333755688576151","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.628732028648648"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.9592767044354882"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4218631289034491"}],"id":"n0.7601888966815635"}],"id":"n0.04550619551919688"}},"id":"n0.2917956954443315"}],"id":"n0.5997785509889499"}],"id":"n0.589789168719923"},"powerValue":{"lines":[{"blocks":[{"text":"T","id":"n0.9344458859699847"}],"id":"n0.35296799842200977"}],"id":"n0.6893288478455344"}},"id":"n0.20085229161538964"}],"id":"n0.6878304647006728"}],"id":"n0.19734605494092916"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9749987698326703"}],"id":"n0.12341831089898059"}],"shape":{"data":{"p":{"x":527.9827880859375,"y":35.78239979743955}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de766426490560322":{"id":"de766426490560322","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Depth: ","id":"n0.5943425507311662"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|𝛺","id":"n0.5567072858792346"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.22011040074090626"}],"id":"n0.9621017955017688"}],"id":"n0.2887825406954372"}},"id":"n0.5756253396206454"},{"text":"|","id":"n0.001745476231194365"}],"id":"n0.8879719304316316"}],"id":"n0.8377316246435462"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8200746325948032"}],"id":"n0.9479074159109457"}],"shape":{"data":{"p":{"x":113.0172119140625,"y":93.28239979743955},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8769763256636647":{"id":"de8769763256636647","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"One hot mapping","id":"n0.3575034704393769"}],"id":"n0.07564267257534452"}],"shape":{"data":{"p":{"x":120.0172119140625,"y":84.78239979743955},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9077288866210012":{"id":"de9077288866210012","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.3459030011878128"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"o","id":"n0.8691611673216317"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7171822782864585"}],"id":"n0.36414181906030185"}],"id":"n0.8201563634585598"}},"id":"n0.9643486708720748"}],"id":"n0.09770634088915475"}],"id":"n0.052403244615391475"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.6797348567627706"}],"id":"n0.017755115192927606"}],"id":"n0.9814357810390177"}},"id":"n0.09398349921211446"}],"id":"n0.560660220226239"}],"id":"n0.11712223778126041"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.33479771380700796"}],"id":"n0.9732905260302813"}],"shape":{"data":{"p":{"x":203.0172119140625,"y":91.78239979743955}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de0427991193329158":{"id":"de0427991193329158","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.6464133006231938"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.14579720940771201","text":"j"}],"id":"n0.288130680137366"}],"id":"n0.03781615706224151"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.18815728479516247"}],"id":"n0.8259113629013399"}],"id":"n0.39119061776319053"}},"id":"n0.4867090870517434"}],"id":"n0.2652112962808757"}],"id":"n0.7646762117471588"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6089176068916575"}],"id":"n0.6015078732153858"}],"shape":{"data":{"p":{"x":60,"y":58.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de4185709066586074":{"id":"de4185709066586074","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.01688425792416437"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.18718254922497635"}],"id":"n0.14289521987802023"}],"id":"n0.2931294741383166"}},"id":"n0.7833519614394571"},{"text":"|","id":"n0.6768902994582451"}],"id":"n0.2421330624441942"}],"id":"n0.8656149269890585"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6159887899805114"}],"style":{"align":"center"},"id":"n0.10572795347500286"}],"shape":{"data":{"p":{"x":154.5172119140625,"y":60.093511247634865},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de27900670992145105":{"id":"de27900670992145105","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.31966651560539705"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7017088864578898"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6530735648959431"}],"id":"n0.14134950566231863"}],"id":"n0.3159090075051221"}},"id":"n0.30743404375942074"}],"id":"n0.23765680276781453"}],"id":"n0.00421906309059672"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.529727692702963"}],"id":"n0.5877611847771624"}],"id":"n0.28055451097523876"}},"id":"n0.7247943503531769"}],"id":"n0.3745027443049487"}],"id":"n0.8432401649435193"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9287469860935853"}],"id":"n0.7791566836714905"}],"shape":{"data":{"p":{"x":164.0172119140625,"y":48.78239979743955}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de8772525490309724":{"id":"de8772525490309724","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.5762133858478438"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.35169004439343365"},{"id":"n0.05925589579167889","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9534903422146683","lines":[{"id":"n0.38955445239343356","blocks":[{"id":"n0.45261265864650935","text":"j"}]}]}}}],"id":"n0.4781498140780698"}],"id":"n0.9221215572847408"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.8968006244869051"}],"id":"n0.29773686256620446"}],"id":"n0.28245853278929767"}},"id":"n0.13292216965562553"}],"id":"n0.43454788566174973"}],"id":"n0.865317173645763"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8002820603523662"}],"id":"n0.2343795510721598"}],"shape":{"data":{"p":{"x":164.0172119140625,"y":73.78239979743955}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":false},"de3319413261208979":{"id":"de3319413261208979","lines":[{"blocks":[{"text":"Training","style":{"fontSize":"\\tiny"},"id":"n0.402568375570203"}],"style":{"align":"center"},"id":"n0.7404299373178662"}],"shape":{"data":{"p":{"x":380.0588687896727,"y":196.0441082000733},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3684156015585027":{"id":"de3684156015585027","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.46054203308809494"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.08317265649526884"}],"id":"n0.5136127675548985"}],"id":"n0.39013289935446305"}},"id":"n0.3484831224478835"},{"text":"|","id":"n0.34630089461119784"}],"id":"n0.6856134748473006"}],"id":"n0.6037157092616128"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3351997587724176"}],"style":{"align":"center"},"id":"n0.20760977007595005"}],"shape":{"data":{"p":{"x":409.4827880859375,"y":214.8249053955078},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5137422723619176":{"id":"de5137422723619176","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.9519679578948306"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.37842720917881234"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.14778329563842507","text":"j"}],"id":"n0.7452891669254227"}],"id":"n0.3652473407083463"}},"id":"n0.10937835340226632"}],"id":"n0.24057415195939091"}],"id":"n0.6737937491681296"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.03573371875191578"}],"id":"n0.028060102656048302"}],"id":"n0.42105302242493625"}},"id":"n0.12730810685656668"}],"id":"n0.9405832457870693"}],"id":"n0.6370642722097213"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.904836261877364"}],"id":"n0.1041501006626171"}],"shape":{"data":{"p":{"x":420.9827880859375,"y":204.5137939453125}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de1747952617436006":{"id":"de1747952617436006","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.03826382342507961"}],"id":"n0.0776788625298026"}],"id":"n0.2299585495929235"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.6855413346855017"}],"id":"n0.8056632706985383"}],"shape":{"data":{"p":{"x":560.6399488179964,"y":24.429167183044143}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de23076532693712015":{"id":"de23076532693712015","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"}","id":"n0.21852843029975233"}],"id":"n0.4472116882434696"}],"id":"n0.7046338254291307"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.35303218499510725"}],"style":{"align":"center"},"id":"n0.711907666288109"}],"shape":{"data":{"p":{"x":596,"y":23.369590963121993},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3021532720703066":{"id":"de3021532720703066","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.9425366060270881"}],"id":"n0.49535503691405913"}],"id":"n0.7689628952048579"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6794254891499345"}],"style":{"align":"center"},"id":"n0.3203984774618396"}],"shape":{"data":{"p":{"x":542,"y":23.369590963121993},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5428744539157133":{"id":"de5428744539157133","lines":[{"blocks":[{"text":"step size","style":{"fontSize":"\\tiny"},"id":"n0.8164605120701358"}],"style":{"align":"center"},"id":"n0.9911689156348542"}],"shape":{"data":{"p":{"x":557.5649331774448,"y":35.94894342945699},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de130364287178661":{"id":"de130364287178661","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.14205109947688643"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.24760638775722588"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.5366232895398386","text":"j"}],"id":"n0.573209120508704"}],"id":"n0.2540251173041572"}},"id":"n0.21577099400758604"}],"id":"n0.49356680643817796"}],"id":"n0.37710113689268754"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.9814172621566803"}],"id":"n0.02602213798203934"}],"id":"n0.7250091879301446"}},"id":"n0.8271830445251864"}],"id":"n0.7399053922658398"}],"id":"n0.5800614332963825"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.08352580501640494"}],"id":"n0.29497144120326313"}],"shape":{"data":{"p":{"x":554.9827880859375,"y":23.575582170486427},"rotation":0},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de13864094431472274":{"id":"de13864094431472274","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.2209383974902177"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.23721481739277217"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.825655967369261","text":"j"}],"id":"n0.15501530759379012"}],"id":"n0.025376741285212612"}},"id":"n0.6662269310487501"}],"id":"n0.5077589861101615"}],"id":"n0.07061986568419831"},"powerValue":{"lines":[{"blocks":[{"text":"T","id":"n0.777430048423563"}],"id":"n0.5462382795226342"}],"id":"n0.6925090740158706"}},"id":"n0.49438988759218017"}],"id":"n0.7748604418054355"}],"id":"n0.5054730445479463"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.044365918439071894"}],"id":"n0.7878884391656515"}],"shape":{"data":{"p":{"x":587.9827880859375,"y":23.782399797439552}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de8858027549359482":{"id":"de8858027549359482","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7771409182943738"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.08850067954682905","text":"j"}],"id":"n0.4151627584541755"}],"id":"n0.571046075525246"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.8278723054805401"}],"id":"n0.924538771173768"}],"id":"n0.8240977136423435"}},"id":"n0.1878142525060167"}],"id":"n0.7205301889098097"}],"id":"n0.3935563474086412"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.874871017068152"}],"id":"n0.18953854390260982"}],"shape":{"data":{"p":{"x":77.0172119140625,"y":58.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de01737361400489701":{"id":"de01737361400489701","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.5028186364995297"}],"id":"n0.639855730025886"}],"id":"n0.9680449396846869"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9793774702776521"}],"style":{"align":"center"},"id":"n0.6803018614918244"}],"shape":{"data":{"p":{"x":51.0172119140625,"y":59.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2338077860981691":{"id":"de2338077860981691","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"}","id":"n0.30890644878022244"}],"id":"n0.5961478322886438"}],"id":"n0.4581428332056161"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.2728615589727075"}],"style":{"align":"center"},"id":"n0.5587154326885382"}],"shape":{"data":{"p":{"x":115.0172119140625,"y":59.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7448435430529068":{"id":"de7448435430529068","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.24419843608862757"}],"id":"n0.6186090930591632"}],"id":"n0.27072142324195303"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.5416380547548176"}],"id":"n0.49359294107359974"}],"shape":{"data":{"p":{"x":83.0172119140625,"y":60.30042969200531}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9645011963385512":{"id":"de9645011963385512","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.5491078512601584"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.2671504875624111","text":"j"}],"id":"n0.32536765922598"}],"id":"n0.920316694189353"},"powerValue":{"lines":[{"blocks":[{"text":"T","id":"n0.3958005480412661"}],"id":"n0.45718673014618805"}],"id":"n0.8929803939717895"}},"id":"n0.9621800921619503"}],"id":"n0.37647153187475135"}],"id":"n0.39136111084628955"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4692029339746646"}],"id":"n0.5362876157300336"}],"shape":{"data":{"p":{"x":107.0172119140625,"y":58.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de756467946908294":{"id":"de756467946908294","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜏","id":"n0.09040024633854027"},{"id":"n0.9414271134932601","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.8539008977666882","lines":[{"id":"n0.4518242293028474","blocks":[{"id":"n0.3965299041617616","text":"a"},{"id":"n0.5950237375304415","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2004556375558837","lines":[{"id":"n0.9786636017007695","blocks":[{"id":"n0.2720602468752946","text":"i"}]}]}}}]}]}}}],"id":"n0.9903605090117544"}],"id":"n0.7968369877522394"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.640509913467499"}],"style":{"align":"center"},"id":"n0.4390753621173462"}],"shape":{"data":{"p":{"x":41.0172119140625,"y":36.54835681521689},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de49310965300164167":{"id":"de49310965300164167","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜏","id":"n0.5029595600631078"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.49474462952339593"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.10050877597725605","text":"j"}],"id":"n0.7137077923863049"}],"id":"n0.03814875876868795"}},"id":"n0.6702518299974569"}],"id":"n0.14156621606474862"}],"id":"n0.19597520547224634"}},"id":"n0.28104078261921317"}],"id":"n0.6777525444975907"}],"id":"n0.43200332154226206"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.38503797423491215"}],"style":{"align":"center"},"id":"n0.5344267510048109"}],"shape":{"data":{"p":{"x":41.0172119140625,"y":57.54835681521689},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7539779953399748":{"id":"de7539779953399748","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.12071300230555493"}],"id":"n0.6389586816019504"}],"id":"n0.09302421410022554"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.17799468051078948"}],"style":{"align":"center"},"id":"n0.020294695836960752"}],"shape":{"data":{"p":{"x":15.0172119140625,"y":81.369590963122},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5911363371170728":{"id":"de5911363371170728","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"}","id":"n0.7564784181513657"}],"id":"n0.9518648643126093"}],"id":"n0.13123680074453592"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.30217654976660224"}],"style":{"align":"center"},"id":"n0.7625369652930956"}],"shape":{"data":{"p":{"x":79.0172119140625,"y":81.369590963122},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2874148039921536":{"id":"de2874148039921536","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.20746859696009823"}],"id":"n0.9625692368785876"}],"id":"n0.21744012313887917"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.719910678243934"}],"id":"n0.3953473469356017"}],"shape":{"data":{"p":{"x":47.0172119140625,"y":82.30042969200531}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de09506015339513452":{"id":"de09506015339513452","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜏","id":"n0.8056760836355961"},{"id":"n0.19700486811713191","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.1118667355180678","lines":[{"id":"n0.10776605706493791","blocks":[{"id":"n0.007754824021389384","text":"o"},{"id":"n0.7267764500012224","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.022645884654262094","lines":[{"id":"n0.07291715931053155","blocks":[{"id":"n0.3681933782261868","text":"i"}]}]}}}]}]}}}],"id":"n0.574213430457988"}],"id":"n0.7879157549084901"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5808192267936789"}],"style":{"align":"center"},"id":"n0.7728223320223773"}],"shape":{"data":{"p":{"x":5.0172119140625,"y":79.54835681521689},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de02747343053030571":{"id":"de02747343053030571","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"o","id":"n0.44625754460905753"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8893678335268238"}],"id":"n0.6884801257066628"}],"id":"n0.7120420318740519"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.9570091548721635"}],"id":"n0.24447494473767573"}],"id":"n0.37374589938555314"}},"id":"n0.9463720171867886"}],"id":"n0.6003475309273705"}],"id":"n0.9901597008831791"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.10003632182033839"}],"id":"n0.7822660415586566"}],"shape":{"data":{"p":{"x":26.5172119140625,"y":79.78239979743955}},"anchor":"left-top"},"isTextMode":true},"de34785104329949257":{"id":"de34785104329949257","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"o","id":"n0.11075842681461645"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.1605187139634474"}],"id":"n0.8013424382554843"}],"id":"n0.20474298201342234"},"powerValue":{"lines":[{"blocks":[{"text":"t+1","id":"n0.8826139000039472"}],"id":"n0.2829897872364435"}],"id":"n0.18076721689238662"}},"id":"n0.504632079602521"}],"id":"n0.3470720973214332"}],"id":"n0.9801920815872638"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.08243843502458148"}],"id":"n0.2792151759161037"}],"shape":{"data":{"p":{"x":38.5172119140625,"y":79.78239979743955}},"anchor":"left-top"},"isTextMode":true},"de7172149586802281":{"id":"de7172149586802281","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"o","id":"n0.8047526366647146"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9174964467470521"}],"id":"n0.41886824368367015"}],"id":"n0.4847380786298725"},"powerValue":{"lines":[{"blocks":[{"id":"n0.23309421944975073","text":"T+1"}],"id":"n0.9393771506272504"}],"id":"n0.8359339654331044"}},"id":"n0.3938671942741456"}],"id":"n0.9544275247121161"}],"id":"n0.7593809752282012"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5184485551626943"}],"id":"n0.06640259461733056"}],"shape":{"data":{"p":{"x":68.5172119140625,"y":79.78239979743955}},"anchor":"left-top"},"isTextMode":true},"de8555181190209911":{"id":"de8555181190209911","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.12155272212617074"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.49906942447057334"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.8214858544308155"}],"id":"n0.5043969874613548"}],"id":"n0.11478171217302191"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.37179947470330266"}],"id":"n0.5457666319441228"}],"id":"n0.6519377455991147"}},"id":"n0.008212787674330091"}],"id":"n0.3157526464422953"}],"id":"n0.4254440358615659"}},"id":"n0.32299234035675894"},{"type":"single","text":"(","id":"n0.811637462333094"},{"text":"s,a","id":"n0.9580426701193052"},{"type":"single","text":")","id":"n0.8869435608132157"}],"id":"n0.15940430690943685"}],"id":"n0.3132924567681319"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5994810916217608"}],"style":{"align":"center"},"id":"n0.3803486414737671"}],"shape":{"data":{"p":{"x":98.40112242936175,"y":216.66248913204873},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6117269236688183":{"id":"de6117269236688183","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"X","id":"n0.5568546759848911"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.539093983180535"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.5504994157337477"}],"id":"n0.6602808463544139"}],"id":"n0.386195782177984"},"indexValue":{"lines":[{"blocks":[{"id":"n0.9047892248610752","text":"R"}],"id":"n0.5516441822744349"}],"id":"n0.9424196624443812"}},"id":"n0.9900286822571793"}],"id":"n0.7841050325873038"}],"id":"n0.8155590170099274"}},"id":"n0.2971341695350542"},{"type":"single","text":"(","id":"n0.6350491494159667"},{"text":"s,a","id":"n0.42438966136036904"},{"type":"single","text":")","id":"n0.9925009236370999"}],"id":"n0.3226085603936859"}],"id":"n0.7590487519403368"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9494209754238183"}],"style":{"align":"center"},"id":"n0.19546139395537332"}],"shape":{"data":{"p":{"x":150.58166565657575,"y":218.18984940756428},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de311792193101031":{"id":"de311792193101031","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.6057829974237232"}],"id":"n0.7516130028137709"}],"id":"n0.6909822130568688"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.18647341392534633"}],"style":{"align":"center"},"id":"n0.11009329718912242"}],"shape":{"data":{"p":{"x":60.5752569651695,"y":257.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6715154092032498":{"id":"de6715154092032498","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.002121963406264138"}],"id":"n0.12942752166974025"}],"id":"n0.608719912583584"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5822546705489986"}],"style":{"align":"center"},"id":"n0.7119450236672624"}],"shape":{"data":{"p":{"x":180.31076744317738,"y":258.2583716044299},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4793583580341598":{"id":"de4793583580341598","lines":[{"blocks":[{"text":"Nested MDP module","style":{"fontSize":"\\tiny"},"id":"n0.8448358206245414"}],"style":{"align":"center"},"id":"n0.5997765310201999"}],"shape":{"data":{"p":{"x":288.1061553955079,"y":204.60139017105115},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5251325581597752":{"id":"de5251325581597752","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"One hot mapping","id":"n0.1311128344440089"}],"id":"n0.9208219994297089"}],"shape":{"data":{"p":{"x":158.0172119140625,"y":48.78239979743955},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de047770060574601425":{"id":"de047770060574601425","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Depth: ","id":"n0.8608065394806057"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.1517757797109054"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5305308657982704"}],"id":"n0.8293462318848102"}],"id":"n0.46725334418639997"}},"id":"n0.14390605202063256"},{"text":"|","id":"n0.4459980056293207"}],"id":"n0.9142747805274785"}],"id":"n0.6638238662000462"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.053809341239267505"},{"id":"n0.06962374744131217","text":",","style":{"fontSize":{"value":0.4}}},{"id":"n0.23137954604272326","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.27431182150181543","lines":[{"id":"n0.9452261389098291","blocks":[{"id":"n0.6323810685373348","text":"|A"},{"id":"n0.7581772681461316","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6622233094117673","lines":[{"id":"n0.019564322462538808","blocks":[{"id":"n0.2997409476047901","text":"j"}]}]}}},{"text":"|","id":"n0.2897989632134057"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}}}],"id":"n0.0012820744010371143"}],"shape":{"data":{"p":{"x":151.0172119140625,"y":51.28239979743955},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di3840833210691088","items":[],"style":{}},"shapes":[{"id":"dp47291887025148904","type":"rectangle","data":{"p1":{"x":32.21372256017689,"y":176.57503948597804},"p2":{"x":61.536182406122975,"y":205.89749933192408}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp33270367186104255","type":"rectangle","data":{"p1":{"x":178.53618240612298,"y":177.57503948597804},"p2":{"x":207.85864225206907,"y":206.89749933192408}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp3686329362905836","type":"doc-rounded-rect","data":{"p1":{"x":273.39875726699836,"y":204.36876454353347},"p2":{"x":379.02362060546886,"y":230.0662476062774}},"style":{"fillColor":[140,200,240,1]}},{"id":"dp5007381791832946","type":"doc-rounded-rect","data":{"p1":{"x":274.39875726699825,"y":168.188744354248},"p2":{"x":377.026611328125,"y":193.88622741699214}},"style":{"fillColor":[140,200,240,1]}},{"id":"da6392114586352498","data":[{"x":61.0093994140625,"y":192.28239979743955},{"x":177.026611328125,"y":192.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp5349757603446712","type":"square","data":{"p1":{"x":62.0172119140625,"y":45.28239979743955},"p2":{"x":74.5172119140625,"y":57.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp7720825853344573","type":"rectangle","data":{"p1":{"x":133.0172119140625,"y":50.78239979743955},"p2":{"x":149.02362060546875,"y":99.78239979743955}}},{"id":"da030927197472309542","data":[{"x":33.0093994140625,"y":105.28239979743955},{"x":95.0093994140625,"y":105.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da953350202160437","data":[{"x":69.0093994140625,"y":83.28239979743955},{"x":132.0093994140625,"y":83.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da11428665306721131","data":[{"x":149.02362060546875,"y":86.28239979743955},{"x":162.02362060546875,"y":86.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg8117454392492514","entities":[{"id":"dp6894444328881189","type":"rectangle","data":{"p1":{"x":163.0172119140625,"y":78.7643699028738},"p2":{"x":175.67437264612136,"y":91.42153063493265}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp7867069659758521","type":"rectangle","data":{"p1":{"x":164.59935700556986,"y":80.34651499438115},"p2":{"x":177.2565177376287,"y":93.00367572644001}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp8906719224066897","type":"rectangle","data":{"p1":{"x":166.1815020970772,"y":81.92866008588851},"p2":{"x":178.83866282913607,"y":94.58582081794736}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dg025260480365929094","entities":[{"id":"dg6091432848288012","entities":[{"id":"dp898136671828403","type":"rectangle","data":{"p1":{"x":200.0172119140625,"y":96.7643699028738},"p2":{"x":212.67437264612136,"y":109.42153063493265}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp6715600294846531","type":"rectangle","data":{"p1":{"x":201.59935700556986,"y":98.34651499438115},"p2":{"x":214.2565177376287,"y":111.00367572644001}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp99606808320349","type":"rectangle","data":{"p1":{"x":203.1815020970772,"y":99.92866008588851},"p2":{"x":215.83866282913607,"y":112.58582081794736}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl11878088651665242","linkedId":"de9077288866210012"}]},{"id":"da49805112140537133","data":[{"x":111.0093994140625,"y":105.28239979743955},{"x":199.0172119140625,"y":105.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp8861163273406749","type":"square","data":{"p1":{"x":77.0172119140625,"y":45.28239979743955},"p2":{"x":89.5172119140625,"y":57.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp42447876275798024","type":"square","data":{"p1":{"x":107.0172119140625,"y":45.28239979743955},"p2":{"x":119.5172119140625,"y":57.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"da5907703484136553","data":[{"x":97.9664306640625,"y":34.3687645435333},{"x":352.026611328125,"y":34.3687645435333}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da12041695999585555","data":[{"x":97.9664306640625,"y":34.3687645435333},{"x":97.9664306640625,"y":38.4984032154083}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg8979656007400847","entities":[{"id":"dp8714920450744359","type":"rectangle","data":{"p1":{"x":95.0172119140625,"y":86.78239979743955},"p2":{"x":111.02362060546875,"y":135.78239979743955}}},{"id":"dl3810803124023281","linkedId":"de8769763256636647"},{"id":"dl8502562526816417","linkedId":"de766426490560322"}]},{"id":"dp2743939152477397","type":"doc-rounded-rect","data":{"p1":{"x":228.3987572669983,"y":72.3687645435333},"p2":{"x":387.346923828125,"y":98.06624760627744}},"style":{"fillColor":[140,200,240,1]}},{"id":"dp13836120411734676","type":"doc-cube","data":{"p1":{"x":66.0172119140625,"y":138.24594116210938},"p2":{"x":104.10756690024687,"y":175.95588793598483},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da9034582338657684","data":[{"x":179.02362060546875,"y":86.28239979743955},{"x":228.0093994140625,"y":86.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da3568795922343908","data":[{"x":208.026611328125,"y":92.58582081794736},{"x":228.026611328125,"y":92.58582081794736}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp5854503391049615","type":"doc-cube","data":{"p1":{"x":411.0172119140625,"y":65.24594116210938},"p2":{"x":449.10756690024687,"y":102.95588793598483},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da15955639931239407","data":[{"x":388.0172119140625,"y":85.28239979743955},{"x":411.0093994140625,"y":85.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da0683073607586604","data":[{"x":245.026611328125,"y":155.3687645435333},{"x":245.026611328125,"y":98.53384399414062}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da8342047457852937","data":[{"x":250.026611328125,"y":59.3687645435333},{"x":430.026611328125,"y":59.3687645435333}],"head":"no","tail":"no","shaft":{"type":"dash","pattern":[5,4,10,2]},"headScale":0.6},{"id":"da1240180229856167","data":[{"x":250.026611328125,"y":59.3687645435333},{"x":250.026611328125,"y":71.40420532226562}],"head":"fh>","tail":"no","shaft":{"type":"dash","pattern":[5,4,10,2]},"headScale":0.6},{"id":"da35220081363584743","data":[{"x":430.026611328125,"y":65.61519384384155},{"x":430.026611328125,"y":59.3687645435333}],"head":"no","tail":"no","shaft":"--","headScale":0.6},{"id":"da3297076579890863","data":[{"x":430.026611328125,"y":102.61519384384155},{"x":430.026611328125,"y":141.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da3354121762434161","data":[{"x":486.026611328125,"y":48.3687645435333},{"x":458.026611328125,"y":48.3687645435333}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp9444187807371747","type":"doc-rounded-rect","data":{"p1":{"x":352.3987572669983,"y":27.368764543533302},"p2":{"x":458.02362060546875,"y":53.06624760627744}},"style":{"fillColor":[255,100,100,1]}},{"id":"dp14401954448631438","type":"doc-rounded-rect","data":{"p1":{"x":466.026611328125,"y":1.5379272937775},"p2":{"x":545.026611328125,"y":26.368764543533302}},"style":{"fillColor":[255,100,100,1]}},{"id":"dg5964008931601581","entities":[{"id":"dg13729603557708514","entities":[{"id":"dp8608226067570728","type":"rectangle","data":{"p1":{"x":524.9827880859375,"y":40.764369902873796},"p2":{"x":537.6399488179964,"y":53.42153063493265}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp33308955013887354","type":"rectangle","data":{"p1":{"x":526.5649331774448,"y":42.34651499438115},"p2":{"x":539.2220939095037,"y":55.00367572644001}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp08325441009202605","type":"rectangle","data":{"p1":{"x":528.1470782689522,"y":43.92866008588851},"p2":{"x":540.8042390010111,"y":56.585820817947365}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl04227117205865438","linkedId":"de7333755688576151"}]},{"id":"dg07971275407612999","entities":[{"id":"dg10005593632932497","entities":[{"id":"dp2595396412152444","type":"rectangle","data":{"p1":{"x":491.9827880859375,"y":40.42916718304414},"p2":{"x":504.63994881799636,"y":53.335634957633346}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp7503940593260996","type":"rectangle","data":{"p1":{"x":493.5649331774448,"y":42.042475654867786},"p2":{"x":506.22209390950366,"y":54.94894342945699}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp4255756058740263","type":"rectangle","data":{"p1":{"x":495.1470782689522,"y":43.65578412669143},"p2":{"x":507.80423900101107,"y":56.562251901280646}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{"rotation":0}},{"id":"dl6550347857907792","linkedId":"de11067232215210976"}]},{"id":"dp7344263155280306","type":"square","data":{"p1":{"x":529,"y":194.0137939453125},"p2":{"x":541.5,"y":206.5137939453125}},"style":{"fillColor":[248,231,28,1]}},{"id":"da6087127329803084","data":[{"x":473.026611328125,"y":180.76184458732604},{"x":514.9260864257812,"y":180.76184458732604}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg28665975456564574","entities":[{"id":"dg1220839973179737","entities":[{"id":"dp02859167077177971","type":"rectangle","data":{"p1":{"x":457,"y":172.49576405074674},"p2":{"x":469.65716073205886,"y":185.1529247828056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp7557740031830245","type":"rectangle","data":{"p1":{"x":458.5821450915073,"y":174.0779091422541},"p2":{"x":471.23930582356616,"y":186.73506987431296}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp05921587767632008","type":"rectangle","data":{"p1":{"x":460.1642901830147,"y":175.66005423376146},"p2":{"x":472.82145091507357,"y":188.3172149658203}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl7884950672888991","linkedId":"de5551324285345347"}]},{"id":"da4360362968208855","data":[{"x":514.9260864257812,"y":180.76184458732604},{"x":514.9260864257812,"y":66.08636474609375}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da1365254495516297","data":[{"x":406.026611328125,"y":27.615193843841553},{"x":406.026611328125,"y":14.316253662109375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7266274650303373","data":[{"x":406.026611328125,"y":14.316253662109375},{"x":465.026611328125,"y":14.316253662109375}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da7146537518216651","data":[{"x":47.026611328125,"y":155.3687645435333},{"x":65.026611328125,"y":155.3687645435333}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da3822054179326899","data":[{"x":47.026611328125,"y":176.08636474609375},{"x":47.026611328125,"y":155.3687645435333}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg31479627254461207","entities":[{"id":"dg04182556084429523","entities":[{"id":"dp8222555557078086","type":"rectangle","data":{"p1":{"x":126.2857093811034,"y":267.5552864074705},"p2":{"x":135.42856979370129,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[248,231,28,1]}},{"id":"dl8712823427166769","linkedId":"de157530155636616"}]},{"id":"dg039684418290218515","entities":[{"id":"dp8400337706125396","type":"rectangle","data":{"p1":{"x":191.2857093811034,"y":267.5552864074705},"p2":{"x":200.42856979370129,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[80,227,194,1]}},{"id":"dl9055472886924096","linkedId":"de9474792898469997"}]},{"id":"dg9466631126217466","entities":[{"id":"dp052026641018338315","type":"rectangle","data":{"p1":{"x":321.2857093811034,"y":267.5552864074705},"p2":{"x":330.4285697937013,"y":330.5552864074705},"rotation":270}},{"id":"dl1370376181394557","linkedId":"de38901163369922753"}]},{"id":"dg00781979238143271","entities":[{"id":"dp779255616671013","type":"rectangle","data":{"p1":{"x":386.2857093811034,"y":267.5552864074705},"p2":{"x":395.4285697937013,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[184,233,134,1]}},{"id":"dl7466420505056555","linkedId":"de7846039342937636"}]},{"id":"dg6978924027490241","entities":[{"id":"dp2553832889138268","type":"rectangle","data":{"p1":{"x":516.2857093811034,"y":267.5552864074705},"p2":{"x":525.4285697937013,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[255,100,100,1]}},{"id":"dl5551832308589866","linkedId":"de6916130444344799"}]},{"id":"dg27173311021871127","entities":[{"id":"dp5838520968227427","type":"rectangle","data":{"p1":{"x":581.2857093811034,"y":267.5552864074705},"p2":{"x":590.4285697937013,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[74,144,226,0.5]}},{"id":"dl5405692283635466","linkedId":"de6830316854968421"}]},{"id":"dg818223334097526","entities":[{"id":"dp09610739516205102","type":"rectangle","data":{"p1":{"x":451.2857093811034,"y":267.5552864074705},"p2":{"x":460.4285697937013,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[180,180,180,1]}},{"id":"dl677683996301746","linkedId":"de6581424833173313"}]},{"id":"dg8743036343367914","entities":[{"id":"dp8550898217750769","type":"rectangle","data":{"p1":{"x":256.2857093811034,"y":267.53902053832985},"p2":{"x":265.4285697937013,"y":330.53902053832985},"rotation":270},"style":{"fillColor":[245,166,35,1]}},{"id":"dl5117518334725439","linkedId":"de03535318107247609"}]}]},{"id":"dp36530934611293553","type":"doc-cube","data":{"p1":{"x":175.0172119140625,"y":135.24594116210938},"p2":{"x":213.10756690024687,"y":172.95588793598483},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da9137409352026389","data":[{"x":159.0093994140625,"y":155.3687645435333},{"x":175.026611328125,"y":155.3687645435333}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp3354267807849822","type":"square","data":{"p1":{"x":62,"y":66.28239979743955},"p2":{"x":74.5,"y":78.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"da5895173336123907","data":[{"x":47.026611328125,"y":206.61519384384155},{"x":47.026611328125,"y":244.89722917234633}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da4759367535608223","data":[{"x":104.026611328125,"y":155.3687645435333},{"x":136.0093994140625,"y":155.3687645435333}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da23401725323007638","data":[{"x":69.0172119140625,"y":57.78239979743955},{"x":69.0093994140625,"y":62.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da4417642064933385","data":[{"x":69.0093994140625,"y":62.21600341796875},{"x":132.0093994140625,"y":62.21600341796875}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da16723585432262245","data":[{"x":149.02362060546875,"y":62.28239979743955},{"x":162.02362060546875,"y":62.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6204603852043595","entities":[{"id":"dg34507822073433725","entities":[{"id":"dp6767493988125446","type":"rectangle","data":{"p1":{"x":163.0172119140625,"y":54.764369902873796},"p2":{"x":175.67437264612136,"y":67.42153063493265}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp8378712102252863","type":"rectangle","data":{"p1":{"x":164.59935700556986,"y":56.34651499438115},"p2":{"x":177.2565177376287,"y":69.00367572644001}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp9340856766244212","type":"rectangle","data":{"p1":{"x":166.1815020970772,"y":57.92866008588851},"p2":{"x":178.83866282913607,"y":70.58582081794736}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl5674564919174834","linkedId":"de27900670992145105"}]},{"id":"da8657778222710852","data":[{"x":206.0093994140625,"y":79.50826115608213},{"x":228.3987572669983,"y":79.50826115608213}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9090319524213821","data":[{"x":179.02362060546875,"y":62.28239979743955},{"x":206.0093994140625,"y":62.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7933468941224051","data":[{"x":206.0093994140625,"y":79.50826115608213},{"x":206.0093994140625,"y":62.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da2634070014092007","data":[{"x":172.0172119140625,"y":70.78239979743955},{"x":172.0093994140625,"y":75.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da5045693654670567","data":[{"x":172.0172119140625,"y":94.78239979743955},{"x":172.0093994140625,"y":102.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7005836873374018","data":[{"x":172.0093994140625,"y":75.21600341796875},{"x":189.0093994140625,"y":75.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9975072723287093","data":[{"x":172.0093994140625,"y":102.21600341796875},{"x":189.0093994140625,"y":102.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9717334391214678","data":[{"x":189.0093994140625,"y":131.21600341796875},{"x":189.0093994140625,"y":75.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da23462799332701567","data":[{"x":189.0093994140625,"y":131.21600341796875},{"x":305.0093994140625,"y":131.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da05639754580279521","data":[{"x":233.0093994140625,"y":178.28239979743955},{"x":273.92608642578125,"y":178.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da41048600073210206","data":[{"x":194.0093994140625,"y":221.32824096679684},{"x":273.39875726699836,"y":221.32824096679684}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da4130143203023442","data":[{"x":327.39875726699825,"y":141.28239979743955},{"x":430.026611328125,"y":141.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da027523619528937227","data":[{"x":379.1072021484375,"y":217.35307836532593},{"x":416.9921875,"y":217.35307836532593}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg9275159137300206","entities":[{"id":"dg03931437452152142","entities":[{"id":"dp2612886007456432","type":"rectangle","data":{"p1":{"x":417.9827880859375,"y":209.49576405074674},"p2":{"x":430.63994881799636,"y":222.1529247828056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp703123805601543","type":"rectangle","data":{"p1":{"x":419.5649331774448,"y":211.0779091422541},"p2":{"x":432.22209390950366,"y":223.73506987431296}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp7783348813475786","type":"rectangle","data":{"p1":{"x":421.1470782689522,"y":212.66005423376146},"p2":{"x":433.80423900101107,"y":225.3172149658203}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl9045323818869151","linkedId":"de5137422723619176"}]},{"id":"da76520212951226","data":[{"x":327.39875726699825,"y":168.32824096679684},{"x":327.39875726699825,"y":141.28239979743955}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da8231706178092588","data":[{"x":327.39875726699825,"y":193.32824096679684},{"x":327.39875726699825,"y":199.76184458732604}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8843110333077893","data":[{"x":327.39875726699825,"y":199.76184458732604},{"x":529.026611328125,"y":199.76184458732604}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da5408394447346849","data":[{"x":377.39875726699825,"y":180.76184458732604},{"x":457.026611328125,"y":180.76184458732604}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg010187030176750156","entities":[{"id":"dg7740502244820402","entities":[{"id":"dp30502397317802865","type":"rectangle","data":{"p1":{"x":584.9827880859375,"y":28.764369902873796},"p2":{"x":597.6399488179964,"y":41.42153063493265}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp6929910450011407","type":"rectangle","data":{"p1":{"x":586.5649331774448,"y":30.346514994381153},"p2":{"x":599.2220939095037,"y":43.00367572644001}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp14312062962951622","type":"rectangle","data":{"p1":{"x":588.1470782689522,"y":31.92866008588851},"p2":{"x":600.8042390010111,"y":44.585820817947365}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl937254962591253","linkedId":"de13864094431472274"}]},{"id":"dg14381181430645285","entities":[{"id":"dg851948865293015","entities":[{"id":"dp6449076364831263","type":"rectangle","data":{"p1":{"x":551.9827880859375,"y":28.429167183044143},"p2":{"x":564.6399488179964,"y":41.335634957633346}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp5027674435197778","type":"rectangle","data":{"p1":{"x":553.5649331774448,"y":30.042475654867786},"p2":{"x":566.2220939095037,"y":42.94894342945699}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp5393966062547468","type":"rectangle","data":{"p1":{"x":555.1470782689522,"y":31.65578412669143},"p2":{"x":567.8042390010111,"y":44.562251901280646}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{"rotation":0}},{"id":"dl9970922422977695","linkedId":"de130364287178661"}]},{"id":"da7287519209547981","data":[{"x":574.9260864257812,"y":217.35307836532593},{"x":574.9260864257812,"y":55.08636474609375}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da8134947108062274","data":[{"x":433.9921875,"y":217.35307836532593},{"x":574.9260864257812,"y":217.35307836532593}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9462672208237359","data":[{"x":327.39875726699825,"y":244.89722917234633},{"x":327.39875726699825,"y":229.76184458732604}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9177471098672696","data":[{"x":181.26448952199212,"y":244.89722917234633},{"x":327.39875726699825,"y":244.89722917234633}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7862100457272858","data":[{"x":305.0093994140625,"y":168.08636474609375},{"x":305.0093994140625,"y":131.21600341796875}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da8237929411758496","data":[{"x":545.9260864257812,"y":36.50826115608213},{"x":458.02362060546875,"y":36.50826115608213}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da784974372238094","data":[{"x":213.0093994140625,"y":155.3687645435333},{"x":245.026611328125,"y":155.3687645435333}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da5017675230909444","data":[{"x":261.0093994140625,"y":212.08636474609375},{"x":261.0093994140625,"y":131.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7847399800114798","data":[{"x":261.0093994140625,"y":212.50826115608226},{"x":273.39875726699836,"y":212.50826115608226}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da04620954595561888","data":[{"x":254.39875726699825,"y":245.21600341796875},{"x":254.39875726699825,"y":185.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da3986932486764072","data":[{"x":254.39875726699825,"y":185.28239979743955},{"x":273.66242184638975,"y":185.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp8618704677398219","type":"square","data":{"p1":{"x":77.0172119140625,"y":66.28239979743955},"p2":{"x":89.5172119140625,"y":78.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp4220243817144764","type":"square","data":{"p1":{"x":107.0172119140625,"y":66.28239979743955},"p2":{"x":119.5172119140625,"y":78.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"da6000787670579764","data":[{"x":69.0093994140625,"y":83.28239979743955},{"x":69.0093994140625,"y":79.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp40504580124109624","type":"square","data":{"p1":{"x":26.0172119140625,"y":88.28239979743955},"p2":{"x":38.5172119140625,"y":100.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp05521779590020026","type":"square","data":{"p1":{"x":41.0172119140625,"y":88.28239979743955},"p2":{"x":53.5172119140625,"y":100.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp5297858632182728","type":"square","data":{"p1":{"x":71.0172119140625,"y":88.28239979743955},"p2":{"x":83.5172119140625,"y":100.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"da9760486685833776","data":[{"x":33.0093994140625,"y":105.28239979743955},{"x":33.0093994140625,"y":101.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da5414642445065745","data":[{"x":233.0093994140625,"y":168.21600341796875},{"x":252.0093994140625,"y":168.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8874845382551191","data":[{"x":252.0093994140625,"y":168.21600341796875},{"x":252.0093994140625,"y":98.21600341796875}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da3614163071748169","data":[{"x":194.0093994140625,"y":221.32824096679684},{"x":194.0093994140625,"y":207.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da6285132337880759","data":[{"x":233.0093994140625,"y":192.21600341796875},{"x":233.0093994140625,"y":168.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da36703405582495274","data":[{"x":208.0093994140625,"y":192.21600341796875},{"x":233.0093994140625,"y":192.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp31192838658068833","type":"doc-cube","data":{"p1":{"x":80.31076744317738,"y":229.9559559513225},"p2":{"x":118.40112242936175,"y":267.66590272519784},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp21586068142524484","type":"doc-cube","data":{"p1":{"x":80.31076744317738,"y":197.65354029821492},"p2":{"x":118.40112242936175,"y":235.36348707209038},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp3674475134050299","type":"doc-cube","data":{"p1":{"x":90.99359130859375,"y":240.2549580112808},"p2":{"x":129.08394629477812,"y":277.96490478515625},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp5033659830497497","type":"doc-cube","data":{"p1":{"x":90.99359130859375,"y":208.2549580112808},"p2":{"x":129.08394629477812,"y":245.96490478515625},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp23700482503033227","type":"doc-cube","data":{"p1":{"x":132.49131067039139,"y":230.48331622683804},"p2":{"x":170.58166565657575,"y":268.1932630007134},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp6002948552391556","type":"doc-cube","data":{"p1":{"x":132.49131067039139,"y":198.18090057373047},"p2":{"x":170.58166565657575,"y":235.89084734760593},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp21640677116835727","type":"doc-cube","data":{"p1":{"x":143.17413453580775,"y":241.2549580112808},"p2":{"x":181.26448952199212,"y":278.96490478515625},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp23699338099923106","type":"doc-cube","data":{"p1":{"x":143.17413453580775,"y":209.2549580112808},"p2":{"x":181.26448952199212,"y":246.96490478515625},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da6761432924104998","data":[{"x":47.026611328125,"y":244.89722917234633},{"x":80.0093994140625,"y":244.89722917234633}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da05559165748430894","data":[{"x":208.0093994140625,"y":96.50826115608213},{"x":208.0093994140625,"y":92.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da5357038925844808","data":[{"x":124.0093994140625,"y":184.21600341796875},{"x":124.0093994140625,"y":126.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da07608551579945444","data":[{"x":124.0093994140625,"y":126.21600341796875},{"x":238.026611328125,"y":126.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9064000025688352","data":[{"x":238.026611328125,"y":126.21600341796875},{"x":238.026611328125,"y":98.53384399414062}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da00021660160795677896","data":[{"x":98.0093994140625,"y":184.21600341796875},{"x":124.0093994140625,"y":184.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da6273542180639886","data":[{"x":98.0093994140625,"y":197.21600341796875},{"x":98.0093994140625,"y":184.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6}],"settings":{"grid":true,"diagramHeight":304.9266357421875}}]},{"id":"n0.9182410738498363","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":5062,"delayRenderCache":{"av":5062,"map":{"n0.2798165469167486":{"n0.8584969463576833":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.0956182946294597":{"n0.35156619811075585":{"w":11.6193,"h":8.4545,"bl":0.8214}},"n0.4915964638796144":{"n0.6764598294619883":{"w":13.4368,"h":41.6667,"bl":0.8333}},"n0.44181901465933904":{"n0.19455039516198558":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.8377316246435462":{"n0.8879719304316316":{"w":11.6193,"h":8.4545,"bl":0.8214}},"n0.6638238662000462":{"n0.9142747805274785":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.8656149269890585":{"n0.2421330624441942":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.6037157092616128":{"n0.6856134748473006":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.7968369877522394":{"n0.9903605090117544":{"w":7.5955,"h":8.988,"bl":0.7726}},"n0.43200332154226206":{"n0.6777525444975907":{"w":7.7673,"h":8.988,"bl":0.7726}},"n0.7879157549084901":{"n0.574213430457988":{"w":7.5955,"h":8.988,"bl":0.7726}},"n0.6909822130568688":{"n0.7516130028137709":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.608719912583584":{"n0.12942752166974025":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.9805767880860297":{"n0.8796898714453854":{"w":10.6518,"h":9.1146,"bl":0.7619}},"n0.8192672737499627":{"n0.4046619303284873":{"w":5.3982,"h":9.1146,"bl":0.7619}},"n0.8865234094211434":{"n0.7670471443345628":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.9553225079236318":{"n0.36904407403017525":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.07663451775769459":{"n0.21276920260652177":{"w":6.7184,"h":9.1146,"bl":0.7619}},"n0.05892219861296333":{"n0.6634858829152157":{"w":16.8457,"h":12.5054,"bl":0.7021}},"n0.8095639861826163":{"n0.6922443966909593":{"w":15.8511,"h":12.5054,"bl":0.7021}},"n0.7620537820832181":{"n0.6042093799923687":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.9087874361013744":{"n0.31153597860941096":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.678448619782392":{"n0.07297285074437698":{"w":5.3982,"h":9.1146,"bl":0.7619}},"n0.2860407715183735":{"n0.4675833849066542":{"w":22.4157,"h":12.5054,"bl":0.7021}},"n0.8842098281055866":{"n0.7129346546594733":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.6926625074118744":{"n0.8820827388445249":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.19734605494092916":{"n0.6878304647006728":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.11712223778126041":{"n0.560660220226239":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.7646762117471588":{"n0.2652112962808757":{"w":10.6518,"h":9.1146,"bl":0.7619}},"n0.8432401649435193":{"n0.3745027443049487":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.865317173645763":{"n0.43454788566174973":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.6370642722097213":{"n0.9405832457870693":{"w":7.6317,"h":9.6481,"bl":0.7198}},"n0.7046338254291307":{"n0.4472116882434696":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.7689628952048579":{"n0.49535503691405913":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.5800614332963825":{"n0.7399053922658398":{"w":7.6317,"h":9.6481,"bl":0.7198}},"n0.5054730445479463":{"n0.7748604418054355":{"w":7.6317,"h":9.6481,"bl":0.7198}},"n0.3935563474086412":{"n0.7205301889098097":{"w":5.3982,"h":9.1146,"bl":0.7619}},"n0.9680449396846869":{"n0.639855730025886":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.4581428332056161":{"n0.5961478322886438":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.39136111084628955":{"n0.37647153187475135":{"w":6.7184,"h":9.1146,"bl":0.7619}},"n0.09302421410022554":{"n0.6389586816019504":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.13123680074453592":{"n0.9518648643126093":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.9901597008831791":{"n0.6003475309273705":{"w":5.3982,"h":9.1146,"bl":0.7619}},"n0.9801920815872638":{"n0.3470720973214332":{"w":10.9502,"h":9.1146,"bl":0.7619}},"n0.7593809752282012":{"n0.9544275247121161":{"w":12.2703,"h":9.1146,"bl":0.7619}},"n0.3132924567681319":{"n0.15940430690943685":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.7590487519403368":{"n0.3226085603936859":{"w":24.2965,"h":9.9736,"bl":0.6963}},"n0.27431182150181543":{"n0.9452261389098291":{"w":11.3661,"h":8.4545,"bl":0.8214}}}}}

==> sIPOMDPLite-Net(arXiv)/plots/docs/595142f9-809a-4354-8218-28db58f80e34 <==
{"id":"n0.27567949884143794","lines":[{"id":"n0.040192133545799535","blocks":[]},{"id":"n0.9895876271290234","blocks":[{"id":"n0.9173890258494699","text":"\\diagram","type":"composite","elements":{"de11223966794022666":{"id":"de11223966794022666","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.7905678483945358"}],"id":"n0.19836934953297547"}],"id":"n0.3697409210978573"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.431063176229344"}],"id":"n0.45841864014718414"}],"shape":{"data":{"p":{"x":43.51719895786459,"y":44.62593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9324197589956453":{"id":"de9324197589956453","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"K","id":"n0.7854313636540744"}],"id":"n0.985214144221201"}],"id":"n0.6661812810602377"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.40559890186951475"},{"text":"-recurrence","style":{"fontSize":{"value":0.4}},"id":"n0.003152585387300899"}],"style":{"align":"center"},"id":"n0.061334301092576204"}],"shape":{"data":{"p":{"x":40.48858574589599,"y":50.62593476262708},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8259787715425368":{"id":"de8259787715425368","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"U","id":"n0.6399712608665704"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"0","id":"n0.3151872604159556"}],"id":"n0.47592403312866116"}],"id":"n0.39645060429578693"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5919786388654495"}],"id":"n0.27736361760795636"}],"id":"n0.8097852380933599"}},"id":"n0.02702932545878034"},{"type":"single","text":"(","id":"n0.5606333216341286"},{"text":"s","id":"n0.2292691114706389"},{"type":"single","text":")","id":"n0.04269859187998892"}],"id":"n0.9283375581593811"}],"id":"n0.89449632340263"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5147011925460008"}],"style":{"align":"center"},"id":"n0.4152486386943557"}],"shape":{"data":{"p":{"x":15.006408691406207,"y":47.249469301363774},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8042430803808909":{"id":"de8042430803808909","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"R","id":"n0.5002283888487531"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7783614614964984"}],"id":"n0.297961339951891"}],"id":"n0.06678040051567691"}},"id":"n0.14844533386117065"}],"id":"n0.4081166751938259"}],"id":"n0.811386407261955"}},"id":"n0.3493723863456686"},{"type":"single","text":"(","id":"n0.46907936726833777"},{"text":"s","id":"n0.805370084609033"},{"id":"n0.12240558766567688","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6473433520604324","lines":[{"id":"n0.6655299740628118","blocks":[{"id":"n0.6759078268102778","text":"i"}]}]}}},{"text":",a","id":"n0.7948022804344625"},{"id":"n0.6913558726770317","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.39601115625214267","lines":[{"id":"n0.5983353018248478","blocks":[{"id":"n0.9802798100220826","text":"i"}]}]}}},{"type":"single","text":")","id":"n0.6212127400771796"}],"id":"n0.8011604082776529"}],"id":"n0.5585144594769098"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6409273035569256"}],"style":{"align":"center"},"id":"n0.5580434371713094"}],"shape":{"data":{"p":{"x":105.62584124487336,"y":234.71144772630112},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de23431970431903837":{"id":"de23431970431903837","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.1170102216432789"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K-1","id":"n0.2677685535824075"}],"id":"n0.2888280766334479"}],"id":"n0.10385750759248502"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.1512838805908041"}],"id":"n0.45970722336055814"}],"id":"n0.4227015986382636"}},"id":"n0.8477961955365088"},{"type":"single","text":"(","id":"n0.25677412994056237"},{"text":"s,a","id":"n0.9172064599053886"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4704409906674023"}],"id":"n0.7906745514798215"}],"id":"n0.21186906296159402"}},"id":"n0.38745424536614315"},{"type":"single","text":")","id":"n0.8400134290375487"}],"id":"n0.0860315124689226"}],"id":"n0.03458318572511776"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9650773898812901"}],"style":{"align":"center"},"id":"n0.3927604683534769"}],"shape":{"data":{"p":{"x":88.99999999999994,"y":28.307382940085972},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de9220101954817366":{"id":"de9220101954817366","lines":[{"blocks":[{"style":{"fontSize":"\\tiny"},"text":"max","id":"n0.5759991411766465"}],"id":"n0.17437563620620256"}],"shape":{"data":{"p":{"x":132.9161720677406,"y":43.48307625737806},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2451984776153353":{"id":"de2451984776153353","lines":[{"blocks":[{"text":"over ","style":{"fontSize":{"value":0.4}},"id":"n0.18585304985235784"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.35282676690819437"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.261625646233296"}],"id":"n0.8542118915203367"}],"id":"n0.9393992909034548"}},"id":"n0.6361202043302763"}],"id":"n0.9225802517691526"}],"id":"n0.6358514931961325"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.13620027133852997"}],"style":{"align":"center"},"id":"n0.5598413358017083"}],"shape":{"data":{"p":{"x":130.02611356688283,"y":57.07236067739149},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1899635654055294":{"id":"de1899635654055294","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"U","id":"n0.006068972938334527"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K-1","id":"n0.30327497430878814"}],"id":"n0.6266768437911552"}],"id":"n0.6259082828332134"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.05812691300451456"}],"id":"n0.5793854272311463"}],"id":"n0.6155248479809592"}},"id":"n0.1756386388594553"},{"type":"single","text":"(","id":"n0.6122476690348917"},{"text":"s","id":"n0.779005463770509"},{"type":"single","text":")","id":"n0.5228856643868618"}],"id":"n0.6037200504114792"}],"id":"n0.5587516503235763"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.19403745428148667"}],"style":{"align":"center"},"id":"n0.10508473415509534"}],"shape":{"data":{"p":{"x":173.0064086914062,"y":48.249469301363774},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de13873359332904545":{"id":"de13873359332904545","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.5747433247274787"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.8035317098087782"}],"id":"n0.6941594324020373"}],"id":"n0.5354791515466708"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.19124892957484718"}],"id":"n0.03189260206184197"}],"id":"n0.4123760353214514"}},"id":"n0.20407435975599109"},{"type":"single","text":"(","id":"n0.39395424899370446"},{"text":"s,a","id":"n0.9496317673458718"},{"type":"single","text":")","id":"n0.6571442186758487"}],"id":"n0.8042656885336161"}],"id":"n0.7264028620765699"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.06254498850303825"}],"style":{"align":"center"},"id":"n0.5971366396022255"}],"shape":{"data":{"p":{"x":434,"y":32.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8441154366127299":{"id":"de8441154366127299","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.146835922766952"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.4090732188892696"}],"id":"n0.31365306684005234"}],"id":"n0.40282909853865134"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.08719815994861824"}],"id":"n0.0908462187955954"}],"id":"n0.740663028209978"}},"id":"n0.11371273039382412"},{"type":"single","text":"(","id":"n0.6107997469772355"},{"text":"s,a","id":"n0.8706452099791198"},{"type":"single","text":")","id":"n0.688112252668329"}],"id":"n0.49246669600141635"}],"id":"n0.04583797116036181"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.003118688884779619"}],"style":{"align":"center"},"id":"n0.11301351693347028"}],"shape":{"data":{"p":{"x":627,"y":185.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de5537087275522437":{"id":"de5537087275522437","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"id":"n0.7694279464781144","text":"X"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.8126849532753888"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.9976485833903799"}],"id":"n0.20559309011582427"}],"id":"n0.15112809974544295"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.3556677777254764"}],"id":"n0.12221687328765296"}],"id":"n0.4633494985314448"}},"id":"n0.8614895912338203"}],"id":"n0.1361849523883183"}],"id":"n0.8873242276899993"}},"id":"n0.21849965246663694"},{"type":"single","text":"(","id":"n0.23386516712588956"},{"text":"s,a","id":"n0.31656162311839675"},{"type":"single","text":")","id":"n0.5296909722044236"}],"id":"n0.25330121363332925"}],"id":"n0.5175725534760129"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4369764114799277"}],"style":{"align":"center"},"id":"n0.13265684890715912"}],"shape":{"data":{"p":{"x":485.58166565657575,"y":105.83474321560152},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6990293149639712":{"id":"de6990293149639712","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1-","id":"n0.8220898377435071"},{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.03681549327761591"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.42292628840796764"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.6360884816366903"}],"id":"n0.6075766201412931"}],"id":"n0.1831481499402674"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.3255229490058702"}],"id":"n0.45556410972655126"}],"id":"n0.6017480792671808"}},"id":"n0.1374571125358317"}],"id":"n0.9273496428839458"}],"id":"n0.3620504825259647"}},"id":"n0.29790768148228053"}],"id":"n0.5159037234950323"}],"id":"n0.8764715381876009"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.2441893047384185"}],"style":{"align":"center"},"id":"n0.9480269161627728"}],"shape":{"data":{"p":{"x":545.5816656565758,"y":106.30738294008597},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8785973636687534":{"id":"de8785973636687534","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.9171824590138633"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.44672021196848055"}],"id":"n0.7818607430779412"}],"id":"n0.2424766441816495"}},"id":"n0.8387742053728955"},{"text":"|","id":"n0.02119829929289274"}],"id":"n0.19818936353891803"}],"id":"n0.10534765439253158"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.32943218763312565"}],"style":{"align":"center"},"id":"n0.507418967455411"}],"shape":{"data":{"p":{"x":-4,"y":2.983856201171875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de706628072537445":{"id":"de706628072537445","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.8759636294784048"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.22156309198850188"}],"id":"n0.866329597589272"}],"id":"n0.3327842032733004"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.01853059314001615"}],"id":"n0.41932018945465765"}],"id":"n0.36034326364212843"}},"id":"n0.608825440438538"},{"type":"single","text":"(","id":"n0.9080770702919103"},{"text":"s,a","id":"n0.19498244033844703"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5678821319862739"}],"id":"n0.9238863149011765"}],"id":"n0.5554338636934399"}},"id":"n0.49702652107349476"},{"type":"single","text":")","id":"n0.4577386658511726"}],"id":"n0.3821079040693218"}],"id":"n0.7324353081628885"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8702381870656417"}],"style":{"align":"center"},"id":"n0.5788367918750632"}],"shape":{"data":{"p":{"x":314.4011224293617,"y":33.68144817745889},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de3825894104169385":{"id":"de3825894104169385","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.028112752972151878"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.4472931034526244"}],"id":"n0.9460204965180818"}],"id":"n0.929472850259067"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.28759584258667403"}],"id":"n0.7787886247668507"}],"id":"n0.21699811384766154"}},"id":"n0.8602692990204304"},{"type":"single","text":"(","id":"n0.6777985648016569"},{"text":"s,a","id":"n0.2706690081177474"},{"type":"single","text":")","id":"n0.5167559890629587"}],"id":"n0.8353405095841582"}],"id":"n0.7820935964803029"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.023554338098733085"}],"style":{"align":"center"},"id":"n0.5130102994810564"}],"shape":{"data":{"p":{"x":325,"y":150.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de3664569806969358":{"id":"de3664569806969358","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"R","id":"n0.6926896140574603"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.17437436458251"}],"id":"n0.500450634251201"}],"id":"n0.5707162910337331"}},"id":"n0.8753640369280276"},{"type":"single","text":"(","id":"n0.3654602825647988"},{"text":"s,a","id":"n0.8464509719784241"},{"type":"single","text":")","id":"n0.21823688730695134"}],"id":"n0.8957631635704928"}],"id":"n0.43208464797421753"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8053380576443636"}],"style":{"align":"center"},"id":"n0.506790653356602"}],"shape":{"data":{"p":{"x":106.99999999999994,"y":149.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de6614622216116961":{"id":"de6614622216116961","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.4016781716870128"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.7877869983749566"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.5103569650418229"}],"id":"n0.10297667539010713"}],"id":"n0.24180552040286263"},"indexValue":{"lines":[{"blocks":[{"id":"n0.34845711097347976","text":"R"}],"id":"n0.41998310362694125"}],"id":"n0.645825499301385"}},"id":"n0.270161409778235"}],"id":"n0.8589650799408448"}],"id":"n0.4728382713070429"}},"id":"n0.07072152856983616"},{"type":"single","text":"(","id":"n0.5616600331440771"},{"text":"s,a","id":"n0.17714782829713904"},{"type":"single","text":")","id":"n0.022167164478694046"}],"id":"n0.16188097070730345"}],"id":"n0.2601044691611345"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.995238850418787"}],"style":{"align":"center"},"id":"n0.10232456325390626"}],"shape":{"data":{"p":{"x":267.58166565657575,"y":283.8347432156015},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6133498609024188":{"id":"de6133498609024188","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1-","id":"n0.7130969737888468"},{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.07721349329427385"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.35828667211669396"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.7749033135304042"}],"id":"n0.2482949363799123"}],"id":"n0.3471541028459606"},"indexValue":{"lines":[{"blocks":[{"id":"n0.5448587495264856","text":"R"}],"id":"n0.2807781437837287"}],"id":"n0.44844167584069505"}},"id":"n0.7952041490495199"}],"id":"n0.3574751371814284"}],"id":"n0.09241515757786978"}},"id":"n0.39464029862294425"}],"id":"n0.14935564515850985"}],"id":"n0.1395073386628325"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7253802699131924"}],"style":{"align":"center"},"id":"n0.9517478242664072"}],"shape":{"data":{"p":{"x":197.5816656565757,"y":285.8347432156015},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2819300277576777":{"id":"de2819300277576777","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"R","id":"n0.5080333992027091"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.05988815671987924"}],"id":"n0.8677746219753883"}],"id":"n0.3330801148958591"}},"id":"n0.04931305154863108"},{"type":"single","text":"(","id":"n0.7438265313295498"},{"text":"s,a","id":"n0.9416925031222689"},{"type":"single","text":")","id":"n0.27548838127387"}],"id":"n0.8304290040433637"}],"id":"n0.8840114401506087"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6375920278393064"}],"style":{"align":"center"},"id":"n0.9746471312645337"}],"shape":{"data":{"p":{"x":374.99999999999994,"y":234.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de9417082366336318":{"id":"de9417082366336318","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.03835443573157615"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.24142218287449624"}],"id":"n0.5162121360533385"}],"id":"n0.6195838386917736"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9092287203107567"}],"id":"n0.5174839387703523"}],"id":"n0.6673525200226891"}},"id":"n0.7347679435219794"},{"type":"single","text":"(","id":"n0.28843414602820805"},{"text":"s,a","id":"n0.6083528317729592"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6610000866890124"}],"id":"n0.8139612448440854"}],"id":"n0.5390876427499873"}},"id":"n0.23308836377708442"},{"type":"single","text":")","id":"n0.5120386048257137"}],"id":"n0.14721663159612897"}],"id":"n0.6997469764205988"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.2885185327931037"}],"style":{"align":"center"},"id":"n0.9110026451703763"}],"shape":{"data":{"p":{"x":616,"y":62.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de4462760249275344":{"id":"de4462760249275344","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.6097464845282279"}],"id":"n0.8832627046842543"}],"id":"n0.8247489543416093"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.2450296951090163"}],"id":"n0.2552966683935185"}],"shape":{"data":{"p":{"x":615.5171989578646,"y":131.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8948224066984556":{"id":"de8948224066984556","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.10857956305467842"}],"id":"n0.421574138797302"}],"id":"n0.7424021727233538"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6055471072451277"}],"id":"n0.7705004067186279"}],"shape":{"data":{"p":{"x":280.16577825936406,"y":232.6259652802052},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4331374139554627":{"id":"de4331374139554627","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.5027133070605017"}],"id":"n0.5355959891214823"}],"id":"n0.005551580701313341"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6075118873025613"}],"id":"n0.0914600554525753"}],"shape":{"data":{"p":{"x":253.5171989578646,"y":209.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de26192952769719957":{"id":"de26192952769719957","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.8888688572006751"}],"id":"n0.3267010850773666"}],"id":"n0.8041508784277376"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7720336149755831"}],"id":"n0.1346588330455778"}],"shape":{"data":{"p":{"x":487.5171989578646,"y":185.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6035267197891458":{"id":"de6035267197891458","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.6543152002270076"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7334742889692814"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.3242040524010321"}],"id":"n0.32644845688640456"}],"id":"n0.6312958751544981"}},"id":"n0.8409088613073215"}],"id":"n0.42302298582626086"}],"id":"n0.779041171275882"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.6188405926277076"}],"id":"n0.3493043981926587"}],"id":"n0.8508007860753459"}},"id":"n0.49707329322549"}],"id":"n0.6768200944743077"}],"id":"n0.976576704540332"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9023187988105708"}],"id":"n0.16337623688328828"}],"shape":{"data":{"p":{"x":9.99359130859375,"y":-3.4417227080760426}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de9760449880962501":{"id":"de9760449880962501","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.7644474351444859"}],"id":"n0.38534861850241797"}],"id":"n0.03316696426389476"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.35057284840972147"}],"id":"n0.5048663397251856"}],"shape":{"data":{"p":{"x":535.5171989578646,"y":43.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8954529408852401":{"id":"de8954529408852401","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.848393679454543"}],"id":"n0.25456691959311417"}],"id":"n0.8389529357060233"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8813460424744157"}],"id":"n0.5735294397612922"}],"shape":{"data":{"p":{"x":182.5171989578646,"y":232.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6584387665735523":{"id":"de6584387665735523","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.47807419727561884"}],"id":"n0.9207113995253955"}],"id":"n0.36444411269043075"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.27754890264373744"}],"id":"n0.9494594229882736"}],"shape":{"data":{"p":{"x":576.1657782593641,"y":185.6259652802052},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de012480490536642463":{"id":"de012480490536642463","lines":[{"blocks":[{"text":"Env of ","style":{"fontSize":"\\tiny"},"id":"n0.40909545976344974"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"i","id":"n0.35427989374640023"}],"id":"n0.6918224794336232"}],"id":"n0.6716473402196932"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.939569616596925"}],"style":{"align":"center"},"id":"n0.01145179328720447"}],"shape":{"data":{"p":{"x":0.0172119140625,"y":229.83665721496357},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de12292055506100197":{"id":"de12292055506100197","lines":[{"blocks":[{"text":"Envs","style":{"fontSize":"\\tiny"},"id":"n0.9459702196038209"}],"style":{"align":"center"},"id":"n0.7056217977509271"}],"shape":{"data":{"p":{"x":5.0172119140625,"y":146.83665721496357},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6435602377123977":{"id":"de6435602377123977","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.6970003767302986"}],"id":"n0.5950220408018525"}],"shape":{"data":{"p":{"x":42.0093994140625,"y":146},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9996999739406618":{"id":"de9996999739406618","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.5369596322341148"}],"id":"n0.26726632531312156"}],"shape":{"data":{"p":{"x":48.0093994140625,"y":230},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de45926917840285286":{"id":"de45926917840285286","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.33193660410626946"},{"id":"n0.05791779870879621","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.08047694735007327","lines":[{"id":"n0.7816226269678082","blocks":[{"id":"n0.2919634577615382","text":"i"}]}]}}},{"text":"|×|A","id":"n0.2065855154668208"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.02735575627040654","text":"i"}],"id":"n0.5841678693928647"}],"id":"n0.7970017989912566"}},"id":"n0.5110727722053909"},{"text":"|","id":"n0.27034545581103564"}],"id":"n0.8261875009076476"}],"id":"n0.5201323123537056"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4154985234933193"}],"style":{"align":"center"},"id":"n0.9504786860991157"}],"shape":{"data":{"p":{"x":90,"y":254.6290170380177},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9696621953343205":{"id":"de9696621953343205","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.9651143315377548"}],"id":"n0.638304223722447"}],"id":"n0.6627150763848109"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.733350121176997"}],"style":{"align":"center"},"id":"n0.037480843957762966"}],"shape":{"data":{"p":{"x":157.5752569651695,"y":328.3740652373729},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6152157786158032":{"id":"de6152157786158032","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.35880572400619837"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4362084347082764","text":"i"}],"id":"n0.2651270788247402"}],"id":"n0.5355411334500058"}},"id":"n0.2929620259609331"},{"text":"|","id":"n0.2764586619464937"}],"id":"n0.2801977747612696"}],"id":"n0.7073291188234092"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5683464147187822"}],"style":{"align":"center"},"id":"n0.3977797917887649"}],"shape":{"data":{"p":{"x":595,"y":113.41412353515625},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de37492081981477954":{"id":"de37492081981477954","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.06361873532402695"}],"id":"n0.794438943756369"}],"id":"n0.3742890977156048"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.29726610735971226"}],"style":{"align":"center"},"id":"n0.8524771677097138"}],"shape":{"data":{"p":{"x":231.5752569651695,"y":326.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de16483016651040594":{"id":"de16483016651040594","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.3307254272736544"}],"id":"n0.35570128805688106"}],"id":"n0.5843063118814504"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6800433846893965"}],"style":{"align":"center"},"id":"n0.1382199641670081"}],"shape":{"data":{"p":{"x":349.5752569651695,"y":286.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5858435209175927":{"id":"de5858435209175927","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.8630724159830749"}],"id":"n0.10997170062610095"}],"id":"n0.19884001565883946"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6946453596836426"}],"style":{"align":"center"},"id":"n0.5052580844707351"}],"shape":{"data":{"p":{"x":66.5752569651695,"y":191.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de739105016409006":{"id":"de739105016409006","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.8463427624385094"}],"id":"n0.8677445567741551"}],"id":"n0.9523563334968661"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5938522470819092"}],"style":{"align":"center"},"id":"n0.39782059849775453"}],"shape":{"data":{"p":{"x":593.5752569651695,"y":231.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de08038848791315778":{"id":"de08038848791315778","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.5637792325450797"}],"id":"n0.8153682870047718"}],"id":"n0.06429032264958878"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.12068162773028224"}],"style":{"align":"center"},"id":"n0.5359962618215615"}],"shape":{"data":{"p":{"x":469.5752569651695,"y":158.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de05131004919843152":{"id":"de05131004919843152","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.4601600173245559"}],"id":"n0.4702891312583537"}],"id":"n0.951802252792926"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.003195231366954765"}],"style":{"align":"center"},"id":"n0.9309387342842783"}],"shape":{"data":{"p":{"x":532.8988417911593,"y":158.83815680875063},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de540773596056596":{"id":"de540773596056596","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.2238645459187596"}],"id":"n0.272353911420099"}],"id":"n0.15126697453981852"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9917190814756962"}],"style":{"align":"center"},"id":"n0.7553146006612377"}],"shape":{"data":{"p":{"x":424.592468879232,"y":85.20226747242553},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9293029664421679":{"id":"de9293029664421679","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.3570916261199457"},{"id":"n0.12845562270225908","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.978783111912851","lines":[{"id":"n0.9922824075722854","blocks":[{"id":"n0.9781673696109443","text":"j"}]}]}}},{"text":"|","id":"n0.7968331349165683"}],"id":"n0.18387064331058434"}],"id":"n0.3497007107320673"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5747667428587113"}],"style":{"align":"center"},"id":"n0.19820451369007985"}],"shape":{"data":{"p":{"x":306.5752569651695,"y":85.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6039595436159426":{"id":"de6039595436159426","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.351398805520563"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.48442315345149445"}],"id":"n0.22172692899803725"}],"id":"n0.7109090021080886"}},"id":"n0.8245989377973624"},{"text":"|","id":"n0.9453516569619351"}],"id":"n0.8496850694621101"}],"id":"n0.4240221115956506"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9664372514825414"}],"style":{"align":"center"},"id":"n0.711141130846596"}],"shape":{"data":{"p":{"x":81,"y":80.41412353515625},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1822628181115682":{"id":"de1822628181115682","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.009072567688456878"}],"id":"n0.9987810547036093"}],"id":"n0.9056280993433128"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.10645997671208307"}],"style":{"align":"center"},"id":"n0.3764724270291231"}],"shape":{"data":{"p":{"x":157,"y":63.41412353515625},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de023526756442026064":{"id":"de023526756442026064","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.6169616174939561"}],"id":"n0.5542460624761409"}],"id":"n0.09762454449042579"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.09210366129022729"}],"style":{"align":"center"},"id":"n0.6764899055842895"}],"shape":{"data":{"p":{"x":-3.401122429361749,"y":64.14435383370333},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de018726185476633628":{"id":"de018726185476633628","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|×|S|","id":"n0.6493944792796353"}],"id":"n0.31216705932647026"}],"id":"n0.6077529724013804"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3531479305094207"}],"style":{"align":"center"},"id":"n0.60399643863951"}],"shape":{"data":{"p":{"x":146.08394629477812,"y":200.27918469789847},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6841190142781819":{"id":"de6841190142781819","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"T","id":"n0.7683100035109409"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.17581462020855665"}],"id":"n0.7885134808056073"}],"id":"n0.42320818106422853"}},"id":"n0.4859395402433364"},{"type":"single","text":"(","id":"n0.7342047706442416"},{"text":"s,a,s","id":"n0.9242146215609002"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"′","id":"n0.6976639139776573"}],"id":"n0.36649137880757676"}],"id":"n0.9077109131461794"}},"id":"n0.858637279194232"},{"type":"single","text":")","id":"n0.610314329815818"}],"id":"n0.9108959058111366"}],"id":"n0.8756710985439298"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.19642713448145832"}],"style":{"align":"center"},"id":"n0.5922218887012953"}],"shape":{"data":{"p":{"x":201.40112242936175,"y":149.27918469789847},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de04293699428649078":{"id":"de04293699428649078","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.6711516206867614"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.6293012772485833"}],"id":"n0.5099188220776707"}],"id":"n0.9515726342974276"}},"id":"n0.6397086361121886"}],"id":"n0.9016597190644242"}],"id":"n0.966922485547485"}},"id":"n0.7201687800889225"},{"type":"single","text":"(","id":"n0.19871584948867915"},{"text":"s","id":"n0.7082896529787819"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5336131573454217"}],"id":"n0.747649878480164"}],"id":"n0.906764969168768"}},"id":"n0.12002761346059354"},{"text":",a","id":"n0.46186803180346914"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.7591372230431157"}],"id":"n0.036654965525058314"}],"id":"n0.11558220844431832"}},"id":"n0.8274900593397492"},{"text":",s","id":"n0.33558272570819203"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.9182511567605076"}],"id":"n0.6823208742583062"}],"id":"n0.9715224083047242"},"powerValue":{"lines":[{"blocks":[{"text":"′","id":"n0.3099759867848324"}],"id":"n0.07252454170979417"}],"id":"n0.8433207561155169"}},"id":"n0.011563720551354795"},{"type":"single","text":")","id":"n0.14740387727406978"}],"id":"n0.364707453151766"}],"id":"n0.49009001515426154"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.1290575271160015"}],"style":{"align":"center"},"id":"n0.3646082883528139"}],"shape":{"data":{"p":{"x":236.610837007667,"y":90.439940578934},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de60646713842523":{"id":"de60646713842523","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.24591902022735268"}],"id":"n0.4565708745568702"}],"id":"n0.7236458004147461"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\scriptsize"},"id":"n0.5289197316272096"}],"id":"n0.29687791418063103"}],"shape":{"data":{"p":{"x":230.47431307477996,"y":61},"rotation":49.5},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de4411629295441355":{"id":"de4411629295441355","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.16870340820175111"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5279456732104058"}],"id":"n0.12907670911963076"}],"id":"n0.7822700061057228"}},"id":"n0.9377404542125218"}],"id":"n0.6706446933400576"}],"id":"n0.5656938308129515"}},"id":"n0.8013307877816385"},{"type":"single","text":"(","id":"n0.985266238712871"},{"text":"s","id":"n0.8271638019349599"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.06183936664223566"}],"id":"n0.13660785462172242"}],"id":"n0.12229695282215336"}},"id":"n0.6613803536952751"},{"text":",a","id":"n0.6015032396773592"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.46374276792931335"}],"id":"n0.7886303216702921"}],"id":"n0.5157308854738447"}},"id":"n0.22909248342684418"},{"text":",s","id":"n0.06235965186953618"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6566980955979471"}],"id":"n0.40280214465327213"}],"id":"n0.40557309953903786"},"powerValue":{"lines":[{"blocks":[{"text":"′","id":"n0.1289725219965525"}],"id":"n0.9746657310057514"}],"id":"n0.44363044936039064"}},"id":"n0.21824669956570997"},{"type":"single","text":")","id":"n0.07911624592295463"}],"id":"n0.09034195018334379"}],"id":"n0.37394730600376547"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.10719803903126146"}],"style":{"align":"center"},"id":"n0.034145748460466585"}],"shape":{"data":{"p":{"x":372.610837007667,"y":110.439940578934},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7010281499379019":{"id":"de7010281499379019","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.06144083114826682"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.596816246871475"}],"id":"n0.19270499103072902"}],"id":"n0.8765824185576179"}},"id":"n0.8940663977104886"},{"text":"|×|A","id":"n0.4445514206699219"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3255236756072324"}],"id":"n0.5545628363138091"}],"id":"n0.9438628177208579"}},"id":"n0.607005841235837"},{"text":"|×|S","id":"n0.7903939639174105"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.0903889441191188"}],"id":"n0.3812769088406949"}],"id":"n0.3831188775016634"}},"id":"n0.601211045335968"},{"text":"|","id":"n0.7474402100335875"}],"id":"n0.8416491680664595"}],"id":"n0.9767225469188732"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7795950076246325"}],"style":{"align":"center"},"id":"n0.38039104499447296"}],"shape":{"data":{"p":{"x":356.9753875732422,"y":129.96709218025205},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de04664323127911296":{"id":"de04664323127911296","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.49813709848875276"}],"id":"n0.9006780350873496"}],"id":"n0.08373904856088688"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\scriptsize"},"id":"n0.37196203298005615"}],"id":"n0.3491212219072135"}],"shape":{"data":{"p":{"x":366.47431307477996,"y":81},"rotation":49.5},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de16198272348575138":{"id":"de16198272348575138","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.5636079506241669"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.15201140972725113"}],"id":"n0.46390307381875373"}],"id":"n0.3033384222360125"}},"id":"n0.9640682618822976"},{"text":"|×|A","id":"n0.06376856138854725"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.4422875989040669"}],"id":"n0.2998811529747065"}],"id":"n0.9577409964156021"}},"id":"n0.25467665850738963"},{"text":"|×|S","id":"n0.8145614275243673"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8770746409066634"}],"id":"n0.39414625675950643"}],"id":"n0.8650993523594279"}},"id":"n0.8556409230193665"},{"text":"|","id":"n0.3813771503877965"}],"id":"n0.08228083687322618"}],"id":"n0.5587680319929698"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.06469661490070111"}],"style":{"align":"center"},"id":"n0.529015195049134"}],"shape":{"data":{"p":{"x":182.9753875732422,"y":93.96709218025205},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1255655849801256":{"id":"de1255655849801256","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.5775081849637576"}],"id":"n0.21811485831728739"}],"id":"n0.7666737289493661"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.24860653849838377"}],"id":"n0.4062273037250861"}],"shape":{"data":{"p":{"x":246.5171989578646,"y":44.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9161591960896418":{"id":"de9161591960896418","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.6318104962220974"}],"id":"n0.5925370726888699"}],"id":"n0.9498508894605631"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6701633702433445"}],"id":"n0.11559847239060783"}],"shape":{"data":{"p":{"x":242.5171989578646,"y":154.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8296046118428881":{"id":"de8296046118428881","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.6398689401106215"}],"id":"n0.4033876395448901"}],"id":"n0.28320581281574864"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.4349597993383858"}],"id":"n0.9448347503743157"}],"shape":{"data":{"p":{"x":274.398973109876,"y":154.85714149475098},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9797287230713403":{"id":"de9797287230713403","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.9505870200032105"}],"id":"n0.5894585729573776"}],"id":"n0.7671618023231281"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.31054545845421266"}],"id":"n0.5076526454333599"}],"shape":{"data":{"p":{"x":278.398973109876,"y":44.85714149475098},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de5739134075838137":{"id":"de5739134075838137","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.3944069710959337"}],"id":"n0.19451179227559212"}],"id":"n0.4663649957506413"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.10051684038523878"}],"id":"n0.9672525642765821"}],"shape":{"data":{"p":{"x":385.398973109876,"y":44.85714149475098},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de03130277592898212":{"id":"de03130277592898212","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.5534333454181448"}],"id":"n0.3072371727743546"}],"id":"n0.631865547408381"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.1458376395512646"}],"id":"n0.17811759237737768"}],"shape":{"data":{"p":{"x":352.5171989578646,"y":44.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6378018078330772":{"id":"de6378018078330772","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.7208760412987405"}],"id":"n0.2624712398833211"}],"shape":{"data":{"p":{"x":42.0093994140625,"y":86},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8481258525974809":{"id":"de8481258525974809","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.4863560218411527"}],"id":"n0.9159159238454151"}],"shape":{"data":{"p":{"x":42.0093994140625,"y":109},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8476603362025159":{"id":"de8476603362025159","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.4501116586327565"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.17091706834106257"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.025782905093796105"}],"id":"n0.4042546801411979"}],"id":"n0.022720621996522583"}},"id":"n0.22476328518358057"}],"id":"n0.3055198623290718"}],"id":"n0.4989652670930218"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6324025007844765"}],"style":{"align":"center"},"id":"n0.24964510519829197"}],"shape":{"data":{"p":{"x":273.6132065083135,"y":56.495030879974365},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8143133125744644":{"id":"de8143133125744644","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.9086075456708929"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.8370412454432139"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7703327140987262"}],"id":"n0.5389871057488758"}],"id":"n0.7381776497761259"}},"id":"n0.33824744641281645"}],"id":"n0.5481934605797949"}],"id":"n0.8829924132636315"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.36829213278754924"}],"style":{"align":"center"},"id":"n0.6450954768629698"}],"shape":{"data":{"p":{"x":381.6132065083135,"y":56.96521918264051},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3476499031597826":{"id":"de3476499031597826","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.30390839200015485"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.729990596735663"}],"id":"n0.7424364242976345"}],"id":"n0.6780372454725427"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.15414247250504576"}],"style":{"align":"center"},"id":"n0.7413564731553903"}],"shape":{"data":{"p":{"x":269.6132065083135,"y":167.49503087997437},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5306365077124713":{"id":"de5306365077124713","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"optionally dependent","id":"n0.8993394473941201"}],"id":"n0.7761974801344702"}],"shape":{"data":{"p":{"x":-6.990600585937493,"y":145.48763757301705},"rotation":270},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di12183456471916898","items":[],"style":{}},"shapes":[{"id":"dp5580500491360401","type":"doc-cube","data":{"p1":{"x":413.89243309975313,"y":45.5022752722482},"p2":{"x":451.9827880859375,"y":83.21222204612354},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp7412593590357124","type":"doc-cube","data":{"p1":{"x":413.89243309975313,"y":13.199859619140625},"p2":{"x":451.9827880859375,"y":50.90980639301608},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"da19200039013523407","data":[{"x":40.01719895786459,"y":57.34437565321065},{"x":51.206092622831534,"y":57.34437565321065}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp0239657809852718","type":"doc-cube","data":{"p1":{"x":1.5988775706382512,"y":37.84193818059583},"p2":{"x":39.68923255682262,"y":75.55188495447129},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp7194803427767733","type":"doc-cube","data":{"p1":{"x":83.17413453580775,"y":51.42721209483358},"p2":{"x":121.26448952199212,"y":89.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp8282129066226385","type":"doc-cube","data":{"p1":{"x":83.17413453580775,"y":19.42721209483358},"p2":{"x":121.26448952199212,"y":57.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da853407251837732","data":[{"x":121.26448952199212,"y":57.13715886870904},{"x":133.1304054661781,"y":57.13715886870904}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da8231681129714354","data":[{"x":152.66612152300183,"y":56.729627747941095},{"x":163.74979117488306,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp2827788892463312","type":"circle","data":{"p1":{"x":133.1304054661781,"y":47.30450264897962},"p2":{"x":152.66612152300183,"y":66.84021870580335}}},{"id":"dp532548436215186","type":"doc-cube","data":{"p1":{"x":163.59887757063825,"y":38.84193818059583},"p2":{"x":201.68923255682262,"y":76.55188495447129},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da308102308085787","data":[{"x":202.0093994140625,"y":56.729627747941095},{"x":248.7314323563021,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da6021732396444412","data":[{"x":297.14892256513724,"y":56.729627747941095},{"x":306.7314323563021,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4489210612652541","data":[{"x":404.14892256513724,"y":56.215249700218635},{"x":414.60827698470075,"y":56.215249700218635}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp5238821890873124","type":"doc-cube","data":{"p1":{"x":424.592468879232,"y":55.89985181931803},"p2":{"x":462.68282386541637,"y":93.60979859319349},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp7110419585223715","type":"doc-cube","data":{"p1":{"x":424.592468879232,"y":23.89985181931803},"p2":{"x":462.68282386541637,"y":61.60979859319349},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dg9204957316369451","entities":[{"id":"dp10499838332590139","type":"circle","data":{"p1":{"x":575.3800116578016,"y":188.44739167180677},"p2":{"x":594.9157277146253,"y":207.9831077286305}}},{"id":"dl1391479758821974","linkedId":"de6584387665735523"}]},{"id":"da2979160721047991","data":[{"x":509.2671484131258,"y":198.21524970021864},{"x":575.3800116578016,"y":198.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da27089434828529035","data":[{"x":585.1478696862134,"y":55.96521918264051},{"x":585.1478696862134,"y":188.44739167180677}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp6621931347037233","type":"doc-cube","data":{"p1":{"x":606.9096450138156,"y":198.12821003487528},"p2":{"x":645,"y":235.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp5776503678584604","type":"doc-cube","data":{"p1":{"x":606.9096450138156,"y":165.8257943817677},"p2":{"x":645,"y":203.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp22224605199990788","type":"doc-cube","data":{"p1":{"x":617.592468879232,"y":208.89985181931803},"p2":{"x":655.6828238654164,"y":246.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp8386984456762969","type":"doc-cube","data":{"p1":{"x":617.592468879232,"y":176.89985181931803},"p2":{"x":655.6828238654164,"y":214.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp5226002240201779","type":"doc-cube","data":{"p1":{"x":467.4913106703914,"y":119.12821003487528},"p2":{"x":505.58166565657575,"y":156.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp3137025663850519","type":"doc-cube","data":{"p1":{"x":467.4913106703914,"y":86.82579438176771},"p2":{"x":505.58166565657575,"y":124.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp6642259953317995","type":"doc-cube","data":{"p1":{"x":478.17413453580775,"y":129.42721209483358},"p2":{"x":516.2644895219921,"y":167.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp41047603791401865","type":"doc-cube","data":{"p1":{"x":478.17413453580775,"y":97.42721209483358},"p2":{"x":516.2644895219921,"y":135.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp2404545538889784","type":"doc-cube","data":{"p1":{"x":525.4913106703914,"y":119.12821003487528},"p2":{"x":563.5816656565758,"y":156.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp6064438594718595","type":"doc-cube","data":{"p1":{"x":525.4913106703914,"y":86.82579438176771},"p2":{"x":563.5816656565758,"y":124.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp5149951155315287","type":"doc-cube","data":{"p1":{"x":536.1741345358078,"y":129.89985181931803},"p2":{"x":574.2644895219921,"y":167.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp3108225276141863","type":"doc-cube","data":{"p1":{"x":536.1741345358078,"y":97.89985181931803},"p2":{"x":574.2644895219921,"y":135.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dg15563367846213083","entities":[{"id":"dp21043865271157292","type":"circle","data":{"p1":{"x":184.7314323563021,"y":235.19736115422864},"p2":{"x":204.26714841312582,"y":254.73307721105238}}},{"id":"dl12406206773144723","linkedId":"de8954529408852401"}]},{"id":"da5150116280603851","data":[{"x":462.60827698470075,"y":56.215249700218635},{"x":537.7314323563021,"y":56.215249700218635}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg954465914639369","entities":[{"id":"dp12510303758397479","type":"circle","data":{"p1":{"x":537.7314323563021,"y":46.197361154228645},"p2":{"x":557.2671484131258,"y":65.73307721105238}}},{"id":"dl6457629730029077","linkedId":"de9760449880962501"}]},{"id":"da6958538552085018","data":[{"x":547.499290384714,"y":65.73307721105238},{"x":547.499290384714,"y":86.21600341796875}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da7778825022864237","data":[{"x":404.0093994140625,"y":245.21524970021864},{"x":585.1478696862134,"y":245.21524970021864}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg41545057312416156","entities":[{"id":"dg8271149987198114","entities":[{"id":"dp31161403196624216","type":"rectangle","data":{"p1":{"x":8.99359130859375,"y":1.5402473973582005},"p2":{"x":21.650752040652606,"y":14.197408129417056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp6085656917177373","type":"rectangle","data":{"p1":{"x":10.57573640010105,"y":3.1223924888655574},"p2":{"x":23.232897132159906,"y":15.779553220924413}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp41813287093409257","type":"rectangle","data":{"p1":{"x":12.157881491608464,"y":4.704537580372914},"p2":{"x":24.81504222366732,"y":17.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl8322524008366461","linkedId":"de6035267197891458"}]},{"id":"dp942503727628808","type":"doc-cube","data":{"p1":{"x":306.5752569651695,"y":56.801277332206496},"p2":{"x":344.66561195135387,"y":94.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp8281586097067699","type":"doc-cube","data":{"p1":{"x":306.5752569651695,"y":24.801277332206496},"p2":{"x":344.66561195135387,"y":62.511224106081954},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da03822030711492408","data":[{"x":345.2671484131258,"y":56.96521918264051},{"x":355.0093994140625,"y":56.96521918264051}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da059191563599135355","data":[{"x":70.0093994140625,"y":57.13715886870904},{"x":83.0093994140625,"y":57.13715886870904}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da13306965166562712","data":[{"x":557.2671484131258,"y":55.96521918264051},{"x":585.1478696862134,"y":55.96521918264051}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg7539883759791381","entities":[{"id":"dp7497877315179022","type":"circle","data":{"p1":{"x":489.7314323563021,"y":188.19736115422864},"p2":{"x":509.2671484131258,"y":207.73307721105238}}},{"id":"dl6687676709899761","linkedId":"de26192952769719957"}]},{"id":"da9415792104793081","data":[{"x":499.49929038471396,"y":167.31321716308594},{"x":499.49929038471396,"y":189.19736115422864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp38660432328521854","type":"doc-cube","data":{"p1":{"x":304.89243309975313,"y":163.5022752722482},"p2":{"x":342.9827880859375,"y":201.21222204612354},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp7338164304551018","type":"doc-cube","data":{"p1":{"x":304.89243309975313,"y":131.19985961914062},"p2":{"x":342.9827880859375,"y":168.90980639301608},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp39348646886366523","type":"doc-cube","data":{"p1":{"x":315.592468879232,"y":173.89985181931803},"p2":{"x":353.68282386541637,"y":211.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp590233598124545","type":"doc-cube","data":{"p1":{"x":315.592468879232,"y":141.89985181931803},"p2":{"x":353.68282386541637,"y":179.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da05971979951523476","data":[{"x":293.14892256513724,"y":166.5022752722482},{"x":304.89243309975313,"y":166.5022752722482}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da42104124445416335","data":[{"x":375.0093994140625,"y":197.9652191826405},{"x":489.7314323563021,"y":197.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da8186217197536731","data":[{"x":354.0093994140625,"y":166.5022752722482},{"x":375.0093994140625,"y":166.5022752722482}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da05615183153668801","data":[{"x":375.0093994140625,"y":166.5022752722482},{"x":375.0093994140625,"y":197.9652191826405}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da673169699290058","data":[{"x":29.563405007743967,"y":160.9336164882478},{"x":41.42493473559304,"y":160.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da5645555795798565","data":[{"x":29.563405007743967,"y":244.9336164882478},{"x":46.42493473559304,"y":244.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da8738004703581135","data":[{"x":82.42493473559304,"y":244.9336164882478},{"x":99.0093994140625,"y":244.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da10460833736657693","data":[{"x":76.42493473559304,"y":160.9336164882478},{"x":87.0093994140625,"y":160.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"dp7869297321934083","type":"doc-cube","data":{"p1":{"x":85.90964501381563,"y":161.12821003487528},"p2":{"x":124,"y":198.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp13484715726844398","type":"doc-cube","data":{"p1":{"x":85.90964501381563,"y":128.8257943817677},"p2":{"x":124,"y":166.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp12477969564605385","type":"doc-cube","data":{"p1":{"x":96.592468879232,"y":171.89985181931803},"p2":{"x":134.68282386541637,"y":209.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp7903226572786035","type":"doc-cube","data":{"p1":{"x":96.592468879232,"y":139.89985181931803},"p2":{"x":134.68282386541637,"y":177.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp031755431326810024","type":"doc-cube","data":{"p1":{"x":176.49131067039139,"y":298.1282100348753},"p2":{"x":214.58166565657575,"y":335.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp3584813595344112","type":"doc-cube","data":{"p1":{"x":176.49131067039139,"y":265.8257943817677},"p2":{"x":214.58166565657575,"y":303.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp007099428310750833","type":"doc-cube","data":{"p1":{"x":187.17413453580775,"y":308.4272120948336},"p2":{"x":225.26448952199212,"y":346.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp22821526251270785","type":"doc-cube","data":{"p1":{"x":187.17413453580775,"y":276.4272120948336},"p2":{"x":225.26448952199212,"y":314.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp7185805497173068","type":"doc-cube","data":{"p1":{"x":249.49131067039139,"y":296.1282100348753},"p2":{"x":287.58166565657575,"y":333.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp018846218146621796","type":"doc-cube","data":{"p1":{"x":249.49131067039139,"y":263.8257943817677},"p2":{"x":287.58166565657575,"y":301.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp5690368574792177","type":"doc-cube","data":{"p1":{"x":260.17413453580775,"y":306.89985181931803},"p2":{"x":298.2644895219921,"y":344.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp38381778786212895","type":"doc-cube","data":{"p1":{"x":260.17413453580775,"y":274.89985181931803},"p2":{"x":298.2644895219921,"y":312.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da5658381447269285","data":[{"x":135.0093994140625,"y":244.9652191826405},{"x":184.7314323563021,"y":244.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da9995455804626399","data":[{"x":194.49929038471396,"y":254.73307721105238},{"x":194.49929038471396,"y":264.94285583496094}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da8640106553630609","data":[{"x":120.0093994140625,"y":209.5022752722482},{"x":120.0093994140625,"y":221.94285583496094}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da18632054957436273","data":[{"x":120.0093994140625,"y":221.94285583496094},{"x":255.7314323563021,"y":221.94285583496094}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"dg8055008932284284","entities":[{"id":"dp03367387182029269","type":"circle","data":{"p1":{"x":255.7314323563021,"y":212.19736115422864},"p2":{"x":275.2671484131258,"y":231.73307721105238}}},{"id":"dl20198523491621545","linkedId":"de4331374139554627"}]},{"id":"da8012264691401934","data":[{"x":265.49929038471396,"y":231.73307721105238},{"x":265.49929038471396,"y":264.21600341796875}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da7835806906210396","data":[{"x":204.26714841312582,"y":244.9652191826405},{"x":279.0093994140625,"y":244.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg7875487562730157","entities":[{"id":"dp578508923349293","type":"circle","data":{"p1":{"x":279.38001165780156,"y":235.44739167180677},"p2":{"x":298.9157277146253,"y":254.9831077286305}}},{"id":"dl1612850971509283","linkedId":"de8948224066984556"}]},{"id":"da9579582551601642","data":[{"x":289.1478696862134,"y":221.9652191826405},{"x":289.1478696862134,"y":235.44739167180677}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da59415295926599","data":[{"x":275.2671484131258,"y":221.9652191826405},{"x":289.1478696862134,"y":221.9652191826405}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp8939365025742361","type":"doc-cube","data":{"p1":{"x":354.90964501381563,"y":246.12821003487528},"p2":{"x":393,"y":283.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp048707061335577784","type":"doc-cube","data":{"p1":{"x":354.90964501381563,"y":213.8257943817677},"p2":{"x":393,"y":251.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp23688862660102084","type":"doc-cube","data":{"p1":{"x":365.592468879232,"y":256.89985181931803},"p2":{"x":403.68282386541637,"y":294.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp23160303178682695","type":"doc-cube","data":{"p1":{"x":365.592468879232,"y":224.89985181931803},"p2":{"x":403.68282386541637,"y":262.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da3866850608376675","data":[{"x":585.1478696862134,"y":207.9831077286305},{"x":585.1478696862134,"y":245.21524970021864}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da9337052957580414","data":[{"x":594.9157277146253,"y":198.21524970021864},{"x":606.9096450138156,"y":198.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp0349412583949118","type":"doc-cube","data":{"p1":{"x":608.1741345358078,"y":85.42721209483358},"p2":{"x":646.2644895219921,"y":123.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp9379059187709777","type":"doc-cube","data":{"p1":{"x":608.1741345358078,"y":53.42721209483358},"p2":{"x":646.2644895219921,"y":91.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da5343953893264877","data":[{"x":60.49929038471396,"y":8.21600341796875},{"x":60.49929038471396,"y":52.197361154228645}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9677469206122253","data":[{"x":24.81504222366732,"y":8.704537580372914},{"x":597.0093994140625,"y":8.704537580372914}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg6752644909371888","entities":[{"id":"dp43033051061531813","type":"circle","data":{"p1":{"x":617.7314323563021,"y":134.19736115422864},"p2":{"x":637.2671484131258,"y":153.73307721105238}}},{"id":"dl377456144583618","linkedId":"de4462760249275344"}]},{"id":"da17224206150215826","data":[{"x":627.499290384714,"y":153.73307721105238},{"x":627.499290384714,"y":165.94285583496094}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da9982300639182866","data":[{"x":627.499290384714,"y":123.21600341796875},{"x":627.499290384714,"y":134.19736115422864}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da7416010416599621","data":[{"x":597.0093994140625,"y":143.9652191826405},{"x":617.7314323563021,"y":143.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9022639564636132","data":[{"x":597.0093994140625,"y":8.704537580372914},{"x":597.0093994140625,"y":143.9652191826405}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp6501577681335067","type":"rectangle","data":{"p1":{"x":1.5361824061229754,"y":228.57503948597804},"p2":{"x":30.858642252069075,"y":257.8974993319241}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp6877052913645814","type":"rectangle","data":{"p1":{"x":1.5361824061229754,"y":145.57503948597804},"p2":{"x":30.858642252069075,"y":174.8974993319241}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"da4090530237206933","data":[{"x":16.49929038471396,"y":174.31321716308594},{"x":16.49929038471396,"y":228.21600341796875}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg6734392125901896","entities":[{"id":"dp2789239062719051","type":"rectangle","data":{"p1":{"x":48.0093994140625,"y":143},"p2":{"x":69.0093994140625,"y":178},"rotation":90}},{"id":"dl3628216806984257","linkedId":"de6435602377123977"}]},{"id":"dg22534662588403087","entities":[{"id":"dp13538335494399356","type":"rectangle","data":{"p1":{"x":54.0093994140625,"y":227},"p2":{"x":75.0093994140625,"y":262},"rotation":90}},{"id":"dl755351049022529","linkedId":"de9996999739406618"}]},{"id":"dg24449934841418952","entities":[{"id":"dp15533761819139724","type":"rectangle","data":{"p1":{"x":99.54648398243944,"y":227.63370702366495},"p2":{"x":128.9300421516284,"y":257.00945182101134}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp4643139166564427","type":"rectangle","data":{"p1":{"x":102.58616261365637,"y":230.67257737498306},"p2":{"x":131.96972078284546,"y":260.04832217232934}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp49163915811603554","type":"rectangle","data":{"p1":{"x":105.62584124487336,"y":233.71144772630112},"p2":{"x":135.0093994140625,"y":263.08719252364745}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{}},{"id":"da7872979366862605","data":[{"x":298.9157277146253,"y":245.21524970021864},{"x":354.0093994140625,"y":245.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp09732505074373066","type":"doc-cube","data":{"p1":{"x":184.31076744317738,"y":161.10001179268778},"p2":{"x":222.40112242936175,"y":198.80995856656313},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp18274731608286587","type":"doc-cube","data":{"p1":{"x":184.31076744317738,"y":128.7975961395802},"p2":{"x":222.40112242936175,"y":166.50754291345567},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp12130929956941183","type":"doc-cube","data":{"p1":{"x":194.99359130859375,"y":171.87165357713053},"p2":{"x":233.08394629477812,"y":209.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp028256799555335776","type":"doc-cube","data":{"p1":{"x":194.99359130859375,"y":139.87165357713053},"p2":{"x":233.08394629477812,"y":177.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5171751511814839","type":"doc-cube","data":{"p1":{"x":152.20960923433677,"y":161.10001179268778},"p2":{"x":190.29996422052113,"y":198.80995856656313},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp5608329832553007","type":"doc-cube","data":{"p1":{"x":152.20960923433677,"y":128.7975961395802},"p2":{"x":190.29996422052113,"y":166.50754291345567},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp7156234666550425","type":"doc-cube","data":{"p1":{"x":162.89243309975313,"y":171.87165357713053},"p2":{"x":200.9827880859375,"y":209.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp15378440916480773","type":"doc-cube","data":{"p1":{"x":162.89243309975313,"y":139.87165357713053},"p2":{"x":200.9827880859375,"y":177.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dg08929290825571146","entities":[{"id":"dp8942136593530361","type":"rectangle","data":{"p1":{"x":215.81933178116822,"y":67.40107022761589},"p2":{"x":247.89927876415908,"y":96.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp7590754257443322","type":"rectangle","data":{"p1":{"x":219.13794720457258,"y":70.439940578934},"p2":{"x":251.21789418756362,"y":99.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp6292476093797723","type":"rectangle","data":{"p1":{"x":222.456562627977,"y":73.47881093025205},"p2":{"x":254.5365096109681,"y":102.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"dg7711569844652904","entities":[{"id":"dp4908467651489763","type":"rectangle","data":{"p1":{"x":233.29222158426262,"y":83.40107022761589},"p2":{"x":266.20073998648286,"y":112.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp798959070951937","type":"rectangle","data":{"p1":{"x":236.69655129805233,"y":86.439940578934},"p2":{"x":269.6050697002727,"y":115.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp02317091301376495","type":"rectangle","data":{"p1":{"x":240.10088101184203,"y":89.47881093025205},"p2":{"x":273.0093994140625,"y":118.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{}},{"id":"dg19964813928951308","entities":[{"id":"dp034934788017860985","type":"rectangle","data":{"p1":{"x":351.8193317811682,"y":87.40107022761589},"p2":{"x":383.89927876415913,"y":116.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp900240286070412","type":"rectangle","data":{"p1":{"x":355.1379472045726,"y":90.439940578934},"p2":{"x":387.2178941875636,"y":119.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp3947392159799368","type":"rectangle","data":{"p1":{"x":358.45656262797706,"y":93.47881093025205},"p2":{"x":390.5365096109681,"y":122.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"dg19029399184522622","entities":[{"id":"dp4240042237526809","type":"rectangle","data":{"p1":{"x":369.2922215842626,"y":103.40107022761589},"p2":{"x":402.20073998648286,"y":132.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp24142162592296623","type":"rectangle","data":{"p1":{"x":372.6965512980523,"y":106.439940578934},"p2":{"x":405.6050697002727,"y":135.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp5443187775637572","type":"rectangle","data":{"p1":{"x":376.10088101184203,"y":109.47881093025205},"p2":{"x":409.0093994140625,"y":138.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{}},{"id":"da637809167456008","data":[{"x":258.49929038471396,"y":66.73307721105238},{"x":258.49929038471396,"y":83.21600341796875}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"dg006391677294819154","entities":[{"id":"dp7771922235587243","type":"circle","data":{"p1":{"x":248.7314323563021,"y":47.197361154228645},"p2":{"x":268.2671484131258,"y":66.73307721105238}}},{"id":"dl389019327591694","linkedId":"de1255655849801256"}]},{"id":"da5209013767862236","data":[{"x":16.49929038471396,"y":100.77681502496227},{"x":16.49929038471396,"y":145.31321716308594}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da7917530330246885","data":[{"x":76.0093994140625,"y":100.77681502496227},{"x":217.81933178116822,"y":100.77681502496227}],"head":"fh>","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da38135419526097825","data":[{"x":76.0093994140625,"y":122.77681502496227},{"x":358.45656262797706,"y":122.77681502496227}],"head":"fh>","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da09903958236513599","data":[{"x":183.4779265063455,"y":76.24041288683861},{"x":183.4779265063455,"y":117.21600341796875}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4673472459214669","data":[{"x":183.4779265063455,"y":117.21600341796875},{"x":236.0093994140625,"y":117.21600341796875}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da3357191226606715","data":[{"x":236.0093994140625,"y":117.21600341796875},{"x":236.0093994140625,"y":137.21600341796875}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da7674599403021374","data":[{"x":236.0093994140625,"y":137.21600341796875},{"x":254.49929038471396,"y":137.21600341796875}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg3111258413323337","entities":[{"id":"dp527895228022196","type":"circle","data":{"p1":{"x":244.7314323563021,"y":157.19736115422864},"p2":{"x":264.2671484131258,"y":176.73307721105238}}},{"id":"dl34043414874577427","linkedId":"de9161591960896418"}]},{"id":"dg6145165827194954","entities":[{"id":"dp261344319135447","type":"circle","data":{"p1":{"x":273.6132065083135,"y":156.67856788635257},"p2":{"x":293.14892256513724,"y":176.2142839431763}}},{"id":"dl21460496321325784","linkedId":"de8296046118428881"}],"data":{"rotation":0}},{"id":"da6657225238385869","data":[{"x":232.9879218216862,"y":166.9652191826405},{"x":244.7314323563021,"y":166.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da36307604254714243","data":[{"x":264.2671484131258,"y":166.9652191826405},{"x":273.6132065083135,"y":166.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da07983334347477489","data":[{"x":254.49929038471396,"y":137.21600341796875},{"x":254.49929038471396,"y":157.19736115422864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da2811500562982141","data":[{"x":140.49929038471396,"y":122.77681502496227},{"x":140.49929038471396,"y":167.31321716308594}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da35308780946559915","data":[{"x":140.49929038471396,"y":167.31321716308594},{"x":152.0093994140625,"y":167.31321716308594}],"head":"fh>","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"dg6474901284015173","entities":[{"id":"dp23763267875478333","type":"circle","data":{"p1":{"x":277.6132065083135,"y":46.67856788635257},"p2":{"x":297.14892256513724,"y":66.2142839431763}}},{"id":"dl023538663551297745","linkedId":"de9797287230713403"}],"data":{"rotation":0}},{"id":"da38022140950114736","data":[{"x":268.2671484131258,"y":56.96521918264051},{"x":277.6132065083135,"y":56.96521918264051}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg27597926385049165","entities":[{"id":"dp10151926770216746","type":"circle","data":{"p1":{"x":354.7314323563021,"y":47.197361154228645},"p2":{"x":374.2671484131258,"y":66.73307721105238}}},{"id":"dl7669813038971061","linkedId":"de03130277592898212"}]},{"id":"dg5771720689263735","entities":[{"id":"dp3859604845475457","type":"circle","data":{"p1":{"x":384.6132065083135,"y":46.67856788635257},"p2":{"x":404.14892256513724,"y":66.2142839431763}}},{"id":"dl6079264183911899","linkedId":"de5739134075838137"}],"data":{"rotation":0}},{"id":"da3886363031679785","data":[{"x":374.2671484131258,"y":56.96521918264051},{"x":384.6132065083135,"y":56.96521918264051}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg12964984834139792","entities":[{"id":"dp5857498755316624","type":"rectangle","data":{"p1":{"x":48.0093994140625,"y":83},"p2":{"x":69.0093994140625,"y":118},"rotation":90}},{"id":"dl7825586801032587","linkedId":"de6378018078330772"}]},{"id":"dg8834776660883104","entities":[{"id":"dp3330655612344646","type":"rectangle","data":{"p1":{"x":48.0093994140625,"y":106},"p2":{"x":69.0093994140625,"y":141},"rotation":90}},{"id":"dl4102774702186407","linkedId":"de8481258525974809"}]},{"id":"da8265208003206985","data":[{"x":16.49929038471396,"y":100.77681502496227},{"x":41.0093994140625,"y":100.77681502496227}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da60878731726692","data":[{"x":16.49929038471396,"y":122.77681502496227},{"x":41.0093994140625,"y":122.77681502496227}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6,"style":{"thickness":2}},{"id":"da034831188233359844","data":[{"x":364.49929038471396,"y":66.73307721105238},{"x":364.49929038471396,"y":87.21600341796875}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6,"style":{"thickness":2}}],"settings":{"grid":true,"diagramHeight":347.94146728515625}}]},{"id":"n0.3042139671924857","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":1347,"delayRenderCache":{"av":1347,"map":{"n0.10534765439253158":{"n0.19818936353891803":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.5201323123537056":{"n0.8261875009076476":{"w":28.1756,"h":8.4545,"bl":0.8214}},"n0.6627150763848109":{"n0.638304223722447":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.7073291188234092":{"n0.2801977747612696":{"w":26.2496,"h":8.4545,"bl":0.8214}},"n0.3742890977156048":{"n0.794438943756369":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.5843063118814504":{"n0.35570128805688106":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.19884001565883946":{"n0.10997170062610095":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.9523563334968661":{"n0.8677445567741551":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.89449632340263":{"n0.9283375581593811":{"w":15.625,"h":9.1146,"bl":0.7619}},"n0.5585144594769098":{"n0.8011604082776529":{"w":24.2151,"h":9.4491,"bl":0.8402}},"n0.03458318572511776":{"n0.0860315124689226":{"w":29.6766,"h":9.1146,"bl":0.7619}},"n0.6358514931961325":{"n0.9225802517691526":{"w":7.0349,"h":8.4545,"bl":0.8214}},"n0.5587516503235763":{"n0.6037200504114792":{"w":21.6743,"h":9.1146,"bl":0.7619}},"n0.7264028620765699":{"n0.8042656885336161":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.04583797116036181":{"n0.49246669600141635":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.5175725534760129":{"n0.25330121363332925":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.8764715381876009":{"n0.5159037234950323":{"w":20.7972,"h":9.9736,"bl":0.6963}},"n0.7324353081628885":{"n0.3821079040693218":{"w":24.6672,"h":9.1146,"bl":0.7619}},"n0.7820935964803029":{"n0.8353405095841582":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.43208464797421753":{"n0.8957631635704928":{"w":19.694,"h":8.4545,"bl":0.8214}},"n0.2601044691611345":{"n0.16188097070730345":{"w":23.9981,"h":9.9736,"bl":0.6963}},"n0.1395073386628325":{"n0.14935564515850985":{"w":20.9871,"h":9.9736,"bl":0.6963}},"n0.8840114401506087":{"n0.8304290040433637":{"w":19.694,"h":8.4545,"bl":0.8214}},"n0.6997469764205988":{"n0.14721663159612897":{"w":24.4231,"h":9.1146,"bl":0.7619}},"n0.976576704540332":{"n0.6768200944743077":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.06429032264958878":{"n0.8153682870047718":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.951802252792926":{"n0.4702891312583537":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.15126697453981852":{"n0.272353911420099":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.3497007107320673":{"n0.18387064331058434":{"w":26.4938,"h":8.4545,"bl":0.8214}},"n0.4240221115956506":{"n0.8496850694621101":{"w":26.2496,"h":8.4545,"bl":0.8214}},"n0.8756710985439298":{"n0.9108959058111366":{"w":28.9804,"h":11.348,"bl":0.6717}},"n0.9767225469188732":{"n0.8416491680664595":{"w":45.2293,"h":8.4545,"bl":0.8214}},"n0.5587680319929698":{"n0.08228083687322618":{"w":45.9617,"h":8.4545,"bl":0.8214}},"n0.49009001515426154":{"n0.364707453151766":{"w":34.2972,"h":12.6682,"bl":0.6267}},"n0.37394730600376547":{"n0.09034195018334379":{"w":33.5015,"h":12.6682,"bl":0.6267}},"n0.6077529724013804":{"n0.31216705932647026":{"w":39.4513,"h":8.1019,"bl":0.8571}},"n0.4989652670930218":{"n0.3055198623290718":{"w":5.9498,"h":8.4545,"bl":0.8214}},"n0.8829924132636315":{"n0.5481934605797949":{"w":5.7057,"h":8.4545,"bl":0.8214}}}}}

==> sIPOMDPLite-Net(arXiv)/plots/docs/59fdd8c4-a9f1-485d-b49e-4c7bfbd03d27 <==
{"id":"n0.7456383844689902","lines":[{"id":"n0.8763064465791919","blocks":[]},{"id":"n0.44711846644901","blocks":[{"id":"n0.9288385843406479","text":"\\diagram","type":"composite","elements":{"de7404139643581418":{"id":"de7404139643581418","lines":[{"blocks":[{"text":"Value iteration solver","style":{"fontSize":"\\tiny"},"id":"n0.19770521534247454"}],"style":{"align":"center"},"id":"n0.0030156944848367395"}],"shape":{"data":{"p":{"x":234.49359130859375,"y":16.635022970635077},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de949941888849803":{"id":"de949941888849803","lines":[{"blocks":[{"text":"Value iteration solver","style":{"fontSize":"\\tiny"},"id":"n0.4593913524176294"}],"style":{"align":"center"},"id":"n0.443496815967684"}],"shape":{"data":{"p":{"x":234.49359130859375,"y":104.63502297063508},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de32130721406148366":{"id":"de32130721406148366","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.8797025232152835"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"L-2,K","id":"n0.7574525922899173"}],"id":"n0.6792864006937782"}],"id":"n0.4871679788236192"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3983774231491659"}],"id":"n0.17604683573999136"}],"id":"n0.7520448645232582"}},"id":"n0.6169344591193611"},{"type":"single","text":"(","id":"n0.247693808610445"},{"text":"s,a","id":"n0.4968446333492895"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6906023085940054"}],"id":"n0.33010937497493464"}],"id":"n0.1641173131260556"}},"id":"n0.7238556114449535"},{"type":"single","text":")","id":"n0.982544451005702"}],"id":"n0.8091899817257213"}],"id":"n0.49121514402082456"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.22186047312577228"}],"style":{"align":"center"},"id":"n0.797204439117494"}],"shape":{"data":{"p":{"x":332.4011224293617,"y":97.72752972042764},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de9910374172859537":{"id":"de9910374172859537","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.005737793719555517"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8383320490845296"}],"id":"n0.7977828385970613"}],"id":"n0.8416031365428731"}},"id":"n0.8044300209222583"},{"text":"|","id":"n0.30338364897354686"}],"id":"n0.6479673560913659"}],"id":"n0.878034595656866"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.009638223477540953"}],"style":{"align":"center"},"id":"n0.04633807084968611"}],"shape":{"data":{"p":{"x":298.99359130859375,"y":141.42014678034167},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9448075050931994":{"id":"de9448075050931994","lines":[{"blocks":[{"text":"Softmax","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.3881871005493689"}],"style":{"align":"center"},"id":"n0.9932399499088576"}],"shape":{"data":{"p":{"x":399.9827880859375,"y":105.47110766449265},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7963858066415856":{"id":"de7963858066415856","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.3905984278663106"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"L-1,K","id":"n0.7986457472156983"}],"id":"n0.5996773595196319"}],"id":"n0.5085266219885212"},"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.3863209742516749"}],"id":"n0.6152400257446515"}],"id":"n0.0400742394500917"}},"id":"n0.5473655481704303"},{"type":"single","text":"(","id":"n0.19500742768663515"},{"text":"s,a","id":"n0.21247214621856103"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.7358306889430006"}],"id":"n0.5656120957983657"}],"id":"n0.9216699336648997"}},"id":"n0.8566877677939349"},{"type":"single","text":")","id":"n0.15889176983574416"}],"id":"n0.624454071858985"}],"id":"n0.5762378149466976"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5245830463600181"}],"style":{"align":"center"},"id":"n0.0717754399241497"}],"shape":{"data":{"p":{"x":332.4011224293617,"y":9.72752972042764},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de030313905425286558":{"id":"de030313905425286558","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.2240811407333707"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.0676601920612836"}],"id":"n0.13277312603126212"}],"id":"n0.7545877627634885"}},"id":"n0.04813229485411008"},{"text":"|","id":"n0.5427307784547795"}],"id":"n0.564695130185312"}],"id":"n0.7620427428820304"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6477223589534982"}],"style":{"align":"center"},"id":"n0.42293417942939726"}],"shape":{"data":{"p":{"x":298.99359130859375,"y":53.42014678034167},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5663753911346638":{"id":"de5663753911346638","lines":[{"blocks":[{"text":"Softmax","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.6609290096212981"}],"style":{"align":"center"},"id":"n0.3977909836140512"}],"shape":{"data":{"p":{"x":399.9827880859375,"y":17.47110766449265},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de0550914994150582":{"id":"de0550914994150582","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.5140039025205387"}],"id":"n0.3709058944946262"}],"id":"n0.47706945579402205"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9035451130987506"}],"id":"n0.38722324292532817"}],"shape":{"data":{"p":{"x":285.5,"y":174.54608154296875},"rotation":90},"anchor":"left-top"},"isTextMode":true},"de9740250816234686":{"id":"de9740250816234686","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.4016400439397185"}],"id":"n0.3934814190940734"}],"id":"n0.5457109854785729"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7604199860398932"}],"id":"n0.5009673578426002"}],"shape":{"data":{"p":{"x":363.5,"y":174.54608154296875},"rotation":90},"anchor":"left-top"},"isTextMode":true},"de9385566531380667":{"id":"de9385566531380667","lines":[{"blocks":[{"text":"Value iteration solver","style":{"fontSize":"\\tiny"},"id":"n0.7217592392524406"}],"style":{"align":"center"},"id":"n0.7213343873567817"}],"shape":{"data":{"p":{"x":235.49359130859375,"y":242.63502297063508},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9230782278135958":{"id":"de9230782278135958","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.1380841457076989"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"0,K","id":"n0.5116599012581777"}],"id":"n0.07456673727038288"}],"id":"n0.742823387835992"},"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5193821290096721"}],"id":"n0.04841632932536677"}],"id":"n0.9650646770652205"}},"id":"n0.9039984150883122"},{"type":"single","text":"(","id":"n0.8842144191413104"},{"text":"s,a","id":"n0.822359185523424"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.05419841640105538"}],"id":"n0.4594820213704369"}],"id":"n0.5705112118491114"}},"id":"n0.6090589366914465"},{"type":"single","text":")","id":"n0.26344848149904343"}],"id":"n0.16312157425304696"}],"id":"n0.5421621652642399"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.11454114241444535"}],"style":{"align":"center"},"id":"n0.034864380703128584"}],"shape":{"data":{"p":{"x":335.4011224293617,"y":235.72752972042764},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de13776807857324536":{"id":"de13776807857324536","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.9813758713228182"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.25818223492049186"}],"id":"n0.08476983469556298"}],"id":"n0.5732016289079991"}},"id":"n0.7340773131771539"},{"text":"|","id":"n0.7212270463159804"}],"id":"n0.4521066476362081"}],"id":"n0.021551824456943036"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7877763209738127"}],"style":{"align":"center"},"id":"n0.047020047972589296"}],"shape":{"data":{"p":{"x":300.99359130859375,"y":279.42014678034167},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9826326892666628":{"id":"de9826326892666628","lines":[{"blocks":[{"text":"Softmax","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.3123466420650318"}],"style":{"align":"center"},"id":"n0.8430356477283305"}],"shape":{"data":{"p":{"x":397.9827880859375,"y":243.47110766449265},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6123916227603201":{"id":"de6123916227603201","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.7284304063632188"}],"id":"n0.9893739898342253"}],"id":"n0.09492127571336417"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6928984319873144"}],"id":"n0.16728586144452362"}],"shape":{"data":{"p":{"x":434.5,"y":174.54608154296875},"rotation":90},"anchor":"left-top"},"isTextMode":true},"de39438104803862406":{"id":"de39438104803862406","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\hat","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"𝜋","id":"n0.7586939751845192"}],"id":"n0.8019077953128695"}],"id":"n0.16274775883676695"}},"id":"n0.6354860275022087"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4097985681310048"}],"id":"n0.5576389802155606"}],"id":"n0.46948006831709677"},"powerValue":{"lines":[{"blocks":[{"text":"0","id":"n0.3771778972134905"}],"id":"n0.3491918701529553"}],"id":"n0.6804177236712141"}},"id":"n0.8564787329672008"},{"type":"single","text":"(","id":"n0.07632820792608874"},{"text":"s,a","id":"n0.37648471103085024"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.775601513941599"}],"id":"n0.40374530105673934"}],"id":"n0.12508214063133827"}},"id":"n0.2606369486644555"},{"type":"single","text":")","id":"n0.8835602704953642"}],"id":"n0.43201992570641323"}],"id":"n0.6639940912465938"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.016141386358724086"}],"style":{"align":"center"},"id":"n0.6607706569816483"}],"shape":{"data":{"p":{"x":460,"y":279.6975843468925},"rotation":0},"anchor":"left-top","style":{"fillColor":[80,227,194,1]}},"isTextMode":true,"isInGroup":false},"de2579719695378768":{"id":"de2579719695378768","lines":[{"blocks":[{"text":"Level ","style":{"fontSize":"\\tiny"},"id":"n0.3632367527785749"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"L-1","id":"n0.20846838892596553"}],"id":"n0.5835614246651424"}],"id":"n0.4508209020473879"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.6120189070802013"}],"style":{"align":"center"},"id":"n0.8349679808894037"}],"shape":{"data":{"p":{"x":182.49359130859375,"y":17.635022970635077},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6314113770356831":{"id":"de6314113770356831","lines":[{"blocks":[{"text":"Level ","style":{"fontSize":"\\tiny"},"id":"n0.21504016787584845"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"L-2","id":"n0.21266299444689585"}],"id":"n0.6814644698850401"}],"id":"n0.20834096396169643"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.09669984625424677"}],"style":{"align":"center"},"id":"n0.9433971486576183"}],"shape":{"data":{"p":{"x":183,"y":105.63502297063508},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de19675038100118147":{"id":"de19675038100118147","lines":[{"blocks":[{"text":"Level ","style":{"fontSize":"\\tiny"},"id":"n0.4665094201284141"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"0","id":"n0.4041203922664638"}],"id":"n0.35536501373177276"}],"id":"n0.542136158452516"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.7350935049092755"}],"style":{"align":"center"},"id":"n0.018888212550350003"}],"shape":{"data":{"p":{"x":183,"y":241.63502297063508},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3793798924569056":{"id":"de3793798924569056","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.8934204249110584"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.8340023940541792","text":"i"}],"id":"n0.990519759646665"}],"id":"n0.6266561818284284"}},"id":"n0.7459659549277033"},{"text":"|","id":"n0.02530197623617303"}],"id":"n0.6296807647435203"}],"id":"n0.8814959856119453"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6089052983923968"}],"style":{"align":"center"},"id":"n0.3309086780043087"}],"shape":{"data":{"p":{"x":402,"y":306.4255789092479},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de02539145642801577":{"id":"de02539145642801577","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.056371739255644204"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.13174007075183192"}],"id":"n0.248403283253676"}],"id":"n0.3661469535821704"}},"id":"n0.9569596830675164"},{"text":"|","id":"n0.2533120784434968"}],"id":"n0.593332307309044"}],"id":"n0.3838513742554275"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.18568227913067625"}],"style":{"align":"center"},"id":"n0.06428877903424657"}],"shape":{"data":{"p":{"x":402,"y":253.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de05168791060859412":{"id":"de05168791060859412","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.6582585624233113"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.788965801871945"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.12614605121514644","text":"i"}],"id":"n0.021324803176446805"}],"id":"n0.10482432157327626"}},"id":"n0.04797838599969828"}],"id":"n0.8901422202213247"}],"id":"n0.8788180716067089"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.3044316332222887"}],"id":"n0.6868342941933696"}],"id":"n0.25994957128260676"}},"id":"n0.8499402048082008"}],"id":"n0.47796249916056044"}],"id":"n0.6748794387292034"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.14765023594948823"}],"id":"n0.4677300447181276"}],"shape":{"data":{"p":{"x":414.99359130859375,"y":296}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de33489281180821995":{"id":"de33489281180821995","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.09407891212168473"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.34600370469723996"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.22683942594424145"}],"id":"n0.010431547090191229"}],"id":"n0.1709610314528911"}},"id":"n0.9697516612181147"}],"id":"n0.37307691542753463"}],"id":"n0.15252746660662364"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.63917899335727"}],"id":"n0.6436412748391367"}],"id":"n0.1347447194698812"}},"id":"n0.3152914544875969"}],"id":"n0.772350973034134"}],"id":"n0.20568306821556503"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4577189107404238"}],"id":"n0.5423432343479035"}],"shape":{"data":{"p":{"x":414.99359130859375,"y":243.55827729192396}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de599100908346867":{"id":"de599100908346867","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.4866774580992028"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9967038337399736"}],"id":"n0.8694528209142025"}],"id":"n0.7855968366770971"}},"id":"n0.6221054991623272"},{"text":"|","id":"n0.23801682853525774"}],"id":"n0.9293510086231909"}],"id":"n0.34935182724472136"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5628668240365013"}],"style":{"align":"center"},"id":"n0.7885752919089821"}],"shape":{"data":{"p":{"x":402,"y":114.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7808512405889996":{"id":"de7808512405889996","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.7362026767584469"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.8163758712340334"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8725591332626943"}],"id":"n0.892491453782452"}],"id":"n0.11958147842711542"}},"id":"n0.8848331183670357"}],"id":"n0.6007899845556632"}],"id":"n0.6118672296885168"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.7993776462627542"}],"id":"n0.025512495977708438"}],"id":"n0.5357554047434483"}},"id":"n0.9984456052965838"}],"id":"n0.6102202981030778"}],"id":"n0.7990525584386923"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6148671870434375"}],"id":"n0.6565569611219635"}],"shape":{"data":{"p":{"x":414.99359130859375,"y":104.55827729192396}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de6183527944901863":{"id":"de6183527944901863","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.6147068921960703"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7066805573624653"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4942985658276202"}],"id":"n0.7086286483486222"}],"id":"n0.17496155535778413"}},"id":"n0.3122931531715807"}],"id":"n0.9201585131605319"}],"id":"n0.07909149458138565"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.19903607225869724"}],"id":"n0.67779796803327"}],"id":"n0.680415402902476"}},"id":"n0.4640400734380665"}],"id":"n0.8325561577006042"}],"id":"n0.6833550991018396"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.960391229975732"}],"id":"n0.3488295089348885"}],"shape":{"data":{"p":{"x":414.99359130859375,"y":17.558277291923957}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de10775284719956923":{"id":"de10775284719956923","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.25871157002202505"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9276959523680952","text":"j"}],"id":"n0.9479672303757438"}],"id":"n0.26069607650483806"}},"id":"n0.906468976536928"},{"text":"|","id":"n0.6566745052972824"}],"id":"n0.6389208899453975"}],"id":"n0.37277273316714243"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4332897151220161"}],"style":{"align":"center"},"id":"n0.06291855946151559"}],"shape":{"data":{"p":{"x":404.08829782270914,"y":28.1858628361133},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di41729058265448593","items":[],"style":{}},"shapes":[{"id":"dp47833610138437277","type":"doc-rounded-rect","data":{"p1":{"x":229.3642310148602,"y":17.810200449549598},"p2":{"x":312.91291638898514,"y":41.7005827509488},"rotation":0},"style":{"fillColor":[140,200,240,1]}},{"id":"dp7252990734982117","type":"doc-rounded-rect","data":{"p1":{"x":229.3642310148602,"y":105.8102004495496},"p2":{"x":312.91291638898514,"y":129.7005827509488},"rotation":0},"style":{"fillColor":[140,200,240,1]}},{"id":"dp5238403623954342","type":"doc-cube","data":{"p1":{"x":326.5752569651695,"y":120.84735887517525},"p2":{"x":369.92608642578125,"y":158.5573056490507},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp3426937152560734","type":"doc-cube","data":{"p1":{"x":326.5752569651695,"y":88.84735887517525},"p2":{"x":369.92608642578125,"y":126.5573056490507},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da3764417224670913","data":[{"x":313.0093994140625,"y":118.1858628361133},{"x":325.93050100541586,"y":118.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9225803741722312","data":[{"x":370.93050100541586,"y":118.1858628361133},{"x":382.0093994140625,"y":118.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp8261396135456109","type":"rectangle","data":{"p1":{"x":382.54710037167024,"y":94.04608154296875},"p2":{"x":390.1573101697012,"y":141.04608154296875}}},{"id":"da06700100677924525","data":[{"x":391.0093994140625,"y":118.1858628361133},{"x":413.08829782270914,"y":118.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp8553147868712787","type":"doc-cube","data":{"p1":{"x":326.5752569651695,"y":32.847358875175246},"p2":{"x":369.92608642578125,"y":70.5573056490507},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp2137631360458554","type":"doc-cube","data":{"p1":{"x":326.5752569651695,"y":0.8473588751752459},"p2":{"x":369.92608642578125,"y":38.557305649050704},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da15943921980254028","data":[{"x":313.0672439523636,"y":30.1858628361133},{"x":325.93050100541586,"y":30.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da8049389990280313","data":[{"x":369.93050100541586,"y":30.1858628361133},{"x":383.0093994140625,"y":30.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp8184268731954947","type":"rectangle","data":{"p1":{"x":382.54710037167024,"y":6.04608154296875},"p2":{"x":390.1573101697012,"y":53.04608154296875}}},{"id":"da45763509473825215","data":[{"x":390.0093994140625,"y":30.1858628361133},{"x":412.08829782270914,"y":30.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da23976988799793553","data":[{"x":271.9004128140757,"y":82.1858628361133},{"x":420.0093994140625,"y":82.1858628361133}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9389736317801487","data":[{"x":420.0093994140625,"y":109.5402473973582},{"x":420.0093994140625,"y":82.1858628361133}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp7423675029202152","type":"doc-rounded-rect","data":{"p1":{"x":230.3642310148602,"y":243.8102004495496},"p2":{"x":313.91291638898514,"y":267.7005827509488},"rotation":0},"style":{"fillColor":[140,200,240,1]}},{"id":"da9790415098060559","data":[{"x":272.9004128140757,"y":308.1858628361133},{"x":272.9004128140757,"y":268.14283514022827}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp7435646245202219","type":"doc-cube","data":{"p1":{"x":328.5752569651695,"y":258.84735887517525},"p2":{"x":366.66561195135387,"y":296.5573056490507},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp08033017088121319","type":"doc-cube","data":{"p1":{"x":328.5752569651695,"y":226.84735887517525},"p2":{"x":366.66561195135387,"y":264.5573056490507},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da8713163721465647","data":[{"x":314.0672439523636,"y":256.1858628361133},{"x":327.93050100541586,"y":256.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da2411252945849418","data":[{"x":366.93050100541586,"y":256.1858628361133},{"x":381.0093994140625,"y":256.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp9011794347447228","type":"rectangle","data":{"p1":{"x":380.54710037167024,"y":232.04608154296875},"p2":{"x":388.1573101697012,"y":279.04608154296875}}},{"id":"da20364951303761303","data":[{"x":388.0093994140625,"y":256.1858628361133},{"x":412.99359130859375,"y":256.1858628361133}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9481886775137895","data":[{"x":273.9004128140757,"y":219.02993774414062},{"x":273.9004128140757,"y":204.1324462890625}],"head":"fh>","tail":"no","shaft":"--","middle":"no","headScale":0.6},{"id":"da16940211400592764","data":[{"x":273.9004128140757,"y":219.02993774414062},{"x":421.0093994140625,"y":219.02993774414062}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6},{"id":"da3473100070999804","data":[{"x":421.0093994140625,"y":248.5402473973582},{"x":421.0093994140625,"y":219.1858628361133}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6},{"id":"dp12319438729391963","type":"right-arrow","data":{"p1":{"x":436.68282386541637,"y":24.471092435162753},"p2":{"x":449.68282386541637,"y":36.97583639268228},"arrowPercentage":0.4}},{"id":"dp7125078369975848","type":"doc-cube","data":{"p1":{"x":453.592468879232,"y":303.29005322612454},"p2":{"x":491.68282386541637,"y":341},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp9152516441590235","type":"doc-cube","data":{"p1":{"x":453.592468879232,"y":271.29005322612454},"p2":{"x":491.68282386541637,"y":309},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da909845752930831","data":[{"x":272.9004128140757,"y":176.1324462890625},{"x":420.0093994140625,"y":176.1324462890625}],"head":"no","tail":"no","shaft":"--","middle":"no","headScale":0.6},{"id":"da09205056674657586","data":[{"x":271.9004128140757,"y":82.1858628361133},{"x":271.9004128140757,"y":41.15322399139404}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da44421738044179104","data":[{"x":272.9004128140757,"y":176.1324462890625},{"x":272.9004128140757,"y":130.15322399139404}],"head":"fh>","tail":"no","shaft":"--","middle":"no","headScale":0.6},{"id":"da9378807022106552","data":[{"x":272.9004128140757,"y":308.1858628361133},{"x":413.0093994140625,"y":308.1858628361133}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg5752425887968442","entities":[{"id":"dg8348766324290573","entities":[{"id":"dp9208284147887935","type":"rectangle","data":{"p1":{"x":412.99359130859375,"y":300.98197010543424},"p2":{"x":425.6507520406526,"y":313.6391308374931}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp008477122704914297","type":"rectangle","data":{"p1":{"x":414.57573640010105,"y":302.5641151969416},"p2":{"x":427.2328971321599,"y":315.22127592900046}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp3642009145930136","type":"rectangle","data":{"p1":{"x":416.15788149160846,"y":304.14626028844896},"p2":{"x":428.8150422236673,"y":316.8034210205078}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl04460893008583788","linkedId":"de05168791060859412"}]},{"id":"da7912672485721097","data":[{"x":428.99359130859375,"y":308.1858628361133},{"x":453.0093994140625,"y":308.1858628361133}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"dg9035236793094654","entities":[{"id":"dg5023454242459575","entities":[{"id":"dp4101738498195575","type":"rectangle","data":{"p1":{"x":412.99359130859375,"y":248.5402473973582},"p2":{"x":425.6507520406526,"y":261.19740812941706}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp5331236483757704","type":"rectangle","data":{"p1":{"x":414.57573640010105,"y":250.12239248886556},"p2":{"x":427.2328971321599,"y":262.7795532209244}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp9471391528134872","type":"rectangle","data":{"p1":{"x":416.15788149160846,"y":251.70453758037291},"p2":{"x":428.8150422236673,"y":264.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl2659154614400385","linkedId":"de33489281180821995"}]},{"id":"dg45923819168090696","entities":[{"id":"dg390100338337527","entities":[{"id":"dp6129333426434289","type":"rectangle","data":{"p1":{"x":412.99359130859375,"y":109.5402473973582},"p2":{"x":425.6507520406526,"y":122.19740812941706}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp32210977992707734","type":"rectangle","data":{"p1":{"x":414.57573640010105,"y":111.12239248886556},"p2":{"x":427.2328971321599,"y":123.77955322092441}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp7088279109032376","type":"rectangle","data":{"p1":{"x":416.15788149160846,"y":112.70453758037291},"p2":{"x":428.8150422236673,"y":125.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl8128743428252136","linkedId":"de7808512405889996"}]},{"id":"dg8422714549228933","entities":[{"id":"dg8749080403551495","entities":[{"id":"dp04357528838072988","type":"rectangle","data":{"p1":{"x":412.99359130859375,"y":22.5402473973582},"p2":{"x":425.6507520406526,"y":35.197408129417056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp7977411862931905","type":"rectangle","data":{"p1":{"x":414.57573640010105,"y":24.122392488865557},"p2":{"x":427.2328971321599,"y":36.77955322092441}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp013304563458476082","type":"rectangle","data":{"p1":{"x":416.15788149160846,"y":25.704537580372914},"p2":{"x":428.8150422236673,"y":38.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl4309794460639673","linkedId":"de6183527944901863"}]},{"id":"dp10615464469127711","type":"right-arrow","data":{"p1":{"x":436.68282386541637,"y":111.97583639268228},"p2":{"x":449.68282386541637,"y":124.48058035020182},"arrowPercentage":0.4}},{"id":"dp11234244974403396","type":"right-arrow","data":{"p1":{"x":436.68282386541637,"y":250.48058035020182},"p2":{"x":449.68282386541637,"y":262.9853243077214},"arrowPercentage":0.4}}],"settings":{"grid":true,"diagramHeight":341.9701232910156}}]},{"id":"n0.5773724414561772","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":1699,"delayRenderCache":{"av":1699,"map":{"n0.878034595656866":{"n0.6479673560913659":{"w":26.2496,"h":8.4545,"bl":0.8214}},"n0.7620427428820304":{"n0.564695130185312":{"w":26.4938,"h":8.4545,"bl":0.8214}},"n0.021551824456943036":{"n0.4521066476362081":{"w":26.4938,"h":8.4545,"bl":0.8214}},"n0.49121514402082456":{"n0.8091899817257213":{"w":33.5015,"h":9.1146,"bl":0.7619}},"n0.5762378149466976":{"n0.624454071858985":{"w":33.7457,"h":9.1146,"bl":0.7619}},"n0.5421621652642399":{"n0.16312157425304696":{"w":28.2208,"h":9.1146,"bl":0.7619}},"n0.6639940912465938":{"n0.43201992570641323":{"w":28.465,"h":15.4984,"bl":0.7264}},"n0.8814959856119453":{"n0.6296807647435203":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.3838513742554275":{"n0.593332307309044":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.6748794387292034":{"n0.47796249916056044":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.34935182724472136":{"n0.9293510086231909":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.7990525584386923":{"n0.6102202981030778":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.6833550991018396":{"n0.8325561577006042":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.37277273316714243":{"n0.6389208899453975":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.20568306821556503":{"n0.772350973034134":{"w":7.4599,"h":9.6481,"bl":0.7198}}}}}

==> sIPOMDPLite-Net(arXiv)/plots/docs/5ff3344f-e3ef-49c3-9fc8-e6006ee92bde <==
{"id":"n0.9735571899555475","lines":[{"id":"n0.09626705958257009","blocks":[]},{"id":"n0.2918628718558065","blocks":[{"id":"n0.37860086508951385","text":"\\diagram","type":"composite","elements":{"de0634562876505389":{"id":"de0634562876505389","lines":[{"blocks":[{"text":"Value iteration solver","style":{"fontSize":"\\tiny"},"id":"n0.2393113020621569"}],"style":{"align":"center"},"id":"n0.7036002702805659"}],"shape":{"data":{"p":{"x":190,"y":39.248550073937906},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7452464315882257":{"id":"de7452464315882257","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.8293342112764326"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6364811329040743"}],"id":"n0.09795120049062156"}],"id":"n0.328815333454892"}},"id":"n0.6905435550237693"},{"text":"|","id":"n0.6451205917090073"}],"id":"n0.1154698172732449"}],"id":"n0.4639640815729844"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9594496036142959"}],"style":{"align":"center"},"id":"n0.3990772838906833"}],"shape":{"data":{"p":{"x":281.5752569651695,"y":83.90358032942736},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de30539217550006503":{"id":"de30539217550006503","lines":[{"blocks":[{"text":"Softmax","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.5380915526612213"}],"style":{"align":"center"},"id":"n0.9635321019519416"}],"shape":{"data":{"p":{"x":443.48919677734375,"y":12.084634767795478},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6158175282739142":{"id":"de6158175282739142","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.6454358308840946"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"L,K","id":"n0.7684800122204358"}],"id":"n0.7190303345779496"}],"id":"n0.5721805846990413"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5245745158244517"}],"id":"n0.7086308650615849"}],"id":"n0.283793262999148"}},"id":"n0.172266758285198"},{"type":"single","text":"(","id":"n0.9033436097145575"},{"text":"s,a","id":"n0.10996256372674273"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8067534064680955"}],"id":"n0.30546746033830807"}],"id":"n0.779788527208449"}},"id":"n0.18425677171769483"},{"type":"single","text":")","id":"n0.1760959765402652"}],"id":"n0.1781866772261569"}],"id":"n0.45802729846083956"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6479475484287407"}],"style":{"align":"center"},"id":"n0.34957141144569714"}],"shape":{"data":{"p":{"x":287.4011224293617,"y":31.481335521572248},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7578803692968976":{"id":"de7578803692968976","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.6735115506100067"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8910240050030935"}],"id":"n0.492933483487094"}],"id":"n0.5543595260820138"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.025605870710162293"}],"id":"n0.2899697062197255"}],"id":"n0.250689808273159"}},"id":"n0.35261412989877283"},{"type":"single","text":"(","id":"n0.8513162358432065"},{"text":"s","id":"n0.040384118441435746"},{"type":"single","text":")","id":"n0.616977251271351"}],"id":"n0.5361220979168753"}],"id":"n0.16920259577024832"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.32636677561643945"}],"style":{"align":"center"},"id":"n0.09078805888162278"}],"shape":{"data":{"p":{"x":333.9827880859375,"y":86.934645988932},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6802701882630025":{"id":"de6802701882630025","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.1346456291087723"}],"id":"n0.04427435903979493"}],"id":"n0.24530697980996785"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.05328824754854278"}],"style":{"align":"center"},"id":"n0.4266733370356186"}],"shape":{"data":{"p":{"x":316.5752569651695,"y":100.82953052127158},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de45675243102562924":{"id":"de45675243102562924","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.8342108437915399"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.5616116446250121"}],"id":"n0.28707750677524335"}],"id":"n0.3709395641010995"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5291916187896755"}],"style":{"align":"center"},"id":"n0.8710600789821672"}],"shape":{"data":{"p":{"x":360.0379365869461,"y":53.79938993941613},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de29561144923861726":{"id":"de29561144923861726","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"q","id":"n0.7861428367417931"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"L,K","id":"n0.8357121406402748"}],"id":"n0.5227598617191422"}],"id":"n0.3628902113797876"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.712903964628566"}],"id":"n0.31475679751150354"}],"id":"n0.7407370441747998"}},"id":"n0.1391651580626443"},{"type":"single","text":"(","id":"n0.2635047033354987"},{"text":"a","id":"n0.36959698716328204"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.24175630353672606"}],"id":"n0.30304596472597756"}],"id":"n0.6422484908790382"}},"id":"n0.34631958848430067"},{"type":"single","text":")","id":"n0.19016959825871682"}],"id":"n0.17101577099144838"}],"id":"n0.8479159783897559"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.06257449221844236"}],"style":{"align":"center"},"id":"n0.8975266426892756"}],"shape":{"data":{"p":{"x":392.9593927759736,"y":37.245461431688},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de15477765764642415":{"id":"de15477765764642415","lines":[{"blocks":[{"text":"Argmax","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.5927037459254869"}],"style":{"align":"center"},"id":"n0.18987849489526099"}],"shape":{"data":{"p":{"x":443.9827880859375,"y":66.73613757171921},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de22048441519143336":{"id":"de22048441519143336","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7153442312137162"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6821186587904562"}],"id":"n0.544484029247013"}],"id":"n0.14612408706422375"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.20960450932884633"}],"id":"n0.747255326029669"}],"id":"n0.7712424245331346"}},"id":"n0.346101542372347"}],"id":"n0.7253550691720647"}],"id":"n0.07047354575524611"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3540147473589985"}],"id":"n0.6466078670383382"}],"shape":{"data":{"p":{"x":446,"y":64.56357350349424}},"anchor":"left-top"},"isTextMode":true},"de6172859081567905":{"id":"de6172859081567905","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.29745597199177953"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.600571084112483"}],"id":"n0.996951432460681"}],"id":"n0.22174708464338644"}},"id":"n0.16095678407547664"},{"text":"|","id":"n0.12931111642842286"}],"id":"n0.4249884359941296"}],"id":"n0.18027727489244993"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.758609235691853"}],"style":{"align":"center"},"id":"n0.578764375406543"}],"shape":{"data":{"p":{"x":437.4827880859375,"y":22.311111450195312},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de029769300904883833":{"id":"de029769300904883833","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.16059604139512107"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.14509492759894793"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9295753376642859"}],"id":"n0.27376384560424927"}],"id":"n0.10688134315026021"}},"id":"n0.23859632174727086"}],"id":"n0.4708863947241193"}],"id":"n0.06716223629911067"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.6027299015914285"}],"id":"n0.15347978730734502"}],"id":"n0.019425296462810104"}},"id":"n0.9321418717828704"}],"id":"n0.3935658500937744"}],"id":"n0.9992338966947969"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5355528677259982"}],"id":"n0.7623875181255182"}],"shape":{"data":{"p":{"x":448.9827880859375,"y":12}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de1929515620516158":{"id":"de1929515620516158","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.15411396745112516"}],"id":"n0.06625770994633151"}],"id":"n0.16559125385250617"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7008248018013283"}],"id":"n0.3962088806452788"}],"shape":{"data":{"p":{"x":363.8237031885086,"y":41.210105519402646},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9533855630629304":{"id":"de9533855630629304","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.803168905710903"}],"id":"n0.595609449097565"}],"id":"n0.6114877208310152"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3396408939754496"}],"id":"n0.3955509286506018"}],"shape":{"data":{"p":{"x":329.4247300786326,"y":40.40960864627158}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true}},"connections":[],"intersections":{"id":"di37777461296401205","items":[],"style":{}},"shapes":[{"id":"dp003544426753230079","type":"doc-rounded-rect","data":{"p1":{"x":184.87063970626645,"y":40.42372755285243},"p2":{"x":268.4193250803914,"y":64.31410985425163},"rotation":0},"style":{"fillColor":[140,200,240,1]}},{"id":"da5945521334690271","data":[{"x":268.57365264376983,"y":52.79938993941613},{"x":280.4369096968221,"y":52.79938993941613}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da3960110458681976","data":[{"x":406.40682150548196,"y":24.79938993941613},{"x":426.51580810546875,"y":24.79938993941613}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp6988907231690673","type":"rectangle","data":{"p1":{"x":426.0535090630765,"y":0.6596086462715789},"p2":{"x":433.66371886110744,"y":47.65960864627158}}},{"id":"da3908323885544205","data":[{"x":433.51580810546875,"y":24.79938993941613},{"x":445.5947065141154,"y":24.79938993941613}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp4210477301545459","type":"doc-cube","data":{"p1":{"x":281.5752569651695,"y":54.601164676319854},"p2":{"x":319.66561195135387,"y":92.31111145019531},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp5009696529486707","type":"doc-cube","data":{"p1":{"x":281.5752569651695,"y":22.601164676319854},"p2":{"x":319.66561195135387,"y":60.31111145019531},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp10826384287995405","type":"doc-cube","data":{"p1":{"x":324.5752569651695,"y":77.52711486816406},"p2":{"x":362.66561195135387,"y":115.23706164203952},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da01663430025434587","data":[{"x":319.4369096968221,"y":52.79938993941613},{"x":331.6389634770701,"y":52.79938993941613}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg5248469829845708","entities":[{"id":"dp14571626825558615","type":"circle","data":{"p1":{"x":331.6389634770701,"y":43.23103503787314},"p2":{"x":351.1746795338938,"y":62.76675109469687}}},{"id":"dl4804558576697693","linkedId":"de9533855630629304"}]},{"id":"da979653912349423","data":[{"x":341.40682150548196,"y":77.52711486816406},{"x":341.40682150548196,"y":62.76675109469687}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da7884999857903685","data":[{"x":351.1746795338938,"y":52.99889306628501},{"x":363.3767333141418,"y":52.99889306628501}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg2725140409654083","entities":[{"id":"dp07794459160541112","type":"circle","data":{"p1":{"x":363.0379365869461,"y":43.031531911004265},"p2":{"x":382.57365264376983,"y":62.567247967827996}}},{"id":"dl6796094159610477","linkedId":"de1929515620516158"}],"data":{"rotation":0}},{"id":"da9333930392682195","data":[{"x":382.57365264376983,"y":52.79938993941613},{"x":394.7757064240178,"y":52.79938993941613}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp718863484943477","type":"rectangle","data":{"p1":{"x":395.0093994140625,"y":37.245461431688},"p2":{"x":418.0093994140625,"y":66.56792127763404}},"style":{"fillColor":[245,166,35,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp8753097908953678","type":"rectangle","data":{"p1":{"x":426.0535090630765,"y":55.65960864627158},"p2":{"x":433.66371886110744,"y":102.65960864627158}}},{"id":"dp6584784912429689","type":"square","data":{"p1":{"x":446,"y":72.56357350349424},"p2":{"x":458.5,"y":85.06357350349424}},"style":{"fillColor":[248,231,28,1]}},{"id":"da1725587121521539","data":[{"x":406.5093994140625,"y":78.90669135466102},{"x":406.5093994140625,"y":66.14632758119383}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da8991990548373658","data":[{"x":406.40682150548196,"y":36.52711486816406},{"x":406.40682150548196,"y":24.527114868164062}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4919998310196001","data":[{"x":406.5093994140625,"y":78.90669135466102},{"x":426.6183860140493,"y":78.90669135466102}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9029528484206584","data":[{"x":433.6183860140493,"y":78.90669135466102},{"x":445.69728442269593,"y":78.90669135466102}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg5700695566556591","entities":[{"id":"dg8570720766417066","entities":[{"id":"dp6218468945744007","type":"rectangle","data":{"p1":{"x":445.9827880859375,"y":16.981970105434243},"p2":{"x":458.63994881799636,"y":29.6391308374931}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp289772994101404","type":"rectangle","data":{"p1":{"x":447.5649331774448,"y":18.5641151969416},"p2":{"x":460.22209390950366,"y":31.221275929000456}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp6286541772730896","type":"rectangle","data":{"p1":{"x":449.1470782689522,"y":20.146260288448957},"p2":{"x":461.80423900101107,"y":32.80342102050781}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl9671172040205072","linkedId":"de029769300904883833"}]}],"settings":{"grid":true,"diagramHeight":122.98385620117188}}]},{"id":"n0.0733441201018945","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":321,"delayRenderCache":{"av":321,"map":{"n0.4639640815729844":{"n0.1154698172732449":{"w":26.2496,"h":8.4545,"bl":0.8214}},"n0.18027727489244993":{"n0.4249884359941296":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.45802729846083956":{"n0.1781866772261569":{"w":28.248,"h":9.1146,"bl":0.7619}},"n0.16920259577024832":{"n0.5361220979168753":{"w":22.4157,"h":12.5054,"bl":0.7021}},"n0.8479159783897559":{"n0.17101577099144838":{"w":20.4083,"h":9.1146,"bl":0.7619}},"n0.07047354575524611":{"n0.7253550691720647":{"w":5.3982,"h":9.1146,"bl":0.7619}},"n0.9992338966947969":{"n0.3935658500937744":{"w":7.4599,"h":9.6481,"bl":0.7198}}}}}

==> sIPOMDPLite-Net(arXiv)/plots/docs/8d120bbf-8ed1-48f8-be65-4a481f7a1e35 <==
{"id":"n0.28715960587730205","lines":[{"id":"n0.29452044693609114","blocks":[]},{"id":"n0.20454292606745117","blocks":[{"id":"n0.6840725551755149","text":"\\diagram","type":"composite","elements":{"de830133496527524":{"id":"de830133496527524","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.888716145367255"},{"id":"n0.15104764783136782","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.36671146661237697","lines":[{"id":"n0.8179473477339385","blocks":[{"id":"n0.9550966687339157","text":"i"}]}]}}},{"text":"×W","id":"n0.5599012392663407"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.41671340239262555"}],"id":"n0.7908228230325796"}],"id":"n0.46363745184185046"}},"id":"n0.678323976462252"},{"text":"×H","id":"n0.16969816635029078"},{"id":"n0.039609500242658635","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.17353734365161166","lines":[{"id":"n0.038406751864820565","blocks":[{"id":"n0.39762182261952717","text":"j"}]}]}}},{"text":"×W","id":"n0.3008060942961859"},{"id":"n0.3607380716179993","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7303295250166091","lines":[{"id":"n0.9959625119092972","blocks":[{"id":"n0.24721289861843165","text":"j"}]}]}}},{"text":"×|A","id":"n0.7472395874987383"},{"id":"n0.3920680333441362","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.8195620441773821","lines":[{"id":"n0.580356851690097","blocks":[{"id":"n0.019039025036673207","text":"i"}]}]}}},{"text":"|×|𝛺","id":"n0.5911674285490001"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3521376731337347"}],"id":"n0.12198891662407862"}],"id":"n0.6303078999133256"}},"id":"n0.8010527248379509"},{"text":"|","id":"n0.09645521585780603"}],"id":"n0.22684036926304696"}],"id":"n0.12264719501879284"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8934350916238187"}],"style":{"align":"center"},"id":"n0.26840922209508244"}],"shape":{"data":{"p":{"x":274,"y":71.05827729192396},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de31428410007153573":{"id":"de31428410007153573","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"2D convolutional layer","id":"n0.16885513588950096"}],"id":"n0.06845146326372276"}],"shape":{"data":{"p":{"x":139.7593994140625,"y":11.070138759285399},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5068466687657365":{"id":"de5068466687657365","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.6485921189478068"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×200×|A","id":"n0.09462604923524598"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7357774409027493"}],"id":"n0.8321220245420999"}],"id":"n0.056047845178978095"}},"id":"n0.34039756771574803"},{"text":"×𝛺","id":"n0.10022572740377522"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.018645629099951266"}],"id":"n0.2507497419973437"}],"id":"n0.5522533401755028"}},"id":"n0.6223560424619412"},{"text":"|","id":"n0.14742117445867353"}],"id":"n0.9045013624179807"}],"id":"n0.28195840591444044"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.27517338485264564"}],"id":"n0.11799573819626064"}],"shape":{"data":{"p":{"x":132.7593994140625,"y":0.07013875928538482},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de546742242883713":{"id":"de546742242883713","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.872383021644545"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1","id":"n0.7272182565354888"}],"id":"n0.9042131022522326"}],"id":"n0.038708607070670586"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7164403655705867"}],"id":"n0.31004931376728595"}],"shape":{"data":{"p":{"x":125.75939941406247,"y":24.0701387592854},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5705596917101636":{"id":"de5705596917101636","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"2D convolutional layer","id":"n0.5472261254339543"}],"id":"n0.08300183269532035"}],"shape":{"data":{"p":{"x":113.2593994140625,"y":10.570138759285385},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6002399326791896":{"id":"de6002399326791896","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.5163073951096822"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3×3×1×200","id":"n0.03293938249114303"}],"id":"n0.8635446728446938"}],"id":"n0.00554654937310417"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.09854121342956024"}],"id":"n0.4855904436457106"}],"shape":{"data":{"p":{"x":105.2593994140625,"y":10.570138759285392},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9263864201631913":{"id":"de9263864201631913","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.020891449239466064"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1","id":"n0.7882173865781894"}],"id":"n0.956542045504768"}],"id":"n0.8597594355492408"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9753627930496795"}],"id":"n0.867659227440186"}],"shape":{"data":{"p":{"x":98.2593994140625,"y":23.570138759285385},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de30334807816745935":{"id":"de30334807816745935","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Activation: sigmoid","id":"n0.3095276842699177"}],"id":"n0.6203656270879352"}],"shape":{"data":{"p":{"x":151.7593994140625,"y":15.070138759285399},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7476602457265411":{"id":"de7476602457265411","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.6928414408579382"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7696527085094487"}],"id":"n0.9249682609169809"}],"id":"n0.6033597829383572"}},"id":"n0.796271880879913"},{"text":"×W","id":"n0.8124065052244716"},{"id":"n0.5558073109510935","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.26051854782853656","lines":[{"id":"n0.9510684309087385","blocks":[{"id":"n0.021780209106427417","text":"i"}]}]}}},{"text":"×|A","id":"n0.7399565040359255"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.15565566038690504"}],"id":"n0.9036242193532307"}],"id":"n0.5163854680637376"}},"id":"n0.19101800992060047"},{"text":"×𝛺","id":"n0.6221485586612392"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.91989118239133"}],"id":"n0.1277352944004988"}],"id":"n0.8165743475653806"}},"id":"n0.958018226031242"},{"text":"|","id":"n0.6820777378036293"}],"id":"n0.7635730023714855"}],"id":"n0.7636721946274969"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.026328566609607806"}],"style":{"align":"center"},"id":"n0.7961220810897758"}],"shape":{"data":{"p":{"x":157.9753875732422,"y":48.560739345222885},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2201987216315624":{"id":"de2201987216315624","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.7132498602809136"}],"id":"n0.3466031727800791"}],"id":"n0.27484400963508127"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\scriptsize"},"id":"n0.6677785758317261"}],"id":"n0.08446180503343959"}],"shape":{"data":{"p":{"x":172.49811067557866,"y":-0.4063528350291712},"rotation":49.5},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8364529015502058":{"id":"de8364529015502058","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.8599819514151139"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5284243819925398"}],"id":"n0.43397894302458195"}],"id":"n0.5203002474914415"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.7093998630382501"}],"id":"n0.8794057646934292"}],"id":"n0.13734081724066582"}},"id":"n0.9586627531781591"},{"type":"single","text":"(","id":"n0.2277236073298805"},{"text":"s","id":"n0.7235534741127996"},{"type":"single","text":")","id":"n0.5423795029927823"}],"id":"n0.008391880325343104"}],"id":"n0.8068253129909273"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.7783573921404539"}],"style":{"align":"center"},"id":"n0.4805870590674932"}],"shape":{"data":{"p":{"x":54.31714561700551,"y":172.21718170370752},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7069425642293998":{"id":"de7069425642293998","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.005083172132470448"},{"id":"n0.6011201773360508","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2905804311605169","lines":[{"id":"n0.9714403353577845","blocks":[{"id":"n0.9660014246304194","text":"i"}]}]}}},{"id":"n0.8703022194174608","text":"×W"},{"id":"n0.7524534765602964","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.08243965341437276","lines":[{"id":"n0.8151768469634642","blocks":[{"id":"n0.5103346716209716","text":"i"}]}]}}}],"id":"n0.9115976780097668"}],"id":"n0.2742966032445735"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8503622370030484"}],"style":{"align":"center"},"id":"n0.7049519028495159"}],"shape":{"data":{"p":{"x":20.909614496237566,"y":184.1120662360471},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de09279253696072942":{"id":"de09279253696072942","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.4910014458934293"},{"id":"n0.8615066548897736","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9575001423927905","lines":[{"id":"n0.27052359880341914","blocks":[{"id":"n0.8845606799651806","text":"i"}]}]}}},{"text":"×W","id":"n0.659142267370771"},{"id":"n0.6083060945162448","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7126463045547087","lines":[{"id":"n0.8733096058843968","blocks":[{"id":"n0.015992116033920034","text":"i"}]}]}}},{"text":"×H","id":"n0.32992532734899993"},{"id":"n0.33587015564662304","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.11277231313626235","lines":[{"id":"n0.4319993442378911","blocks":[{"id":"n0.3045815083089889","text":"j"}]}]}}},{"text":"×W","id":"n0.06804613915010371"},{"id":"n0.38530347794077335","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.06629092672006331","lines":[{"id":"n0.30582049305888703","blocks":[{"id":"n0.6796539873208021","text":"j"}]}]}}},{"text":"×|A","id":"n0.795047829499475"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.30683837280018733"}],"id":"n0.05876238109896281"}],"id":"n0.8536749608131902"}},"id":"n0.12748157878062338"},{"text":"×A","id":"n0.7742199666318177"},{"id":"n0.6456645765287621","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7418617950362201","lines":[{"id":"n0.3239890683037132","blocks":[{"id":"n0.1956380655810923","text":"j"}]}]}}},{"text":"|","id":"n0.5271039502302577"}],"id":"n0.27881606013744675"}],"id":"n0.3566822829252332"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.02033497072142687"}],"style":{"align":"center"},"id":"n0.07737509054617053"}],"shape":{"data":{"p":{"x":281.29996422052113,"y":305.8058692110944},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5724928845451427":{"id":"de5724928845451427","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.6209544034078567"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9240656630032333"}],"id":"n0.6953438142929429"}],"id":"n0.40078647540400847"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.9680237366661995"}],"id":"n0.19941693119236126"}],"id":"n0.9183308773255874"}},"id":"n0.749968146026206"},{"type":"single","text":"(","id":"n0.36590915762485476"},{"text":"s","id":"n0.8817001599358769"},{"type":"single","text":")","id":"n0.7877088141325723"}],"id":"n0.15906262428338502"}],"id":"n0.10589766223614272"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.05246689859301301"}],"style":{"align":"center"},"id":"n0.3289653371420669"}],"shape":{"data":{"p":{"x":563.407531120768,"y":31.217181703707524},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8862399825472123":{"id":"de8862399825472123","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜂","id":"n0.08841301020629855"}],"id":"n0.9389266420440985"}],"id":"n0.838979028267915"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6644917188788857"}],"id":"n0.7384985395864783"}],"shape":{"data":{"p":{"x":517.398973109876,"y":26.45078865972181},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de5631212479888772":{"id":"de5631212479888772","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.9525486490876891"}],"id":"n0.2317967537056933"}],"id":"n0.8247411379987435"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.47255320127532596"}],"id":"n0.08230385127998541"}],"shape":{"data":{"p":{"x":627,"y":170.34364716497083}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de943353730681556":{"id":"de943353730681556","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.5584175853313227"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.6259426616056865"}],"id":"n0.4664845985318422"}],"id":"n0.7533964028274516"}},"id":"n0.3603030527412392"}],"id":"n0.7886272795362079"}],"id":"n0.5054452515819241"}},"id":"n0.8511512956512159"}],"id":"n0.30799020377446107"}],"id":"n0.5973717047898972"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9046484463074862"}],"id":"n0.8574308925216818"}],"shape":{"data":{"p":{"x":201,"y":227.6290170380177}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de7017196159240964":{"id":"de7017196159240964","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.8419303604558264"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8744834530110013"}],"id":"n0.9787111276864338"}],"id":"n0.9250652536355461"}},"id":"n0.8370633037128976"}],"id":"n0.9804800724410077"}],"id":"n0.5276168185965409"}},"id":"n0.16378716658177073"}],"id":"n0.13534933903798363"}],"id":"n0.04010641624309197"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.871833201414649"}],"id":"n0.4971954423167957"}],"shape":{"data":{"p":{"x":438,"y":197.39167897191663}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de8939303688783218":{"id":"de8939303688783218","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⊤","id":"n0.051813233084192944"}],"id":"n0.960716301838975"}],"id":"n0.2991346959721153"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.10743327573701134"}],"id":"n0.4445115508842854"}],"shape":{"data":{"p":{"x":314.31729449710235,"y":171.1441440381019},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de42671147127769893":{"id":"de42671147127769893","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.2105991058479868"}],"id":"n0.6898669597151807"}],"id":"n0.8636088782949856"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.17690363562700084"}],"id":"n0.6977511955253459"}],"shape":{"data":{"p":{"x":104,"y":170.34364716497083}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de0077756148427987615":{"id":"de0077756148427987615","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.7808842253596036"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.8412023551991661"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.2392245969950375"}],"id":"n0.6702209885816119"}],"id":"n0.6981445718985935"}},"id":"n0.18404916440608687"}],"id":"n0.6311475456865279"}],"id":"n0.49059051491697736"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.23131975052950882"}],"id":"n0.7578890736339061"}],"id":"n0.07250555470401698"}},"id":"n0.010866027179482707"}],"id":"n0.22137403373846753"}],"id":"n0.8554662319877668"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.39843064903810554"}],"id":"n0.40498540954485573"}],"shape":{"data":{"p":{"x":64.99359130859375,"y":104.55827729192396}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de9839075823404071":{"id":"de9839075823404071","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.46107283295633916"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.07797177132489064"}],"id":"n0.8192352865137036"}],"id":"n0.8533218395760711"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.2784785651723245"}],"id":"n0.9599880442014379"}],"id":"n0.8570434995157119"}},"id":"n0.4243079250467019"},{"id":"n0.2933130695804871","type":"single","text":"("},{"id":"n0.5444368383855107","text":"s,a"},{"id":"n0.5854650558170484","type":"single","text":")"}],"id":"n0.4664481726460583"}],"id":"n0.3223836254719801"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.5308587113556174"}],"style":{"align":"center"},"id":"n0.7266358655856826"}],"shape":{"data":{"p":{"x":169.9827880859375,"y":162.80245561794527},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1090782511171895":{"id":"de1090782511171895","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.7707876775405613"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.12008251905162615","text":"i"}],"id":"n0.4973178642373326"}],"id":"n0.24065984544285235"}},"id":"n0.20692698822685096"},{"text":"|×H","id":"n0.13077721782901275"},{"id":"n0.6298403962112051","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.1684123085518181","lines":[{"id":"n0.607684858931526","blocks":[{"id":"n0.7642240954984785","text":"j"}]}]}}}],"id":"n0.48014294592380113"}],"id":"n0.12142712283211354"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7113835606186685"}],"style":{"align":"center"},"id":"n0.9140171115099107"}],"shape":{"data":{"p":{"x":146.29996422052108,"y":212.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de27818778541908484":{"id":"de27818778541908484","lines":[{"blocks":[{"id":"n0.19811593342069855","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.27303294008700485","lines":[{"id":"n0.20807316996563263","blocks":[{"id":"n0.8476450789047942","text":"⟨s,a⟩∈"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}}}],"id":"n0.315154072876368"}],"shape":{"data":{"p":{"x":172.2593994140625,"y":188.57013875928538},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5665977907448196":{"id":"de5665977907448196","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"P","id":"n0.307663362192103"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.10623070241454569"}],"id":"n0.8827687096036736"}],"id":"n0.5503718734749985"},"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.8967256030802724"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.46344775539216965"}],"id":"n0.0910101533328953"}],"id":"n0.3890398752134623"}},"id":"n0.7392678537130051"}],"id":"n0.8408046439029846"}],"id":"n0.24075512889589712"}},"id":"n0.24299648297894794"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"∁","id":"n0.9559161988759053"}],"id":"n0.0614877672214893"}],"id":"n0.08636211467259147"}},"id":"n0.8633596343116492"}],"id":"n0.13555213879565464"}],"id":"n0.8868465557438261"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6149708464894408"}],"id":"n0.8085337507563177"}],"shape":{"data":{"p":{"x":173.2593994140625,"y":200.57013875928538},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de30843334298970215":{"id":"de30843334298970215","lines":[{"blocks":[{"id":"n0.32033707080720686","text":"reshape","style":{"fontSize":{"value":0.4}}}],"style":{"align":"center"},"id":"n0.3735752378184525"}],"shape":{"data":{"p":{"x":124.29996422052108,"y":160.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9248573790762489":{"id":"de9248573790762489","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.7603334384584806"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.3217610877936177"},{"id":"n0.21383482447251523","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9825801512442374","lines":[{"id":"n0.07189415363336216","blocks":[{"id":"n0.04384100305856253","text":"j"}]}]}}}],"id":"n0.16362173088793375"}],"id":"n0.16619311131198167"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.6632166449495389"}],"id":"n0.3737897722083008"}],"id":"n0.7585584777622782"}},"id":"n0.2518456284544879"}],"id":"n0.9369673044431397"}],"id":"n0.1167764301657912"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.23477981152773864"}],"id":"n0.6641020234620718"}],"shape":{"data":{"p":{"x":64.99359130859375,"y":125.55827729192396}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de4498440874344303":{"id":"de4498440874344303","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.8588232679304955"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.18868339216376362","text":"j"}],"id":"n0.4414432983578507"}],"id":"n0.08884608357346835"}},"id":"n0.5391030170731603"},{"text":"|","id":"n0.6639977883797332"}],"id":"n0.5903833754603707"}],"id":"n0.33986799877509544"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4046521967791459"}],"style":{"align":"center"},"id":"n0.6302171432238233"}],"shape":{"data":{"p":{"x":51,"y":131.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de19860656186876802":{"id":"de19860656186876802","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.9728792456619699"}],"id":"n0.3614715090637004"}],"id":"n0.31851350704837644"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6103450736207618"}],"id":"n0.22301542229688098"}],"shape":{"data":{"p":{"x":276,"y":170.34364716497083}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de17895393746656385":{"id":"de17895393746656385","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.2225457776491735"}],"style":{"align":"center"},"id":"n0.48149747604985205"}],"shape":{"data":{"p":{"x":342.2999642205211,"y":160.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de0956511130065969":{"id":"de0956511130065969","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.21684088306783855"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8810173732013185"}],"id":"n0.09244370019065884"}],"id":"n0.9908347680288985"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.2171008019923657"}],"id":"n0.7344164383742948"}],"id":"n0.10489682643546083"}},"id":"n0.7092440768028014"},{"type":"single","text":"(","id":"n0.1630181873482086"},{"text":"s,a","id":"n0.32282624326485454"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.45678412884730646","text":"i"}],"id":"n0.0872462204668929"}],"id":"n0.0441292851971995"}},"id":"n0.37481095126090547"},{"type":"single","text":")","id":"n0.029012923234883692"}],"id":"n0.25774265518288164"}],"id":"n0.1846677557628713"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.8537851218944812"}],"style":{"align":"center"},"id":"n0.7254641411995377"}],"shape":{"data":{"p":{"x":390.9827880859375,"y":157.80245561794527},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9168744279554575":{"id":"de9168744279554575","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.8973834832800198"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.08165736455520789","text":"j"}],"id":"n0.19048861557441343"}],"id":"n0.11691188405925867"}},"id":"n0.23522145637931424"},{"text":"|×H","id":"n0.13561582343082956"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4348102888760459","text":"i"}],"id":"n0.9816122324013963"}],"id":"n0.645012438850548"}},"id":"n0.47560350934855466"},{"text":"×W","id":"n0.13212722290639367"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.8609083576254704","text":"i"}],"id":"n0.8165011523965076"}],"id":"n0.7742212388926979"}},"id":"n0.9032057221818466"},{"text":"×|A","id":"n0.05523285678774892"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.6954448285145305","text":"i"}],"id":"n0.9349445110858419"}],"id":"n0.3074719355739637"}},"id":"n0.23130510103780288"},{"text":"|","id":"n0.907281144214686"}],"id":"n0.5592823458575049"}],"id":"n0.8891057395138631"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.03796355660326678"}],"style":{"align":"center"},"id":"n0.87548864355613"}],"shape":{"data":{"p":{"x":373.2999642205211,"y":208.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3279148366297122":{"id":"de3279148366297122","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.9764923833878913"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"o","id":"n0.8545723140790371"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.656088695208134"}],"id":"n0.9423376863555075"}],"id":"n0.05268244245386278"}},"id":"n0.13117074509106152"}],"id":"n0.8149136508863273"}],"id":"n0.5320387796314341"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.6071295041600127"}],"id":"n0.8125459681939333"}],"id":"n0.6267102920693011"}},"id":"n0.12500792441251707"}],"id":"n0.20304082800058465"}],"id":"n0.009969838646760376"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3074931501193965"}],"id":"n0.09711639066157196"}],"shape":{"data":{"p":{"x":66.99359130859375,"y":83.2140237518849}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de37592669576036997":{"id":"de37592669576036997","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.37140121002635285"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.8222042970629553","text":"i"}],"id":"n0.8532041137459934"}],"id":"n0.6723412507106035"}},"id":"n0.43193967528583666"},{"text":"|","id":"n0.29947608577971097"}],"id":"n0.08150258236245111"}],"id":"n0.4797470730986"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5563251825052116"}],"style":{"align":"center"},"id":"n0.256507361805991"}],"shape":{"data":{"p":{"x":51,"y":111.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de21007012170022854":{"id":"de21007012170022854","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|𝛺","id":"n0.36016219737294297"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4393028134718642"}],"id":"n0.6659609798693562"}],"id":"n0.5437564035996625"}},"id":"n0.10133264164423617"},{"text":"|","id":"n0.7224327312760754"}],"id":"n0.4032393424919807"}],"id":"n0.8679679641366074"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7382787493809047"}],"style":{"align":"center"},"id":"n0.3534678316598481"}],"shape":{"data":{"p":{"x":51,"y":90.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4170855423696589":{"id":"de4170855423696589","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.8667350681769705"}],"id":"n0.45712645502986815"}],"id":"n0.6457390848865447"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9794651469988409"}],"id":"n0.5564923070041499"}],"shape":{"data":{"p":{"x":495,"y":170.34364716497083}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8293020670412787":{"id":"de8293020670412787","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⊤","id":"n0.6140443696320139"}],"id":"n0.7432367586553266"}],"id":"n0.07659008397190314"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.868990594364446"}],"id":"n0.9922236445990658"}],"shape":{"data":{"p":{"x":528.3172944971024,"y":171.1441440381019},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de669945869924045":{"id":"de669945869924045","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.34518448981183725"}],"style":{"align":"center"},"id":"n0.8690897824719104"}],"shape":{"data":{"p":{"x":544.2999642205211,"y":160.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8145527982242438":{"id":"de8145527982242438","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.4267226079420261"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.2937109514143881"}],"id":"n0.19683042376548032"}],"id":"n0.5952520400922403"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.062236602762587356"}],"id":"n0.5664962141458856"}],"id":"n0.3577607064246804"}},"id":"n0.09695746678638462"},{"type":"single","text":"(","id":"n0.6281659403480571"},{"text":"s","id":"n0.7022231872432894"},{"type":"single","text":")","id":"n0.185653476301755"}],"id":"n0.12698408810015294"}],"id":"n0.8024924706930465"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.32891985484141095"}],"style":{"align":"center"},"id":"n0.8824838961846289"}],"shape":{"data":{"p":{"x":583.407531120768,"y":172.21718170370752},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6553654751023015":{"id":"de6553654751023015","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.394426262818969"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.23499173389848416"}],"id":"n0.005625112307531932"}],"id":"n0.796539540727877"}},"id":"n0.12271738779981445"},{"text":"×W","id":"n0.34614302360500226"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7421539385815077"}],"id":"n0.35134270037528714"}],"id":"n0.7583559929329973"}},"id":"n0.5521611919047027"},{"text":"×H","id":"n0.36205238542179075"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5906657040606391"}],"id":"n0.2317659176249558"}],"id":"n0.49004230698462936"}},"id":"n0.7758571018564613"},{"text":"×W","id":"n0.24293871410295753"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.005343589685217642"}],"id":"n0.3650620138975105"}],"id":"n0.45390929658934875"}},"id":"n0.5378082324788938"}],"id":"n0.864399840513006"}],"id":"n0.4464515627733918"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6578105722546257"}],"style":{"align":"center"},"id":"n0.40036281772086113"}],"shape":{"data":{"p":{"x":560,"y":193.1120662360471},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4773866742381614":{"id":"de4773866742381614","lines":[{"blocks":[{"text":"Expand along dimensions ","style":{"fontSize":{"value":0.4}},"id":"n0.4777894131524951"},{"id":"n0.8336835840112506","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.766638339102051","lines":[{"id":"n0.7058263596247902","blocks":[{"id":"n0.766599551830595","text":"H"},{"id":"n0.06466344616431674","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.0037084846037074293","lines":[{"id":"n0.18954123602279727","blocks":[{"id":"n0.7103732797925326","text":"j"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}}},{"id":"n0.12596522527849463","text":",","style":{"fontSize":{"value":0.4}}},{"id":"n0.810974683227552","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.47147723642626493","lines":[{"id":"n0.6254596818194615","blocks":[{"id":"n0.516270729737571","text":"W"},{"id":"n0.6497664086249271","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6505778140428289","lines":[{"id":"n0.42528586649288136","blocks":[{"id":"n0.10351850513902994","text":"j"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}}}],"style":{"align":"center"},"id":"n0.675126439532246"}],"shape":{"data":{"p":{"x":214.29996422052108,"y":19.805869211094375},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de39442010604872957":{"id":"de39442010604872957","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.14714877240293278"}],"id":"n0.13157685618989423"}],"id":"n0.23581435920432314"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6573834073407789"}],"id":"n0.5823267703072419"}],"shape":{"data":{"p":{"x":395.99359130859375,"y":28.905746459960938}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de0411298464122003":{"id":"de0411298464122003","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.980927202048494"}],"id":"n0.974705051418195"}],"id":"n0.47526699081088797"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5398708628961781"}],"id":"n0.2768969188858561"}],"shape":{"data":{"p":{"x":363.99359130859375,"y":28.870376586914062}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de7388266462341742":{"id":"de7388266462341742","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.5071050351318276"}],"style":{"align":"center"},"id":"n0.13105491006599146"}],"shape":{"data":{"p":{"x":247.29996422052108,"y":32.805869211094375},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de0830381032376537":{"id":"de0830381032376537","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.8965425373877725","type":"composite","text":"\\Pr","elements":{}},{"id":"n0.3442353613415672","type":"single","text":"("},{"id":"n0.0845208498103871","text":"o"},{"id":"n0.31676876570778445","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.4690998683411016","lines":[{"id":"n0.1330729774493402","blocks":[{"id":"n0.5730378908635343","text":"i"}]}]}}},{"id":"n0.5475042978382414","text":"|s,a"},{"id":"n0.35289670728570566","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5110242207761153","lines":[{"id":"n0.7948905322565856","blocks":[{"id":"n0.30612191359910423","text":"i"}]}]}}},{"id":"n0.3831480288091813","type":"single","text":")"}],"id":"n0.18446577248835783"}],"id":"n0.7503090051164691"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6385329125259112"}],"style":{"align":"center"},"id":"n0.6832618478377599"}],"shape":{"data":{"p":{"x":436.6178159936692,"y":31.565967721611457},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7458997970769539":{"id":"de7458997970769539","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.0718166669177347"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3168480525463271"}],"id":"n0.12648840840709297"}],"id":"n0.15890614400874914"}},"id":"n0.7519119373679519"},{"text":"×W","id":"n0.5920452203425906"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.1776212629466427"}],"id":"n0.14108349465921566"}],"id":"n0.03706276421585164"}},"id":"n0.21062676702879468"},{"text":"×H","id":"n0.05552562153997176"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.06280782700699583"}],"id":"n0.9425552972309041"}],"id":"n0.2761944122243878"}},"id":"n0.2635350789248214"},{"text":"×W","id":"n0.13676684268811634"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.319378960058051"}],"id":"n0.3927870336843269"}],"id":"n0.908260687161133"}},"id":"n0.26239027238645707"}],"id":"n0.7568409456873406"}],"id":"n0.24506231822248026"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7432260243774154"}],"style":{"align":"center"},"id":"n0.007628739367402604"}],"shape":{"data":{"p":{"x":418.9756827354431,"y":51.26288890838623},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2003253275462542":{"id":"de2003253275462542","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.05993666967703404"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9042661943311023"}],"id":"n0.9386350158346954"}],"id":"n0.3995965561196029"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.4199011904587484"}],"id":"n0.8247882463362652"}],"id":"n0.3247054696277607"}},"id":"n0.8299140372309248"},{"type":"single","text":"(","id":"n0.6623530921690994"},{"text":"s","id":"n0.43889332452392593"},{"type":"single","text":")","id":"n0.08122931977256154"}],"id":"n0.14447215791313917"}],"id":"n0.8685308613044107"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.9383609344299102"}],"style":{"align":"center"},"id":"n0.42613163751687644"}],"shape":{"data":{"p":{"x":583.407531120768,"y":273.2171817037075},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7565797893523323":{"id":"de7565797893523323","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.8002262262900506"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.24564655302018923"}],"id":"n0.3088543549628897"}],"id":"n0.8515017815217956"}},"id":"n0.3413536317663919"},{"text":"×W","id":"n0.016568973436302148"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5749350813051146"}],"id":"n0.8332324771261821"}],"id":"n0.4520368826794676"}},"id":"n0.7656998147065233"},{"text":"×H","id":"n0.584135691491046"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.4105217232748377"}],"id":"n0.7144078818603381"}],"id":"n0.5926601031321859"}},"id":"n0.8384180698480208"},{"text":"×W","id":"n0.5376518715799503"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.6088208828591788"}],"id":"n0.526078288818403"}],"id":"n0.33542278812265924"}},"id":"n0.8176488346950643"}],"id":"n0.5064483700922966"}],"id":"n0.6615254849573731"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.1349214364108775"}],"style":{"align":"center"},"id":"n0.7067476805507515"}],"shape":{"data":{"p":{"x":561,"y":294.1120662360471},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5290652384541861":{"id":"de5290652384541861","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.46027237797742626"}],"id":"n0.7177733724273605"}],"id":"n0.6097892962585569"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5473614520072723"}],"id":"n0.9341008659211252"}],"shape":{"data":{"p":{"x":479.9827880859375,"y":28.49939362493177}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de46277186945107696":{"id":"de46277186945107696","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.46771412146034685"}],"style":{"align":"center"},"id":"n0.8110806422154855"}],"shape":{"data":{"p":{"x":352.00939941406244,"y":260.80245561794527},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8463101795697547":{"id":"de8463101795697547","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.2602801313897891"}],"id":"n0.38287986979292277"}],"id":"n0.9651448539051894"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.1141182818123545"}],"id":"n0.8571368685375644"}],"shape":{"data":{"p":{"x":412.99359130859375,"y":270.90574645996094}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de857602324837198":{"id":"de857602324837198","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.1568773903181273"}],"id":"n0.8420086078291884"}],"id":"n0.4282342875453744"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.2084298801907456"}],"id":"n0.7275271279585349"}],"shape":{"data":{"p":{"x":380.99359130859375,"y":270.87037658691406}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9277590802208895":{"id":"de9277590802208895","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.14144761073521783"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6978940101307265"}],"id":"n0.9882271030569612"}],"id":"n0.7190211040442582"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.05348292174395319"}],"id":"n0.6020659708555867"}],"id":"n0.07516815562681134"}},"id":"n0.4392028187363797"},{"type":"single","text":"(","id":"n0.32049668130328013"},{"text":"s,a","id":"n0.8665530680262943"},{"type":"single","text":")","id":"n0.9212341774477784"}],"id":"n0.8414305306060739"}],"id":"n0.2339738641536926"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.4325019727590309"}],"style":{"align":"center"},"id":"n0.7391255984161547"}],"shape":{"data":{"p":{"x":318.15324163402437,"y":254.80245561794527},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6680758227104713":{"id":"de6680758227104713","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.38809881048380124"}],"id":"n0.03754649801948018"}],"id":"n0.9286164676290005"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7589032828734961"}],"id":"n0.3501760318677496"}],"shape":{"data":{"p":{"x":53,"y":208.34364716497083}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de33451906419634647":{"id":"de33451906419634647","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"id":"n0.8372553384111951","text":"X"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.5872417922678372"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.03830798375830846"}],"id":"n0.17834281279956343"}],"id":"n0.235315821971545"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.6277978845181515"}],"id":"n0.94137873539362"}],"id":"n0.5946312346390881"}},"id":"n0.7000175404116691"}],"id":"n0.1963309157355273"}],"id":"n0.4401800566575105"}},"id":"n0.9516233886005141"},{"type":"single","text":"(","id":"n0.5407370816987096"},{"text":"s,a","id":"n0.6564324879943835"},{"type":"single","text":")","id":"n0.48642615921601484"}],"id":"n0.4237285521604277"}],"id":"n0.20649554028200523"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5481037893136345"}],"style":{"align":"center"},"id":"n0.012275783186388889"}],"shape":{"data":{"p":{"x":57.40112242936175,"y":260.20880845297444},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de23024235703851592":{"id":"de23024235703851592","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.9291547683556114"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.5163815412944552","text":"i"}],"id":"n0.18972846315785996"}],"id":"n0.5700081006974362"}},"id":"n0.9827207480147806"},{"text":"×W","id":"n0.2084825202211329"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4251312613811131","text":"i"}],"id":"n0.40357285884537597"}],"id":"n0.08454621183956479"}},"id":"n0.006496406810263533"},{"text":"×H","id":"n0.5574819716886936"},{"id":"n0.8461517982433133","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.32111423845020015","lines":[{"id":"n0.2699080480690079","blocks":[{"id":"n0.8186288242446029","text":"j"}]}]}}}],"id":"n0.8072900678294179"}],"id":"n0.8962696595786119"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.794439420444337"}],"style":{"align":"center"},"id":"n0.06738415328718728"}],"shape":{"data":{"p":{"x":10,"y":302.6290170380177},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de39900376536250404":{"id":"de39900376536250404","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.2723198198313941"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9591550340193618"}],"id":"n0.5964767574562275"}],"id":"n0.6551061619768701"}},"id":"n0.07094054403522487"},{"text":"×W","id":"n0.4674033076598587"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.30931752182513406"}],"id":"n0.5516107555819181"}],"id":"n0.2408426998855402"}},"id":"n0.9568216286077658"},{"text":"×H","id":"n0.2782871445677946"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.18382258695628395"}],"id":"n0.5935551549083624"}],"id":"n0.5186587852573017"}},"id":"n0.6780650757034818"},{"text":"×W","id":"n0.13629958420015487"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.19496263696955318"}],"id":"n0.2519479940241587"}],"id":"n0.24152246688556933"}},"id":"n0.38140606080332695"}],"id":"n0.08267215938659933"}],"id":"n0.7023420069695498"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.16188461314545588"}],"style":{"align":"center"},"id":"n0.38597499972620275"}],"shape":{"data":{"p":{"x":540.3810645367254,"y":50.80793110814713},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1403991638934048":{"id":"de1403991638934048","lines":[{"blocks":[{"text":"Env map for agent ","style":{"fontSize":{"value":0.4}},"id":"n0.9712413089337955"},{"id":"n0.20032978619065522","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.04625616876755467","lines":[{"id":"n0.2585342501714727","blocks":[{"id":"n0.867836739311739","text":"i"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}}}],"style":{"align":"center"},"id":"n0.3435864613679471"}],"shape":{"data":{"p":{"x":18.107566900246866,"y":48.65347228287732},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de21276987906964906":{"id":"de21276987906964906","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.4093467247683491","text":"O"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8166139838940352"}],"id":"n0.043042421802454545"}],"id":"n0.3127550529781269"}},"id":"n0.4603781322459519"},{"type":"single","text":"(","id":"n0.7321504678612816"},{"text":"s,a","id":"n0.005065657196590356"},{"id":"n0.6976724784573709","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.25955722025508643","lines":[{"id":"n0.009544485526986168","blocks":[{"id":"n0.11863656857749305","text":"i"}]}]}}},{"text":",o","id":"n0.2549026018291045"},{"id":"n0.8588600373699287","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.3178461024367669","lines":[{"id":"n0.4778072763325152","blocks":[{"id":"n0.0016428669114334493","text":"i"}]}]}}},{"type":"single","text":")","id":"n0.8624895098210799"}],"id":"n0.8847247660066546"}],"id":"n0.23124838131896186"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5728168841051675"}],"style":{"align":"center"},"id":"n0.16039627818252766"}],"shape":{"data":{"p":{"x":318.4011224293617,"y":17.681440548064366},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de6967035079120742":{"id":"de6967035079120742","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"O","id":"n0.7663962241632654"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7473083347132004"}],"id":"n0.2703144490961966"}],"id":"n0.1991865376500357"}},"id":"n0.5882428150387884"},{"type":"single","text":"(","id":"n0.03746013119834379"},{"text":"s","id":"n0.1985457752930604"},{"id":"n0.5376262985786864","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9078990163736704","lines":[{"id":"n0.5338368310554413","blocks":[{"id":"n0.20146336820493738","text":"i"}]}]}}},{"text":",a","id":"n0.15356174462514338"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4917042302820358"}],"id":"n0.3646442975237121"}],"id":"n0.8832778644999733"}},"id":"n0.6012821954948677"},{"text":",o","id":"n0.292345748241547"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.883382721516984"}],"id":"n0.5450711900828653"}],"id":"n0.191353720293008"}},"id":"n0.44608469355529423"},{"type":"single","text":")","id":"n0.12310447143393777"}],"id":"n0.8935425919742013"}],"id":"n0.5653478407878947"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6368133830903722"}],"style":{"align":"center"},"id":"n0.5620708150660785"}],"shape":{"data":{"p":{"x":178.94530465440607,"y":29.072458095222885},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de41779621283020885":{"id":"de41779621283020885","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.31808763908175397","text":"T"},{"id":"n0.7811607469746116","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9934384487042336","lines":[{"id":"n0.8249034781604134","blocks":[{"id":"n0.38552263098111217","text":"i"}]}]}}}],"id":"n0.5966198281161046"}],"id":"n0.03826225597296773"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7099380664464363"}],"id":"n0.4556250393584236"}],"shape":{"data":{"p":{"x":223,"y":256.6290170380177}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de34251506853038727":{"id":"de34251506853038727","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"3D channel-wise conv layer","id":"n0.45099606085613075"}],"id":"n0.9168304829570921"}],"shape":{"data":{"p":{"x":492.5,"y":158.59364716497083},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de0897703378860828":{"id":"de0897703378860828","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.7713406074602509"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×3×3×|A","id":"n0.8795321550721087"},{"id":"n0.23366925302629848","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2933669962193266","lines":[{"id":"n0.5282555781020577","blocks":[{"id":"n0.15873731962818005","text":"i"}]}]}}},{"text":"|×|A","id":"n0.6430833826318751"},{"id":"n0.4466440054019756","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6784456112344799","lines":[{"id":"n0.481923060795445","blocks":[{"id":"n0.16599295159904703","text":"i"}]}]}}},{"text":"|","id":"n0.8858597521722005"}],"id":"n0.27010289520160713"}],"id":"n0.4916509212070379"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7014747910320709"}],"id":"n0.6812788064366586"}],"shape":{"data":{"p":{"x":485.5,"y":155.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de660336245025593":{"id":"de660336245025593","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.9199440943311219"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1","id":"n0.5215522760989746"}],"id":"n0.7509404326875604"}],"id":"n0.2816604439341721"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5875591290851307"}],"id":"n0.5860391761773773"}],"shape":{"data":{"p":{"x":479.5,"y":174.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9591453651554063":{"id":"de9591453651554063","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"3D channel-wise conv layer","id":"n0.05191440829554517"}],"id":"n0.17237313422475875"}],"shape":{"data":{"p":{"x":252.5,"y":159.59364716497083},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de45735341519520456":{"id":"de45735341519520456","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.3314400328996967"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×3×3×|A","id":"n0.2917759348473479"},{"id":"n0.3609113348534887","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9335465805122038","lines":[{"id":"n0.8435857768293036","blocks":[{"id":"n0.6881939329826796","text":"j"}]}]}}},{"text":"|×|A","id":"n0.5101759115117066"},{"id":"n0.18745062227453024","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.42588280166580916","lines":[{"id":"n0.7479203928049911","blocks":[{"id":"n0.12498090824807195","text":"j"}]}]}}},{"text":"|","id":"n0.9622768332023766"}],"id":"n0.19712993762208386"}],"id":"n0.8920883669508386"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.08525903771344989"}],"id":"n0.5251548027051971"}],"shape":{"data":{"p":{"x":245.5,"y":156.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de52514505709446":{"id":"de52514505709446","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.21377116286758535"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1","id":"n0.8243123237640093"}],"id":"n0.29355940165675376"}],"id":"n0.004686903710433121"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.027630590179415826"}],"id":"n0.7395885647252762"}],"shape":{"data":{"p":{"x":239.5,"y":175.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de117272111129469":{"id":"de117272111129469","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"4D channel-wise conv layer","id":"n0.9306252205114571"}],"id":"n0.39657295829914774"}],"shape":{"data":{"p":{"x":277.5,"y":236.59364716497083},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de7615362257186091":{"id":"de7615362257186091","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.4130287381629909"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3×3×3×3×|A|×|A|","id":"n0.36715312468569916"}],"id":"n0.3200974499624347"}],"id":"n0.08237313594205076"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3510258372240125"}],"id":"n0.6116826147621695"}],"shape":{"data":{"p":{"x":270.5,"y":230.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6516545387625636":{"id":"de6516545387625636","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.500807289500258"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1×1","id":"n0.8113093053356222"}],"id":"n0.35291789532253914"}],"id":"n0.8258704275455162"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6295809682720299"}],"id":"n0.17484403301633678"}],"shape":{"data":{"p":{"x":264.5,"y":246.59364716497078},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de10870917208802044":{"id":"de10870917208802044","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.6447790487623963"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.6169936476655333"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.045612797957085505"}],"id":"n0.22292745515142354"}],"id":"n0.8415070752340081"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.8563935651909795"}],"id":"n0.9684488874652912"}],"id":"n0.5774917245565432"}},"id":"n0.7034740122979639"}],"id":"n0.07669296594331176"}],"id":"n0.0994922811168637"}},"id":"n0.8242576641109514"},{"type":"single","text":"(","id":"n0.5749209994620474"},{"text":"s,a","id":"n0.5092861365050867"},{"type":"single","text":")","id":"n0.5051619485545153"}],"id":"n0.16051818902884407"}],"id":"n0.3114158995400982"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.14258793098244626"}],"style":{"align":"center"},"id":"n0.9960370761185398"}],"shape":{"data":{"p":{"x":116.40112242936175,"y":222.53370987198798},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3162967005585082":{"id":"de3162967005585082","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×H","id":"n0.5084690952694362"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.82135938647904"}],"id":"n0.35478653377661695"}],"id":"n0.23011811938807103"}},"id":"n0.4848196183730935"},{"text":"×W","id":"n0.40299386914870117"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.03503589739992141"}],"id":"n0.9852695233050719"}],"id":"n0.5841533398669001"}},"id":"n0.7007170507377265"}],"id":"n0.2738713707452638"}],"id":"n0.832831636206383"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9604007485113473"}],"style":{"align":"center"},"id":"n0.6776359740492512"}],"shape":{"data":{"p":{"x":20,"y":192.1120662360471},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2104159824026235":{"id":"de2104159824026235","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.7876280219507019"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6290273553863923"}],"id":"n0.07730342401283585"}],"id":"n0.09106588172363139"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.13182050895445974"}],"id":"n0.8009488580250363"}],"id":"n0.28390283275685135"}},"id":"n0.7189470474140787"},{"type":"single","text":"(","id":"n0.9200273278034197"},{"text":"s,a","id":"n0.646388645726921"},{"type":"single","text":")","id":"n0.9214108582392662"}],"id":"n0.19072972727490445"}],"id":"n0.44294341390001013"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.9221759651055457"}],"style":{"align":"center"},"id":"n0.8601035183982335"}],"shape":{"data":{"p":{"x":171.9827880859375,"y":261.80245561794527},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8990960063160915":{"id":"de8990960063160915","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⟨s,a⟩∈P","id":"n0.39889804243963156"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.11906623756041412"}],"id":"n0.2572134513703166"}],"id":"n0.12924158531451835"},"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.6116493305333659"}],"id":"n0.4929970812996085"}],"id":"n0.9343545064639578"}},"id":"n0.8359040854265134"}],"id":"n0.2555656084479139"}],"id":"n0.8001658363143611"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.19978794391158705"}],"id":"n0.578648975033156"}],"shape":{"data":{"p":{"x":171.2593994140625,"y":293.5701387592854},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8745360752140423":{"id":"de8745360752140423","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×W","id":"n0.14771945004597176"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8206652003562014"}],"id":"n0.3071335603483367"}],"id":"n0.0070596474573974"}},"id":"n0.2986233368509299"},{"text":"×|A","id":"n0.6465069551089713"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6825004675603832"}],"id":"n0.029569346878788982"}],"id":"n0.2641187807105312"}},"id":"n0.16309711346390343"},{"text":"|×|A","id":"n0.13113792884500786"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.150293276858394"}],"id":"n0.9495867001768996"}],"id":"n0.3505805194696199"}},"id":"n0.9680356977111231"},{"text":"|","id":"n0.4968696429602695"}],"id":"n0.960824309431972"}],"id":"n0.7546823378521905"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8550027525837427"}],"style":{"align":"center"},"id":"n0.3285386933870884"}],"shape":{"data":{"p":{"x":9,"y":309.95391845703125},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9681358751947411":{"id":"de9681358751947411","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.6735155867197911"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.822951003368392"}],"id":"n0.3875169435950563"}],"id":"n0.5393744984404478"}},"id":"n0.015158075214938282"},{"text":"×W","id":"n0.9328996247353945"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.23811111870702528"}],"id":"n0.7304818694832187"}],"id":"n0.71047928281358"}},"id":"n0.19056974257318737"},{"text":"×H","id":"n0.3445684342557569"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.022240047955429443"}],"id":"n0.09543772425738717"}],"id":"n0.5356780984386695"}},"id":"n0.7251456758815455"}],"id":"n0.7675969773404887"}],"id":"n0.7185940494962384"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.26479353790136995"}],"style":{"align":"center"},"id":"n0.07069884526832615"}],"shape":{"data":{"p":{"x":115,"y":299.6290170380177},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6804744066955923":{"id":"de6804744066955923","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×W","id":"n0.7254971108419839"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8556966236175492"}],"id":"n0.6256926549735815"}],"id":"n0.7314977349612517"}},"id":"n0.9220443438229273"},{"text":"×|A","id":"n0.5642899003657063"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3047713439072508"}],"id":"n0.2869302910733671"}],"id":"n0.2632708866522573"}},"id":"n0.4425430359350071"},{"text":"×A","id":"n0.5442896384796381"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.9472826684666635"}],"id":"n0.7388989824221315"}],"id":"n0.8540986958813741"}},"id":"n0.8917579792144881"},{"text":"|","id":"n0.174251111004877"}],"id":"n0.15127848760257478"}],"id":"n0.934508072726157"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9783427957246185"}],"style":{"align":"center"},"id":"n0.330671341117847"}],"shape":{"data":{"p":{"x":114,"y":306.95391845703125},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5301995220615792":{"id":"de5301995220615792","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×W","id":"n0.6117308415951288"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.40483598555446476"}],"id":"n0.6840556074512587"}],"id":"n0.6126873023620558"}},"id":"n0.063179090824099"},{"text":"×|A","id":"n0.9336298325406398"},{"id":"n0.5162968033203927","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.3059733431069611","lines":[{"id":"n0.6706970193389152","blocks":[{"id":"n0.5994754649617351","text":"i"}]}]}}},{"text":"×A","id":"n0.4450143072946269"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.49680642770751104"}],"id":"n0.32082172568795664"}],"id":"n0.960799079841429"}},"id":"n0.164921740577342"},{"text":"|","id":"n0.541991390065071"}],"id":"n0.8705964676783371"}],"id":"n0.7840692535254685"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6362533217886697"}],"style":{"align":"center"},"id":"n0.8382510826015033"}],"shape":{"data":{"p":{"x":145.29996422052108,"y":220.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de45379357826059574":{"id":"de45379357826059574","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.863071493418518"}],"style":{"align":"center"},"id":"n0.8446101747497616"}],"shape":{"data":{"p":{"x":108.00939941406244,"y":283.80245561794527},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di5159292854007935","items":[],"style":{}},"shapes":[{"id":"dp6622237718632957","type":"doc-cube","data":{"p1":{"x":152.89243309975313,"y":175.09592243721903},"p2":{"x":195.15612200055915,"y":212.80586921109438},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp7977048112572978","type":"doc-cube","data":{"p1":{"x":152.89243309975313,"y":142.79350678411146},"p2":{"x":195.15612200055915,"y":180.50345355798692},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dg8483270993201228","entities":[{"id":"dp7384638156337533","type":"rectangle","data":{"p1":{"x":157.85418515207553,"y":5.994717392586722},"p2":{"x":189.90884998009108,"y":35.37046218993311}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp2742804657475568","type":"rectangle","data":{"p1":{"x":161.1701851799656,"y":9.033587743904832},"p2":{"x":193.22485000798127,"y":38.4093325412511}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp8917185552111246","type":"rectangle","data":{"p1":{"x":164.4861852078557,"y":12.072458095222885},"p2":{"x":196.54085003587147,"y":41.44820289256921}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"dg22710741968910475","entities":[{"id":"dg1612353785263314","entities":[{"id":"dp8411049564449569","type":"rectangle","data":{"p1":{"x":63.99359130859375,"y":109.5402473973582},"p2":{"x":76.6507520406526,"y":122.19740812941706}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp639236493824461","type":"rectangle","data":{"p1":{"x":65.57573640010105,"y":111.12239248886556},"p2":{"x":78.2328971321599,"y":123.77955322092441}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp7897895271166255","type":"rectangle","data":{"p1":{"x":67.15788149160846,"y":112.70453758037291},"p2":{"x":79.81504222366732,"y":125.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl9317274722545805","linkedId":"de0077756148427987615"}]},{"id":"dg5022281278414338","entities":[{"id":"dp6584292212823948","type":"rectangle","data":{"p1":{"x":46.76515712043911,"y":40.457077960817855},"p2":{"x":48.87080794747369,"y":42.56272878785251}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7634301089799995","type":"rectangle","data":{"p1":{"x":32.86592987226048,"y":26.557850712639492},"p2":{"x":62.770035195652184,"y":56.461956036031125}},"style":{"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp941185546601065","type":"rectangle","data":{"p1":{"x":60.74970508255704,"y":42.60671136364056},"p2":{"x":62.855355909591694,"y":44.71236219067538}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp12518955187598535","type":"rectangle","data":{"p1":{"x":44.529110485308124,"y":51.82566063705568},"p2":{"x":46.61544341484719,"y":53.911993566594646}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9425702251933581","type":"rectangle","data":{"p1":{"x":53.78238338576345,"y":40.502153054974656},"p2":{"x":55.88803421279809,"y":42.60780388200919}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp15268933323188394","type":"rectangle","data":{"p1":{"x":51.44491778877999,"y":54.40459995273574},"p2":{"x":53.55056861581458,"y":56.510250779770445}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7349145908262524","type":"rectangle","data":{"p1":{"x":35.20629315386839,"y":49.476155713122694},"p2":{"x":37.31194398090304,"y":51.58180654015723}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp018307640963909133","type":"rectangle","data":{"p1":{"x":51.45135708794521,"y":42.794543557801376},"p2":{"x":53.55700791497986,"y":44.900194384836}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9798505615248356","type":"rectangle","data":{"p1":{"x":37.51027439519254,"y":42.5616362694839},"p2":{"x":39.615925222227204,"y":44.66728709651858}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp054134720767317956","type":"rectangle","data":{"p1":{"x":32.97056848369576,"y":47.24300676261623},"p2":{"x":35.0053870199127,"y":49.277825298833136}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp24121436979654787","type":"rectangle","data":{"p1":{"x":53.78238338576338,"y":52.06713435575227},"p2":{"x":55.888034212797976,"y":54.17278518278687}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5483749790467487","type":"rectangle","data":{"p1":{"x":33.07359727033966,"y":30.958019173714746},"p2":{"x":35.0053870199127,"y":35.41401419606339}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7224264188314182","type":"rectangle","data":{"p1":{"x":33.07359727033966,"y":51.827787768269644},"p2":{"x":37.323534719400456,"y":53.88192420198243}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5887727300494723","type":"rectangle","data":{"p1":{"x":35.2372017898615,"y":42.794543557801376},"p2":{"x":41.959830118376004,"y":44.85511929067934}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp16641140208384075","type":"rectangle","data":{"p1":{"x":39.873497188836936,"y":45.05473756480188},"p2":{"x":48.9335911143348,"y":47.131411545592925}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9404293655527154","type":"rectangle","data":{"p1":{"x":39.873497188836936,"y":47.131411545592925},"p2":{"x":44.29729571535945,"y":49.50751293756787}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5790284043711376","type":"rectangle","data":{"p1":{"x":42.191644888324674,"y":49.739327707516736},"p2":{"x":46.61544341484719,"y":51.82566063705568}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp14115968377148302","type":"rectangle","data":{"p1":{"x":56.04257739276399,"y":28.87599841212699},"p2":{"x":60.46637591928632,"y":30.962331341666015}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9911215666839048","type":"rectangle","data":{"p1":{"x":53.78238338576338,"y":31.13619241912761},"p2":{"x":58.20618191228584,"y":33.222525348666636}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9229359877586667","type":"rectangle","data":{"p1":{"x":60.71750858673076,"y":33.334120565689716},"p2":{"x":62.64929833630396,"y":37.69674575014224}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp03975774153187217","type":"rectangle","data":{"p1":{"x":58.45731457973022,"y":33.43824187070231},"p2":{"x":60.52432961177354,"y":37.91677444012913}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp2688864035259695","type":"rectangle","data":{"p1":{"x":60.71750858673076,"y":47.185053070128816},"p2":{"x":62.784523618774045,"y":51.66358563955592}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp49434807172942263","type":"rectangle","data":{"p1":{"x":56.06189529025964,"y":54.433576798979345},"p2":{"x":60.46637591928632,"y":56.40400234354394}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp3547941895884805","type":"rectangle","data":{"p1":{"x":49.146087986787904,"y":38.148589210078086},"p2":{"x":53.569886513310294,"y":40.23492213961691}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp6149100927668762","type":"rectangle","data":{"p1":{"x":42.18681541395077,"y":31.184487162866958},"p2":{"x":44.29246624098542,"y":33.29013798990161}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp6236361675538047","type":"rectangle","data":{"p1":{"x":49.141258512413984,"y":33.50263486235468},"p2":{"x":51.246909339448706,"y":35.608285689389334}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp33083943579870945","type":"rectangle","data":{"p1":{"x":53.777553911389475,"y":47.46947475176819},"p2":{"x":55.883204738424055,"y":49.57512557880307}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp4059609980214478","type":"rectangle","data":{"p1":{"x":56.09570161087714,"y":45.03541966730623},"p2":{"x":58.201352437911794,"y":47.141070494340795}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7983374591042727","type":"rectangle","data":{"p1":{"x":49.141258512413984,"y":28.92429315586645},"p2":{"x":51.246909339448706,"y":31.02994398290113}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp458619221511277","type":"rectangle","data":{"p1":{"x":39.868667714463015,"y":35.82078256184241},"p2":{"x":41.97431854149774,"y":37.92643338887703}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp760537205040309","type":"rectangle","data":{"p1":{"x":51.45940621190172,"y":26.548191763891396},"p2":{"x":53.565057038936374,"y":28.65384259092619}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}}],"data":{"rotation":0}},{"id":"dp491477702765458","type":"rectangle","data":{"p1":{"x":48.78095245361328,"y":31.495927638679916},"p2":{"x":134.78095245361328,"y":55.62555105176587},"rotation":270}},{"id":"dp30550026210942716","type":"rectangle","data":{"p1":{"x":75.91057586669922,"y":31.495927638679916},"p2":{"x":161.91057586669922,"y":55.625551051765896},"rotation":270}},{"id":"dp205081585511121","type":"rectangle","data":{"p1":{"x":133.9753875732422,"y":0.5607393452228777},"p2":{"x":141.9753875732422,"y":86.5607393452229}}},{"id":"da6255417888001278","data":[{"x":62.85535590959171,"y":42.60671136364056},{"x":80.0093994140625,"y":42.60671136364056}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg4057455004606121","entities":[{"id":"dp8829635558448385","type":"rectangle","data":{"p1":{"x":175.3133045986259,"y":21.994717392586722},"p2":{"x":207.36796942664145,"y":51.37046218993311}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp4576128651121294","type":"rectangle","data":{"p1":{"x":178.629304626516,"y":25.03358774390483},"p2":{"x":210.68396945453168,"y":54.4093325412511}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp9782337459077366","type":"rectangle","data":{"p1":{"x":181.94530465440607,"y":28.072458095222885},"p2":{"x":213.99996948242188,"y":57.44820289256921}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"da5095274510017072","data":[{"x":142.0093994140625,"y":42.60671136364056},{"x":163.0093994140625,"y":42.60671136364056}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da7452683182568292","data":[{"x":213.62422468507543,"y":41.44820289256921},{"x":312.0093994140625,"y":41.44820289256921}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp9101006504208546","type":"doc-cube","data":{"p1":{"x":44.909614496237566,"y":162.80965058293958},"p2":{"x":82.99996948242193,"y":200.51959735681504},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da5647146191766867","data":[{"x":82.98209142684937,"y":182.93293158498426},{"x":106.2142333984375,"y":182.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg9521102190475543","entities":[{"id":"dp19818381292907983","type":"circle","data":{"p1":{"x":106.2142333984375,"y":173.1650735565724},"p2":{"x":125.74994945526123,"y":192.70078961339613}}},{"id":"dl5336932286757903","linkedId":"de42671147127769893"}]},{"id":"da8298169380593463","data":[{"x":205.0093994140625,"y":182.93293158498426},{"x":222.0093994140625,"y":182.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg949991068622825","entities":[{"id":"dp019087905739112232","type":"rectangle","data":{"p1":{"x":222.00640869140625,"y":158.80965058293958},"p2":{"x":243.00640869140625,"y":238.80965058293953}}},{"id":"dl6010164519079402","linkedId":"de9591453651554063"},{"id":"dl9415606179860345","linkedId":"de45735341519520456"},{"id":"dl6861227487454671","linkedId":"de52514505709446"}]},{"id":"da2635283354670219","data":[{"x":207.98209142684937,"y":210.55038849797864},{"x":222.0093994140625,"y":210.55038849797864}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da7988329293723304","data":[{"x":297.74994945526123,"y":182.93293158498426},{"x":313.53152789553985,"y":182.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6451961657470695","entities":[{"id":"dp8738376037206987","type":"circle","data":{"p1":{"x":313.53152789553985,"y":172.96557042970352},"p2":{"x":333.0672439523636,"y":192.50128648652725}}},{"id":"dl07766096735198125","linkedId":"de8939303688783218"}]},{"id":"da48869933214538896","data":[{"x":427.0672439523636,"y":182.73342845811538},{"x":462.0093994140625,"y":182.73342845811538}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg9004625109246001","entities":[{"id":"dg3748164866414456","entities":[{"id":"dp5509037023859227","type":"rectangle","data":{"p1":{"x":436,"y":202.37364907735088},"p2":{"x":448.65716073205886,"y":215.03080980940973}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp2177725905865473","type":"rectangle","data":{"p1":{"x":437.58214509150736,"y":203.95579416885823},"p2":{"x":450.2393058235662,"y":216.6129549009171}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp2982156234219324","type":"rectangle","data":{"p1":{"x":439.1642901830147,"y":205.5379392603656},"p2":{"x":451.82145091507357,"y":218.19509999242445}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}}],"data":{}},{"id":"dl04261871052164312","linkedId":"de7017196159240964"}]},{"id":"dg7770051742104693","entities":[{"id":"dg6879742697168143","entities":[{"id":"dp733881807495532","type":"rectangle","data":{"p1":{"x":199,"y":232.61098714345195},"p2":{"x":211.65716073205886,"y":245.2681478755108}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp9571343654651887","type":"rectangle","data":{"p1":{"x":200.58214509150736,"y":234.1931322349593},"p2":{"x":213.2393058235662,"y":246.85029296701816}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp4276722835541409","type":"rectangle","data":{"p1":{"x":202.1642901830147,"y":235.77527732646666},"p2":{"x":214.82145091507357,"y":248.43243805852552}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}}],"data":{}},{"id":"dl3016453782434083","linkedId":"de943353730681556"}]},{"id":"dg8757060045119001","entities":[{"id":"dp4296214797357958","type":"rectangle","data":{"p1":{"x":462.00640869140625,"y":157.80965058293958},"p2":{"x":483.00640869140625,"y":237.80965058293953}}},{"id":"dl3744631857488627","linkedId":"de34251506853038727"},{"id":"dl19816395846600354","linkedId":"de0897703378860828"},{"id":"dl717557293755684","linkedId":"de660336245025593"}]},{"id":"da4096156558091564","data":[{"x":483.0093994140625,"y":182.73342845811538},{"x":497.2142333984375,"y":182.73342845811538}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp19126358492857554","type":"doc-cube","data":{"p1":{"x":297.89243309975313,"y":267.09592243721903},"p2":{"x":340.15612200055915,"y":304.8058692110944},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp7816021932988355","type":"doc-cube","data":{"p1":{"x":297.89243309975313,"y":234.79350678411146},"p2":{"x":340.15612200055915,"y":272.5034535579869},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp5604777893071713","type":"doc-cube","data":{"p1":{"x":308.7457105132565,"y":277.3949244971773},"p2":{"x":351.0093994140625,"y":315.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp7934318242807215","type":"doc-cube","data":{"p1":{"x":308.7457105132565,"y":245.39492449717733},"p2":{"x":351.0093994140625,"y":283.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da5886723440129011","data":[{"x":610.0093994140625,"y":182.73342845811538},{"x":626.2142333984375,"y":182.73342845811538}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg2711048233910618","entities":[{"id":"dp9744063565275916","type":"circle","data":{"p1":{"x":626.2142333984375,"y":173.1650735565724},"p2":{"x":645.7499494552612,"y":192.70078961339613}}},{"id":"dl8909188918888535","linkedId":"de5631212479888772"}]},{"id":"dp6166308761367747","type":"doc-cube","data":{"p1":{"x":550,"y":21.809650582939582},"p2":{"x":588.0903549861844,"y":59.51959735681504},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"dp35984004071735387","type":"right-arrow","data":{"p1":{"x":591.6828238654164,"y":37.01865805716483},"p2":{"x":604.6828238654164,"y":49.523402014684365},"arrowPercentage":0.4}},{"id":"dp20135056334796086","type":"right-arrow","data":{"p1":{"x":27.682823865416367,"y":175.01865805716483},"p2":{"x":40.68282386541637,"y":187.52340201468436},"arrowPercentage":0.4}},{"id":"dg9794871144668333","entities":[{"id":"dp30648019613019284","type":"circle","data":{"p1":{"x":515.6132065083135,"y":31.2722150513234},"p2":{"x":535.1489225651372,"y":50.80793110814713}}},{"id":"dl9290812430313644","linkedId":"de8862399825472123"}]},{"id":"da874563705382023","data":[{"x":207.98209142684937,"y":232.61098714345195},{"x":207.98209142684937,"y":210.55038849797864}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da060468175387625056","data":[{"x":451.98209142684937,"y":210.55038849797864},{"x":462.0093994140625,"y":210.55038849797864}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg9769168345695671","entities":[{"id":"dg7049738960854695","entities":[{"id":"dp6476120928270528","type":"rectangle","data":{"p1":{"x":63.99359130859375,"y":130.5402473973582},"p2":{"x":76.6507520406526,"y":143.19740812941706}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp140945334013155","type":"rectangle","data":{"p1":{"x":65.57573640010105,"y":132.12239248886556},"p2":{"x":78.2328971321599,"y":144.7795532209244}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp6967821362141615","type":"rectangle","data":{"p1":{"x":67.15788149160846,"y":133.70453758037291},"p2":{"x":79.81504222366732,"y":146.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl2867078864360555","linkedId":"de9248573790762489"}]},{"id":"dp2535340361018632","type":"doc-cube","data":{"p1":{"x":163.5752569651695,"y":185.39492449717733},"p2":{"x":205.0093994140625,"y":223.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp9677376167535234","type":"doc-cube","data":{"p1":{"x":163.5752569651695,"y":153.39492449717733},"p2":{"x":205.0093994140625,"y":191.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da816214625717876","data":[{"x":125.74994945526123,"y":182.93293158498426},{"x":153.0093994140625,"y":183.08636474609375}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6055197197769788","entities":[{"id":"dp3484523225939222","type":"circle","data":{"p1":{"x":278.2142333984375,"y":173.1650735565724},"p2":{"x":297.74994945526123,"y":192.70078961339613}}},{"id":"dl7429748158984153","linkedId":"de19860656186876802"}]},{"id":"da2811811086482159","data":[{"x":243.0093994140625,"y":182.93293158498426},{"x":278.2142333984375,"y":182.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9822177726400323","data":[{"x":287.98209142684937,"y":173.1650735565724},{"x":287.98209142684937,"y":139.08636474609375}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da8248729303496711","data":[{"x":80.0093994140625,"y":139.08636474609375},{"x":287.98209142684937,"y":139.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da5594349890606285","data":[{"x":333.0672439523636,"y":182.73342845811538},{"x":385.5752569651695,"y":182.73342845811538}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp1404845983163685","type":"doc-cube","data":{"p1":{"x":385.5752569651695,"y":180.39492449717733},"p2":{"x":427.0093994140625,"y":218.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp10524773268557919","type":"doc-cube","data":{"p1":{"x":385.5752569651695,"y":148.39492449717733},"p2":{"x":427.0093994140625,"y":186.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"dg8484742129714533","entities":[{"id":"dg9038736138675647","entities":[{"id":"dp9996305414061866","type":"rectangle","data":{"p1":{"x":63.99359130859375,"y":88.19599385731914},"p2":{"x":76.6507520406526,"y":100.853154589378}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp21860303704643136","type":"rectangle","data":{"p1":{"x":65.57573640010105,"y":89.7781389488265},"p2":{"x":78.2328971321599,"y":102.43529968088535}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp8561186880022829","type":"rectangle","data":{"p1":{"x":67.15788149160846,"y":91.36028404033385},"p2":{"x":79.81504222366732,"y":104.01744477239271}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl23537597833849233","linkedId":"de3279148366297122"}]},{"id":"da5893669933322039","data":[{"x":79.81504222366732,"y":118.08636474609375},{"x":507.0093994140625,"y":118.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg5470884334023867","entities":[{"id":"dp7943579170689357","type":"circle","data":{"p1":{"x":497.2142333984375,"y":173.1650735565724},"p2":{"x":516.7499494552612,"y":192.70078961339613}}},{"id":"dl41378762513915945","linkedId":"de4170855423696589"}]},{"id":"da6067276147750311","data":[{"x":506.98209142684937,"y":173.1650735565724},{"x":506.98209142684937,"y":118.08636474609375}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da3658460936994632","data":[{"x":516.7499494552612,"y":182.93293158498426},{"x":527.5315278955399,"y":182.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg8290168484072875","entities":[{"id":"dp43094216648041606","type":"circle","data":{"p1":{"x":527.5315278955399,"y":172.96557042970352},"p2":{"x":547.0672439523636,"y":192.50128648652725}}},{"id":"dl37666879315892676","linkedId":"de8293020670412787"}]},{"id":"da9124292323903822","data":[{"x":547.0672439523636,"y":182.73342845811538},{"x":571.0093994140625,"y":182.73342845811538}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp8563869802684876","type":"doc-cube","data":{"p1":{"x":572,"y":162.80965058293958},"p2":{"x":610.0903549861844,"y":200.51959735681504},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da8350532175954528","data":[{"x":635.9820914268494,"y":283.1048712710528},{"x":635.9820914268494,"y":192.70078961339613}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da14438530859309862","data":[{"x":434.743540763855,"y":283.1048712710528},{"x":572.0093994140625,"y":283.1048712710528}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6552341923862859","entities":[{"id":"dp4114310463952291","type":"circle","data":{"p1":{"x":366.20782470703125,"y":31.691802978515625},"p2":{"x":385.743540763855,"y":51.227519035339355}}},{"id":"dl8524192395429857","linkedId":"de0411298464122003"}]},{"id":"da9857160005357748","data":[{"x":352.0093994140625,"y":41.45966100692749},{"x":366.20782470703125,"y":41.45966100692749}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg5361109596292808","entities":[{"id":"dp3737490376357602","type":"circle","data":{"p1":{"x":398.20782470703125,"y":31.7271728515625},"p2":{"x":417.743540763855,"y":51.26288890838623}}},{"id":"dl06797239555156298","linkedId":"de39442010604872957"}]},{"id":"da4043032123170953","data":[{"x":385.743540763855,"y":41.495030879974365},{"x":398.20782470703125,"y":41.495030879974365}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9273551234543298","data":[{"x":417.743540763855,"y":41.495030879974365},{"x":430.0093994140625,"y":41.495030879974365}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da5120502812969023","data":[{"x":375.9756827354431,"y":96.36028404033385},{"x":375.9756827354431,"y":51.227519035339355}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da41002029497127945","data":[{"x":407.9756827354431,"y":118.21600341796875},{"x":407.9756827354431,"y":51.26288890838623}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da027839575910060255","data":[{"x":79.81504222366732,"y":96.36028404033385},{"x":375.9756827354431,"y":96.36028404033385}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp29147501886307037","type":"doc-cube","data":{"p1":{"x":312.99359130859375,"y":41.27390942729642},"p2":{"x":352.0093994140625,"y":78.98385620117188},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp18465950721045088","type":"doc-cube","data":{"p1":{"x":312.99359130859375,"y":9.273909427296417},"p2":{"x":352.0093994140625,"y":46.983856201171875},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp7293007378919645","type":"doc-cube","data":{"p1":{"x":430.99359130859375,"y":22.273909427296417},"p2":{"x":469.0839462947781,"y":59.983856201171875},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp29862627321028845","type":"doc-cube","data":{"p1":{"x":572,"y":263.8096505829396},"p2":{"x":610.0903549861844,"y":301.51959735681504},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da881050927661438","data":[{"x":610.0093994140625,"y":283.1048712710528},{"x":635.9820914268494,"y":283.1048712710528}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da536505232054884","data":[{"x":351.32182448864523,"y":283.1048712710528},{"x":383.20782470703125,"y":283.1048712710528}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg9352496300077404","entities":[{"id":"dp8381260328807054","type":"circle","data":{"p1":{"x":482.197021484375,"y":31.320820016533332},"p2":{"x":501.73273754119873,"y":50.85653607335706}}},{"id":"dl04218115805922773","linkedId":"de5290652384541861"}]},{"id":"da1671169067994731","data":[{"x":469.0093994140625,"y":41.495030879974365},{"x":482.197021484375,"y":41.495030879974365}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da4434413038574352","data":[{"x":491.96487951278687,"y":95.21600341796875},{"x":491.96487951278687,"y":50.85653607335706}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9824275673759653","data":[{"x":491.96487951278687,"y":95.21600341796875},{"x":635.9820914268494,"y":95.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8315863874944149","data":[{"x":635.9820914268494,"y":173.1650735565724},{"x":635.9820914268494,"y":95.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8675175182676189","data":[{"x":501.73273754119873,"y":41.0886780449452},{"x":515.6132065083135,"y":41.0886780449452}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da1706452397478937","data":[{"x":535.1489225651372,"y":41.040073079735265},{"x":549.029391532252,"y":41.040073079735265}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg8999168748503741","entities":[{"id":"dp7767797686105347","type":"circle","data":{"p1":{"x":383.20782470703125,"y":273.6918029785156},"p2":{"x":402.743540763855,"y":293.22751903533936}}},{"id":"dl6027413285167649","linkedId":"de857602324837198"}]},{"id":"dg6669031335846896","entities":[{"id":"dp8030836569988877","type":"circle","data":{"p1":{"x":415.20782470703125,"y":273.7271728515625},"p2":{"x":434.743540763855,"y":293.26288890838623}}},{"id":"dl9104054636494301","linkedId":"de8463101795697547"}]},{"id":"da007300751910995107","data":[{"x":402.743540763855,"y":283.49503087997437},{"x":415.20782470703125,"y":283.49503087997437}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da10649370567532523","data":[{"x":392.9756827354431,"y":330.08636474609375},{"x":392.9756827354431,"y":293.22751903533936}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da4284726936260912","data":[{"x":424.9756827354431,"y":334.08636474609375},{"x":424.9756827354431,"y":293.26288890838623}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da819754312498066","data":[{"x":6.0093994140625,"y":118.08636474609375},{"x":63.81504222366732,"y":118.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da6859220166447162","data":[{"x":10.982091426849365,"y":139.08636474609375},{"x":64.0093994140625,"y":139.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da16116560471307007","data":[{"x":10.982091426849365,"y":330.08636474609375},{"x":392.9756827354431,"y":330.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da4402995226506323","data":[{"x":10.982091426849365,"y":330.08636474609375},{"x":10.982091426849365,"y":139.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da07365458199363362","data":[{"x":6.0093994140625,"y":334.08636474609375},{"x":6.0093994140625,"y":118.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8609599008450401","data":[{"x":6.0093994140625,"y":334.08636474609375},{"x":424.9756827354431,"y":334.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg18633038966604198","entities":[{"id":"dp23789513342027635","type":"rectangle","data":{"p1":{"x":247.00640869140625,"y":231.08636474609375},"p2":{"x":268.00640869140625,"y":321.08636474609375}}},{"id":"dl5964117034027434","linkedId":"de117272111129469"},{"id":"dl43136719617667074","linkedId":"de7615362257186091"},{"id":"dl848449371733256","linkedId":"de6516545387625636"}]},{"id":"da8132116984781697","data":[{"x":235.98209142684937,"y":269.55038849797864},{"x":247.0093994140625,"y":269.55038849797864}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da2679111615406278","data":[{"x":268.0093994140625,"y":267.09592243721903},{"x":297.8924330997532,"y":267.09592243721903}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg2436496973924449","entities":[{"id":"dp8472658757800087","type":"circle","data":{"p1":{"x":55.2142333984375,"y":211.1650735565724},"p2":{"x":74.74994945526123,"y":230.70078961339613}}},{"id":"dl6546463077814686","linkedId":"de6680758227104713"}]},{"id":"da7870207852415669","data":[{"x":64.98209142684937,"y":211.1650735565724},{"x":64.98209142684937,"y":200.55038849797864}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"dp19398203200317687","type":"doc-cube","data":{"p1":{"x":39.31076744317738,"y":273.5022752722482},"p2":{"x":77.40112242936175,"y":311.21222204612354},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp09881308613683815","type":"doc-cube","data":{"p1":{"x":39.31076744317738,"y":241.19985961914062},"p2":{"x":77.40112242936175,"y":278.9098063930161},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp45325200116230313","type":"doc-cube","data":{"p1":{"x":49.99359130859375,"y":283.8012773322065},"p2":{"x":88.08394629477812,"y":321.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp7083211951380533","type":"doc-cube","data":{"p1":{"x":49.99359130859375,"y":251.8012773322065},"p2":{"x":88.08394629477812,"y":289.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da6699254290055761","data":[{"x":93.0093994140625,"y":290.93293158498426},{"x":154.0093994140625,"y":290.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da5597155529763433","data":[{"x":64.98209142684937,"y":241.51122410608195},{"x":64.98209142684937,"y":230.70078961339613}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg299842150815365","entities":[{"id":"dp8541761199432887","type":"doc-cube","data":{"p1":{"x":219.62434362521276,"y":261.21600341796875},"p2":{"x":236.08394629477812,"y":277.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dl3981580537257483","linkedId":"de41779621283020885"}]},{"id":"dp1231293400345943","type":"doc-cube","data":{"p1":{"x":98.31076744317738,"y":235.82717669126174},"p2":{"x":136.40112242936175,"y":273.5371234651371},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp9189534433042095","type":"doc-cube","data":{"p1":{"x":98.31076744317738,"y":203.52476103815417},"p2":{"x":136.40112242936175,"y":241.23470781202963},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp07285677194005613","type":"doc-cube","data":{"p1":{"x":108.99359130859375,"y":246.12617875122004},"p2":{"x":147.08394629477812,"y":283.8361255250955},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp5541115348388084","type":"doc-cube","data":{"p1":{"x":108.99359130859375,"y":214.12617875122004},"p2":{"x":147.08394629477812,"y":251.8361255250955},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da7225287201552757","data":[{"x":115.98209142684937,"y":203.51122410608195},{"x":115.98209142684937,"y":192.70078961339613}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da1495707413591436","data":[{"x":74.74994945526123,"y":220.93293158498426},{"x":93.0093994140625,"y":220.93293158498426}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9737361179617816","data":[{"x":93.0093994140625,"y":290.93293158498426},{"x":93.0093994140625,"y":220.93293158498426}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp47773940152606587","type":"doc-cube","data":{"p1":{"x":153.89243309975313,"y":274.09592243721903},"p2":{"x":196.15612200055915,"y":311.8058692110944},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp6190514455540355","type":"doc-cube","data":{"p1":{"x":153.89243309975313,"y":241.79350678411146},"p2":{"x":196.15612200055915,"y":279.5034535579869},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp39046556118951337","type":"doc-cube","data":{"p1":{"x":164.5752569651695,"y":284.3949244971773},"p2":{"x":206.0093994140625,"y":322.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp9887279274745566","type":"doc-cube","data":{"p1":{"x":164.5752569651695,"y":252.39492449717733},"p2":{"x":206.0093994140625,"y":290.1048712710528},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da9292084301369448","data":[{"x":206.0093994140625,"y":290.93293158498426},{"x":247.0093994140625,"y":290.93293158498426}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6}],"settings":{"grid":true,"diagramHeight":337.95391845703125}}]},{"id":"n0.8643197968059031","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":5643,"delayRenderCache":{"av":5643,"map":{"n0.12264719501879284":{"n0.22684036926304696":{"w":90.6576,"h":8.4545,"bl":0.8214}},"n0.28195840591444044":{"n0.9045013624179807":{"w":64.6792,"h":8.4545,"bl":0.8214}},"n0.00554654937310417":{"n0.8635446728446938":{"w":42.164,"h":8.1019,"bl":0.8571}},"n0.7636721946274969":{"n0.7635730023714855":{"w":55.9986,"h":8.4545,"bl":0.8214}},"n0.3566822829252332":{"n0.27881606013744675":{"w":86.3173,"h":8.4545,"bl":0.8214}},"n0.4916509212070379":{"n0.27010289520160713":{"w":61.4873,"h":8.4545,"bl":0.8214}},"n0.2816604439341721":{"n0.7509404326875604":{"w":24.7215,"h":8.1019,"bl":0.8571}},"n0.004686903710433121":{"n0.29355940165675376":{"w":24.7215,"h":8.1019,"bl":0.8571}},"n0.8920883669508386":{"n0.19712993762208386":{"w":61.9755,"h":8.4545,"bl":0.8214}},"n0.8068253129909273":{"n0.008391880325343104":{"w":22.4157,"h":12.5054,"bl":0.7021}},"n0.10589766223614272":{"n0.15906262428338502":{"w":15.8511,"h":12.5054,"bl":0.7021}},"n0.5973717047898972":{"n0.30799020377446107":{"w":6.9897,"h":9.4491,"bl":0.8402}},"n0.04010641624309197":{"n0.13534933903798363":{"w":6.7455,"h":9.4491,"bl":0.8402}},"n0.8554662319877668":{"n0.22137403373846753":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.2742966032445735":{"n0.9115976780097668":{"w":22.8226,"h":8.4545,"bl":0.8214}},"n0.12142712283211354":{"n0.48014294592380113":{"w":24.5135,"h":8.4545,"bl":0.8214}},"n0.3223836254719801":{"n0.4664481726460583":{"w":30.0022,"h":12.5054,"bl":0.7021}},"n0.27303294008700485":{"n0.20807316996563263":{"w":21.8099,"h":8.1019,"bl":0.8571}},"n0.8868465557438261":{"n0.13555213879565464":{"w":12.424,"h":12.5326,"bl":0.8268}},"n0.33986799877509544":{"n0.5903833754603707":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.8891057395138631":{"n0.5592823458575049":{"w":58.5033,"h":8.4545,"bl":0.8214}},"n0.1846677557628713":{"n0.25774265518288164":{"w":32.4165,"h":12.5054,"bl":0.7021}},"n0.009969838646760376":{"n0.20304082800058465":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.4797470730986":{"n0.08150258236245111":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.8679679641366074":{"n0.4032393424919807":{"w":11.6193,"h":8.4545,"bl":0.8214}},"n0.4464515627733918":{"n0.864399840513006":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.8024924706930465":{"n0.12698408810015294":{"w":18.1297,"h":12.5054,"bl":0.7021}},"n0.766638339102051":{"n0.7058263596247902":{"w":7.4599,"h":8.4545,"bl":0.8214}},"n0.47147723642626493":{"n0.6254596818194615":{"w":8.5901,"h":8.4545,"bl":0.8214}},"n0.1167764301657912":{"n0.9369673044431397":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.7503090051164691":{"n0.18446577248835783":{"w":28.9352,"h":8.4545,"bl":0.8214}},"n0.24506231822248026":{"n0.7568409456873406":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.6615254849573731":{"n0.5064483700922966":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.8685308613044107":{"n0.14447215791313917":{"w":18.1297,"h":12.5054,"bl":0.7021}},"n0.8258704275455162":{"n0.35291789532253914":{"w":35.3823,"h":8.1019,"bl":0.8571}},"n0.08237313594205076":{"n0.3200974499624347":{"w":68.2961,"h":8.1019,"bl":0.8571}},"n0.2339738641536926":{"n0.8414305306060739":{"w":25.7161,"h":12.5054,"bl":0.7021}},"n0.20649554028200523":{"n0.4237285521604277":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.7023420069695498":{"n0.08267215938659933":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.23124838131896186":{"n0.8847247660066546":{"w":30.3819,"h":8.4545,"bl":0.8214}},"n0.5653478407878947":{"n0.8935425919742013":{"w":32.3079,"h":8.4545,"bl":0.8214}},"n0.03826225597296773":{"n0.5966198281161046":{"w":6.0764,"h":8.4545,"bl":0.8214}},"n0.3114158995400982":{"n0.16051818902884407":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.832831636206383":{"n0.2738713707452638":{"w":30.5718,"h":8.4545,"bl":0.8214}},"n0.44294341390001013":{"n0.19072972727490445":{"w":30.0022,"h":12.5054,"bl":0.7021}},"n0.8001658363143611":{"n0.2555656084479139":{"w":29.4687,"h":9.1146,"bl":0.7619}},"n0.8962696595786119":{"n0.8072900678294179":{"w":37.5434,"h":8.4545,"bl":0.8214}},"n0.7546823378521905":{"n0.960824309431972":{"w":52.861,"h":8.4545,"bl":0.8214}},"n0.7185940494962384":{"n0.7675969773404887":{"w":37.5434,"h":8.4545,"bl":0.8214}},"n0.934508072726157":{"n0.15127848760257478":{"w":48.7739,"h":8.4545,"bl":0.8214}},"n0.7840692535254685":{"n0.8705964676783371":{"w":48.7739,"h":8.4545,"bl":0.8214}}}}}

==> sIPOMDPLite-Net(arXiv)/plots/docs/b89772eb-8011-46b7-a78f-95fb2bd8066b <==
{"id":"n0.8628316918407355","lines":[{"id":"n0.562747597967387","blocks":[]},{"id":"n0.5273559793818359","blocks":[{"id":"n0.8236255645064039","text":"\\diagram","type":"composite","elements":{"de49825060737485827":{"id":"de49825060737485827","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.49455426490344423"}],"id":"n0.3700714401035192"}],"id":"n0.507439450247194"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.05259571325594736"}],"id":"n0.03200298763200937"}],"shape":{"data":{"p":{"x":43.51719895786459,"y":44.62593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8392772638175428":{"id":"de8392772638175428","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"K","id":"n0.3280016587529575"}],"id":"n0.16000872253933585"}],"id":"n0.8754298217202812"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.24308943320830023"},{"text":"-recurrence","style":{"fontSize":{"value":0.4}},"id":"n0.21761928944529574"}],"style":{"align":"center"},"id":"n0.6188698522177833"}],"shape":{"data":{"p":{"x":40.48858574589599,"y":50.62593476262708},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7341561404291017":{"id":"de7341561404291017","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"U","id":"n0.14414333629632226"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"0","id":"n0.5905869300100071"}],"id":"n0.4959477743407148"}],"id":"n0.8219514388463278"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.26550122080025473"}],"id":"n0.9834551544666157"}],"id":"n0.027947209104751458"}},"id":"n0.860745668223655"},{"type":"single","text":"(","id":"n0.32172556728556234"},{"text":"s","id":"n0.23871287102752237"},{"type":"single","text":")","id":"n0.32322946097667593"}],"id":"n0.13909617635472848"}],"id":"n0.3405674873132667"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6065860912160819"}],"style":{"align":"center"},"id":"n0.9330200118644694"}],"shape":{"data":{"p":{"x":15.006408691406207,"y":47.249469301363774},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de878652079817785":{"id":"de878652079817785","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.9958750569996075","text":"\\overline","type":"composite","elements":{"value":{"id":"n0.8274210037083352","lines":[{"id":"n0.7895789030039244","blocks":[{"id":"n0.43073904367060356","text":"R"},{"id":"n0.9535602388338378","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.536952360116205","lines":[{"id":"n0.5762810627605497","blocks":[{"id":"n0.3884757344320906","text":"i"}]}]}}}]}]}}},{"type":"single","text":"(","id":"n0.15628260744819755"},{"text":"s,a","id":"n0.1681254651066575"},{"type":"single","text":")","id":"n0.8467666474282782"}],"id":"n0.960706236887447"}],"id":"n0.019004960502556623"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7380032901435976"}],"style":{"align":"center"},"id":"n0.5577433365257503"}],"shape":{"data":{"p":{"x":182.99999999999994,"y":219.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7882416035892696":{"id":"de7882416035892696","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.8070505170474311"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K-1","id":"n0.7820588648858702"}],"id":"n0.05204179071363346"}],"id":"n0.7461165093705924"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6797434591650722"}],"id":"n0.9780683932837613"}],"id":"n0.20405798469217795"}},"id":"n0.6767929484781436"},{"type":"single","text":"(","id":"n0.2979368193140759"},{"text":"s,a","id":"n0.6780472158337372"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.16812272379692583"}],"id":"n0.48746411688136204"}],"id":"n0.8678109095937245"}},"id":"n0.8473536042680254"},{"type":"single","text":")","id":"n0.4158045198032194"}],"id":"n0.6959331038941989"}],"id":"n0.4540862647774402"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8650872834849428"}],"style":{"align":"center"},"id":"n0.7460705152308109"}],"shape":{"data":{"p":{"x":97.99999999999994,"y":28.307382940085972},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8829192640173664":{"id":"de8829192640173664","lines":[{"blocks":[{"style":{"fontSize":"\\tiny"},"text":"max","id":"n0.09150222951303144"}],"id":"n0.41006002604551295"}],"shape":{"data":{"p":{"x":141.9161720677406,"y":43.48307625737806},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6212929260153228":{"id":"de6212929260153228","lines":[{"blocks":[{"text":"over ","style":{"fontSize":{"value":0.4}},"id":"n0.3759199150140131"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"A","id":"n0.8115277575240654"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7678858912569642"}],"id":"n0.27427660411047583"}],"id":"n0.7064297452925781"}},"id":"n0.5252128827500564"}],"id":"n0.4306183045431822"}],"id":"n0.7517415472449318"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.09107955876747975"}],"style":{"align":"center"},"id":"n0.1754719445147397"}],"shape":{"data":{"p":{"x":139.02611356688283,"y":57.07236067739149},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6961368095322311":{"id":"de6961368095322311","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"U","id":"n0.7420053721935991"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K-1","id":"n0.8374766026964253"}],"id":"n0.9292519201634248"}],"id":"n0.678570655622885"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.20744229043569407"}],"id":"n0.6341865633801596"}],"id":"n0.13966502816369797"}},"id":"n0.451547018102906"},{"type":"single","text":"(","id":"n0.83564795344481"},{"text":"s","id":"n0.9551868824980847"},{"type":"single","text":")","id":"n0.05549337685606481"}],"id":"n0.04906427405686231"}],"id":"n0.408476759756512"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5547124045533918"}],"style":{"align":"center"},"id":"n0.8132906214521824"}],"shape":{"data":{"p":{"x":182.0064086914062,"y":48.249469301363774},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de04836713429619688":{"id":"de04836713429619688","lines":[{"blocks":[{"text":"3D convolutional layer","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.9255886619942555"}],"style":{"align":"center"},"id":"n0.5044981362680492"}],"shape":{"data":{"p":{"x":400.7522976254404,"y":20.737859009608997},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4304294819132035":{"id":"de4304294819132035","lines":[{"blocks":[{"text":"Filter: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.7411218868021072"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×3×3×1×|A","style":{"mathModeType":"\\displaystyle"},"id":"n0.7439831288651368"},{"id":"n0.20038780616676166","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5273071114603862","lines":[{"id":"n0.2630313592514699","blocks":[{"id":"n0.9486521416434981","text":"i"}]}]}},"style":{"mathModeType":"\\displaystyle"}},{"text":"|","id":"n0.4331918560462156","style":{"mathModeType":"\\displaystyle"}}],"id":"n0.24224066795434895"}],"id":"n0.4948186869059896"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8823231620659291"}],"style":{"align":"center"},"id":"n0.063711797895871"}],"shape":{"data":{"p":{"x":392.51716844028647,"y":13.625934762627082},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1540081823410162":{"id":"de1540081823410162","lines":[{"blocks":[{"text":"Stride: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.04887852559195127"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1","id":"n0.0006046228652674124"}],"id":"n0.8114851563395926"}],"id":"n0.03631791790874783"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.37639896831524444"}],"style":{"align":"center"},"id":"n0.08980327572054025"}],"shape":{"data":{"p":{"x":385.52020640099363,"y":25.813468264617768},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6418911130447893":{"id":"de6418911130447893","lines":[{"blocks":[{"text":"3D convolutional layer","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.5579558575718451"}],"style":{"align":"center"},"id":"n0.9240321464139629"}],"shape":{"data":{"p":{"x":269.7522976254404,"y":23.737859009608997},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4386358202714504":{"id":"de4386358202714504","lines":[{"blocks":[{"text":"Filter: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.9095064291184971"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×3×3×1×|A","style":{"mathModeType":"\\displaystyle"},"id":"n0.805560192272305"},{"id":"n0.1918696226589085","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.4184995246269638","lines":[{"id":"n0.20172986713473895","blocks":[{"id":"n0.2338179798265101","text":"j"}]}]}},"style":{"mathModeType":"\\displaystyle"}},{"text":"|","id":"n0.6775938225632441","style":{"mathModeType":"\\displaystyle"}}],"id":"n0.10192837968410129"}],"id":"n0.10368321027700222"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6585904782524061"}],"style":{"align":"center"},"id":"n0.2141492919151311"}],"shape":{"data":{"p":{"x":261.51716844028647,"y":16.625934762627082},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9007883307111533":{"id":"de9007883307111533","lines":[{"blocks":[{"text":"Stride: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.24564546709807833"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1","id":"n0.788064759206107"}],"id":"n0.1471848314421922"}],"id":"n0.6113778876903095"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.542137284137528"}],"style":{"align":"center"},"id":"n0.15125705242321952"}],"shape":{"data":{"p":{"x":254.52020640099363,"y":28.813468264617768},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5541208246815192":{"id":"de5541208246815192","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.5041178283729908"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.9002246682459194"}],"id":"n0.5324681959368309"}],"id":"n0.5467348900570257"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5764000405107381"}],"id":"n0.7042306286918925"}],"id":"n0.8276904729959691"}},"id":"n0.24336808018267586"},{"type":"single","text":"(","id":"n0.8353469868189909"},{"text":"s,a","id":"n0.26468356341896015"},{"type":"single","text":")","id":"n0.30937765220020563"}],"id":"n0.25329414575928455"}],"id":"n0.8174948536978763"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5628238923487163"}],"style":{"align":"center"},"id":"n0.2604262847326111"}],"shape":{"data":{"p":{"x":424,"y":32.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de6127666039309161":{"id":"de6127666039309161","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.27594370866893114"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.3189564528479387"}],"id":"n0.8008403275771725"}],"id":"n0.16008272810937152"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5568189705645645"}],"id":"n0.9004139476633783"}],"id":"n0.9550466807690905"}},"id":"n0.38090799160040656"},{"type":"single","text":"(","id":"n0.3822111221954114"},{"text":"s,a","id":"n0.2356453221454542"},{"type":"single","text":")","id":"n0.8604232677303914"}],"id":"n0.7081331412186238"}],"id":"n0.6850706070771972"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.028734220868174454"}],"style":{"align":"center"},"id":"n0.43185577108968776"}],"shape":{"data":{"p":{"x":627,"y":185.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de28435527997219756":{"id":"de28435527997219756","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.08705093799143793"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.5891023591185407"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.9745168370340724"}],"id":"n0.958791673039098"}],"id":"n0.5039758522513191"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.5077092681029911"}],"id":"n0.864499051948938"}],"id":"n0.8320198695658971"}},"id":"n0.33459736015383257"}],"id":"n0.7615972764891554"}],"id":"n0.7244497752506611"}},"id":"n0.9720753771004256"},{"type":"single","text":"(","id":"n0.8591747481643697"},{"text":"s,a","id":"n0.17031193184549975"},{"type":"single","text":")","id":"n0.26795896373366945"}],"id":"n0.36970927642703466"}],"id":"n0.9153175281526549"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.30265450177445663"}],"style":{"align":"center"},"id":"n0.13500136400373175"}],"shape":{"data":{"p":{"x":477.58166565657575,"y":105.83474321560152},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de23402032048605892":{"id":"de23402032048605892","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1-","id":"n0.9148565968805094"},{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.06176305597570009"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.9604509141810909"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.6769009588768056"}],"id":"n0.8034744293145191"}],"id":"n0.06201144688230409"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.18625086752317932"}],"id":"n0.5951331231125816"}],"id":"n0.394072288365348"}},"id":"n0.20412815548829943"}],"id":"n0.7549304966285213"}],"id":"n0.4586129786426738"}},"id":"n0.7666961378815713"}],"id":"n0.31354421293919166"}],"id":"n0.047463607109459405"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.06354871958030639"}],"style":{"align":"center"},"id":"n0.8712918476355476"}],"shape":{"data":{"p":{"x":545.5816656565758,"y":106.30738294008597},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5414059609216073":{"id":"de5414059609216073","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⊤","id":"n0.3037765506455372"}],"id":"n0.3258322941087266"}],"id":"n0.38197129936659513"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7703953942288464"}],"id":"n0.5926678419513765"}],"shape":{"data":{"p":{"x":483.9161720677406,"y":44.17643163575815},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de5279245661967291":{"id":"de5279245661967291","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.1348097845975078"}],"id":"n0.09263916432355268"}],"id":"n0.4522059294213938"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.40620553658268865"}],"id":"n0.5650827310011799"}],"shape":{"data":{"p":{"x":535.5171989578646,"y":43.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de3842459334625856":{"id":"de3842459334625856","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.09128646721982836"}],"id":"n0.1645121089452033"}],"id":"n0.30112295613345186"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9229260139686721"}],"id":"n0.9912310077698254"}],"shape":{"data":{"p":{"x":230.5171989578646,"y":220.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6724674073740904":{"id":"de6724674073740904","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.6536524566939939"}],"id":"n0.8208839175415283"}],"id":"n0.07669072170856572"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5594436296680694"}],"id":"n0.77373365802956"}],"shape":{"data":{"p":{"x":576.1657782593641,"y":185.6259652802052},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de16664139451638227":{"id":"de16664139451638227","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⊤","id":"n0.2968545073165423"}],"id":"n0.3700267897409688"}],"id":"n0.687359062348055"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.29203876646287985"}],"id":"n0.5391793768832565"}],"shape":{"data":{"p":{"x":323.9161720677406,"y":45.17643163575815},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8268699887031468":{"id":"de8268699887031468","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.3915984754793784"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.3417202940877271"}],"id":"n0.7534884352237681"}],"id":"n0.7440048651355136"}},"id":"n0.05589435437227719"}],"id":"n0.4447440037807877"}],"id":"n0.7100476968630136"}},"id":"n0.4846887253442911"}],"id":"n0.7635891487221897"}],"id":"n0.6377335918019102"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.09659427055567638"}],"id":"n0.19349664935775568"}],"shape":{"data":{"p":{"x":209.59887757063825,"y":13.661304635673957}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de8705375563265205":{"id":"de8705375563265205","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.9552801703362863"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.34683177399551446"}],"id":"n0.30677207232372883"}],"id":"n0.355649984111561"}},"id":"n0.14589399605715192"}],"id":"n0.07548818109930044"}],"id":"n0.8021436907932609"}},"id":"n0.7115273960748678"}],"id":"n0.773475139164786"}],"id":"n0.769201243672291"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.00392747107489777"}],"id":"n0.8926299965974056"}],"shape":{"data":{"p":{"x":326.59887757063825,"y":12.625934762627082}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de23681891905315045":{"id":"de23681891905315045","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.8953639408865319"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.4149842063285205"}],"id":"n0.19796433252479173"}],"id":"n0.7872800310627679"}},"id":"n0.7339670170784438"},{"text":"|","id":"n0.6835423634317954"}],"id":"n0.9774562041920496"}],"id":"n0.04103796103922863"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.020117516451057416"}],"style":{"align":"center"},"id":"n0.34896747346457"}],"shape":{"data":{"p":{"x":-4,"y":2.983856201171875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de48398552182920707":{"id":"de48398552182920707","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.9266641391509445"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.5568862477146572"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.33934474488506416"}],"id":"n0.931750154936541"}],"id":"n0.057924422351373295"}},"id":"n0.8902100788558625"}],"id":"n0.4967429723445542"}],"id":"n0.36540566276141506"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.38746857642979204"}],"id":"n0.8869775529225605"}],"id":"n0.526142623353475"}},"id":"n0.5603748434152191"}],"id":"n0.6524612630217288"}],"id":"n0.8651163527017454"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7428763826954485"}],"id":"n0.5887641859815747"}],"shape":{"data":{"p":{"x":9.99359130859375,"y":-3.4417227080760426}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de48673237968752736":{"id":"de48673237968752736","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.23292943631388763"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.3016682683679175"}],"id":"n0.025440374297824198"}],"id":"n0.6127761903648783"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4666539713796616"}],"id":"n0.668351275345753"}],"id":"n0.2767409612998937"}},"id":"n0.724881061692201"},{"type":"single","text":"(","id":"n0.31414876243208134"},{"text":"s,a","id":"n0.9864117007105992"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.1248712269325194"}],"id":"n0.06525388807431942"}],"id":"n0.5646104364600255"}},"id":"n0.07435533398861138"},{"type":"single","text":")","id":"n0.5624481888687876"}],"id":"n0.4248082564228923"}],"id":"n0.6138080945790303"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.10695921374173234"}],"style":{"align":"center"},"id":"n0.7097339872021309"}],"shape":{"data":{"p":{"x":278.4011224293617,"y":33.68144817745889},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8846298562061499":{"id":"de8846298562061499","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.9240098393557779"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.15499462180864287"}],"id":"n0.4318738583219519"}],"id":"n0.5324136919490754"}},"id":"n0.03725379254995542"},{"text":"×W","id":"n0.5377241879080408"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.006083119336494969"}],"id":"n0.7914171866983244"}],"id":"n0.09591925744493657"}},"id":"n0.3132651821130823"},{"text":"×H","id":"n0.5004129826576436"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.7914725656335135"}],"id":"n0.1666645969839271"}],"id":"n0.21297786696722532"}},"id":"n0.8885724783469957"},{"text":"×W","id":"n0.6576475851357684"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.811406949344728"}],"id":"n0.3269255955473507"}],"id":"n0.9914809921042727"}},"id":"n0.649669996204548"},{"text":"×|A","id":"n0.3569691578905021"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.0812859212449546"}],"id":"n0.44980866937891073"}],"id":"n0.9576709953840956"}},"id":"n0.5893869902083619"},{"text":"|×|A","id":"n0.9021067821601803"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8935952646673961"}],"id":"n0.16896322121170715"}],"id":"n0.5754560664408199"}},"id":"n0.3914541099875819"},{"text":"|","id":"n0.8576312480942625"}],"id":"n0.15286703063243756"}],"id":"n0.9346331450716716"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7420023035191288"}],"style":{"align":"center"},"id":"n0.28601838441576555"}],"shape":{"data":{"p":{"x":354,"y":281.9838562011719},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9056851396423851":{"id":"de9056851396423851","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.3975583049207363"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.06300427758300442"}],"id":"n0.20985140923926293"}],"id":"n0.7920020741174281"}},"id":"n0.6124542089220948"},{"text":"×W","id":"n0.52786224995756"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6476996367412975"}],"id":"n0.19763128347540593"}],"id":"n0.5508098725003492"}},"id":"n0.1896532976045786"},{"text":"×H","id":"n0.6288155425985547"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.007222502636268002"}],"id":"n0.054198563577345205"}],"id":"n0.6690767590448217"}},"id":"n0.43593740460130137"},{"text":"×W","id":"n0.5201671469445934"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.828782969496656"}],"id":"n0.11314837801358313"}],"id":"n0.7490363675695493"}},"id":"n0.8263341454929529"}],"id":"n0.522341707304876"}],"id":"n0.4658812440199587"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5435050101233148"}],"style":{"align":"center"},"id":"n0.9664266160818378"}],"shape":{"data":{"p":{"x":-2,"y":66.80793110814716},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de17725590586649997":{"id":"de17725590586649997","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.7697015924694854"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9255487288302668","text":"i"}],"id":"n0.7188220392736842"}],"id":"n0.6556097098409805"}},"id":"n0.9550082434015339"},{"text":"×W","id":"n0.22086728083849638"},{"id":"n0.10686891860923686","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7950620791776775","lines":[{"id":"n0.9773869714200802","blocks":[{"id":"n0.7852054377104776","text":"i"}]}]}}},{"text":"×H","id":"n0.17503155648954793"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.2236222367379872"}],"id":"n0.015536579478339307"}],"id":"n0.4474869123314231"}},"id":"n0.7683706952890572"},{"text":"×W","id":"n0.37544184562018157"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.26205685100766263"}],"id":"n0.8192353100200187"}],"id":"n0.9808450237463693"}},"id":"n0.7732845998155922"}],"id":"n0.7037197434395268"}],"id":"n0.6779540611266668"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.832519388159987"}],"style":{"align":"center"},"id":"n0.7153854145196572"}],"shape":{"data":{"p":{"x":139,"y":68.80793110814716},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8020780160490844":{"id":"de8020780160490844","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.19254118440377188"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.026708629040808507"}],"id":"n0.09432173819124712"}],"id":"n0.8686400357039945"}},"id":"n0.4802286381463339"},{"text":"×W","id":"n0.17312173914197304"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.2786013489390031"}],"id":"n0.16553076516208476"}],"id":"n0.0593824842978008"}},"id":"n0.882010426100716"},{"text":"×H","id":"n0.41778977561438135"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.08879210981933316"}],"id":"n0.52338464392984"}],"id":"n0.7557619000986653"}},"id":"n0.0884478826117927"},{"text":"×W","id":"n0.27385964723967615"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.1339468242647479"}],"id":"n0.7932762094562638"}],"id":"n0.7933576266650011"}},"id":"n0.10511854772275031"},{"text":"×|A","id":"n0.992631034430089"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.21675636965666656"}],"id":"n0.7762497937584696"}],"id":"n0.42825336586871243"}},"id":"n0.5203396537118956"},{"text":"|","id":"n0.9659200368612286"}],"id":"n0.3315585301606032"}],"id":"n0.2594341695196014"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.42799371253152896"}],"style":{"align":"center"},"id":"n0.6841868762211407"}],"shape":{"data":{"p":{"x":81.49929038471396,"y":80.21600341796875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de35837508646930627":{"id":"de35837508646930627","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.6752105647865525"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.5421777995235713","text":"i"}],"id":"n0.6673260548869122"}],"id":"n0.9149894207372442"}},"id":"n0.4884171265223254"},{"text":"|×H","id":"n0.31802552971937215"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8552332406632621"}],"id":"n0.0023972541780015177"}],"id":"n0.9653179998027317"}},"id":"n0.10300070602660427"},{"text":"×W","id":"n0.8554204348452248"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8818196953034094"}],"id":"n0.6501696933127412"}],"id":"n0.8035121608949127"}},"id":"n0.24019777675753962"},{"text":"×|A","id":"n0.9243501476649474"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.6066945677921896","text":"j"}],"id":"n0.0752357949125324"}],"id":"n0.005099696887602478"}},"id":"n0.3694483709039966"},{"text":"|","id":"n0.22700339936023584"}],"id":"n0.035945705013095575"}],"id":"n0.8035966151360414"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9934441125242666"}],"style":{"align":"center"},"id":"n0.7339952625586599"}],"shape":{"data":{"p":{"x":254.49929038471396,"y":86.21600341796875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de44431680897613113":{"id":"de44431680897613113","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.30503785226816715"},{"id":"n0.12058067480096524","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.14472103467257824","lines":[{"id":"n0.47748592585873983","blocks":[{"id":"n0.017744946456977884","text":"j"}]}]}}},{"text":"×A","id":"n0.8678266411174607"},{"id":"n0.3546478795143535","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9368869249435956","lines":[{"id":"n0.706322193982863","blocks":[{"id":"n0.7336895096776936","text":"j"}]}]}}},{"text":"|×H","id":"n0.09055987566643942"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4715056720982993","text":"i"}],"id":"n0.010659160438502013"}],"id":"n0.4276082222151729"}},"id":"n0.468399590720896"},{"text":"×W","id":"n0.8798716378432485"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7710942261178746","text":"i"}],"id":"n0.750499963069041"}],"id":"n0.2905758440450652"}},"id":"n0.5549385663006416"},{"text":"×|A","id":"n0.06074146956194504"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9280595346450058","text":"i"}],"id":"n0.7785574871342951"}],"id":"n0.4945902397594186"}},"id":"n0.6548284470302579"},{"text":"|","id":"n0.20016963550019895"}],"id":"n0.9974246527053048"}],"id":"n0.8652985179455455"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9486350789859588"}],"style":{"align":"center"},"id":"n0.041652101070513536"}],"shape":{"data":{"p":{"x":380.49929038471396,"y":86.21600341796875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de11129279367613587":{"id":"de11129279367613587","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.43190907136130297"}],"style":{"align":"center"},"id":"n0.9233886406772411"}],"shape":{"data":{"p":{"x":209.59887757063825,"y":34.300435473167056},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4390051875579064":{"id":"de4390051875579064","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.28249310277124473"}],"style":{"align":"center"},"id":"n0.33436862044616644"}],"shape":{"data":{"p":{"x":339.76316775365297,"y":34.429355783134895},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1507135434759932":{"id":"de1507135434759932","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.4872662421724989"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.1096318083339114","text":"j"}],"id":"n0.08828378784498514"}],"id":"n0.4313687052503603"}},"id":"n0.602195369768934"},{"text":"×A","id":"n0.9082697695415494"},{"id":"n0.2835671734457961","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6971546230925536","lines":[{"id":"n0.7992977157443393","blocks":[{"id":"n0.8876145669787254","text":"j"}]}]}}},{"text":"|×H","id":"n0.716329668428678"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9107067680455683","text":"i"}],"id":"n0.5384319111418014"}],"id":"n0.3603334496393018"}},"id":"n0.2766257768924789"},{"text":"×W","id":"n0.5241081903205831"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.46252002726247676","text":"i"}],"id":"n0.35424214207291405"}],"id":"n0.7505731487542968"}},"id":"n0.8393193586503307"}],"id":"n0.4120157811821672"}],"id":"n0.40235662659270877"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.07942332055987467"}],"style":{"align":"center"},"id":"n0.8941317310966974"}],"shape":{"data":{"p":{"x":306.2671484131258,"y":57.96521918264051},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de522171948209275":{"id":"de522171948209275","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.07347982487587168"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6943621769917845"}],"id":"n0.8538407585486798"}],"id":"n0.23779598982390726"}},"id":"n0.9994533451097276"},{"text":"×W","id":"n0.5641323880399061"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7655910428307564"}],"id":"n0.0744036343268597"}],"id":"n0.8624241408950293"}},"id":"n0.5632405278854995"},{"text":"×H","id":"n0.38042025325061846"},{"id":"n0.6900959648010496","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.11219020746017283","lines":[{"id":"n0.03178520695856757","blocks":[{"id":"n0.5553908242528094","text":"j"}]}]}}},{"text":"×W","id":"n0.454434201497254"},{"id":"n0.5384307991107282","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7520327457247449","lines":[{"id":"n0.7277586400121654","blocks":[{"id":"n0.7354762063033926","text":"j"}]}]}}},{"text":"×|A","id":"n0.22485390461849852"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.408823091251288"}],"id":"n0.16585619659351103"}],"id":"n0.2924015559398825"}},"id":"n0.9146328100298982"},{"text":"|×|A","id":"n0.6720662299968945"},{"id":"n0.2227552496632479","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5039818588024179","lines":[{"id":"n0.9567124009660033","blocks":[{"id":"n0.758271073863773","text":"j"}]}]}}},{"text":"|","id":"n0.4681849489955767"}],"id":"n0.8672176115946004"}],"id":"n0.5663416250436877"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7955583954820513"}],"style":{"align":"center"},"id":"n0.524381383059356"}],"shape":{"data":{"p":{"x":450.60827698470075,"y":57.215249700218635},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de04941809146159737":{"id":"de04941809146159737","lines":[{"blocks":[{"text":"reshape","style":{"fontSize":{"value":0.4}},"id":"n0.916266029563227"}],"style":{"align":"center"},"id":"n0.0991665152370298"}],"shape":{"data":{"p":{"x":452.68282386541637,"y":34.30738294008598},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6620171831553086":{"id":"de6620171831553086","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.06644675650866261"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5812713175375215"}],"id":"n0.9600611837462389"}],"id":"n0.08529489713954752"}},"id":"n0.8646489637780295"},{"text":"×W","id":"n0.8089785591043599"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.07684623624518028"}],"id":"n0.29565576360943635"}],"id":"n0.35672593270715947"}},"id":"n0.6798175258010559"},{"text":"×H","id":"n0.5071816299008141"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5787419699083496"}],"id":"n0.844131361406786"}],"id":"n0.6818487507936537"}},"id":"n0.15833282812438276"},{"text":"×W","id":"n0.9130348269297166"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.3777307375122563"}],"id":"n0.24573635349157308"}],"id":"n0.10589104972322194"}},"id":"n0.07698402670484605"},{"text":"×|A","id":"n0.8504775928759356"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7788587289830557"}],"id":"n0.22215615429686775"}],"id":"n0.20835969360451156"}},"id":"n0.4127374457395061"},{"text":"|×|A","id":"n0.028993692012068584"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.6303562730740266"}],"id":"n0.12768825363388836"}],"id":"n0.9790385343606987"}},"id":"n0.46668316132436494"},{"text":"|","id":"n0.837018209659206"}],"id":"n0.4139531593661605"}],"id":"n0.2688194492057001"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7634823240114856"}],"style":{"align":"center"},"id":"n0.7873382932403481"}],"shape":{"data":{"p":{"x":490.60827698470075,"y":159.21524970021864},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de11098522098733432":{"id":"de11098522098733432","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.30690009171114196"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5919306379608547"}],"id":"n0.7979906207756955"}],"id":"n0.3081021407237814"}},"id":"n0.8316015393846763"},{"text":"×W","id":"n0.8769431682553834"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.40798222036222587"}],"id":"n0.7503499867028827"}],"id":"n0.3148845401510407"}},"id":"n0.8642976180964292"},{"text":"×H","id":"n0.2519436465858962"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.03898210518009182"}],"id":"n0.7871624906068271"}],"id":"n0.787894730359483"}},"id":"n0.9967576722087257"},{"text":"×W","id":"n0.16617853467699106"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.6465546664341582"}],"id":"n0.0544832208057191"}],"id":"n0.34225070472881414"}},"id":"n0.8689876849907643"},{"text":"×|A","id":"n0.738367115137506"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7432839740810651"}],"id":"n0.2521045996472795"}],"id":"n0.3590950542783178"}},"id":"n0.8911538754232573"},{"text":"|×|A","id":"n0.33713830235063225"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.1799236854589148"}],"id":"n0.09029960826674222"}],"id":"n0.7852857038869694"}},"id":"n0.40885625536349934"},{"text":"|","id":"n0.7311220792156645"}],"id":"n0.3127101080275474"}],"id":"n0.8434406802059295"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6334771093928775"}],"style":{"align":"center"},"id":"n0.24022153427204107"}],"shape":{"data":{"p":{"x":376.60827698470075,"y":149.21524970021864},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9498932232987138":{"id":"de9498932232987138","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.05817662287806291"}],"id":"n0.8226545479203107"}],"id":"n0.14671194271672894"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.16502998636958033"}],"id":"n0.24002220610340408"}],"shape":{"data":{"p":{"x":479.5171989578646,"y":185.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de21836601327672356":{"id":"de21836601327672356","lines":[{"blocks":[{"text":"4D convolutional layer","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.5581912545269967"}],"style":{"align":"center"},"id":"n0.2222051032077259"}],"shape":{"data":{"p":{"x":260.7522976254404,"y":113.11192424698191},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5046958092324985":{"id":"de5046958092324985","lines":[{"blocks":[{"text":"Filter: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.808913255521164"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3×3×3×3×1×|A|","style":{"mathModeType":"\\displaystyle"},"id":"n0.614441534176204"}],"id":"n0.2070918756904696"}],"id":"n0.8084507466865571"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.06910730168479695"}],"style":{"align":"center"},"id":"n0.9327962624050163"}],"shape":{"data":{"p":{"x":252.51716844028647,"y":101},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de20876449516190876":{"id":"de20876449516190876","lines":[{"blocks":[{"text":"Stride: ","style":{"fontSize":{"value":0.4},"fontName":"ptm"},"id":"n0.6171687124432887"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1×1","id":"n0.5768882542983327"}],"id":"n0.5764231602461787"}],"id":"n0.4078630694843064"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.18145225750901695"}],"style":{"align":"center"},"id":"n0.981925283009887"}],"shape":{"data":{"p":{"x":245.52020640099363,"y":115.18753350199069},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5418541516011492":{"id":"de5418541516011492","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"T","id":"n0.7688004359587917"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3796404679311245"}],"id":"n0.2753147448993347"}],"id":"n0.9936634121326251"}},"id":"n0.49998465427461736"}],"id":"n0.29351627084059895"}],"id":"n0.1325705150031895"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5881905538269003"}],"id":"n0.05491706422767484"}],"shape":{"data":{"p":{"x":195,"y":141.6290170380177}},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de593748394392474":{"id":"de593748394392474","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.2024513439070299"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.6079080211235881"}],"id":"n0.039372446555006935"}],"id":"n0.17424852726676154"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.27754197573671946"}],"id":"n0.9898910152004727"}],"id":"n0.9131833576629502"}},"id":"n0.06928870624904726"},{"type":"single","text":"(","id":"n0.36341506215089003"},{"text":"s,a","id":"n0.34063805430204086"},{"type":"single","text":")","id":"n0.0880183115160802"}],"id":"n0.011029513288379977"}],"id":"n0.5354735391707355"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3680450720683681"}],"style":{"align":"center"},"id":"n0.3056060788524073"}],"shape":{"data":{"p":{"x":287,"y":126.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8913158837985631":{"id":"de8913158837985631","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Activation: ReLU","id":"n0.05693186723663479"}],"id":"n0.7546118539131947"}],"shape":{"data":{"p":{"x":100.5172119140625,"y":204.4443130493164},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de49845263097063075":{"id":"de49845263097063075","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.3561453397862475"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1","id":"n0.4691350123111182"}],"id":"n0.5771846971278596"}],"id":"n0.42747229650193197"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5927800692205678"}],"id":"n0.8453167772585206"}],"shape":{"data":{"p":{"x":74.5172119140625,"y":208.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de19958885418575512":{"id":"de19958885418575512","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.8237715942731867"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3×3×4×200","id":"n0.14754586405517744"}],"id":"n0.3382643066492892"}],"id":"n0.0671748381274353"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5746527989732806"}],"id":"n0.8533482083801416"}],"shape":{"data":{"p":{"x":81.5172119140625,"y":196.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9991017222779492":{"id":"de9991017222779492","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"2D convolutional layer","id":"n0.3305531879713304"}],"id":"n0.796093615307945"}],"shape":{"data":{"p":{"x":89.5172119140625,"y":196.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de7794946484826855":{"id":"de7794946484826855","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.24491485485523845"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1","id":"n0.34253594693251954"}],"id":"n0.8201033238122026"}],"id":"n0.35431681432038165"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.1461140221830728"}],"id":"n0.21950866463284258"}],"shape":{"data":{"p":{"x":112.0172119140625,"y":209.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9437130437561829":{"id":"de9437130437561829","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.5979703033955528"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×200×|A","id":"n0.9453268524544269"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.630998937819023"}],"id":"n0.8083322454877857"}],"id":"n0.3487417949962308"}},"id":"n0.7879825099348208"},{"text":"|","id":"n0.35092453772066623"}],"id":"n0.9924403943583895"}],"id":"n0.12323602675056611"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3716906131006634"}],"id":"n0.8408340296938122"}],"shape":{"data":{"p":{"x":119.0172119140625,"y":192.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de3957690388394757":{"id":"de3957690388394757","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"2D convolutional layer","id":"n0.2831710279467221"}],"id":"n0.13269695582335794"}],"shape":{"data":{"p":{"x":127.0172119140625,"y":196.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de5805238498780745":{"id":"de5805238498780745","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Activation: ReLU","id":"n0.9772703803458971"}],"id":"n0.6842961852820442"}],"shape":{"data":{"p":{"x":100.5172119140625,"y":119.4443130493164},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4297722923504397":{"id":"de4297722923504397","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"4D convolutional layer","id":"n0.6128428799527574"}],"id":"n0.1863077684458414"}],"shape":{"data":{"p":{"x":89.5172119140625,"y":113.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9970137941515702":{"id":"de9970137941515702","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.8551779072921222"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"3×3×3×3×2×100","id":"n0.5894255189656732"}],"id":"n0.7063629133230427"}],"id":"n0.3210884854241822"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3397182068614162"}],"id":"n0.3961409225340591"}],"shape":{"data":{"p":{"x":81.5172119140625,"y":101.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de618679292194954":{"id":"de618679292194954","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.9710282475795413"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1×1","id":"n0.7066017249082943"}],"id":"n0.5611562227899454"}],"id":"n0.14206887739882257"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7443737249209761"}],"id":"n0.7181779079849848"}],"shape":{"data":{"p":{"x":74.5172119140625,"y":115.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4392674425233447":{"id":"de4392674425233447","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"4D convolutional layer","id":"n0.5301660593230821"}],"id":"n0.3958610824559792"}],"shape":{"data":{"p":{"x":127.0172119140625,"y":112.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de04204407547054956":{"id":"de04204407547054956","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Filter: ","id":"n0.10551866878206084"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1×1×100×|A|","id":"n0.8656058523394414"}],"id":"n0.02722195288173035"}],"id":"n0.633784928341107"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.16890997532945828"}],"id":"n0.5765982436223782"}],"shape":{"data":{"p":{"x":119.0172119140625,"y":98.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8792070875119302":{"id":"de8792070875119302","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Stride: ","id":"n0.8513302607064426"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1×1×1×1","id":"n0.32634089926763865"}],"id":"n0.31301881936258424"}],"id":"n0.36024324575911404"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.07486874930869836"}],"id":"n0.5385064198666598"}],"shape":{"data":{"p":{"x":112.0172119140625,"y":116.27590942382812},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7209237783119844":{"id":"de7209237783119844","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.9729776412783562","text":"R"},{"id":"n0.2835126069111431","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.08389011410193059","lines":[{"id":"n0.9819171012848007","blocks":[{"id":"n0.047536987371397776","text":"i"}]}]}}},{"type":"single","text":"(","id":"n0.8691568773847549"},{"text":"s,a","id":"n0.5889567509171811"},{"type":"single","text":")","id":"n0.5276003849362187"}],"id":"n0.2095657756783389"}],"id":"n0.2982039446388105"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.015031633040377246"}],"style":{"align":"center"},"id":"n0.25864148778868534"}],"shape":{"data":{"p":{"x":151.99999999999994,"y":125.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de038275511556437936":{"id":"de038275511556437936","lines":[{"blocks":[{"text":"expand along","style":{"fontSize":{"value":0.4}},"id":"n0.7377298173475393"}],"style":{"align":"center"},"id":"n0.9617942479760144"}],"shape":{"data":{"p":{"x":117.29996422052108,"y":198.80586921109438},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9771146900240346":{"id":"de9771146900240346","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.6399812305379686"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.7507470953748117"}],"id":"n0.6350793290242283"}],"id":"n0.6673921088194974"}},"id":"n0.8403559765691839"}],"id":"n0.6655942045909249"}],"id":"n0.39382613896308327"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.68068017586931"},{"text":",","style":{"fontSize":{"value":0.4}},"id":"n0.6656502821413655"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"W","id":"n0.13463231949855103"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.3824123960513046"}],"id":"n0.9272158036074829"}],"id":"n0.06135171794311067"}},"id":"n0.8809286095868312"},{"id":"n0.22244046571993925","text":",A"},{"id":"n0.004709735571196472","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5915201252700317","lines":[{"id":"n0.9228932234027902","blocks":[{"id":"n0.13351951205842272","text":"j"}]}]}}}],"id":"n0.9862134259506325"}],"id":"n0.7869443691048681"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8476247623710638"}],"style":{"align":"center"},"id":"n0.22591749357595425"}],"shape":{"data":{"p":{"x":120.29996422052108,"y":214},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9138085967477212":{"id":"de9138085967477212","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.5246867276122629"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.44468150511900717"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.28346165577162274"}],"id":"n0.13986293163761343"}],"id":"n0.2918402784940872"},"indexValue":{"lines":[{"blocks":[{"id":"n0.8675891867791983","text":"R"}],"id":"n0.5950250442193212"}],"id":"n0.9362693118359131"}},"id":"n0.1802718268590522"}],"id":"n0.9060303829634953"}],"id":"n0.6254132286642293"}},"id":"n0.6166884885015271"},{"type":"single","text":"(","id":"n0.8913429643789912"},{"text":"s,a","id":"n0.039437228771850075"},{"type":"single","text":")","id":"n0.12396919054212252"}],"id":"n0.1563681651083162"}],"id":"n0.3888587151739875"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.2655067483208675"}],"style":{"align":"center"},"id":"n0.590575319588402"}],"shape":{"data":{"p":{"x":308.58166565657575,"y":271.8347432156015},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de20514259198876084":{"id":"de20514259198876084","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"1-","id":"n0.668198392710996"},{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.7571321692537014"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.5272197079611174"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.8937534642238385"}],"id":"n0.4214733950927938"}],"id":"n0.7177250752548958"},"indexValue":{"lines":[{"blocks":[{"id":"n0.7474702890391776","text":"R"}],"id":"n0.5319220509984435"}],"id":"n0.2693561890123892"}},"id":"n0.8118552033966404"}],"id":"n0.7837346203169866"}],"id":"n0.009197237518780765"}},"id":"n0.3760909778409871"}],"id":"n0.2830138817581649"}],"id":"n0.4091118874775652"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.904834482548242"}],"style":{"align":"center"},"id":"n0.08067293266874409"}],"shape":{"data":{"p":{"x":245.5816656565757,"y":273.8347432156015},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7312818138853312":{"id":"de7312818138853312","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.129410645790617"}],"id":"n0.0932584376979364"}],"id":"n0.6176372360853613"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7572352029835652"}],"id":"n0.013809604713022283"}],"shape":{"data":{"p":{"x":294.5171989578646,"y":200.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de18788604977197143":{"id":"de18788604977197143","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.7208189660776849"}],"id":"n0.6520254498093123"}],"id":"n0.4440631194786806"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.818256381077096"}],"id":"n0.5427659946248642"}],"shape":{"data":{"p":{"x":337.16577825936406,"y":220.6259652802052},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4165371666675024":{"id":"de4165371666675024","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"R","id":"n0.0853109433397754"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9419594729096477"}],"id":"n0.968664482499086"}],"id":"n0.9296545885225689"}},"id":"n0.8016860732170108"},{"type":"single","text":"(","id":"n0.013403756317966753"},{"text":"s,a","id":"n0.6226098915614835"},{"type":"single","text":")","id":"n0.6431540514618153"}],"id":"n0.9579442511261114"}],"id":"n0.747319571117421"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8339656140112792"}],"style":{"align":"center"},"id":"n0.7419316581247017"}],"shape":{"data":{"p":{"x":391.99999999999994,"y":228.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de4583001414534833":{"id":"de4583001414534833","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.921779451769565"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8518855671786338"}],"id":"n0.11299044556288429"}],"id":"n0.7604477425721416"}},"id":"n0.9296973827163246"},{"text":"×W","id":"n0.1538161200467536"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8171545339012034"}],"id":"n0.9385952818455519"}],"id":"n0.1867963143872604"}},"id":"n0.587800547063406"},{"text":"×H","id":"n0.46918365779553817"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.008491500153849252"}],"id":"n0.02332069353328614"}],"id":"n0.828953364810201"}},"id":"n0.340743747243319"},{"text":"×W","id":"n0.7074877741896182"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.7296990462222239"}],"id":"n0.8203240114425976"}],"id":"n0.8593990452589579"}},"id":"n0.4786005730910594"},{"text":"×|A","id":"n0.7863315375672915"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3876218112318073"}],"id":"n0.11576612414543375"}],"id":"n0.4475959595518957"}},"id":"n0.20566171753843232"},{"text":"|×|A","id":"n0.5637944255714951"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.9738597378483855"}],"id":"n0.45027017249932344"}],"id":"n0.8867471707265016"}},"id":"n0.3206198173113135"},{"text":"|","id":"n0.06621334827614778"}],"id":"n0.3805910514369335"}],"id":"n0.7089762412406253"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8667210386776814"}],"style":{"align":"center"},"id":"n0.5745830515114823"}],"shape":{"data":{"p":{"x":565,"y":238.98385620117188},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1583966116698592":{"id":"de1583966116698592","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.25051324056472835"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5104485528147293"}],"id":"n0.7119266041364181"}],"id":"n0.6720067974614112"}},"id":"n0.22417906398881216"},{"text":"×W","id":"n0.38694565250942947"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.11308467701634828"}],"id":"n0.2561855248327065"}],"id":"n0.8964395188293126"}},"id":"n0.873709845049295"},{"text":"×H","id":"n0.07805176795000945"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.5261696737053156"}],"id":"n0.9217072167579223"}],"id":"n0.508954517101174"}},"id":"n0.9127868590808386"},{"text":"×W","id":"n0.4359191161625884"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8355586213743413"}],"id":"n0.28414560810793055"}],"id":"n0.02678663819435756"}},"id":"n0.7433295513012017"},{"text":"×|A","id":"n0.7044446941084268"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.13006501606547882"}],"id":"n0.0153861215235791"}],"id":"n0.4633317385584048"}},"id":"n0.7469097027384985"},{"text":"|×|A","id":"n0.6972895534173722"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.2138797359882061"}],"id":"n0.17566364102152088"}],"id":"n0.2007068588156009"}},"id":"n0.35156909735178665"},{"text":"|","id":"n0.11037384940026396"}],"id":"n0.08339218194311648"}],"id":"n0.4177074897863875"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.32265772539243165"}],"style":{"align":"center"},"id":"n0.43506864788632593"}],"shape":{"data":{"p":{"x":286,"y":324.9838562011719},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7104577832050005":{"id":"de7104577832050005","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.8075229294190343"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.22083786699300711"}],"id":"n0.5255935204300768"}],"id":"n0.4311607854420607"}},"id":"n0.0914520644866017"},{"text":"×W","id":"n0.2652626755745493"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.16552874564810538"}],"id":"n0.8782516293388296"}],"id":"n0.85421562944347"}},"id":"n0.4873403498265405"},{"text":"×H","id":"n0.8038175045166087"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.08554711175121255"}],"id":"n0.6725093589093312"}],"id":"n0.5375129209530072"}},"id":"n0.6141587701812863"},{"text":"×W","id":"n0.01933840850697721"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.020443097004659405"}],"id":"n0.522494558892066"}],"id":"n0.21268471635124353"}},"id":"n0.8246463885708728"},{"text":"×|A","id":"n0.4801458926047433"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.21798914880275522"}],"id":"n0.7652275275201048"}],"id":"n0.9870166818264658"}},"id":"n0.06268927174621086"},{"text":"|×|A","id":"n0.1087166598051661"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.1336164611793449"}],"id":"n0.8600008500233927"}],"id":"n0.362784223053767"}},"id":"n0.05402756018969823"},{"text":"|","id":"n0.6466916443560289"}],"id":"n0.9209111051638239"}],"id":"n0.26785386114980914"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7785792835100691"}],"style":{"align":"center"},"id":"n0.6668498709114434"}],"shape":{"data":{"p":{"x":189,"y":324.9838562011719},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5557732641915689":{"id":"de5557732641915689","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"H","id":"n0.9221364007242416"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8708924348985256"}],"id":"n0.4361484756663945"}],"id":"n0.44176253688535194"}},"id":"n0.04716332947140223"},{"text":"×W","id":"n0.712883274296817"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6132920401588458"}],"id":"n0.7616430739518658"}],"id":"n0.2696234113493192"}},"id":"n0.013541307813835557"},{"text":"×H","id":"n0.7340685198492256"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.20818575598044387"}],"id":"n0.10504536827258204"}],"id":"n0.6062678939699782"}},"id":"n0.111041145839339"},{"text":"×W","id":"n0.45675239871196416"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.8037406560355145"}],"id":"n0.2762161569037047"}],"id":"n0.2607323870924354"}},"id":"n0.35059931187490756"},{"text":"×|A","id":"n0.9153432582945753"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5041720294833045"}],"id":"n0.04667625220583438"}],"id":"n0.9892646631408653"}},"id":"n0.6319894876092336"},{"text":"|×|A","id":"n0.7986057437532796"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.0712045303235258"}],"id":"n0.4180675169846606"}],"id":"n0.3078710101191444"}},"id":"n0.3499893192850838"},{"text":"|","id":"n0.8972496317508627"}],"id":"n0.4931140849769742"}],"id":"n0.9409319662631248"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6201032476437982"}],"style":{"align":"center"},"id":"n0.1098735865660323"}],"shape":{"data":{"p":{"x":129,"y":271.9838562011719},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5375910533835289":{"id":"de5375910533835289","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Q","id":"n0.3818972620683758"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"K","id":"n0.6936000842560022"}],"id":"n0.8834480079197842"}],"id":"n0.47579159718552"},"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.0161172559129108"}],"id":"n0.3091250253697164"}],"id":"n0.04860701906399467"}},"id":"n0.5280536840296086"},{"type":"single","text":"(","id":"n0.3717890650866613"},{"text":"s,a","id":"n0.8688828975071476"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6224899193762006"}],"id":"n0.6917619864650839"}],"id":"n0.7395427912098691"}},"id":"n0.2917797323041105"},{"type":"single","text":")","id":"n0.14063453808692916"}],"id":"n0.19153155965893243"}],"id":"n0.7764373811879"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7429848061739557"}],"style":{"align":"center"},"id":"n0.33650805746857215"}],"shape":{"data":{"p":{"x":616,"y":62.30738294008597},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de9514175999666843":{"id":"de9514175999666843","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.5850924357739005"}],"id":"n0.5376003386086392"}],"id":"n0.0762310102206607"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6456319389028695"}],"id":"n0.11134966197085183"}],"shape":{"data":{"p":{"x":615.5171989578646,"y":131.37593476262708}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true}},"connections":[],"intersections":{"id":"di2780349073832271","items":[],"style":{}},"shapes":[{"id":"dp14990224151474485","type":"doc-cube","data":{"p1":{"x":403.89243309975313,"y":45.5022752722482},"p2":{"x":441.9827880859375,"y":83.21222204612354},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp24405884183873572","type":"doc-cube","data":{"p1":{"x":403.89243309975313,"y":13.199859619140625},"p2":{"x":441.9827880859375,"y":50.90980639301608},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"da6949805193558927","data":[{"x":40.01719895786459,"y":57.34437565321065},{"x":51.206092622831534,"y":57.34437565321065}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp7751921556432406","type":"doc-cube","data":{"p1":{"x":1.5988775706382512,"y":37.84193818059583},"p2":{"x":39.68923255682262,"y":75.55188495447129},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp8785182138928569","type":"doc-cube","data":{"p1":{"x":92.17413453580775,"y":51.42721209483358},"p2":{"x":130.26448952199212,"y":89.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp844065271006349","type":"doc-cube","data":{"p1":{"x":92.17413453580775,"y":19.42721209483358},"p2":{"x":130.26448952199212,"y":57.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp8899522848110837","type":"doc-cube","data":{"p1":{"x":162.90964501381563,"y":231.12821003487528},"p2":{"x":201,"y":268.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp6103754823685426","type":"doc-cube","data":{"p1":{"x":162.90964501381563,"y":198.8257943817677},"p2":{"x":201,"y":236.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp5314894875590921","type":"doc-cube","data":{"p1":{"x":173.592468879232,"y":241.89985181931803},"p2":{"x":211.68282386541637,"y":279.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp7433023052420107","type":"doc-cube","data":{"p1":{"x":173.592468879232,"y":209.89985181931803},"p2":{"x":211.68282386541637,"y":247.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da9197567997449922","data":[{"x":130.26448952199212,"y":57.13715886870904},{"x":142.1304054661781,"y":57.13715886870904}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4367992055092309","data":[{"x":161.66612152300183,"y":56.729627747941095},{"x":172.74979117488306,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp49796068475762456","type":"circle","data":{"p1":{"x":142.1304054661781,"y":47.30450264897962},"p2":{"x":161.66612152300183,"y":66.84021870580335}}},{"id":"dp12323737849555427","type":"doc-cube","data":{"p1":{"x":172.59887757063825,"y":38.84193818059583},"p2":{"x":210.68923255682262,"y":76.55188495447129},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dp9747833728278197","type":"rectangle","data":{"p1":{"x":366.57731762375033,"y":11.841938180595832},"p2":{"x":391.60827698470075,"y":88.84193818059583}}},{"id":"dg48705751945207343","entities":[{"id":"dg5483839555055041","entities":[{"id":"dp575668142911451","type":"rectangle","data":{"p1":{"x":324.59887757063825,"y":17.607904868061325},"p2":{"x":337.2560383026971,"y":30.26506560012018}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp08016503403204545","type":"rectangle","data":{"p1":{"x":326.18102266214555,"y":19.190049959568682},"p2":{"x":338.8381833942044,"y":31.847210691627538}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp2892912392670768","type":"rectangle","data":{"p1":{"x":327.76316775365297,"y":20.77219505107604},"p2":{"x":340.4203284857118,"y":33.429355783134895}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}}],"data":{}},{"id":"dl476644294595165","linkedId":"de8705375563265205"}]},{"id":"dp21090197840764624","type":"rectangle","data":{"p1":{"x":235.57731762375033,"y":14.841938180595832},"p2":{"x":260.60827698470075,"y":91.84193818059583}}},{"id":"da5090470079597946","data":[{"x":210.63773467215037,"y":56.729627747941095},{"x":235.60827698470075,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da16305663881483423","data":[{"x":260.8334608267643,"y":56.729627747941095},{"x":270.7314323563021,"y":56.729627747941095}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg5268113431064796","entities":[{"id":"dg34625322291609306","entities":[{"id":"dp4907438325901321","type":"rectangle","data":{"p1":{"x":207.59887757063825,"y":18.6432747411082},"p2":{"x":220.2560383026971,"y":31.300435473167056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp9607763071254807","type":"rectangle","data":{"p1":{"x":209.1810226621456,"y":20.225419832615557},"p2":{"x":221.83818339420446,"y":32.88258056467441}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}},{"id":"dp9702120349022043","type":"rectangle","data":{"p1":{"x":210.76316775365297,"y":21.807564924122914},"p2":{"x":223.42032848571182,"y":34.46472565618177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[184,233,134,1]}}],"data":{}},{"id":"dl22840323663350937","linkedId":"de8268699887031468"}]},{"id":"dg5119081581839389","entities":[{"id":"dp5997815318584838","type":"circle","data":{"p1":{"x":323.1304054661781,"y":46.99785802735977},"p2":{"x":342.66612152300183,"y":66.5335740841835}}},{"id":"dl051729928572972206","linkedId":"de16664139451638227"}]},{"id":"da41753940725179994","data":[{"x":342.66612152300183,"y":56.765716055771634},{"x":366.60827698470075,"y":56.765716055771634}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4665736284321893","data":[{"x":392.0861485032234,"y":56.215249700218635},{"x":403.60827698470075,"y":56.215249700218635}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp28495266948125453","type":"doc-cube","data":{"p1":{"x":414.592468879232,"y":55.89985181931803},"p2":{"x":452.68282386541637,"y":93.60979859319349},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp8552058952329378","type":"doc-cube","data":{"p1":{"x":414.592468879232,"y":23.89985181931803},"p2":{"x":452.68282386541637,"y":61.60979859319349},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"dg17309319634559373","entities":[{"id":"dp015239561323907358","type":"circle","data":{"p1":{"x":575.3800116578016,"y":188.44739167180677},"p2":{"x":594.9157277146253,"y":207.9831077286305}}},{"id":"dl29152123864399115","linkedId":"de6724674073740904"}]},{"id":"da6983784416503829","data":[{"x":501.2671484131258,"y":198.21524970021864},{"x":575.3800116578016,"y":198.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da3283043273032493","data":[{"x":585.1478696862134,"y":55.96521918264051},{"x":585.1478696862134,"y":188.44739167180677}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp13376537653618326","type":"doc-cube","data":{"p1":{"x":606.9096450138156,"y":198.12821003487528},"p2":{"x":645,"y":235.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp3054749720417138","type":"doc-cube","data":{"p1":{"x":606.9096450138156,"y":165.8257943817677},"p2":{"x":645,"y":203.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp41034984821714504","type":"doc-cube","data":{"p1":{"x":617.592468879232,"y":208.89985181931803},"p2":{"x":655.6828238654164,"y":246.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp8886673172247268","type":"doc-cube","data":{"p1":{"x":617.592468879232,"y":176.89985181931803},"p2":{"x":655.6828238654164,"y":214.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da9953024180193935","data":[{"x":340.2560383026971,"y":26.26506560012018},{"x":366.0093994140625,"y":26.26506560012018}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da449948342434481","data":[{"x":223.42032848571182,"y":28.807564924122914},{"x":235.94245696718917,"y":28.807564924122914}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp19338476574456598","type":"doc-cube","data":{"p1":{"x":459.4913106703914,"y":119.12821003487528},"p2":{"x":497.58166565657575,"y":156.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp8030024715026778","type":"doc-cube","data":{"p1":{"x":459.4913106703914,"y":86.82579438176771},"p2":{"x":497.58166565657575,"y":124.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp125416381304714","type":"doc-cube","data":{"p1":{"x":470.17413453580775,"y":129.42721209483358},"p2":{"x":508.2644895219921,"y":167.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp6916795208149304","type":"doc-cube","data":{"p1":{"x":470.17413453580775,"y":97.42721209483358},"p2":{"x":508.2644895219921,"y":135.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp2468627412531159","type":"doc-cube","data":{"p1":{"x":525.4913106703914,"y":119.12821003487528},"p2":{"x":563.5816656565758,"y":156.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp22016459532661758","type":"doc-cube","data":{"p1":{"x":525.4913106703914,"y":86.82579438176771},"p2":{"x":563.5816656565758,"y":124.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp8150954059179112","type":"doc-cube","data":{"p1":{"x":536.1741345358078,"y":129.89985181931803},"p2":{"x":574.2644895219921,"y":167.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp05758749241223038","type":"doc-cube","data":{"p1":{"x":536.1741345358078,"y":97.89985181931803},"p2":{"x":574.2644895219921,"y":135.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dg7864340864191153","entities":[{"id":"dp18345955570639116","type":"circle","data":{"p1":{"x":232.7314323563021,"y":223.19736115422864},"p2":{"x":252.26714841312582,"y":242.73307721105238}}},{"id":"dl9306573912534319","linkedId":"de3842459334625856"}]},{"id":"da8891685749627016","data":[{"x":452.60827698470075,"y":56.215249700218635},{"x":483.1304054661781,"y":56.215249700218635}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg5666011018312356","entities":[{"id":"dp9124936588147989","type":"circle","data":{"p1":{"x":537.7314323563021,"y":46.197361154228645},"p2":{"x":557.2671484131258,"y":65.73307721105238}}},{"id":"dl7867532605259782","linkedId":"de5279245661967291"}]},{"id":"da8790688520118102","data":[{"x":547.499290384714,"y":65.73307721105238},{"x":547.499290384714,"y":86.21600341796875}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"dg8772277223546896","entities":[{"id":"dp9608104972311906","type":"circle","data":{"p1":{"x":483.1304054661781,"y":45.99785802735977},"p2":{"x":502.66612152300183,"y":65.5335740841835}}},{"id":"dl860205744073318","linkedId":"de5414059609216073"}],"data":{}},{"id":"da4537344221289057","data":[{"x":502.66612152300183,"y":55.96521918264051},{"x":537.7314323563021,"y":55.96521918264051}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da6439031813379001","data":[{"x":419.7987614003159,"y":233.21524970021864},{"x":585.1478696862134,"y":233.21524970021864}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg6839742550484962","entities":[{"id":"dg5310372500915896","entities":[{"id":"dp6417093932066409","type":"rectangle","data":{"p1":{"x":8.99359130859375,"y":1.5402473973582005},"p2":{"x":21.650752040652606,"y":14.197408129417056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp8266435787880344","type":"rectangle","data":{"p1":{"x":10.57573640010105,"y":3.1223924888655574},"p2":{"x":23.232897132159906,"y":15.779553220924413}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp5776532759061219","type":"rectangle","data":{"p1":{"x":12.157881491608464,"y":4.704537580372914},"p2":{"x":24.81504222366732,"y":17.36169831243177}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl7562753566974094","linkedId":"de48398552182920707"}]},{"id":"dp7209277368997147","type":"doc-cube","data":{"p1":{"x":270.5752569651695,"y":56.801277332206496},"p2":{"x":308.66561195135387,"y":94.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp3734636867943475","type":"doc-cube","data":{"p1":{"x":270.5752569651695,"y":24.801277332206496},"p2":{"x":308.66561195135387,"y":62.511224106081954},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da4212914548171849","data":[{"x":309.2671484131258,"y":56.96521918264051},{"x":323.0093994140625,"y":56.96521918264051}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da8328460715812909","data":[{"x":70.0093994140625,"y":57.13715886870904},{"x":92.26448952199212,"y":57.13715886870904}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da5204873677507988","data":[{"x":557.2671484131258,"y":55.96521918264051},{"x":585.1478696862134,"y":55.96521918264051}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg34712524270343836","entities":[{"id":"dp37922344119144635","type":"circle","data":{"p1":{"x":481.7314323563021,"y":188.19736115422864},"p2":{"x":501.2671484131258,"y":207.73307721105238}}},{"id":"dl5441292163557927","linkedId":"de9498932232987138"}]},{"id":"da9848201611653264","data":[{"x":491.49929038471396,"y":167.31321716308594},{"x":491.49929038471396,"y":189.19736115422864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9356199515291648","data":[{"x":198.14786968621343,"y":76.96521918264051},{"x":198.14786968621343,"y":130.21600341796875}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp36614154743620286","type":"rectangle","data":{"p1":{"x":226.57731762375033,"y":101.21600341796875},"p2":{"x":251.60827698470075,"y":185.21600341796875}}},{"id":"dg6506031910909329","entities":[{"id":"dp6523267676928928","type":"doc-cube","data":{"p1":{"x":191.62434362521276,"y":146.21600341796875},"p2":{"x":208.08394629477812,"y":162.51122410608195},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dl7345083637550276","linkedId":"de5418541516011492"}]},{"id":"da7801880500008729","data":[{"x":208.42032848571182,"y":154.80756492412291},{"x":226.0093994140625,"y":154.80756492412291}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da045930330977075995","data":[{"x":198.14786968621343,"y":130.21600341796875},{"x":226.0093994140625,"y":130.21600341796875}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp1009362638384308","type":"doc-cube","data":{"p1":{"x":266.89243309975313,"y":139.5022752722482},"p2":{"x":304.9827880859375,"y":177.21222204612354},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp8845379047524937","type":"doc-cube","data":{"p1":{"x":266.89243309975313,"y":107.19985961914062},"p2":{"x":304.9827880859375,"y":144.90980639301608},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1]}},{"id":"dp5398496350087281","type":"doc-cube","data":{"p1":{"x":277.592468879232,"y":149.89985181931803},"p2":{"x":315.68282386541637,"y":187.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp17001763161707162","type":"doc-cube","data":{"p1":{"x":277.592468879232,"y":117.89985181931803},"p2":{"x":315.68282386541637,"y":155.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da6755513325025082","data":[{"x":252.0093994140625,"y":142.5022752722482},{"x":266.89243309975313,"y":142.5022752722482}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da5839508455852414","data":[{"x":375.0093994140625,"y":197.9652191826405},{"x":481.7314323563021,"y":197.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da6520536481094008","data":[{"x":315.89243309975313,"y":142.5022752722482},{"x":375.0093994140625,"y":142.5022752722482}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da6223170250390233","data":[{"x":375.0093994140625,"y":142.5022752722482},{"x":375.0093994140625,"y":197.9652191826405}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg4876687212389459","entities":[{"id":"dp46454992351115565","type":"rectangle","data":{"p1":{"x":6.743766507919418,"y":101.63121309108607},"p2":{"x":36.79161019925965,"y":130.95367293703205}},"style":{"strokeColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dg8343682138407165","entities":[{"id":"dp776531624489611","type":"rectangle","data":{"p1":{"x":23.558526932530896,"y":118.92873841303452},"p2":{"x":25.66417775956546,"y":121.03438924006917}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp09636319241084101","type":"rectangle","data":{"p1":{"x":9.659299684352277,"y":105.02951116485616},"p2":{"x":39.56340500774397,"y":134.9336164882478}},"style":{"boxShadow":{"fill":[155,155,155,1]},"fillColor":[255,255,255,1]}},{"id":"dp4542673426534998","type":"rectangle","data":{"p1":{"x":37.54307489464884,"y":121.07837181585722},"p2":{"x":39.64872572168349,"y":123.18402264289205}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7517531721738098","type":"rectangle","data":{"p1":{"x":21.32248029739992,"y":130.29732108927234},"p2":{"x":23.408813226938975,"y":132.3836540188113}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7424285459413666","type":"rectangle","data":{"p1":{"x":30.57575319785525,"y":118.97381350719132},"p2":{"x":32.68140402488987,"y":121.07946433422586}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp2187897295217227","type":"rectangle","data":{"p1":{"x":28.238287600871786,"y":132.8762604049524},"p2":{"x":30.34393842790638,"y":134.9819112319871}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp591011055398821","type":"rectangle","data":{"p1":{"x":11.99966296596017,"y":127.94781616533936},"p2":{"x":14.10531379299482,"y":130.0534669923739}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp10549255661273271","type":"rectangle","data":{"p1":{"x":28.244726900036994,"y":121.26620401001804},"p2":{"x":30.350377727071645,"y":123.37185483705267}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp48315751179595523","type":"rectangle","data":{"p1":{"x":14.303644207284322,"y":121.03329672170057},"p2":{"x":16.409295034318973,"y":123.13894754873525}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp09228914560259338","type":"rectangle","data":{"p1":{"x":9.76393829578754,"y":125.7146672148329},"p2":{"x":11.798756832004472,"y":127.7494857510498}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp07696527225880301","type":"rectangle","data":{"p1":{"x":30.575753197855164,"y":130.53879480796894},"p2":{"x":32.68140402488976,"y":132.64444563500354}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5046873712573121","type":"rectangle","data":{"p1":{"x":9.866967082431444,"y":109.42967962593141},"p2":{"x":11.798756832004472,"y":113.88567464828006}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp10639888501546224","type":"rectangle","data":{"p1":{"x":9.866967082431444,"y":130.2994482204863},"p2":{"x":14.116904531492253,"y":132.3535846541991}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp03655512040885056","type":"rectangle","data":{"p1":{"x":12.030571601953284,"y":121.26620401001804},"p2":{"x":18.753199930467787,"y":123.32677974289601}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp10827553729293315","type":"rectangle","data":{"p1":{"x":16.666867000928733,"y":123.52639801701855},"p2":{"x":25.726960926426585,"y":125.6030719978096}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp23537435320969347","type":"rectangle","data":{"p1":{"x":16.666867000928733,"y":125.6030719978096},"p2":{"x":21.090665527451222,"y":127.97917338978453}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp798566212688985","type":"rectangle","data":{"p1":{"x":18.985014700416457,"y":128.2109881597334},"p2":{"x":23.408813226938975,"y":130.29732108927234}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5762405859628885","type":"rectangle","data":{"p1":{"x":32.835947204855756,"y":107.34765886434366},"p2":{"x":37.2597457313781,"y":109.43399179388268}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp52394507536378","type":"rectangle","data":{"p1":{"x":30.575753197855164,"y":109.60785287134428},"p2":{"x":34.999551724377625,"y":111.6941858008833}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp08281576660854384","type":"rectangle","data":{"p1":{"x":37.51087839882254,"y":111.80578101790638},"p2":{"x":39.44266814839574,"y":116.16840620235891}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5577979226831644","type":"rectangle","data":{"p1":{"x":35.250684391822006,"y":111.90990232291898},"p2":{"x":37.31769942386532,"y":116.3884348923458}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5057205085433467","type":"rectangle","data":{"p1":{"x":37.51087839882254,"y":125.65671352234548},"p2":{"x":39.57789343086583,"y":130.1352460917726}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp4512706381415301","type":"rectangle","data":{"p1":{"x":32.85526510235144,"y":132.905237251196},"p2":{"x":37.2597457313781,"y":134.8756627957606}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9794822969993058","type":"rectangle","data":{"p1":{"x":25.939457798879687,"y":116.62024966229475},"p2":{"x":30.363256325402062,"y":118.70658259183358}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp044264019666153454","type":"rectangle","data":{"p1":{"x":18.98018522604255,"y":109.65614761508363},"p2":{"x":21.0858360530772,"y":111.76179844211828}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp1466883217919721","type":"rectangle","data":{"p1":{"x":25.934628324505752,"y":111.97429531457135},"p2":{"x":28.04027915154049,"y":114.079946141606}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp650343481751867","type":"rectangle","data":{"p1":{"x":30.570923723481258,"y":125.94113520398486},"p2":{"x":32.67657455051585,"y":128.04678603101974}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9510716723900396","type":"rectangle","data":{"p1":{"x":32.889071422968925,"y":123.5070801195229},"p2":{"x":34.994722250003576,"y":125.61273094655746}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp49548771039898365","type":"rectangle","data":{"p1":{"x":25.934628324505752,"y":107.39595360808312},"p2":{"x":28.04027915154049,"y":109.5016044351178}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp28752193051771213","type":"rectangle","data":{"p1":{"x":16.662037526554798,"y":114.29244301405907},"p2":{"x":18.767688353589506,"y":116.3980938410937}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp42681388277735866","type":"rectangle","data":{"p1":{"x":28.252776023993505,"y":105.01985221610806},"p2":{"x":30.358426851028156,"y":107.12550304314286}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}}]}]},{"id":"dg7947812146816244","entities":[{"id":"dg42402985072836286","entities":[{"id":"dp5366672673986501","type":"rectangle","data":{"p1":{"x":6.754925534814049,"y":138.60033347539206},"p2":{"x":36.80276922615428,"y":167.92279332133808}},"style":{"strokeColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp01476874744542922","type":"rectangle","data":{"p1":{"x":9.75492553481405,"y":141.60033347539206},"p2":{"x":39.80276922615428,"y":170.92279332133808}},"style":{"strokeColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]},"fillColor":[255,255,255,1]}}]},{"id":"dp6630803563195715","type":"rectangle","data":{"p1":{"x":32.93896497293281,"y":154.25366925943968},"p2":{"x":35.022598812787294,"y":156.33730309929422}},"style":{"fillColor":[245,166,35,1],"strokeColor":[245,166,35,1],"boxShadow":{"fill":[155,155,155,1]}}}]},{"id":"dp2657910889604185","type":"rectangle","data":{"p1":{"x":83.026611328125,"y":100.21600341796875},"p2":{"x":91.0093994140625,"y":189.21600341796875}}},{"id":"dp08631295206854994","type":"rectangle","data":{"p1":{"x":94.026611328125,"y":100.21600341796875},"p2":{"x":118.026611328125,"y":189.21600341796875}}},{"id":"dp5015713956466579","type":"rectangle","data":{"p1":{"x":56.026611328125,"y":100.21600341796875},"p2":{"x":80.026611328125,"y":189.21600341796875}}},{"id":"da2316879304074464","data":[{"x":38.56340500774397,"y":136.9336164882478},{"x":55.42493473559304,"y":136.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da7603240354022516","data":[{"x":24.49929038471396,"y":171.31321716308594},{"x":24.49929038471396,"y":188.19736115422864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg1092150889775978","entities":[{"id":"dp9954113311031296","type":"rectangle","data":{"p1":{"x":23.558526932530896,"y":202.92873841303452},"p2":{"x":25.66417775956546,"y":205.03438924006917}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp13339104191848405","type":"rectangle","data":{"p1":{"x":9.659299684352277,"y":189.02951116485616},"p2":{"x":39.56340500774397,"y":218.9336164882478}},"style":{"boxShadow":{"fill":[155,155,155,1]},"fillColor":[255,255,255,1]}},{"id":"dp9215697306740127","type":"rectangle","data":{"p1":{"x":37.54307489464884,"y":205.07837181585722},"p2":{"x":39.64872572168349,"y":207.18402264289205}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9893460518428052","type":"rectangle","data":{"p1":{"x":21.32248029739992,"y":214.29732108927234},"p2":{"x":23.408813226938975,"y":216.3836540188113}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp8627106894066896","type":"rectangle","data":{"p1":{"x":30.57575319785525,"y":202.97381350719132},"p2":{"x":32.68140402488987,"y":205.07946433422586}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp5575418095764657","type":"rectangle","data":{"p1":{"x":28.238287600871786,"y":216.8762604049524},"p2":{"x":30.34393842790638,"y":218.9819112319871}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp1290207446549887","type":"rectangle","data":{"p1":{"x":11.99966296596017,"y":211.94781616533936},"p2":{"x":14.10531379299482,"y":214.0534669923739}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9442750653267553","type":"rectangle","data":{"p1":{"x":28.244726900036994,"y":205.26620401001804},"p2":{"x":30.350377727071645,"y":207.37185483705267}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp4802362519752237","type":"rectangle","data":{"p1":{"x":14.303644207284322,"y":205.03329672170057},"p2":{"x":16.409295034318973,"y":207.13894754873525}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp2723767529078016","type":"rectangle","data":{"p1":{"x":9.76393829578754,"y":209.7146672148329},"p2":{"x":11.798756832004472,"y":211.7494857510498}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7569028132398223","type":"rectangle","data":{"p1":{"x":30.575753197855164,"y":214.53879480796894},"p2":{"x":32.68140402488976,"y":216.64444563500354}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9970278121826268","type":"rectangle","data":{"p1":{"x":9.866967082431444,"y":193.4296796259314},"p2":{"x":11.798756832004472,"y":197.88567464828006}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp4036610544119197","type":"rectangle","data":{"p1":{"x":9.866967082431444,"y":214.2994482204863},"p2":{"x":14.116904531492253,"y":216.3535846541991}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp8968742480258425","type":"rectangle","data":{"p1":{"x":12.030571601953284,"y":205.26620401001804},"p2":{"x":18.753199930467787,"y":207.326779742896}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp1899883385859371","type":"rectangle","data":{"p1":{"x":16.666867000928733,"y":207.52639801701855},"p2":{"x":25.726960926426585,"y":209.6030719978096}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp8509824335979563","type":"rectangle","data":{"p1":{"x":16.666867000928733,"y":209.6030719978096},"p2":{"x":21.090665527451222,"y":211.97917338978453}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp6477753281033174","type":"rectangle","data":{"p1":{"x":18.985014700416457,"y":212.2109881597334},"p2":{"x":23.408813226938975,"y":214.29732108927234}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp33687450466130264","type":"rectangle","data":{"p1":{"x":32.835947204855756,"y":191.34765886434366},"p2":{"x":37.2597457313781,"y":193.43399179388268}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp6422861029956799","type":"rectangle","data":{"p1":{"x":30.575753197855164,"y":193.60785287134428},"p2":{"x":34.999551724377625,"y":195.6941858008833}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp16854570501165456","type":"rectangle","data":{"p1":{"x":37.51087839882254,"y":195.80578101790638},"p2":{"x":39.44266814839574,"y":200.1684062023589}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp7190945406323468","type":"rectangle","data":{"p1":{"x":35.250684391822006,"y":195.90990232291898},"p2":{"x":37.31769942386532,"y":200.3884348923458}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp8201804471978769","type":"rectangle","data":{"p1":{"x":37.51087839882254,"y":209.65671352234548},"p2":{"x":39.57789343086583,"y":214.1352460917726}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp0978748132177627","type":"rectangle","data":{"p1":{"x":32.85526510235144,"y":216.905237251196},"p2":{"x":37.2597457313781,"y":218.8756627957606}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp17876075451600437","type":"rectangle","data":{"p1":{"x":25.939457798879687,"y":200.62024966229475},"p2":{"x":30.363256325402062,"y":202.70658259183358}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp9290422019998839","type":"rectangle","data":{"p1":{"x":18.98018522604255,"y":193.65614761508363},"p2":{"x":21.0858360530772,"y":195.76179844211828}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp12588320681146237","type":"rectangle","data":{"p1":{"x":25.934628324505752,"y":195.97429531457135},"p2":{"x":28.04027915154049,"y":198.079946141606}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp6519377730025322","type":"rectangle","data":{"p1":{"x":30.570923723481258,"y":209.94113520398486},"p2":{"x":32.67657455051585,"y":212.04678603101974}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp22105976859820342","type":"rectangle","data":{"p1":{"x":32.889071422968925,"y":207.5070801195229},"p2":{"x":34.994722250003576,"y":209.61273094655746}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp1855997675757235","type":"rectangle","data":{"p1":{"x":25.934628324505752,"y":191.39595360808312},"p2":{"x":28.04027915154049,"y":193.5016044351178}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp09107112896950009","type":"rectangle","data":{"p1":{"x":16.662037526554798,"y":198.29244301405907},"p2":{"x":18.767688353589506,"y":200.3980938410937}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}},{"id":"dp410629668178655","type":"rectangle","data":{"p1":{"x":28.252776023993505,"y":189.01985221610806},"p2":{"x":30.358426851028156,"y":191.12550304314286}},"style":{"fillColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]}}}]},{"id":"dg2423948431923939","entities":[{"id":"dp10443581611316621","type":"rectangle","data":{"p1":{"x":9.75492553481405,"y":222.60033347539206},"p2":{"x":39.80276922615428,"y":251.92279332133808}},"style":{"strokeColor":[0,0,0,1],"boxShadow":{"fill":[155,155,155,1]},"fillColor":[255,255,255,1]}},{"id":"dp46357080878324264","type":"rectangle","data":{"p1":{"x":32.93896497293281,"y":236.25366925943968},"p2":{"x":35.022598812787294,"y":238.33730309929422}},"style":{"fillColor":[245,166,35,1],"strokeColor":[245,166,35,1],"boxShadow":{"fill":[155,155,155,1]}}}]},{"id":"dg2629691174216253","entities":[{"id":"dg41920582080262037","entities":[{"id":"dl2645106817182066","linkedId":"de3957690388394757"},{"id":"dl8307616693404456","linkedId":"de9437130437561829"},{"id":"dl5381812000928694","linkedId":"de7794946484826855"}],"data":{"rotation":90}},{"id":"dg9374920961374769","entities":[{"id":"dl3584575941687689","linkedId":"de9991017222779492"},{"id":"dl9100732043267474","linkedId":"de19958885418575512"},{"id":"dl6432441582775346","linkedId":"de49845263097063075"}],"data":{"rotation":90}},{"id":"dp9677582662226305","type":"rectangle","data":{"p1":{"x":83.026611328125,"y":193.1030216217041},"p2":{"x":91.026611328125,"y":264.1030216217041}}},{"id":"dp5483405438508648","type":"rectangle","data":{"p1":{"x":94.026611328125,"y":193.1030216217041},"p2":{"x":118.026611328125,"y":264.1030216217041}}},{"id":"dp6739538718666911","type":"rectangle","data":{"p1":{"x":56.026611328125,"y":193.1030216217041},"p2":{"x":80.026611328125,"y":264.1030216217041}}},{"id":"dl8054083505541851","linkedId":"de8913158837985631"}]},{"id":"da7987444022977732","data":[{"x":38.56340500774397,"y":220.9336164882478},{"x":55.42493473559304,"y":220.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da4833872206251586","data":[{"x":118.42493473559304,"y":220.9336164882478},{"x":162.0093994140625,"y":220.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da28774511274180226","data":[{"x":117.42493473559304,"y":136.9336164882478},{"x":131.0093994140625,"y":136.9336164882478}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp032300108571785335","type":"doc-cube","data":{"p1":{"x":130.90964501381563,"y":137.12821003487528},"p2":{"x":169,"y":174.83815680875063},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp8689638891930163","type":"doc-cube","data":{"p1":{"x":130.90964501381563,"y":104.82579438176771},"p2":{"x":169,"y":142.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp46796818169982624","type":"doc-cube","data":{"p1":{"x":141.592468879232,"y":147.89985181931803},"p2":{"x":179.68282386541637,"y":185.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp18654960695364986","type":"doc-cube","data":{"p1":{"x":141.592468879232,"y":115.89985181931803},"p2":{"x":179.68282386541637,"y":153.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5796097857133129","type":"doc-cube","data":{"p1":{"x":224.49131067039139,"y":286.1282100348753},"p2":{"x":262.58166565657575,"y":323.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp8905943944570951","type":"doc-cube","data":{"p1":{"x":224.49131067039139,"y":253.8257943817677},"p2":{"x":262.58166565657575,"y":291.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp07475380820616206","type":"doc-cube","data":{"p1":{"x":235.17413453580775,"y":296.4272120948336},"p2":{"x":273.2644895219921,"y":334.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp04076385251012349","type":"doc-cube","data":{"p1":{"x":235.17413453580775,"y":264.4272120948336},"p2":{"x":273.2644895219921,"y":302.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp256726783214128","type":"doc-cube","data":{"p1":{"x":290.4913106703914,"y":284.1282100348753},"p2":{"x":328.58166565657575,"y":321.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp02970722890567945","type":"doc-cube","data":{"p1":{"x":290.4913106703914,"y":251.8257943817677},"p2":{"x":328.58166565657575,"y":289.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp15340142017396352","type":"doc-cube","data":{"p1":{"x":301.17413453580775,"y":294.89985181931803},"p2":{"x":339.2644895219921,"y":332.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp3371339396431723","type":"doc-cube","data":{"p1":{"x":301.17413453580775,"y":262.89985181931803},"p2":{"x":339.2644895219921,"y":300.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da1936716116269368","data":[{"x":211.68282386541637,"y":232.9652191826405},{"x":232.7314323563021,"y":232.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da09652295103309871","data":[{"x":242.49929038471396,"y":242.73307721105238},{"x":242.49929038471396,"y":253.38780212402344}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da05570659084657903","data":[{"x":165.0093994140625,"y":185.5022752722482},{"x":165.0093994140625,"y":192.94285583496094}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da503179763891904","data":[{"x":165.0093994140625,"y":192.94285583496094},{"x":306.49929038471396,"y":192.94285583496094}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg8303076532667495","entities":[{"id":"dp9919009890132662","type":"circle","data":{"p1":{"x":296.7314323563021,"y":203.19736115422864},"p2":{"x":316.2671484131258,"y":222.73307721105238}}},{"id":"dl3281941997823845","linkedId":"de7312818138853312"}]},{"id":"da012760867966330913","data":[{"x":306.49929038471396,"y":192.94285583496094},{"x":306.49929038471396,"y":203.19736115422864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da17610889282896403","data":[{"x":306.49929038471396,"y":222.73307721105238},{"x":306.49929038471396,"y":251.94285583496094}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da7954537709950458","data":[{"x":252.26714841312582,"y":232.9652191826405},{"x":336.38001165780156,"y":232.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg022188156504345358","entities":[{"id":"dp882701495807743","type":"circle","data":{"p1":{"x":336.38001165780156,"y":223.44739167180677},"p2":{"x":355.9157277146253,"y":242.9831077286305}}},{"id":"dl5767208896380549","linkedId":"de18788604977197143"}]},{"id":"da007392881901756132","data":[{"x":346.1478696862134,"y":213.19288635253906},{"x":346.1478696862134,"y":223.44739167180677}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da5608151902147727","data":[{"x":316.2671484131258,"y":212.9652191826405},{"x":346.1478696862134,"y":213.19288635253906}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da9982419724932328","data":[{"x":355.9157277146253,"y":233.21524970021864},{"x":370.7987614003159,"y":233.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp5494387577736761","type":"doc-cube","data":{"p1":{"x":371.90964501381563,"y":240.12821003487528},"p2":{"x":410,"y":277.8381568087506},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp9840299030242623","type":"doc-cube","data":{"p1":{"x":371.90964501381563,"y":207.8257943817677},"p2":{"x":410,"y":245.53574115564317},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp0700905801207472","type":"doc-cube","data":{"p1":{"x":382.592468879232,"y":250.89985181931803},"p2":{"x":420.68282386541637,"y":288.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp7358646795505828","type":"doc-cube","data":{"p1":{"x":382.592468879232,"y":218.89985181931803},"p2":{"x":420.68282386541637,"y":256.6097985931935},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da35931337732752766","data":[{"x":585.1478696862134,"y":207.9831077286305},{"x":585.1478696862134,"y":233.21524970021864}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da4465892145796957","data":[{"x":594.9157277146253,"y":198.21524970021864},{"x":606.9096450138156,"y":198.21524970021864}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dp43037807676417295","type":"doc-cube","data":{"p1":{"x":608.1741345358078,"y":85.42721209483358},"p2":{"x":646.2644895219921,"y":123.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[255,220,160,1],"strokeType":"-"}},{"id":"dp46356129901525867","type":"doc-cube","data":{"p1":{"x":608.1741345358078,"y":53.42721209483358},"p2":{"x":646.2644895219921,"y":91.13715886870904},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[245,166,35,1]}},{"id":"da4033821799514925","data":[{"x":60.49929038471396,"y":8.21600341796875},{"x":60.49929038471396,"y":52.197361154228645}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da31513085646614347","data":[{"x":24.81504222366732,"y":8.704537580372914},{"x":597.0093994140625,"y":8.704537580372914}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"dg400068704729871","entities":[{"id":"dp09758932003963472","type":"circle","data":{"p1":{"x":617.7314323563021,"y":134.19736115422864},"p2":{"x":637.2671484131258,"y":153.73307721105238}}},{"id":"dl3052853572706562","linkedId":"de9514175999666843"}]},{"id":"da7860029488436255","data":[{"x":627.499290384714,"y":153.73307721105238},{"x":627.499290384714,"y":165.94285583496094}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da8378432600870507","data":[{"x":627.499290384714,"y":123.21600341796875},{"x":627.499290384714,"y":134.19736115422864}],"head":"no","tail":"fh<","shaft":"-","middle":"no","headScale":0.6},{"id":"da10865471188678466","data":[{"x":597.0093994140625,"y":143.9652191826405},{"x":617.7314323563021,"y":143.9652191826405}],"head":"fh>","tail":"no","shaft":"-","middle":"no","headScale":0.6},{"id":"da43058112228638956","data":[{"x":597.0093994140625,"y":8.704537580372914},{"x":597.0093994140625,"y":143.9652191826405}],"head":"no","tail":"no","shaft":"-","middle":"no","headScale":0.6}],"settings":{"grid":true,"diagramHeight":347.9201354980469}}]},{"id":"n0.3370407539120146","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":3860,"delayRenderCache":{"av":3860,"map":{"n0.4948186869059896":{"n0.24224066795434895":{"w":53.7652,"h":8.4545,"bl":0.8214}},"n0.03631791790874783":{"n0.8114851563395926":{"w":24.7215,"h":8.1019,"bl":0.8571}},"n0.10368321027700222":{"n0.10192837968410129":{"w":54.0093,"h":8.4545,"bl":0.8214}},"n0.6113778876903095":{"n0.1471848314421922":{"w":24.7215,"h":8.1019,"bl":0.8571}},"n0.04103796103922863":{"n0.9774562041920496":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.9346331450716716":{"n0.15286703063243756":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.4658812440199587":{"n0.522341707304876":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.6779540611266668":{"n0.7037197434395268":{"w":53.3945,"h":8.4545,"bl":0.8214}},"n0.2594341695196014":{"n0.3315585301606032":{"w":71.7773,"h":8.4545,"bl":0.8214}},"n0.8035966151360414":{"n0.035945705013095575":{"w":58.9916,"h":8.4545,"bl":0.8214}},"n0.8652985179455455":{"n0.9974246527053048":{"w":73.0433,"h":8.4545,"bl":0.8214}},"n0.3405674873132667":{"n0.13909617635472848":{"w":15.625,"h":9.1146,"bl":0.7619}},"n0.019004960502556623":{"n0.960706236887447":{"w":20.3631,"h":9.4491,"bl":0.8402}},"n0.4540862647774402":{"n0.6959331038941989":{"w":29.6766,"h":9.1146,"bl":0.7619}},"n0.7517415472449318":{"n0.4306183045431822":{"w":7.0349,"h":8.4545,"bl":0.8214}},"n0.408476759756512":{"n0.04906427405686231":{"w":21.6743,"h":9.1146,"bl":0.7619}},"n0.8174948536978763":{"n0.25329414575928455":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.6850706070771972":{"n0.7081331412186238":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.9153175281526549":{"n0.36970927642703466":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.047463607109459405":{"n0.31354421293919166":{"w":20.7972,"h":9.9736,"bl":0.6963}},"n0.6377335918019102":{"n0.7635891487221897":{"w":6.9897,"h":9.4491,"bl":0.8402}},"n0.769201243672291":{"n0.773475139164786":{"w":6.7455,"h":9.4491,"bl":0.8402}},"n0.8651163527017454":{"n0.6524612630217288":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.6138080945790303":{"n0.4248082564228923":{"w":24.6672,"h":9.1146,"bl":0.7619}},"n0.40235662659270877":{"n0.4120157811821672":{"w":54.6604,"h":8.4545,"bl":0.8214}},"n0.5663416250436877":{"n0.8672176115946004":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.2688194492057001":{"n0.4139531593661605":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.8434406802059295":{"n0.3127101080275474":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.8084507466865571":{"n0.2070918756904696":{"w":62.5,"h":8.1019,"bl":0.8571}},"n0.4078630694843064":{"n0.5764231602461787":{"w":35.3823,"h":8.1019,"bl":0.8571}},"n0.1325705150031895":{"n0.29351627084059895":{"w":6.0764,"h":8.4545,"bl":0.8214}},"n0.5354735391707355":{"n0.011029513288379977":{"w":22.4971,"h":9.1146,"bl":0.7619}},"n0.3210884854241822":{"n0.7063629133230427":{"w":63.4856,"h":8.1019,"bl":0.8571}},"n0.633784928341107":{"n0.02722195288173035":{"w":69.2817,"h":8.1019,"bl":0.8571}},"n0.0671748381274353":{"n0.3382643066492892":{"w":42.164,"h":8.1019,"bl":0.8571}},"n0.12323602675056611":{"n0.9924403943583895":{"w":49.8861,"h":8.4545,"bl":0.8214}},"n0.14206887739882257":{"n0.5611562227899454":{"w":35.3823,"h":8.1019,"bl":0.8571}},"n0.36024324575911404":{"n0.31301881936258424":{"w":35.3823,"h":8.1019,"bl":0.8571}},"n0.2982039446388105":{"n0.2095657756783389":{"w":19.694,"h":8.4545,"bl":0.8214}},"n0.39382613896308327":{"n0.6655942045909249":{"w":7.4599,"h":8.4545,"bl":0.8214}},"n0.7869443691048681":{"n0.9862134259506325":{"w":18.9254,"h":8.4545,"bl":0.8214}},"n0.3888587151739875":{"n0.1563681651083162":{"w":23.9981,"h":9.9736,"bl":0.6963}},"n0.4091118874775652":{"n0.2830138817581649":{"w":20.9871,"h":9.9736,"bl":0.6963}},"n0.747319571117421":{"n0.9579442511261114":{"w":19.694,"h":8.4545,"bl":0.8214}},"n0.7089762412406253":{"n0.3805910514369335":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.4177074897863875":{"n0.08339218194311648":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.26785386114980914":{"n0.9209111051638239":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.9409319662631248":{"n0.4931140849769742":{"w":90.4044,"h":8.4545,"bl":0.8214}},"n0.7764373811879":{"n0.19153155965893243":{"w":24.4231,"h":9.1146,"bl":0.7619}}}}}

==> sIPOMDPLite-Net(arXiv)/plots/docs/d31f12dc-761f-4b2e-977d-e46e77d677c6 <==
{"id":"n0.25338045829944633","lines":[{"id":"n0.7943069201579043","blocks":[]},{"id":"n0.8548540010333312","blocks":[{"id":"n0.28855487568557425","text":"\\diagram","type":"composite","elements":{"de5520970398776124":{"id":"de5520970398776124","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A","id":"n0.27151433873504516"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4636885140653977"}],"id":"n0.1117015472631393"}],"id":"n0.7622507405737542"}},"id":"n0.1394569138907935"},{"text":"|×|𝛺","id":"n0.2675884865558562"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.2315164678700763"}],"id":"n0.2749069621900577"}],"id":"n0.34863616730742186"}},"id":"n0.14457479221384584"},{"text":"|","id":"n0.047235420711965403"}],"id":"n0.8622852515762334"}],"id":"n0.6538694462700769"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8783443695980817"}],"style":{"align":"center"},"id":"n0.07846061311474695"}],"shape":{"data":{"p":{"x":189.09038550376243,"y":63.23626428200146},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de828983001736362":{"id":"de828983001736362","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.14179019025753226"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5749151404407025"}],"id":"n0.2143796473185655"}],"id":"n0.09084256075912345"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.4641599294522796"}],"id":"n0.7513396748046104"}],"id":"n0.37517258111186624"}},"id":"n0.3889504856587369"},{"type":"single","text":"(","id":"n0.4153840753872462"},{"text":"s","id":"n0.27379039666989824"},{"type":"single","text":")","id":"n0.4721169865752184"}],"id":"n0.6615510692663404"}],"id":"n0.0967657311158161"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.4013948251365338"}],"style":{"align":"center"},"id":"n0.441050774848742"}],"shape":{"data":{"p":{"x":113.40753112076794,"y":164.39516869378502},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de07208453170872553":{"id":"de07208453170872553","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.9495180972961037"}],"id":"n0.43859045338187364"}],"id":"n0.006608013145942282"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.493594653748731"}],"style":{"align":"center"},"id":"n0.6349481183113024"}],"shape":{"data":{"p":{"x":96,"y":179.2900532261246},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8834167216713067":{"id":"de8834167216713067","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.22364208655963358"}],"id":"n0.08847662245070831"}],"id":"n0.5562758659701175"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6771809112206673"}],"style":{"align":"center"},"id":"n0.19983733450358176"}],"shape":{"data":{"p":{"x":203.39034972428357,"y":297.9838562011719},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de04997776156109879":{"id":"de04997776156109879","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.897803963229926"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.08874136617804429"}],"id":"n0.34502941267511034"}],"id":"n0.4261746236899189"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.94840773762354"}],"id":"n0.2666371980940394"}],"id":"n0.042645947864674794"}},"id":"n0.3816973634716303"},{"type":"single","text":"(","id":"n0.48950838725563806"},{"text":"s","id":"n0.5769828033292839"},{"type":"single","text":")","id":"n0.10888111089770058"}],"id":"n0.9817385017994846"}],"id":"n0.5955230560954696"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.06144290259826923"}],"style":{"align":"center"},"id":"n0.046256853314367685"}],"shape":{"data":{"p":{"x":446.4979166245305,"y":23.395168693785024},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1263861426676729":{"id":"de1263861426676729","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.5579350812384536"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.3478954273203627"}],"id":"n0.19435338820378134"}],"id":"n0.6165632336495481"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.48810065734612507"}],"id":"n0.6527594226319431"}],"id":"n0.9927622996794807"}},"id":"n0.3310870136335953"},{"type":"single","text":"(","id":"n0.24733232207573397"},{"text":"s,a","id":"n0.2640130706228947"},{"type":"single","text":")","id":"n0.320797152671904"}],"id":"n0.12385914641248141"}],"id":"n0.10292510313515457"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.8792233341240645"}],"style":{"align":"center"},"id":"n0.581431440814911"}],"shape":{"data":{"p":{"x":225.07317358969993,"y":153.98044260802277},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7586505332283031":{"id":"de7586505332283031","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.4927180768830606"}],"id":"n0.7049969082472012"}],"id":"n0.5491990457901264"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8331730280336691"}],"style":{"align":"center"},"id":"n0.4908615520610786"}],"shape":{"data":{"p":{"x":217.66564246893194,"y":205.87532714036234},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de769876825831503":{"id":"de769876825831503","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.2476163548834478"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.05289691975208344"}],"id":"n0.9475595525928506"}],"id":"n0.26913830451602294"}},"id":"n0.3823787096886917"},{"text":"|","id":"n0.3572567729085736"}],"id":"n0.6437754419605293"}],"id":"n0.801448369692964"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8248570835206583"}],"style":{"align":"center"},"id":"n0.33378938373308187"}],"shape":{"data":{"p":{"x":125.09038550376243,"y":124.16184319124937},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9878510090899617":{"id":"de9878510090899617","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.26474967983170705"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8971092040815121"}],"id":"n0.589078373381241"}],"id":"n0.6144261277188128"}},"id":"n0.6252549284208646"},{"text":"|","id":"n0.012925371806804309"}],"id":"n0.9645001095314869"}],"id":"n0.16824565767494604"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.36432594095690884"}],"style":{"align":"center"},"id":"n0.9517376011612726"}],"shape":{"data":{"p":{"x":125.09038550376243,"y":104.16184319124937},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de040532016393358905":{"id":"de040532016393358905","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|𝛺","id":"n0.017627045438355138"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.567640267774302"}],"id":"n0.5876253790254438"}],"id":"n0.8016798244873558"}},"id":"n0.29881555110954827"},{"text":"|","id":"n0.5141272299841424"}],"id":"n0.8320770388847725"}],"id":"n0.5233019382756188"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3876548054566744"}],"style":{"align":"center"},"id":"n0.7670897406456516"}],"shape":{"data":{"p":{"x":125.09038550376243,"y":83.16184319124937},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4342493044242768":{"id":"de4342493044242768","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.9688909438345801"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.11465109772496085"}],"id":"n0.805198393901633"}],"id":"n0.9860014414794123"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.3365944052709"}],"id":"n0.24308677305968152"}],"id":"n0.33971423872499673"}},"id":"n0.4481408429704987"},{"type":"single","text":"(","id":"n0.48292648096903945"},{"text":"s","id":"n0.09419811564487834"},{"type":"single","text":")","id":"n0.1532926878468186"}],"id":"n0.9863990264272267"}],"id":"n0.39686664852335385"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.47318647813400827"}],"style":{"align":"center"},"id":"n0.4561115989782121"}],"shape":{"data":{"p":{"x":569.4979166245305,"y":164.39516869378502},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de1069292797428456":{"id":"de1069292797428456","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"composite","text":"\\Pr","elements":{},"id":"n0.893109935736548"},{"type":"single","text":"(","id":"n0.9543708301694047"},{"text":"o","id":"n0.9304630750587284"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7951549406875484"}],"id":"n0.3259176389383067"}],"id":"n0.3838815664172657"}},"id":"n0.012190115400921409"},{"text":"|s,a","id":"n0.6633100830421328"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4796694870508367"}],"id":"n0.08360553435830642"}],"id":"n0.8402381803414027"}},"id":"n0.22742123199036857"},{"type":"single","text":")","id":"n0.9526418894946047"}],"id":"n0.21882807550247785"}],"id":"n0.7414166285458648"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.15957685423588397"}],"style":{"align":"center"},"id":"n0.8382613973508035"}],"shape":{"data":{"p":{"x":319.7082014974316,"y":23.743954711688957},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7272921803134598":{"id":"de7272921803134598","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.6169228088745604"}],"id":"n0.8192075369172236"}],"id":"n0.5053983715856316"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.49323858999303005"}],"style":{"align":"center"},"id":"n0.22946509979998075"}],"shape":{"data":{"p":{"x":308.06606823920555,"y":39.44087589846373},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3762499993351762":{"id":"de3762499993351762","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.07320753465653862"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.46024205589598743"}],"id":"n0.9452681236751148"}],"id":"n0.6955125721326587"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.5312255638734711"}],"id":"n0.39967597290956625"}],"id":"n0.9341639557260559"}},"id":"n0.4175368060735638"},{"type":"single","text":"(","id":"n0.8125475236978077"},{"text":"s","id":"n0.351545201203727"},{"type":"single","text":")","id":"n0.7249340044377426"}],"id":"n0.5234834432647619"}],"id":"n0.8204346809622691"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.1835526429852079"}],"style":{"align":"center"},"id":"n0.36577372130072083"}],"shape":{"data":{"p":{"x":569.4979166245305,"y":265.395168693785},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5537469412531904":{"id":"de5537469412531904","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b′","id":"n0.3444215796140062"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6732995066259508"}],"id":"n0.2317602136179413"}],"id":"n0.04477763558765413"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.24421246794559215"}],"id":"n0.24136736621281973"}],"id":"n0.802362797715338"}},"id":"n0.036129547494320846"},{"type":"single","text":"(","id":"n0.1905873277459469"},{"text":"s,a","id":"n0.7504823179517286"},{"type":"single","text":")","id":"n0.9556456824948709"}],"id":"n0.4968593472306042"}],"id":"n0.6329778626633036"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.5871582382398293"}],"style":{"align":"center"},"id":"n0.031214142057099936"}],"shape":{"data":{"p":{"x":240.2436271377868,"y":254.98044260802277},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de38487360283742666":{"id":"de38487360283742666","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⟨s,a⟩∈P","id":"n0.9493257460171807"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.0637310156548887"}],"id":"n0.6215067546401203"}],"id":"n0.19531961549334165"},"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.010474151883645755"}],"id":"n0.5030753749829053"}],"id":"n0.301602005952047"}},"id":"n0.8037365022814322"}],"id":"n0.7795957295841542"}],"id":"n0.8476611167760499"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6221849330837028"}],"id":"n0.26477504035527244"}],"shape":{"data":{"p":{"x":238.34978491782493,"y":286.7481257493629},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9715702645442834":{"id":"de9715702645442834","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.6249619007940019"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.7804181971152868"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.5010191634308674"}],"id":"n0.09833512951191548"}],"id":"n0.7775190735055468"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.6356951276867575"}],"id":"n0.8668797493357865"}],"id":"n0.32877103183081413"}},"id":"n0.4500177953582223"}],"id":"n0.83712498968937"}],"id":"n0.04838708755876753"}},"id":"n0.7587963723902582"},{"type":"single","text":"(","id":"n0.9035787260749824"},{"text":"s,a","id":"n0.9119426963835975"},{"type":"single","text":")","id":"n0.8996281514045852"}],"id":"n0.44456487845322856"}],"id":"n0.37357327720965383"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3415234652411294"}],"style":{"align":"center"},"id":"n0.08209456400124648"}],"shape":{"data":{"p":{"x":117.49150793312418,"y":254.38679544305194},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de777519150267751":{"id":"de777519150267751","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.708169864947874"}],"id":"n0.4600841538833922"}],"id":"n0.803624317973094"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.15327389506075506"}],"style":{"align":"center"},"id":"n0.13008437109947923"}],"shape":{"data":{"p":{"x":80.09038550376243,"y":295.8070040280952},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2938177892970333":{"id":"de2938177892970333","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.41806308068322995"}],"id":"n0.08978729943238095"}],"id":"n0.2483893817822127"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7966415745224384"}],"style":{"align":"center"},"id":"n0.22000167342181998"}],"shape":{"data":{"p":{"x":426.47145004048775,"y":38.98591809822463},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de49606201729253674":{"id":"de49606201729253674","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.4662020816813366"}],"id":"n0.9923703182999024"}],"id":"n0.10744352025325266"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.24604688373448957"}],"id":"n0.8519992825477789"}],"shape":{"data":{"p":{"x":111.09038550376243,"y":201.52163415504833}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de23325305718254907":{"id":"de23325305718254907","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.7979787517676606"}],"id":"n0.5573311515059192"}],"id":"n0.7963742656758848"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9131254761902869"}],"id":"n0.6855452719069914"}],"shape":{"data":{"p":{"x":481.0839768123562,"y":263.08373345003844}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9752351203905827":{"id":"de9752351203905827","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.5411448237521672"}],"id":"n0.42940441151394837"}],"id":"n0.6249678696487018"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5251141136924362"}],"id":"n0.6205838356665792"}],"shape":{"data":{"p":{"x":451.0839768123562,"y":263.04836357699156}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4427510142690705":{"id":"de4427510142690705","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.6473788903274942"}],"id":"n0.28172712935215594"}],"id":"n0.49565357867421134"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5717228225550308"}],"id":"n0.38989133361763373"}],"shape":{"data":{"p":{"x":363.07317358969993,"y":20.67738061500927}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de21516737336846048":{"id":"de21516737336846048","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.6552982732289234"}],"id":"n0.01837465200897337"}],"id":"n0.03166421290171506"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6980806282271741"}],"id":"n0.700129871063206"}],"shape":{"data":{"p":{"x":279.0839768123562,"y":21.083733450038437}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de66011368422189":{"id":"de66011368422189","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.4181417722821359"}],"id":"n0.2901340212969634"}],"id":"n0.9377912065800365"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7114358006326251"}],"id":"n0.9572312474456759"}],"shape":{"data":{"p":{"x":247.08397681235618,"y":21.048363576991562}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de17339897452830244":{"id":"de17339897452830244","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.32011581099575515"}],"id":"n0.48032552796931505"}],"id":"n0.6098667043946604"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.1918989233501993"}],"id":"n0.1123475664115372"}],"shape":{"data":{"p":{"x":492.09038550376243,"y":162.52163415504833}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6658095144342686":{"id":"de6658095144342686","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.04566694455289677"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"o","id":"n0.4690478936906626"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.26568131608860956"}],"id":"n0.4181611779164287"}],"id":"n0.9796608489781882"}},"id":"n0.19874676327498553"}],"id":"n0.17563860398529862"}],"id":"n0.518107722756628"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.030613434388105487"}],"id":"n0.0857132965788101"}],"id":"n0.5927140745037591"}},"id":"n0.44439756021995347"}],"id":"n0.7050310140621812"}],"id":"n0.5206787888668472"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9436715546247578"}],"id":"n0.8866638644305771"}],"shape":{"data":{"p":{"x":141.08397681235618,"y":75.3920107419624}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de7522212595218865":{"id":"de7522212595218865","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.9201805558857985"}],"id":"n0.4150342211710165"}],"id":"n0.9756851757003704"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.24536760764214205"}],"id":"n0.3505649113359728"}],"shape":{"data":{"p":{"x":299.09038550376243,"y":162.52163415504833}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de41418421309961495":{"id":"de41418421309961495","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.017504874173464913"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.4824121787239064"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.4089467599378185"}],"id":"n0.6951856021652583"}],"id":"n0.3903696214115149"}},"id":"n0.7157059533793924"}],"id":"n0.1548520232970234"}],"id":"n0.4634946863213816"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.44582937785428833"}],"id":"n0.24721055235684797"}],"id":"n0.9602180403860188"}},"id":"n0.6160427835409938"}],"id":"n0.5660597128568199"}],"id":"n0.1301789488913847"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.07306106530879108"}],"id":"n0.5756709131973967"}],"shape":{"data":{"p":{"x":139.08397681235618,"y":117.73626428200146}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de4746109038062831":{"id":"de4746109038062831","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜂","id":"n0.6466061046461433"}],"id":"n0.7302807030126197"}],"id":"n0.7891280452896823"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8189562118218683"}],"id":"n0.5711161538928315"}],"shape":{"data":{"p":{"x":400.4893586136384,"y":18.62877564979931},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de14515593214146394":{"id":"de14515593214146394","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"+","id":"n0.3993967946976933"}],"id":"n0.8513486599475975"}],"id":"n0.7635312661181304"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.3389140722650501"}],"id":"n0.014183471947202264"}],"shape":{"data":{"p":{"x":613.0903855037625,"y":162.52163415504833}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de31945308578801956":{"id":"de31945308578801956","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.6761337058482566"}],"id":"n0.8322914479919379"}],"id":"n0.4975080524356512"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7533020277434055"}],"id":"n0.04571303176510533"}],"shape":{"data":{"p":{"x":172.09038550376243,"y":162.52163415504833}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de3437232299036792":{"id":"de3437232299036792","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.7836336026147002"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.8669790981921077"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.45006927492141435"}],"id":"n0.8432470184549252"}],"id":"n0.7760493020829007"}},"id":"n0.8510052871461884"}],"id":"n0.6085925846811548"}],"id":"n0.7845320934138384"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.7598083618016642"}],"id":"n0.2333118184252101"}],"id":"n0.10901128152382666"}},"id":"n0.22888754770276676"}],"id":"n0.6781410424131757"}],"id":"n0.6933598697700811"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9928222755901932"}],"id":"n0.4175433094163179"}],"shape":{"data":{"p":{"x":139.08397681235618,"y":96.73626428200146}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de7044486226873938":{"id":"de7044486226873938","lines":[{"blocks":[{"text":"Env of ","style":{"fontSize":"\\tiny"},"id":"n0.5099793436595266"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4672407192966339"}],"id":"n0.7945254040989973"}],"id":"n0.5184897446323622"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.3030723685580643"}],"style":{"align":"center"},"id":"n0.6399406701300896"}],"shape":{"data":{"p":{"x":71.0172119140625,"y":19.836657214963566},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de12233133224262716":{"id":"de12233133224262716","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.6066601636292384"}],"id":"n0.17172801310522656"}],"shape":{"data":{"p":{"x":146.0093994140625,"y":18.487637573017054},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de46179107522947693":{"id":"de46179107522947693","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.013630509284332293","text":"\\overline","type":"composite","elements":{"value":{"id":"n0.1758891244744567","lines":[{"id":"n0.5764298561436061","blocks":[{"id":"n0.6936611013083895","text":"T"},{"id":"n0.38120918513713975","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2740917218026975","lines":[{"id":"n0.2623134127841795","blocks":[{"id":"n0.1398397090605179","text":"j"}]}]}}}]}]}}},{"id":"n0.8637212773995331","type":"single","text":"("},{"id":"n0.1184595306083227","text":"s"},{"id":"n0.7995764123716085","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.22694177844776497","lines":[{"id":"n0.9719713993739867","blocks":[{"id":"n0.36678450979810284","text":"j"}]}]}}},{"id":"n0.44743090344259095","text":",a"},{"id":"n0.9732165628501099","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9740311565942015","lines":[{"id":"n0.5282287035504141","blocks":[{"id":"n0.8611731955874364","text":"j"}]}]}}},{"id":"n0.4518938002610928","text":",s"},{"id":"n0.33445895890955124","text":"\\power-index","type":"composite","elements":{"indexValue":{"id":"n0.19409567144365947","lines":[{"id":"n0.21874968140141626","blocks":[{"id":"n0.8869740525148799","text":"j"}]}]},"powerValue":{"id":"n0.9581713259022835","lines":[{"id":"n0.33154237150314714","blocks":[{"id":"n0.5128302910455178","text":"′"}]}]}}},{"id":"n0.5208916699492883","type":"single","text":")"}],"id":"n0.3168167494404379"}],"id":"n0.4767325958984765"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.2627541312577786"}],"style":{"align":"center"},"id":"n0.1063418548762598"}],"shape":{"data":{"p":{"x":285.610837007667,"y":211.439940578934},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7780578807104204":{"id":"de7780578807104204","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.3511778113409634"}],"id":"n0.6791373232583222"}],"id":"n0.9190651324944978"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\scriptsize"},"id":"n0.5102771242337476"}],"id":"n0.727761724805509"}],"shape":{"data":{"p":{"x":279.47431307477996,"y":182},"rotation":49.5},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de7949056139072763":{"id":"de7949056139072763","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.7323452707351161"}],"id":"n0.9998912548605183"}],"id":"n0.2695926434935332"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.06716032875908473"}],"id":"n0.3041700245436336"}],"shape":{"data":{"p":{"x":393.398973109876,"y":163.85714149475098},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de18751418875508108":{"id":"de18751418875508108","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.6657655635791759"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.6988767036565222","text":"S"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"j","id":"n0.9918120171219929"}],"id":"n0.4639519314559222"}],"id":"n0.9002291473294042"}},"id":"n0.3696878338976073"}],"id":"n0.7807554544460695"}],"id":"n0.22070928010431268"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.03709216209504618"}],"style":{"align":"center"},"id":"n0.24756927622662173"}],"shape":{"data":{"p":{"x":387.6132065083135,"y":176.49503087997437},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4732927849438495":{"id":"de4732927849438495","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"\\overline","type":"composite","elements":{"value":{"lines":[{"blocks":[{"text":"T","id":"n0.6690562907245137"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.8251746388397112","text":"i"}],"id":"n0.7872000785640887"}],"id":"n0.5671193837451141"}},"id":"n0.6653553919120421"}],"id":"n0.8743865335203924"}],"id":"n0.7369081718594115"}},"id":"n0.8307042719014721"},{"type":"single","text":"(","id":"n0.8161136531935869"},{"text":"s","id":"n0.6317085800446827"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.863245780817153","text":"i"}],"id":"n0.19411642848546928"}],"id":"n0.15499224249872112"}},"id":"n0.07263915415971667"},{"text":",a","id":"n0.35331379313221434"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.19072136140105989","text":"i"}],"id":"n0.28789446170314803"}],"id":"n0.7535370809803013"}},"id":"n0.5786958769021082"},{"text":",s","id":"n0.8729865630953615"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.27671413047786286","text":"i"}],"id":"n0.0658217758732682"}],"id":"n0.8357421006926671"},"powerValue":{"lines":[{"blocks":[{"text":"′","id":"n0.38218768799271197"}],"id":"n0.4181362511671829"}],"id":"n0.5053937731298157"}},"id":"n0.35834813904867335"},{"type":"single","text":")","id":"n0.9331666725428862"}],"id":"n0.6269908053119784"}],"id":"n0.8307652002174195"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.2505705598926036"}],"style":{"align":"center"},"id":"n0.6554982900972093"}],"shape":{"data":{"p":{"x":480.610837007667,"y":210.439940578934},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de050079977272444065":{"id":"de050079977272444065","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.1738546458892547"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5114629739047636"}],"id":"n0.2614889628337296"}],"id":"n0.48558053202701057"}},"id":"n0.031390229467598285"},{"text":"|×|A","id":"n0.44019166576794566"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4637563564016487"}],"id":"n0.8669426250713395"}],"id":"n0.22756702503613369"}},"id":"n0.9448409720070239"},{"text":"|×|S","id":"n0.6901681656015859"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9829367529890434"}],"id":"n0.14589201133848984"}],"id":"n0.4412492132056076"}},"id":"n0.15350060445090596"},{"text":"|","id":"n0.6097945030746335"}],"id":"n0.359211311045716"}],"id":"n0.5307342112945057"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.960813422623283"}],"style":{"align":"center"},"id":"n0.9181020972926659"}],"shape":{"data":{"p":{"x":444.9753875732422,"y":229.96709218025205},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6309121644461761":{"id":"de6309121644461761","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.7226923294314347"}],"id":"n0.18588346131724376"}],"id":"n0.771851697492894"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\scriptsize"},"id":"n0.8944203923289638"}],"id":"n0.22539485656992042"}],"shape":{"data":{"p":{"x":474.47431307477996,"y":181},"rotation":49.5},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de9901244604061572":{"id":"de9901244604061572","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.6103673174997359"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.983002655974881"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7018351678973132","text":"i"}],"id":"n0.7010329296925055"}],"id":"n0.7244476972754041"}},"id":"n0.17542069322933473"}],"id":"n0.19976495412619033"}],"id":"n0.9154711282656824"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.21271815915282222"}],"style":{"align":"center"},"id":"n0.5686213055828779"}],"shape":{"data":{"p":{"x":520.6132065083135,"y":176.49503087997437},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4468797854678037":{"id":"de4468797854678037","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.9747497283041866"}],"id":"n0.08076912011418358"}],"id":"n0.5883148292773521"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.866124436049301"}],"id":"n0.8475282880647284"}],"shape":{"data":{"p":{"x":526.398973109876,"y":163.85714149475098},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6963008676951739":{"id":"de6963008676951739","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.9467432607928974"}],"id":"n0.38641848532049905"}],"id":"n0.5349620693643276"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7052032195921623"}],"style":{"align":"center"},"id":"n0.006805448686313831"}],"shape":{"data":{"p":{"x":551.4714500404878,"y":179.98591809822463},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5307733598657904":{"id":"de5307733598657904","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.07306710235810865"}],"id":"n0.37648057370659616"}],"id":"n0.10130076633391227"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.7743980585092951"}],"style":{"align":"center"},"id":"n0.9014467266778325"}],"shape":{"data":{"p":{"x":549.4714500404878,"y":279.9859180982246},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de35702312713851314":{"id":"de35702312713851314","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|×|S|","id":"n0.9098320743091413"}],"id":"n0.28064584064339515"}],"id":"n0.31823182025495567"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8374452296648147"}],"style":{"align":"center"},"id":"n0.9010594346309162"}],"shape":{"data":{"p":{"x":301.99359130859375,"y":278.9718017578125},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9284763344198799":{"id":"de9284763344198799","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.3777097004849297","text":"T"},{"id":"n0.6035946850133376","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6458733035771684","lines":[{"id":"n0.8996133625620213","blocks":[{"id":"n0.04865555559290735","text":"i"}]}]}}},{"type":"single","text":"(","id":"n0.9430238294952795"},{"text":"s,a,s","id":"n0.5718031955471183"},{"id":"n0.2761454214500738","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.7897967364936616","lines":[{"id":"n0.9758438418244391","blocks":[{"id":"n0.4895623117809469","text":"′"}]}]}}},{"type":"single","text":")","id":"n0.47133613654659334"}],"id":"n0.45421291588955426"}],"id":"n0.803263754257443"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.24979216144084027"}],"style":{"align":"center"},"id":"n0.8280339397799843"}],"shape":{"data":{"p":{"x":379.40112242936175,"y":233.27918469789847},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de8341143779891083":{"id":"de8341143779891083","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"×","id":"n0.919589422656347"}],"id":"n0.507537421036887"}],"id":"n0.25074793897328806"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.04248175548225519"}],"id":"n0.32866920481796"}],"shape":{"data":{"p":{"x":420.0839768123562,"y":263.04836357699156}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de40063125596160476":{"id":"de40063125596160476","lines":[{"blocks":[{"text":"along ","style":{"fontSize":{"value":0.4}},"id":"n0.30820532932014166"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"S","id":"n0.33575061932716554"}],"id":"n0.22267003548064213"}],"id":"n0.7776956814282687"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4572670445753324"}],"style":{"align":"center"},"id":"n0.22331571707557485"}],"shape":{"data":{"p":{"x":513.6132065083135,"y":276.49503087997437},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de24456460257009915":{"id":"de24456460257009915","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"Σ","id":"n0.537723752459317"}],"id":"n0.36660980309716384"}],"id":"n0.013381938972016005"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.14629858535251006"}],"id":"n0.8005719086749645"}],"shape":{"data":{"p":{"x":517.398973109876,"y":263.857141494751},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de1363233054056363":{"id":"de1363233054056363","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S","id":"n0.2640899370100982"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7957312675333303","text":"j"}],"id":"n0.4289763060352012"}],"id":"n0.5636851996964858"}},"id":"n0.6200066969093145"},{"text":"|×|A","id":"n0.24931989747100292"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7061769676734742","text":"j"}],"id":"n0.8338566948931943"}],"id":"n0.6497095558154655"}},"id":"n0.6467263721354128"},{"text":"|×|S","id":"n0.681059980774184"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4234643670864695","text":"j"}],"id":"n0.2839239830649629"}],"id":"n0.9936617197736568"}},"id":"n0.10945988810950902"},{"text":"|","id":"n0.2779183338745703"}],"id":"n0.06478265473108147"}],"id":"n0.5747157058513406"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.07143623474426697"}],"style":{"align":"center"},"id":"n0.9594258614626692"}],"shape":{"data":{"p":{"x":231.9753875732422,"y":214.96709218025205},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8164181201179905":{"id":"de8164181201179905","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.36909629287933576"}],"id":"n0.23203813653136018"}],"shape":{"data":{"p":{"x":69.5093994140625,"y":86.98763757301705},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de917768460299415":{"id":"de917768460299415","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.810206964359198"}],"id":"n0.987302506030517"}],"shape":{"data":{"p":{"x":54.5093994140625,"y":161.98763757301705},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de577878045869977":{"id":"de577878045869977","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"NN layers","id":"n0.4064584503096027"}],"id":"n0.6168405228893412"}],"shape":{"data":{"p":{"x":39.5093994140625,"y":238.98763757301705},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de25110577288426494":{"id":"de25110577288426494","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"optionally dependent","id":"n0.4294657609427419"}],"id":"n0.2075778433860329"}],"shape":{"data":{"p":{"x":26.0093994140625,"y":44.487637573017054},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9499061837025173":{"id":"de9499061837025173","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"O","id":"n0.03930271760983639"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9011877772769519"}],"id":"n0.2388782643341718"}],"id":"n0.7468827239368123"}},"id":"n0.6953668642779995"},{"type":"single","text":"(","id":"n0.867129969382012"},{"text":"s,a","id":"n0.14021984306407043"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7655408689436833"}],"id":"n0.6550037690461015"}],"id":"n0.40458429035569443"}},"id":"n0.12811158542692813"},{"text":",o","id":"n0.04109526130856023"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9264905662614205"}],"id":"n0.6836812671851038"}],"id":"n0.696923725427885"}},"id":"n0.13306711535718385"},{"type":"single","text":")","id":"n0.06019184064626515"}],"id":"n0.4699397483891101"}],"id":"n0.7532302997838924"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9532813190383616"}],"style":{"align":"center"},"id":"n0.6075074297187724"}],"shape":{"data":{"p":{"x":201.41693053483044,"y":10.859427538141873},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":false},"de5622973739907038":{"id":"de5622973739907038","lines":[{"blocks":[{"text":"Envs","style":{"fontSize":"\\tiny"},"id":"n0.21323080848364517"}],"style":{"align":"center"},"id":"n0.5256645226151633"}],"shape":{"data":{"p":{"x":14.0172119140625,"y":19.836657214963566},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6571793473371186":{"id":"de6571793473371186","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.5029636989508328","text":"1-"},{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.5923570668684544"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.4834162458318534"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.32720262256835997"}],"id":"n0.48124815737646"}],"id":"n0.6927750915470068"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.5237791160596883"}],"id":"n0.6078049422868859"}],"id":"n0.6621310130027627"}},"id":"n0.2934739111828135"}],"id":"n0.01844241672470992"}],"id":"n0.6640143275241097"}},"id":"n0.10774757238169008"}],"id":"n0.5698678369589656"}],"id":"n0.9213915518587037"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6941094154964307"}],"style":{"align":"center"},"id":"n0.5991071178838041"}],"shape":{"data":{"p":{"x":183.49150793312418,"y":214.5206788661286},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8759589275482531":{"id":"de8759589275482531","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⟨s,a⟩∈","id":"n0.07936266846190287"}],"id":"n0.8149341385306228"}],"id":"n0.13020470631706216"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5524560793549289"}],"id":"n0.4859903828788752"}],"shape":{"data":{"p":{"x":229.07317358969988,"y":180.2828582611303},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de027912896577368507":{"id":"de027912896577368507","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"P","id":"n0.8348951616133002"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.294027956435992"}],"id":"n0.9879948918298702"}],"id":"n0.7322371853995608"},"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.8647546073343904"}],"id":"n0.8126379184044228"}],"id":"n0.462874068420569"}},"id":"n0.19183621734909861"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"∁","id":"n0.8307733655110068"}],"id":"n0.8500675537164684"}],"id":"n0.21676817271064475"}},"id":"n0.5730612827824997"}],"id":"n0.10160514417398603"}],"id":"n0.8721596412132258"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5086512898297695"}],"id":"n0.8667644861112345"}],"shape":{"data":{"p":{"x":235.07317358969988,"y":191.2828582611303},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di11968482578171047","items":[],"style":{}},"shapes":[{"id":"dp736494545583406","type":"doc-cube","data":{"p1":{"x":206.98281860351562,"y":166.27390942729653},"p2":{"x":249.24650750432158,"y":203.98385620117188},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp3937974403007931","type":"doc-cube","data":{"p1":{"x":206.98281860351562,"y":133.97149377418896},"p2":{"x":249.24650750432158,"y":171.68144054806442},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dg4857174382127132","entities":[{"id":"dg3449782978264446","entities":[{"id":"dp06947519900625876","type":"rectangle","data":{"p1":{"x":138.08397681235618,"y":101.7182343874357},"p2":{"x":150.74113754441504,"y":114.37539511949456}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp20987111150207616","type":"rectangle","data":{"p1":{"x":139.66612190386348,"y":103.30037947894306},"p2":{"x":152.32328263592234,"y":115.95754021100191}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp49462251128848367","type":"rectangle","data":{"p1":{"x":141.2482669953709,"y":104.88252457045041},"p2":{"x":153.90542772742975,"y":117.53968530250927}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl42310251642970464","linkedId":"de3437232299036792"}]},{"id":"da8512811121136399","data":[{"x":179.9299333078854,"y":33.451896417373916},{"x":195.08397681235618,"y":33.451896417373916}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dp9164171276212354","type":"doc-cube","data":{"p1":{"x":104,"y":154.98763757301708},"p2":{"x":142.09035498618437,"y":192.69758434689254},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da36194738276189287","data":[{"x":142.0724769306118,"y":175.26897912575146},{"x":174.30461890219993,"y":175.26897912575146}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6925834452262651","entities":[{"id":"dp7122737596261504","type":"circle","data":{"p1":{"x":174.30461890219993,"y":165.3430605466499},"p2":{"x":193.84033495902366,"y":184.87877660347363}}},{"id":"dl21082570538075251","linkedId":"de31945308578801956"}]},{"id":"da9781576713698847","data":[{"x":184.0724769306118,"y":195.5987463529243},{"x":184.0724769306118,"y":184.87877660347363}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9130259516533765","data":[{"x":259.09978491782493,"y":175.11091857506176},{"x":301.30461890219993,"y":175.11091857506176}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da8078770409643174","data":[{"x":320.84033495902366,"y":175.44642591476443},{"x":392.6132065083135,"y":175.44642591476443}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da5717337911460176","data":[{"x":412.14892256513724,"y":174.91141544819288},{"x":494.30461890219993,"y":174.91141544819288}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp015528813822181187","type":"doc-cube","data":{"p1":{"x":219.98281860351557,"y":267.27390942729653},"p2":{"x":262.2465075043216,"y":304.9838562011719},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp10757977244525407","type":"doc-cube","data":{"p1":{"x":219.98281860351557,"y":234.97149377418896},"p2":{"x":262.2465075043216,"y":272.6814405480644},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1]}},{"id":"dp8961558328475161","type":"doc-cube","data":{"p1":{"x":230.83609601701892,"y":277.5729114872548},"p2":{"x":273.09978491782493,"y":315.2828582611303},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp6167927249451948","type":"doc-cube","data":{"p1":{"x":230.83609601701892,"y":245.57291148725483},"p2":{"x":273.09978491782493,"y":283.2828582611303},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da5541931341066593","data":[{"x":596.099784917825,"y":174.91141544819288},{"x":612.3046189022,"y":174.91141544819288}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg5507586732404957","entities":[{"id":"dp2474566988972675","type":"circle","data":{"p1":{"x":612.3046189022,"y":165.3430605466499},"p2":{"x":631.8403349590237,"y":184.87877660347363}}},{"id":"dl9309649904975439","linkedId":"de14515593214146394"}]},{"id":"dp25197333914514775","type":"doc-cube","data":{"p1":{"x":433.0903855037625,"y":13.987637573017082},"p2":{"x":471.18074048994686,"y":51.69758434689254},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"dp37574443914210653","type":"right-arrow","data":{"p1":{"x":474.77320936917886,"y":29.196645047242328},"p2":{"x":487.77320936917886,"y":41.701389004761864},"arrowPercentage":0.4}},{"id":"dp08763935736717032","type":"right-arrow","data":{"p1":{"x":86.7732093691788,"y":167.19664504724233},"p2":{"x":99.7732093691788,"y":179.70138900476186},"arrowPercentage":0.4}},{"id":"dg13119570528477054","entities":[{"id":"dp646631666663311","type":"circle","data":{"p1":{"x":398.7035920120759,"y":23.4502020414009},"p2":{"x":418.2393080688996,"y":42.98591809822463}}},{"id":"dl6858481371533711","linkedId":"de4746109038062831"}]},{"id":"dg7135466245084179","entities":[{"id":"dg8432308452604242","entities":[{"id":"dp8942514088023354","type":"rectangle","data":{"p1":{"x":138.08397681235618,"y":122.7182343874357},"p2":{"x":150.74113754441504,"y":135.37539511949456}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp35227720864097356","type":"rectangle","data":{"p1":{"x":139.66612190386348,"y":124.30037947894306},"p2":{"x":152.32328263592234,"y":136.9575402110019}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp32821010554962604","type":"rectangle","data":{"p1":{"x":141.2482669953709,"y":125.88252457045041},"p2":{"x":153.90542772742975,"y":138.53968530250927}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl31480972409938146","linkedId":"de41418421309961495"}]},{"id":"dp1387905064421593","type":"doc-cube","data":{"p1":{"x":217.66564246893194,"y":176.57291148725483},"p2":{"x":259.09978491782493,"y":214.2828582611303},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[190,255,240,1],"strokeType":"-"}},{"id":"dp19759085845352287","type":"doc-cube","data":{"p1":{"x":217.66564246893194,"y":144.57291148725483},"p2":{"x":259.09978491782493,"y":182.2828582611303},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da3810595798413534","data":[{"x":193.84033495902366,"y":175.11091857506176},{"x":206.0093994140625,"y":175.11091857506176}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg14935737342636268","entities":[{"id":"dp7130874326641121","type":"circle","data":{"p1":{"x":301.30461890219993,"y":165.3430605466499},"p2":{"x":320.84033495902366,"y":184.87877660347363}}},{"id":"dl3679786690104043","linkedId":"de7522212595218865"}]},{"id":"da6732502125459128","data":[{"x":311.0724769306118,"y":165.3430605466499},{"x":311.0724769306118,"y":131.26435173617125}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da6645842690011527","data":[{"x":154.09978491782493,"y":131.26435173617125},{"x":311.0724769306118,"y":131.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg034018568564376794","entities":[{"id":"dg010410268580065107","entities":[{"id":"dp2671548493581788","type":"rectangle","data":{"p1":{"x":138.08397681235618,"y":80.37398084739664},"p2":{"x":150.74113754441504,"y":93.0311415794555}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp39155139166343367","type":"rectangle","data":{"p1":{"x":139.66612190386348,"y":81.956125938904},"p2":{"x":152.32328263592234,"y":94.61328667096285}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp9534721276938438","type":"rectangle","data":{"p1":{"x":141.2482669953709,"y":83.53827103041135},"p2":{"x":153.90542772742975,"y":96.1954317624702}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl8828715697007943","linkedId":"de6658095144342686"}]},{"id":"da5686891709937563","data":[{"x":153.90542772742975,"y":110.26435173617125},{"x":504.07247693061186,"y":110.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg22020581913434567","entities":[{"id":"dp1786034723960801","type":"circle","data":{"p1":{"x":494.30461890219993,"y":165.3430605466499},"p2":{"x":513.8403349590237,"y":184.87877660347363}}},{"id":"dl5377592576205668","linkedId":"de17339897452830244"}]},{"id":"da6626157824412076","data":[{"x":504.07247693061186,"y":165.3430605466499},{"x":504.07247693061186,"y":110.26435173617125}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da007611409748998321","data":[{"x":513.8403349590237,"y":175.11091857506176},{"x":525.6132065083135,"y":175.11091857506176}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp23841769197210172","type":"doc-cube","data":{"p1":{"x":558.0903855037625,"y":154.98763757301708},"p2":{"x":596.1807404899469,"y":192.69758434689254},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da014232816717384411","data":[{"x":622.0724769306119,"y":275.2828582611303},{"x":622.0724769306119,"y":184.87877660347363}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da3514202122360184","data":[{"x":536.1489225651372,"y":275.4464259147644},{"x":557.0093994140625,"y":275.4464259147644}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg42312302720444395","entities":[{"id":"dp4114507869592985","type":"circle","data":{"p1":{"x":249.29821021079368,"y":23.869789968593125},"p2":{"x":268.8339262676174,"y":43.405506025416855}}},{"id":"dl8024629095656042","linkedId":"de66011368422189"}]},{"id":"da12461802170632863","data":[{"x":235.09978491782493,"y":33.63764799700499},{"x":249.29821021079368,"y":33.63764799700499}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg22448264621035063","entities":[{"id":"dp1224597961569569","type":"circle","data":{"p1":{"x":281.2982102107937,"y":23.90515984164},"p2":{"x":300.8339262676174,"y":43.44087589846373}}},{"id":"dl4891615338121085","linkedId":"de21516737336846048"}]},{"id":"da038265993665470566","data":[{"x":268.8339262676174,"y":33.673017870051865},{"x":281.2982102107937,"y":33.673017870051865}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da4303535348042271","data":[{"x":300.8339262676174,"y":33.673017870051865},{"x":313.09978491782493,"y":33.673017870051865}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da12991360138833485","data":[{"x":259.06606823920555,"y":88.53827103041135},{"x":259.06606823920555,"y":43.405506025416855}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da8630138130538123","data":[{"x":291.06606823920555,"y":110.39399040804625},{"x":291.06606823920555,"y":43.44087589846373}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da4687117982275335","data":[{"x":153.90542772742975,"y":88.53827103041135},{"x":259.06606823920555,"y":88.53827103041135}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp2833493815756354","type":"doc-cube","data":{"p1":{"x":195.0093994140625,"y":33.451896417373916},"p2":{"x":235.17433179854055,"y":71.16184319124937},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp7211172021631458","type":"doc-cube","data":{"p1":{"x":195.0093994140625,"y":1.4518964173739164},"p2":{"x":235.17433179854055,"y":39.161843191249375},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp28182991976211436","type":"doc-cube","data":{"p1":{"x":314.0839768123562,"y":14.451896417373916},"p2":{"x":352.17433179854055,"y":52.161843191249375},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp41233534794370286","type":"doc-cube","data":{"p1":{"x":558.0903855037625,"y":255.98763757301708},"p2":{"x":596.1807404899469,"y":293.69758434689254},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da3578566881853964","data":[{"x":596.099784917825,"y":275.2828582611303},{"x":622.0724769306119,"y":275.2828582611303}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da22910905289663774","data":[{"x":441.8339262676174,"y":275.2828582611303},{"x":453.2982102107937,"y":275.2828582611303}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6119160641031665","entities":[{"id":"dp6940299382763646","type":"circle","data":{"p1":{"x":365.28740698813743,"y":23.498807006610832},"p2":{"x":384.8231230449612,"y":43.03452306343456}}},{"id":"dl8194607481224132","linkedId":"de4427510142690705"}]},{"id":"da06170766786087989","data":[{"x":352.09978491782493,"y":33.673017870051865},{"x":365.28740698813743,"y":33.673017870051865}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da7661767127582952","data":[{"x":375.0552650165493,"y":87.39399040804625},{"x":375.0552650165493,"y":43.03452306343456}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da5904324486887984","data":[{"x":375.0552650165493,"y":87.39399040804625},{"x":622.0724769306119,"y":87.39399040804625}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da39666738665513357","data":[{"x":622.0724769306119,"y":165.3430605466499},{"x":622.0724769306119,"y":87.39399040804625}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8621241068926349","data":[{"x":384.8231230449612,"y":33.2666650350227},{"x":398.7035920120759,"y":33.2666650350227}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da15883595570438813","data":[{"x":418.2393080688996,"y":33.218060069812765},{"x":432.1197770360145,"y":33.218060069812765}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg5665293210572151","entities":[{"id":"dp5223536771260155","type":"circle","data":{"p1":{"x":453.2982102107937,"y":265.8697899685931},"p2":{"x":472.8339262676174,"y":285.40550602541686}}},{"id":"dl9856755625912192","linkedId":"de9752351203905827"}]},{"id":"dg2859204043050667","entities":[{"id":"dp27442180512290504","type":"circle","data":{"p1":{"x":483.2982102107937,"y":265.90515984164},"p2":{"x":502.8339262676174,"y":285.44087589846373}}},{"id":"dl09600199380841445","linkedId":"de23325305718254907"}]},{"id":"da8204967439508815","data":[{"x":472.8339262676174,"y":275.67301787005186},{"x":483.2982102107937,"y":275.67301787005186}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da6400775207512097","data":[{"x":463.06606823920555,"y":319.26435173617125},{"x":463.06606823920555,"y":285.40550602541686}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9515171657668875","data":[{"x":493.06606823920555,"y":326.26435173617125},{"x":493.06606823920555,"y":285.44087589846373}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da10613409214611624","data":[{"x":72.09978491782493,"y":110.26435173617125},{"x":137.90542772742975,"y":110.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da2953123613930908","data":[{"x":77.0724769306118,"y":131.26435173617125},{"x":138.09978491782493,"y":131.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da4221174999797901","data":[{"x":77.0724769306118,"y":319.26435173617125},{"x":463.06606823920555,"y":319.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da2519721272826567","data":[{"x":77.0724769306118,"y":319.26435173617125},{"x":77.0724769306118,"y":131.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da32642060477246626","data":[{"x":72.09978491782493,"y":326.26435173617125},{"x":72.09978491782493,"y":110.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da6097416351721896","data":[{"x":72.09978491782493,"y":326.26435173617125},{"x":493.06606823920555,"y":326.26435173617125}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg28288844823488657","entities":[{"id":"dp21529388042290099","type":"circle","data":{"p1":{"x":113.30461890219993,"y":204.3430605466499},"p2":{"x":132.84033495902366,"y":223.87877660347363}}},{"id":"dl2703305754153198","linkedId":"de49606201729253674"}]},{"id":"da19119945301524477","data":[{"x":123.0724769306118,"y":204.3430605466499},{"x":123.0724769306118,"y":193.08636474609375}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"dp7751841189826612","type":"doc-cube","data":{"p1":{"x":99.40115294693982,"y":267.6802622623257},"p2":{"x":137.49150793312418,"y":305.39020903620104},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp09191320884543552","type":"doc-cube","data":{"p1":{"x":99.40115294693982,"y":235.37784660921812},"p2":{"x":137.49150793312418,"y":273.0877933830936},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp3598762218995919","type":"doc-cube","data":{"p1":{"x":110.08397681235618,"y":277.979264322284},"p2":{"x":148.17433179854055,"y":315.68921109615945},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp9971546776994589","type":"doc-cube","data":{"p1":{"x":110.08397681235618,"y":245.979264322284},"p2":{"x":148.17433179854055,"y":283.68921109615945},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp678013530603216","type":"rectangle","data":{"p1":{"x":72.53618240612298,"y":18.57503948597804},"p2":{"x":101.85864225206907,"y":47.89749933192411}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"da12399125708023151","data":[{"x":101.92993330788539,"y":33.451896417373916},{"x":144.0093994140625,"y":33.451896417373916}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dg03257418016404867","entities":[{"id":"dp3152110579077312","type":"rectangle","data":{"p1":{"x":152.0093994140625,"y":15.487637573017054},"p2":{"x":173.0093994140625,"y":50.487637573017054},"rotation":90}},{"id":"dl06335489444716114","linkedId":"de12233133224262716"}]},{"id":"dg022598253553454573","entities":[{"id":"dp7162741970895288","type":"rectangle","data":{"p1":{"x":264.8193317811682,"y":188.4010702276159},"p2":{"x":296.8992787641591,"y":217.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp7166353491492305","type":"rectangle","data":{"p1":{"x":268.1379472045726,"y":191.439940578934},"p2":{"x":300.2178941875636,"y":220.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp45092874176182973","type":"rectangle","data":{"p1":{"x":271.456562627977,"y":194.47881093025205},"p2":{"x":303.5365096109681,"y":223.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"dg9063844885927825","entities":[{"id":"dp3324864871780777","type":"rectangle","data":{"p1":{"x":282.2922215842626,"y":204.4010702276159},"p2":{"x":315.20073998648286,"y":233.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp16290898091617434","type":"rectangle","data":{"p1":{"x":285.6965512980523,"y":207.439940578934},"p2":{"x":318.6050697002727,"y":236.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp45688045414785683","type":"rectangle","data":{"p1":{"x":289.10088101184203,"y":210.47881093025205},"p2":{"x":322.0093994140625,"y":239.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{}},{"id":"da16784612594529036","data":[{"x":311.0724769306118,"y":204.21600341796875},{"x":311.0724769306118,"y":184.87877660347363}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dg18184788905852511","entities":[{"id":"dp8646170164656934","type":"circle","data":{"p1":{"x":392.6132065083135,"y":165.67856788635257},"p2":{"x":412.14892256513724,"y":185.2142839431763}}},{"id":"dl6828844980552891","linkedId":"de7949056139072763"}],"data":{"rotation":0}},{"id":"dg6537970351311602","entities":[{"id":"dp40893869773660274","type":"rectangle","data":{"p1":{"x":459.8193317811682,"y":187.4010702276159},"p2":{"x":491.8992787641591,"y":216.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp48003443565701986","type":"rectangle","data":{"p1":{"x":463.1379472045726,"y":190.439940578934},"p2":{"x":495.2178941875636,"y":219.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp7658880754652924","type":"rectangle","data":{"p1":{"x":466.456562627977,"y":193.47881093025205},"p2":{"x":498.5365096109681,"y":222.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{"rotation":0}},{"id":"dg8118707468459647","entities":[{"id":"dp5740912673943488","type":"rectangle","data":{"p1":{"x":477.2922215842626,"y":203.4010702276159},"p2":{"x":510.20073998648286,"y":232.77681502496227}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp35219300120680974","type":"rectangle","data":{"p1":{"x":480.6965512980523,"y":206.439940578934},"p2":{"x":513.6050697002727,"y":235.81568537628027}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp6242015767297737","type":"rectangle","data":{"p1":{"x":484.10088101184203,"y":209.47881093025205},"p2":{"x":517.0093994140625,"y":238.85455572759838}},"style":{"fillColor":[184,233,134,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}}],"data":{}},{"id":"da7178618526318812","data":[{"x":504.07247693061186,"y":203.4010702276159},{"x":504.07247693061186,"y":184.87877660347363}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dg21946987099562154","entities":[{"id":"dp08167676563876336","type":"circle","data":{"p1":{"x":525.6132065083135,"y":165.67856788635257},"p2":{"x":545.1489225651372,"y":185.2142839431763}}},{"id":"dl9823479464918712","linkedId":"de4468797854678037"}],"data":{"rotation":0}},{"id":"da7528501861897603","data":[{"x":545.1489225651372,"y":175.44642591476443},{"x":558.0093994140625,"y":175.44642591476443}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da06891007608653754","data":[{"x":273.0093994140625,"y":285.2828582611303},{"x":291.0093994140625,"y":285.2828582611303}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp36222220506471525","type":"doc-cube","data":{"p1":{"x":362.3107674431774,"y":245.10001179268778},"p2":{"x":400.40112242936175,"y":282.8099585665631},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp49160010269192633","type":"doc-cube","data":{"p1":{"x":362.3107674431774,"y":212.7975961395802},"p2":{"x":400.40112242936175,"y":250.50754291345567},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp028345364209015234","type":"doc-cube","data":{"p1":{"x":372.99359130859375,"y":255.87165357713053},"p2":{"x":411.0839462947781,"y":293.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp08300142719153847","type":"doc-cube","data":{"p1":{"x":372.99359130859375,"y":223.87165357713053},"p2":{"x":411.0839462947781,"y":261.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp20157966704302677","type":"doc-cube","data":{"p1":{"x":330.20960923433677,"y":245.10001179268778},"p2":{"x":368.29996422052113,"y":282.8099585665631},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp840449126725197","type":"doc-cube","data":{"p1":{"x":330.20960923433677,"y":212.7975961395802},"p2":{"x":368.29996422052113,"y":250.50754291345567},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp5184103697755356","type":"doc-cube","data":{"p1":{"x":340.89243309975313,"y":255.87165357713053},"p2":{"x":378.9827880859375,"y":293.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp38152875855088375","type":"doc-cube","data":{"p1":{"x":340.89243309975313,"y":223.87165357713053},"p2":{"x":378.9827880859375,"y":261.581600351006},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"da9346851626995165","data":[{"x":411.0093994140625,"y":275.2828582611303},{"x":422.2982102107937,"y":275.2828582611303}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dg5680346096153936","entities":[{"id":"dp20902577586770232","type":"circle","data":{"p1":{"x":422.2982102107937,"y":265.8697899685931},"p2":{"x":441.8339262676174,"y":285.40550602541686}}},{"id":"dl8017040983907677","linkedId":"de8341143779891083"}]},{"id":"da7586293919208427","data":[{"x":291.0093994140625,"y":303.39399040804625},{"x":432.06606823920555,"y":303.39399040804625}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7560479291363291","data":[{"x":291.0093994140625,"y":303.39399040804625},{"x":291.0093994140625,"y":285.2828582611303}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8899836517412827","data":[{"x":432.06606823920555,"y":303.39399040804625},{"x":432.06606823920555,"y":285.40550602541686}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da6017064760040944","data":[{"x":502.8339262676174,"y":275.4464259147644},{"x":516.6132065083135,"y":275.4464259147644}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg7716441606617934","entities":[{"id":"dp5518051175170133","type":"circle","data":{"p1":{"x":516.6132065083135,"y":265.67856788635254},"p2":{"x":536.1489225651372,"y":285.21428394317627}}},{"id":"dl7634889538117462","linkedId":"de24456460257009915"}],"data":{"rotation":0}},{"id":"da6913802546127341","data":[{"x":507.06606823920555,"y":338.08636474609375},{"x":507.06606823920555,"y":239.44087589846373}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da41338346233577594","data":[{"x":381.4011224293617,"y":344.08636474609375},{"x":381.4011224293617,"y":293.581600351006}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da8829406212403315","data":[{"x":301.4011224293617,"y":332.08636474609375},{"x":301.4011224293617,"y":240.08636474609375}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da6357185847481888","data":[{"x":40.92993330788539,"y":68.45189641737392},{"x":88.06606823920555,"y":68.45189641737392}],"head":"no","tail":"no","shaft":"--","headScale":0.6,"style":{"thickness":2}},{"id":"dg6791254461787495","entities":[{"id":"dp7486564023570643","type":"rectangle","data":{"p1":{"x":45.5093994140625,"y":85.98763757301705},"p2":{"x":66.5093994140625,"y":120.98763757301705},"rotation":180}},{"id":"dl35265567380820073","linkedId":"de8164181201179905"}]},{"id":"da15242885145344998","data":[{"x":88.06606823920555,"y":68.45189641737392},{"x":88.06606823920555,"y":48.8064075697439}],"head":"no","tail":"no","shaft":"--","headScale":0.6,"style":{"thickness":2}},{"id":"dg042014731349737655","entities":[{"id":"dp42646116629358155","type":"rectangle","data":{"p1":{"x":30.5093994140625,"y":160.98763757301705},"p2":{"x":51.5093994140625,"y":195.98763757301705},"rotation":180}},{"id":"dl05036021293983439","linkedId":"de917768460299415"}]},{"id":"dg5545058864855459","entities":[{"id":"dp6893988467776901","type":"rectangle","data":{"p1":{"x":15.5093994140625,"y":237.98763757301705},"p2":{"x":36.5093994140625,"y":272.9876375730171},"rotation":180}},{"id":"dl885283454862652","linkedId":"de577878045869977"}]},{"id":"da856743504473545","data":[{"x":56.92993330788539,"y":86.08636474609375},{"x":56.92993330788539,"y":68.45189641737392}],"head":"no","tail":"fh<","shaft":"--","headScale":0.6,"style":{"thickness":2}},{"id":"da8995970177679058","data":[{"x":40.92993330788539,"y":161.08636474609375},{"x":40.92993330788539,"y":68.08636474609375}],"head":"no","tail":"fh<","shaft":"--","headScale":0.6,"style":{"thickness":2}},{"id":"da6768359987484875","data":[{"x":25.929933307885392,"y":238.08636474609375},{"x":25.929933307885392,"y":47.21600341796875}],"head":"no","tail":"fh<","shaft":"--","headScale":0.6,"style":{"thickness":2}},{"id":"da38251931450937326","data":[{"x":56.92993330788545,"y":332.08636474609375},{"x":301.4011224293617,"y":332.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da7899027626513784","data":[{"x":40.92993330788539,"y":338.08636474609375},{"x":507.06606823920555,"y":338.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da13412493721590724","data":[{"x":25.929933307885392,"y":344.08636474609375},{"x":381.4011224293617,"y":344.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da997526913950449","data":[{"x":56.92993330788545,"y":332.08636474609375},{"x":56.92993330788545,"y":121.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da9611237820087917","data":[{"x":40.92993330788539,"y":338.08636474609375},{"x":40.92993330788539,"y":196.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"da5383501755569913","data":[{"x":25.929933307885392,"y":344.08636474609375},{"x":25.929933307885392,"y":273.08636474609375}],"head":"no","tail":"no","shaft":"-","headScale":0.6,"style":{"thickness":2}},{"id":"dp1794917753730061","type":"rectangle","data":{"p1":{"x":10.536182406122975,"y":18.57503948597804},"p2":{"x":39.858642252069075,"y":47.89749933192408}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"da1035032699410634","data":[{"x":40.0093994140625,"y":33.451896417373916},{"x":71.92993330788539,"y":33.451896417373916}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da656704405537178","data":[{"x":123.0724769306118,"y":235.5987463529243},{"x":123.0724769306118,"y":223.87877660347363}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp1508235303229002","type":"doc-cube","data":{"p1":{"x":163.40115294693982,"y":227.81414568540237},"p2":{"x":201.49150793312418,"y":265.5240924592777},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp9992749909706351","type":"doc-cube","data":{"p1":{"x":163.40115294693982,"y":195.5117300322948},"p2":{"x":201.49150793312418,"y":233.22167680617025},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp7034960302191771","type":"doc-cube","data":{"p1":{"x":174.08397681235618,"y":238.11314774536066},"p2":{"x":212.17433179854055,"y":275.8230945192361},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp49521555987026833","type":"doc-cube","data":{"p1":{"x":174.08397681235618,"y":206.11314774536066},"p2":{"x":212.17433179854055,"y":243.82309451923612},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da8544942580045773","data":[{"x":132.84033495902366,"y":214.11091857506176},{"x":155.0093994140625,"y":214.11091857506176}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8231745533625754","data":[{"x":155.0093994140625,"y":285.2828582611303},{"x":155.0093994140625,"y":214.11091857506176}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9346291681395247","data":[{"x":155.0093994140625,"y":285.2828582611303},{"x":220.0093994140625,"y":285.2828582611303}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6}],"settings":{"grid":true,"diagramHeight":345.9408874511719}}]},{"id":"n0.8469391538169186","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":3261,"delayRenderCache":{"av":3261,"map":{"n0.5562758659701175":{"n0.08847662245070831":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.5491990457901264":{"n0.7049969082472012":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.801448369692964":{"n0.6437754419605293":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.16824565767494604":{"n0.9645001095314869":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.5233019382756188":{"n0.8320770388847725":{"w":11.6193,"h":8.4545,"bl":0.8214}},"n0.803624317973094":{"n0.4600841538833922":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.0967657311158161":{"n0.6615510692663404":{"w":22.4157,"h":12.5054,"bl":0.7021}},"n0.5955230560954696":{"n0.9817385017994846":{"w":15.8511,"h":12.5054,"bl":0.7021}},"n0.10292510313515457":{"n0.12385914641248141":{"w":30.0022,"h":12.5054,"bl":0.7021}},"n0.39686664852335385":{"n0.9863990264272267":{"w":18.1297,"h":12.5054,"bl":0.7021}},"n0.7414166285458648":{"n0.21882807550247785":{"w":28.9352,"h":8.4545,"bl":0.8214}},"n0.8204346809622691":{"n0.5234834432647619":{"w":18.1297,"h":12.5054,"bl":0.7021}},"n0.6329778626633036":{"n0.4968593472306042":{"w":25.7161,"h":12.5054,"bl":0.7021}},"n0.8476611167760499":{"n0.7795957295841542":{"w":29.4687,"h":9.1146,"bl":0.7619}},"n0.37357327720965383":{"n0.44456487845322856":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.5206787888668472":{"n0.7050310140621812":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.1301789488913847":{"n0.5660597128568199":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.6933598697700811":{"n0.6781410424131757":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.6538694462700769":{"n0.8622852515762334":{"w":45.1298,"h":8.4545,"bl":0.8214}},"n0.4767325958984765":{"n0.3168167494404379":{"w":34.2972,"h":12.6682,"bl":0.6267}},"n0.22070928010431268":{"n0.7807554544460695":{"w":5.9498,"h":8.4545,"bl":0.8214}},"n0.5307342112945057":{"n0.359211311045716":{"w":45.2293,"h":8.4545,"bl":0.8214}},"n0.8307652002174195":{"n0.6269908053119784":{"w":33.5015,"h":12.6682,"bl":0.6267}},"n0.9154711282656824":{"n0.19976495412619033":{"w":5.7057,"h":8.4545,"bl":0.8214}},"n0.31823182025495567":{"n0.28064584064339515":{"w":39.4513,"h":8.1019,"bl":0.8571}},"n0.803263754257443":{"n0.45421291588955426":{"w":28.9804,"h":11.348,"bl":0.6717}},"n0.5747157058513406":{"n0.06478265473108147":{"w":45.9617,"h":8.4545,"bl":0.8214}},"n0.7532302997838924":{"n0.4699397483891101":{"w":30.3819,"h":8.4545,"bl":0.8214}},"n0.9213915518587037":{"n0.5698678369589656":{"w":20.7972,"h":9.9736,"bl":0.6963}},"n0.13020470631706216":{"n0.8149341385306228":{"w":21.8099,"h":8.1019,"bl":0.8571}},"n0.8721596412132258":{"n0.10160514417398603":{"w":12.0443,"h":11.0044,"bl":0.8028}}}}}

==> sIPOMDPLite-Net(arXiv)/plots/docs/f2c8181d-ae2e-4c8a-84e1-5fea8033fe03 <==
{"id":"n0.18805762998880904","lines":[{"id":"n0.10628078590158863","blocks":[]},{"id":"n0.04419106341594836","blocks":[{"id":"n0.8838103512889588","text":"\\diagram","type":"composite","elements":{"de6103756180794349":{"id":"de6103756180794349","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜃","style":{"mathType":"\\mathbf"},"id":"n0.22674499425613304"}],"id":"n0.8251165182411753"}],"id":"n0.34276351265372096"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.3104246612387036"}],"style":{"align":"center"},"id":"n0.28170482108071027"}],"shape":{"data":{"p":{"x":39.97359713596575,"y":178.63632516949775},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4921345059974387":{"id":"de4921345059974387","lines":[{"blocks":[{"text":"Envs","style":{"fontSize":"\\tiny"},"id":"n0.7886006601830433"}],"style":{"align":"center"},"id":"n0.2652218053583968"}],"shape":{"data":{"p":{"x":182.0172119140625,"y":178.83665721496357},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de09648216086759942":{"id":"de09648216086759942","lines":[{"blocks":[{"text":"MAQMDP planning module","style":{"fontSize":"\\tiny"},"id":"n0.1692246054674058"}],"style":{"align":"center"},"id":"n0.4574645504738164"}],"shape":{"data":{"p":{"x":277.026611328125,"y":167.7467308044433},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6319421349768997":{"id":"de6319421349768997","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.15166061834504974"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.759422983008895"}],"id":"n0.9918347669429193"}],"id":"n0.7606601194513969"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.09962989669326383"}],"id":"n0.2931944948632237"}],"id":"n0.6156082247263208"}},"id":"n0.31326272255816034"}],"id":"n0.8796898714453854"}],"id":"n0.9805767880860297"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3371603844651063"}],"id":"n0.30306266283677585"}],"shape":{"data":{"p":{"x":60.0172119140625,"y":37.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de9909381176935796":{"id":"de9909381176935796","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.7770745399973855"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.279482495896181","text":"j"}],"id":"n0.049294457730357566"}],"id":"n0.47502194828777755"}},"id":"n0.3104698583774652"},{"text":"|","id":"n0.8069761130046857"}],"id":"n0.8584969463576833"}],"id":"n0.2798165469167486"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6562813764434903"}],"style":{"align":"center"},"id":"n0.363983952699487"}],"shape":{"data":{"p":{"x":154.5172119140625,"y":85.09351124763486},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7940121895808216":{"id":"de7940121895808216","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|𝛺","id":"n0.8392268213222378"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.45931023392974546"}],"id":"n0.4386172708809295"}],"id":"n0.4584664630282278"}},"id":"n0.4763352696187795"},{"text":"|","id":"n0.14967209541319826"}],"id":"n0.35156619811075585"}],"id":"n0.0956182946294597"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9708121693643827"}],"style":{"align":"center"},"id":"n0.35881694925462093"}],"shape":{"data":{"p":{"x":192.02362060546875,"y":103.28239979743955},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3438066760605898":{"id":"de3438066760605898","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.6185751205939924"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7630019635107705"}],"id":"n0.18231221574247525"}],"id":"n0.6089119962955543"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.8931427045562066"}],"id":"n0.45448693554527053"}],"id":"n0.19216976991918355"}},"id":"n0.7171050426488565"}],"id":"n0.4046619303284873"}],"id":"n0.8192672737499627"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5089895969159941"}],"id":"n0.43765832669474447"}],"shape":{"data":{"p":{"x":77.0172119140625,"y":37.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de02563280881487806":{"id":"de02563280881487806","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.48393696995564994"}],"id":"n0.7670471443345628"}],"id":"n0.8865234094211434"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.11082735422175616"}],"style":{"align":"center"},"id":"n0.9320416525991655"}],"shape":{"data":{"p":{"x":51.0172119140625,"y":38.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2952691414875843":{"id":"de2952691414875843","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"}","id":"n0.6356927531194121"}],"id":"n0.36904407403017525"}],"id":"n0.9553225079236318"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8271860448504322"}],"style":{"align":"center"},"id":"n0.6542691589207725"}],"shape":{"data":{"p":{"x":115.0172119140625,"y":38.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2137567380595542":{"id":"de2137567380595542","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.008045371016361047"}],"id":"n0.056940874031297994"}],"id":"n0.4727756332635742"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.9381759798707874"}],"id":"n0.4639351367653197"}],"shape":{"data":{"p":{"x":83.0172119140625,"y":39.30042969200531}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4411703412746728":{"id":"de4411703412746728","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.5673059339913724"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.061383121218202774"}],"id":"n0.6367317616117458"}],"id":"n0.11324966217388632"},"powerValue":{"lines":[{"blocks":[{"text":"T","id":"n0.3556798658020468"}],"id":"n0.25916704271678803"}],"id":"n0.5837359185292408"}},"id":"n0.7818593738823849"}],"id":"n0.21276920260652177"}],"id":"n0.07663451775769459"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6650778724083672"}],"id":"n0.6330050359540009"}],"shape":{"data":{"p":{"x":107.0172119140625,"y":37.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de035400546782350384":{"id":"de035400546782350384","lines":[{"blocks":[{"text":"step size","style":{"fontSize":"\\tiny"},"id":"n0.9764453106149684"}],"style":{"align":"center"},"id":"n0.17208796365792245"}],"shape":{"data":{"p":{"x":80.2672119140625,"y":13.532399797439552},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de011428175050699707":{"id":"de011428175050699707","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.8415160191222524"}],"id":"n0.6764598294619883"}],"id":"n0.4915964638796144"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\huge"},"id":"n0.04242692615873578"}],"style":{"align":"center"},"id":"n0.7062294202886628"}],"shape":{"data":{"p":{"x":123.0172119140625,"y":31.282399797439552},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6537304728518818":{"id":"de6537304728518818","lines":[{"blocks":[{"text":"sIPOMDPLite-net belief update module","style":{"fontSize":"\\tiny"},"id":"n0.7546254988855303"}],"style":{"align":"center"},"id":"n0.8691198432839606"}],"shape":{"data":{"p":{"x":239.0172119140625,"y":72.387485023934},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7705556078782059":{"id":"de7705556078782059","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.008293039797159674"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5216747967197923"}],"id":"n0.35693243297690636"}],"id":"n0.41737925849133406"},"powerValue":{"lines":[{"blocks":[{"text":"0","id":"n0.6979465989849813"}],"id":"n0.14420185103029626"}],"id":"n0.40474595580324424"}},"id":"n0.3277983918828431"},{"type":"single","text":"(","id":"n0.8809554206446106"},{"text":"s","id":"n0.7858656026709734"},{"type":"single","text":")","id":"n0.6124441271549628"}],"id":"n0.6634858829152157"}],"id":"n0.05892219861296333"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.7774372556191349"}],"style":{"align":"center"},"id":"n0.2595929551888332"}],"shape":{"data":{"p":{"x":78.42474303483044,"y":147.65347228287732},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de17319207116005386":{"id":"de17319207116005386","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.780829103006283"}],"id":"n0.6355606499794044"}],"id":"n0.966917583179874"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9759693950963464"}],"style":{"align":"center"},"id":"n0.9848921236101413"}],"shape":{"data":{"p":{"x":58.0172119140625,"y":160.5483568152169},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5959307484371226":{"id":"de5959307484371226","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.6726140179660547"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.762679550225982"}],"id":"n0.8397633926464323"}],"id":"n0.7290894455779042"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.17320945559767842"}],"id":"n0.09662066496380262"}],"id":"n0.25944338759843943"}},"id":"n0.7583015172184857"},{"type":"single","text":"(","id":"n0.3786770174641547"},{"text":"s","id":"n0.7625989177777934"},{"type":"single","text":")","id":"n0.5639546157732511"}],"id":"n0.6922443966909593"}],"id":"n0.8095639861826163"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.3649388247074752"}],"style":{"align":"center"},"id":"n0.5687985959786279"}],"shape":{"data":{"p":{"x":423.42474303483044,"y":74.65347228287732},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de07073982375164545":{"id":"de07073982375164545","lines":[{"blocks":[{"text":"Sparse softmax cross entropy","style":{"fontSize":"\\tiny"},"id":"n0.27095514986534974"}],"style":{"align":"center"},"id":"n0.31120224083679693"}],"shape":{"data":{"p":{"x":352.3273048400878,"y":26.79249272346499},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6830611398030915":{"id":"de6830611398030915","lines":[{"blocks":[{"text":"RMSProp Optimizer","style":{"fontSize":"\\tiny"},"id":"n0.10517431055464077"}],"style":{"align":"center"},"id":"n0.297970068178369"}],"shape":{"data":{"p":{"x":469.3273048400878,"y":0.7924927234649886},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6104984434949119":{"id":"de6104984434949119","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.34613872236485066"}],"id":"n0.15018417810138507"}],"id":"n0.24973157094907705"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.5489273765608476"}],"id":"n0.07614620034088282"}],"shape":{"data":{"p":{"x":500.63994881799636,"y":36.42916718304414}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de8090494859670556":{"id":"de8090494859670556","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"}","id":"n0.16533359404242964"}],"id":"n0.6042093799923687"}],"id":"n0.7620537820832181"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5331785463618879"}],"style":{"align":"center"},"id":"n0.3358850621573517"}],"shape":{"data":{"p":{"x":536,"y":35.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de15916424799553974":{"id":"de15916424799553974","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.16381382403266276"}],"id":"n0.31153597860941096"}],"id":"n0.9087874361013744"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.014338093252062256"}],"style":{"align":"center"},"id":"n0.8352763945462958"}],"shape":{"data":{"p":{"x":482,"y":35.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5571887982091397":{"id":"de5571887982091397","lines":[{"blocks":[{"text":"step size","style":{"fontSize":"\\tiny"},"id":"n0.8485972952380658"}],"style":{"align":"center"},"id":"n0.14538206619684813"}],"shape":{"data":{"p":{"x":497.5649331774448,"y":47.94894342945699},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6104151282223247":{"id":"de6104151282223247","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.5426573890919397"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9965857282116861"}],"id":"n0.676222141387296"}],"id":"n0.21237977565877797"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.7246782685259634"}],"id":"n0.12791338011177222"}],"id":"n0.629879321844137"}},"id":"n0.23433173455375367"}],"id":"n0.07297285074437698"}],"id":"n0.678448619782392"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5031310617013929"}],"id":"n0.6304535325735754"}],"shape":{"data":{"p":{"x":529,"y":186.0137939453125}},"anchor":"left-top"},"isTextMode":true},"de7214680511204863":{"id":"de7214680511204863","lines":[{"blocks":[{"text":"Evaluation","style":{"fontSize":"\\tiny"},"id":"n0.3229327737426322"}],"style":{"align":"center"},"id":"n0.015974279420830406"}],"shape":{"data":{"p":{"x":381.39875726699825,"y":178.76184458732604},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7549900886099203":{"id":"de7549900886099203","lines":[{"blocks":[{"text":"Training","style":{"fontSize":"\\tiny"},"id":"n0.803890300664885"}],"style":{"align":"center"},"id":"n0.03181144687105686"}],"shape":{"data":{"p":{"x":404.0760807037352,"y":159.0441082000733},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5046710934384864":{"id":"de5046710934384864","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.24609779131871923"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.22706401339330085"}],"id":"n0.33524231977662367"}],"id":"n0.5487085448306963"}},"id":"n0.9534120892256168"},{"text":"|","id":"n0.7717020579670113"}],"id":"n0.19455039516198558"}],"id":"n0.44181901465933904"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.11344735225385527"}],"style":{"align":"center"},"id":"n0.19566480723516833"}],"shape":{"data":{"p":{"x":448.5,"y":177.8249053955078},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6139659569366251":{"id":"de6139659569366251","lines":[{"blocks":[{"text":"Recurrent belief update","style":{"fontSize":"\\tiny"},"id":"n0.9792646145620199"}],"style":{"align":"center"},"id":"n0.300225697394062"}],"shape":{"data":{"p":{"x":265.0172119140625,"y":38.35211515088713},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5190732616850979":{"id":"de5190732616850979","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"b","id":"n0.03595251541093991"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5555799269653077"}],"id":"n0.7826657345235788"}],"id":"n0.20729284139918103"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.18543534405426731"}],"id":"n0.4732846757636109"}],"id":"n0.6985821718961494"}},"id":"n0.3199206488286901"},{"type":"single","text":"(","id":"n0.12285033223688102"},{"text":"s","id":"n0.09153978246159955"},{"type":"single","text":")","id":"n0.8513960623698407"}],"id":"n0.4675833849066542"}],"id":"n0.2860407715183735"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\tiny"},"id":"n0.31907694747023063"}],"style":{"align":"center"},"id":"n0.6745466833125002"}],"shape":{"data":{"p":{"x":184.42474303483044,"y":144.65347228287732},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9578891903894824":{"id":"de9578891903894824","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.15860019140094073"}],"id":"n0.526338816874079"}],"id":"n0.14877766752441013"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.02063639735628442"}],"id":"n0.46798948411037133"}],"shape":{"data":{"p":{"x":132.0172119140625,"y":143.04796763870638}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6727368075661122":{"id":"de6727368075661122","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.27279228036029113"}],"id":"n0.7808913629699232"}],"id":"n0.3813400136477225"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6236698896964832"}],"style":{"align":"center"},"id":"n0.362718419602585"}],"shape":{"data":{"p":{"x":163.0172119140625,"y":153.5483568152169},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de12018452445458294":{"id":"de12018452445458294","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|","id":"n0.4304601760832991"}],"id":"n0.7197864701343688"}],"id":"n0.3232354544137075"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.46162195355427316"}],"style":{"align":"center"},"id":"n0.15662968742916283"}],"shape":{"data":{"p":{"x":402.0172119140625,"y":87.28239979743955},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9279013124591611":{"id":"de9279013124591611","lines":[{"blocks":[{"text":"Interaction indicators","style":{"fontSize":{"value":0.4}},"id":"n0.41359606004965843"}],"style":{"align":"center"},"id":"n0.9861904073319885"}],"shape":{"data":{"p":{"x":103.80276922615428,"y":270.28239979743955},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de03535318107247609":{"id":"de03535318107247609","lines":[{"blocks":[{"text":"value","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.1285566936690723"}],"style":{"align":"center"},"id":"n0.9484429575143738"}],"shape":{"data":{"p":{"x":250,"y":284.96759033203125},"rotation":0},"anchor":"left-top","style":{"fillColor":[245,166,35,1]}},"isTextMode":true,"isInGroup":true},"de6581424833173313":{"id":"de6581424833173313","lines":[{"blocks":[{"text":"indexing vector","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.014119603541997483"}],"style":{"align":"center"},"id":"n0.11737167060362119"}],"shape":{"data":{"p":{"x":430.00000000000006,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de6830316854968421":{"id":"de6830316854968421","lines":[{"blocks":[{"text":"sub-module","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.6161909700312669"}],"style":{"align":"center"},"id":"n0.5050592436335899"}],"shape":{"data":{"p":{"x":565,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[74,144,226,0.5]}},"isTextMode":true,"isInGroup":true},"de6916130444344799":{"id":"de6916130444344799","lines":[{"blocks":[{"text":"training algorithm","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.08509839011126474"}],"style":{"align":"center"},"id":"n0.8553495772556003"}],"shape":{"data":{"p":{"x":491,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[255,100,100,1]}},"isTextMode":true,"isInGroup":true},"de7846039342937636":{"id":"de7846039342937636","lines":[{"blocks":[{"text":"model","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.5182017439975346"}],"style":{"align":"center"},"id":"n0.8576427129423225"}],"shape":{"data":{"p":{"x":378,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[184,233,134,1]}},"isTextMode":true,"isInGroup":true},"de38901163369922753":{"id":"de38901163369922753","lines":[{"blocks":[{"text":"trainable variable","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.16199844627080617"}],"style":{"align":"center"},"id":"n0.7231446857744572"}],"shape":{"data":{"p":{"x":296.00000000000006,"y":284.9838562011719},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9474792898469997":{"id":"de9474792898469997","lines":[{"blocks":[{"text":"belief/probability","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.7950880955069464"}],"style":{"align":"center"},"id":"n0.051025330855066775"}],"shape":{"data":{"p":{"x":167.00000000000006,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[80,227,194,1]}},"isTextMode":true,"isInGroup":true},"de157530155636616":{"id":"de157530155636616","lines":[{"blocks":[{"text":"input/output","style":{"fontSize":"\\tiny","fontName":"ptm"},"id":"n0.2070151504513611"}],"style":{"align":"center"},"id":"n0.7316417110811024"}],"shape":{"data":{"p":{"x":110.00000000000006,"y":284.9838562011719},"rotation":0},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de5551324285345347":{"id":"de5551324285345347","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.10112709389658225"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.15719802354624712"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.230433667689528"}],"id":"n0.6000958793716686"}],"id":"n0.15896386458891132"}},"id":"n0.5010451678163392"}],"id":"n0.36143427726355126"}],"id":"n0.6079979627375813"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.9283315301145045"}],"id":"n0.8944995803110658"}],"id":"n0.057705097653189874"}},"id":"n0.967172965753176"}],"id":"n0.7129346546594733"}],"id":"n0.8842098281055866"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.15550535315998992"}],"id":"n0.8290424429158296"}],"shape":{"data":{"p":{"x":460,"y":167.5137939453125}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de11067232215210976":{"id":"de11067232215210976","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.6278015293063248"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.11467269437820349"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.30987021170003315"}],"id":"n0.8111485637648763"}],"id":"n0.605238568977055"}},"id":"n0.44655036459612485"}],"id":"n0.6280076279345186"}],"id":"n0.8328557278802435"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.8653763603017739"}],"id":"n0.1893791319877034"}],"id":"n0.6088615053213609"}},"id":"n0.06539787902914118"}],"id":"n0.8820827388445249"}],"id":"n0.6926625074118744"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.002378739463359425"}],"id":"n0.001579009779701046"}],"shape":{"data":{"p":{"x":494.9827880859375,"y":35.57558217048643},"rotation":0},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de7333755688576151":{"id":"de7333755688576151","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.628732028648648"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.9592767044354882"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.4218631289034491"}],"id":"n0.7601888966815635"}],"id":"n0.04550619551919688"}},"id":"n0.2917956954443315"}],"id":"n0.5997785509889499"}],"id":"n0.589789168719923"},"powerValue":{"lines":[{"blocks":[{"text":"T","id":"n0.9344458859699847"}],"id":"n0.35296799842200977"}],"id":"n0.6893288478455344"}},"id":"n0.20085229161538964"}],"id":"n0.6878304647006728"}],"id":"n0.19734605494092916"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9749987698326703"}],"id":"n0.12341831089898059"}],"shape":{"data":{"p":{"x":527.9827880859375,"y":35.78239979743955}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de766426490560322":{"id":"de766426490560322","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Depth: ","id":"n0.5943425507311662"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|𝛺","id":"n0.5567072858792346"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.22011040074090626"}],"id":"n0.9621017955017688"}],"id":"n0.2887825406954372"}},"id":"n0.5756253396206454"},{"text":"|","id":"n0.001745476231194365"}],"id":"n0.8879719304316316"}],"id":"n0.8377316246435462"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8200746325948032"}],"id":"n0.9479074159109457"}],"shape":{"data":{"p":{"x":113.0172119140625,"y":93.28239979743955},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8769763256636647":{"id":"de8769763256636647","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"One hot mapping","id":"n0.3575034704393769"}],"id":"n0.07564267257534452"}],"shape":{"data":{"p":{"x":120.0172119140625,"y":84.78239979743955},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9077288866210012":{"id":"de9077288866210012","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.3459030011878128"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"o","id":"n0.8691611673216317"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.7171822782864585"}],"id":"n0.36414181906030185"}],"id":"n0.8201563634585598"}},"id":"n0.9643486708720748"}],"id":"n0.09770634088915475"}],"id":"n0.052403244615391475"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.6797348567627706"}],"id":"n0.017755115192927606"}],"id":"n0.9814357810390177"}},"id":"n0.09398349921211446"}],"id":"n0.560660220226239"}],"id":"n0.11712223778126041"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.33479771380700796"}],"id":"n0.9732905260302813"}],"shape":{"data":{"p":{"x":203.0172119140625,"y":91.78239979743955}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de0427991193329158":{"id":"de0427991193329158","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.6464133006231938"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.14579720940771201","text":"j"}],"id":"n0.288130680137366"}],"id":"n0.03781615706224151"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.18815728479516247"}],"id":"n0.8259113629013399"}],"id":"n0.39119061776319053"}},"id":"n0.4867090870517434"}],"id":"n0.2652112962808757"}],"id":"n0.7646762117471588"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6089176068916575"}],"id":"n0.6015078732153858"}],"shape":{"data":{"p":{"x":60,"y":58.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de4185709066586074":{"id":"de4185709066586074","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.01688425792416437"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.18718254922497635"}],"id":"n0.14289521987802023"}],"id":"n0.2931294741383166"}},"id":"n0.7833519614394571"},{"text":"|","id":"n0.6768902994582451"}],"id":"n0.2421330624441942"}],"id":"n0.8656149269890585"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.6159887899805114"}],"style":{"align":"center"},"id":"n0.10572795347500286"}],"shape":{"data":{"p":{"x":154.5172119140625,"y":60.093511247634865},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de27900670992145105":{"id":"de27900670992145105","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.31966651560539705"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7017088864578898"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.6530735648959431"}],"id":"n0.14134950566231863"}],"id":"n0.3159090075051221"}},"id":"n0.30743404375942074"}],"id":"n0.23765680276781453"}],"id":"n0.00421906309059672"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.529727692702963"}],"id":"n0.5877611847771624"}],"id":"n0.28055451097523876"}},"id":"n0.7247943503531769"}],"id":"n0.3745027443049487"}],"id":"n0.8432401649435193"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9287469860935853"}],"id":"n0.7791566836714905"}],"shape":{"data":{"p":{"x":164.0172119140625,"y":48.78239979743955}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":true},"de8772525490309724":{"id":"de8772525490309724","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.5762133858478438"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.35169004439343365"},{"id":"n0.05925589579167889","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9534903422146683","lines":[{"id":"n0.38955445239343356","blocks":[{"id":"n0.45261265864650935","text":"j"}]}]}}}],"id":"n0.4781498140780698"}],"id":"n0.9221215572847408"},"powerValue":{"lines":[{"blocks":[{"text":"t-1","id":"n0.8968006244869051"}],"id":"n0.29773686256620446"}],"id":"n0.28245853278929767"}},"id":"n0.13292216965562553"}],"id":"n0.43454788566174973"}],"id":"n0.865317173645763"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.8002820603523662"}],"id":"n0.2343795510721598"}],"shape":{"data":{"p":{"x":164.0172119140625,"y":73.78239979743955}},"anchor":"left-top","style":{"fillColor":[180,180,180,1]}},"isTextMode":true,"isInGroup":false},"de3319413261208979":{"id":"de3319413261208979","lines":[{"blocks":[{"text":"Training","style":{"fontSize":"\\tiny"},"id":"n0.402568375570203"}],"style":{"align":"center"},"id":"n0.7404299373178662"}],"shape":{"data":{"p":{"x":380.0588687896727,"y":196.0441082000733},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3684156015585027":{"id":"de3684156015585027","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.46054203308809494"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.08317265649526884"}],"id":"n0.5136127675548985"}],"id":"n0.39013289935446305"}},"id":"n0.3484831224478835"},{"text":"|","id":"n0.34630089461119784"}],"id":"n0.6856134748473006"}],"id":"n0.6037157092616128"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.3351997587724176"}],"style":{"align":"center"},"id":"n0.20760977007595005"}],"shape":{"data":{"p":{"x":409.4827880859375,"y":214.8249053955078},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5137422723619176":{"id":"de5137422723619176","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.9519679578948306"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.37842720917881234"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.14778329563842507","text":"j"}],"id":"n0.7452891669254227"}],"id":"n0.3652473407083463"}},"id":"n0.10937835340226632"}],"id":"n0.24057415195939091"}],"id":"n0.6737937491681296"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.03573371875191578"}],"id":"n0.028060102656048302"}],"id":"n0.42105302242493625"}},"id":"n0.12730810685656668"}],"id":"n0.9405832457870693"}],"id":"n0.6370642722097213"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.904836261877364"}],"id":"n0.1041501006626171"}],"shape":{"data":{"p":{"x":420.9827880859375,"y":204.5137939453125}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de1747952617436006":{"id":"de1747952617436006","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.03826382342507961"}],"id":"n0.0776788625298026"}],"id":"n0.2299585495929235"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.6855413346855017"}],"id":"n0.8056632706985383"}],"shape":{"data":{"p":{"x":560.6399488179964,"y":24.429167183044143}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de23076532693712015":{"id":"de23076532693712015","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"}","id":"n0.21852843029975233"}],"id":"n0.4472116882434696"}],"id":"n0.7046338254291307"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.35303218499510725"}],"style":{"align":"center"},"id":"n0.711907666288109"}],"shape":{"data":{"p":{"x":596,"y":23.369590963121993},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de3021532720703066":{"id":"de3021532720703066","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.9425366060270881"}],"id":"n0.49535503691405913"}],"id":"n0.7689628952048579"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6794254891499345"}],"style":{"align":"center"},"id":"n0.3203984774618396"}],"shape":{"data":{"p":{"x":542,"y":23.369590963121993},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5428744539157133":{"id":"de5428744539157133","lines":[{"blocks":[{"text":"step size","style":{"fontSize":"\\tiny"},"id":"n0.8164605120701358"}],"style":{"align":"center"},"id":"n0.9911689156348542"}],"shape":{"data":{"p":{"x":557.5649331774448,"y":35.94894342945699},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de130364287178661":{"id":"de130364287178661","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.14205109947688643"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.24760638775722588"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.5366232895398386","text":"j"}],"id":"n0.573209120508704"}],"id":"n0.2540251173041572"}},"id":"n0.21577099400758604"}],"id":"n0.49356680643817796"}],"id":"n0.37710113689268754"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.9814172621566803"}],"id":"n0.02602213798203934"}],"id":"n0.7250091879301446"}},"id":"n0.8271830445251864"}],"id":"n0.7399053922658398"}],"id":"n0.5800614332963825"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.08352580501640494"}],"id":"n0.29497144120326313"}],"shape":{"data":{"p":{"x":554.9827880859375,"y":23.575582170486427},"rotation":0},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de13864094431472274":{"id":"de13864094431472274","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"v","id":"n0.2209383974902177"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.23721481739277217"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.825655967369261","text":"j"}],"id":"n0.15501530759379012"}],"id":"n0.025376741285212612"}},"id":"n0.6662269310487501"}],"id":"n0.5077589861101615"}],"id":"n0.07061986568419831"},"powerValue":{"lines":[{"blocks":[{"text":"T","id":"n0.777430048423563"}],"id":"n0.5462382795226342"}],"id":"n0.6925090740158706"}},"id":"n0.49438988759218017"}],"id":"n0.7748604418054355"}],"id":"n0.5054730445479463"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.044365918439071894"}],"id":"n0.7878884391656515"}],"shape":{"data":{"p":{"x":587.9827880859375,"y":23.782399797439552}},"anchor":"left-top","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de8858027549359482":{"id":"de8858027549359482","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.7771409182943738"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.08850067954682905","text":"j"}],"id":"n0.4151627584541755"}],"id":"n0.571046075525246"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.8278723054805401"}],"id":"n0.924538771173768"}],"id":"n0.8240977136423435"}},"id":"n0.1878142525060167"}],"id":"n0.7205301889098097"}],"id":"n0.3935563474086412"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.874871017068152"}],"id":"n0.18953854390260982"}],"shape":{"data":{"p":{"x":77.0172119140625,"y":58.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de01737361400489701":{"id":"de01737361400489701","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.5028186364995297"}],"id":"n0.639855730025886"}],"id":"n0.9680449396846869"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9793774702776521"}],"style":{"align":"center"},"id":"n0.6803018614918244"}],"shape":{"data":{"p":{"x":51.0172119140625,"y":59.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2338077860981691":{"id":"de2338077860981691","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"}","id":"n0.30890644878022244"}],"id":"n0.5961478322886438"}],"id":"n0.4581428332056161"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.2728615589727075"}],"style":{"align":"center"},"id":"n0.5587154326885382"}],"shape":{"data":{"p":{"x":115.0172119140625,"y":59.36959096312199},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7448435430529068":{"id":"de7448435430529068","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.24419843608862757"}],"id":"n0.6186090930591632"}],"id":"n0.27072142324195303"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.5416380547548176"}],"id":"n0.49359294107359974"}],"shape":{"data":{"p":{"x":83.0172119140625,"y":60.30042969200531}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9645011963385512":{"id":"de9645011963385512","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"a","id":"n0.5491078512601584"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.2671504875624111","text":"j"}],"id":"n0.32536765922598"}],"id":"n0.920316694189353"},"powerValue":{"lines":[{"blocks":[{"text":"T","id":"n0.3958005480412661"}],"id":"n0.45718673014618805"}],"id":"n0.8929803939717895"}},"id":"n0.9621800921619503"}],"id":"n0.37647153187475135"}],"id":"n0.39136111084628955"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.4692029339746646"}],"id":"n0.5362876157300336"}],"shape":{"data":{"p":{"x":107.0172119140625,"y":58.28239979743955}},"anchor":"left-top"},"isTextMode":true},"de756467946908294":{"id":"de756467946908294","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜏","id":"n0.09040024633854027"},{"id":"n0.9414271134932601","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.8539008977666882","lines":[{"id":"n0.4518242293028474","blocks":[{"id":"n0.3965299041617616","text":"a"},{"id":"n0.5950237375304415","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2004556375558837","lines":[{"id":"n0.9786636017007695","blocks":[{"id":"n0.2720602468752946","text":"i"}]}]}}}]}]}}}],"id":"n0.9903605090117544"}],"id":"n0.7968369877522394"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.640509913467499"}],"style":{"align":"center"},"id":"n0.4390753621173462"}],"shape":{"data":{"p":{"x":41.0172119140625,"y":36.54835681521689},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de49310965300164167":{"id":"de49310965300164167","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜏","id":"n0.5029595600631078"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"a","id":"n0.49474462952339593"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.10050877597725605","text":"j"}],"id":"n0.7137077923863049"}],"id":"n0.03814875876868795"}},"id":"n0.6702518299974569"}],"id":"n0.14156621606474862"}],"id":"n0.19597520547224634"}},"id":"n0.28104078261921317"}],"id":"n0.6777525444975907"}],"id":"n0.43200332154226206"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.38503797423491215"}],"style":{"align":"center"},"id":"n0.5344267510048109"}],"shape":{"data":{"p":{"x":41.0172119140625,"y":57.54835681521689},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de7539779953399748":{"id":"de7539779953399748","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"{","id":"n0.12071300230555493"}],"id":"n0.6389586816019504"}],"id":"n0.09302421410022554"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.17799468051078948"}],"style":{"align":"center"},"id":"n0.020294695836960752"}],"shape":{"data":{"p":{"x":15.0172119140625,"y":81.369590963122},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5911363371170728":{"id":"de5911363371170728","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"type":"single","text":"}","id":"n0.7564784181513657"}],"id":"n0.9518648643126093"}],"id":"n0.13123680074453592"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.30217654976660224"}],"style":{"align":"center"},"id":"n0.7625369652930956"}],"shape":{"data":{"p":{"x":79.0172119140625,"y":81.369590963122},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de2874148039921536":{"id":"de2874148039921536","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"⋯","id":"n0.20746859696009823"}],"id":"n0.9625692368785876"}],"id":"n0.21744012313887917"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\small"},"id":"n0.719910678243934"}],"id":"n0.3953473469356017"}],"shape":{"data":{"p":{"x":47.0172119140625,"y":82.30042969200531}},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de09506015339513452":{"id":"de09506015339513452","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"𝜏","id":"n0.8056760836355961"},{"id":"n0.19700486811713191","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.1118667355180678","lines":[{"id":"n0.10776605706493791","blocks":[{"id":"n0.007754824021389384","text":"o"},{"id":"n0.7267764500012224","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.022645884654262094","lines":[{"id":"n0.07291715931053155","blocks":[{"id":"n0.3681933782261868","text":"i"}]}]}}}]}]}}}],"id":"n0.574213430457988"}],"id":"n0.7879157549084901"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5808192267936789"}],"style":{"align":"center"},"id":"n0.7728223320223773"}],"shape":{"data":{"p":{"x":5.0172119140625,"y":79.54835681521689},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de02747343053030571":{"id":"de02747343053030571","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"o","id":"n0.44625754460905753"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.8893678335268238"}],"id":"n0.6884801257066628"}],"id":"n0.7120420318740519"},"powerValue":{"lines":[{"blocks":[{"text":"t","id":"n0.9570091548721635"}],"id":"n0.24447494473767573"}],"id":"n0.37374589938555314"}},"id":"n0.9463720171867886"}],"id":"n0.6003475309273705"}],"id":"n0.9901597008831791"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.10003632182033839"}],"id":"n0.7822660415586566"}],"shape":{"data":{"p":{"x":26.5172119140625,"y":79.78239979743955}},"anchor":"left-top"},"isTextMode":true},"de34785104329949257":{"id":"de34785104329949257","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"o","id":"n0.11075842681461645"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.1605187139634474"}],"id":"n0.8013424382554843"}],"id":"n0.20474298201342234"},"powerValue":{"lines":[{"blocks":[{"text":"t+1","id":"n0.8826139000039472"}],"id":"n0.2829897872364435"}],"id":"n0.18076721689238662"}},"id":"n0.504632079602521"}],"id":"n0.3470720973214332"}],"id":"n0.9801920815872638"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.08243843502458148"}],"id":"n0.2792151759161037"}],"shape":{"data":{"p":{"x":38.5172119140625,"y":79.78239979743955}},"anchor":"left-top"},"isTextMode":true},"de7172149586802281":{"id":"de7172149586802281","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"o","id":"n0.8047526366647146"},{"text":"\\power-index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.9174964467470521"}],"id":"n0.41886824368367015"}],"id":"n0.4847380786298725"},"powerValue":{"lines":[{"blocks":[{"id":"n0.23309421944975073","text":"T+1"}],"id":"n0.9393771506272504"}],"id":"n0.8359339654331044"}},"id":"n0.3938671942741456"}],"id":"n0.9544275247121161"}],"id":"n0.7593809752282012"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5184485551626943"}],"id":"n0.06640259461733056"}],"shape":{"data":{"p":{"x":68.5172119140625,"y":79.78239979743955}},"anchor":"left-top"},"isTextMode":true},"de8555181190209911":{"id":"de8555181190209911","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"X","id":"n0.12155272212617074"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.49906942447057334"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.8214858544308155"}],"id":"n0.5043969874613548"}],"id":"n0.11478171217302191"},"indexValue":{"lines":[{"blocks":[{"text":"T","id":"n0.37179947470330266"}],"id":"n0.5457666319441228"}],"id":"n0.6519377455991147"}},"id":"n0.008212787674330091"}],"id":"n0.3157526464422953"}],"id":"n0.4254440358615659"}},"id":"n0.32299234035675894"},{"type":"single","text":"(","id":"n0.811637462333094"},{"text":"s,a","id":"n0.9580426701193052"},{"type":"single","text":")","id":"n0.8869435608132157"}],"id":"n0.15940430690943685"}],"id":"n0.3132924567681319"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5994810916217608"}],"style":{"align":"center"},"id":"n0.3803486414737671"}],"shape":{"data":{"p":{"x":98.40112242936175,"y":216.66248913204873},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6117269236688183":{"id":"de6117269236688183","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"X","id":"n0.5568546759848911"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"P","id":"n0.539093983180535"},{"text":"\\power-index","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"text":"I","id":"n0.5504994157337477"}],"id":"n0.6602808463544139"}],"id":"n0.386195782177984"},"indexValue":{"lines":[{"blocks":[{"id":"n0.9047892248610752","text":"R"}],"id":"n0.5516441822744349"}],"id":"n0.9424196624443812"}},"id":"n0.9900286822571793"}],"id":"n0.7841050325873038"}],"id":"n0.8155590170099274"}},"id":"n0.2971341695350542"},{"type":"single","text":"(","id":"n0.6350491494159667"},{"text":"s,a","id":"n0.42438966136036904"},{"type":"single","text":")","id":"n0.9925009236370999"}],"id":"n0.3226085603936859"}],"id":"n0.7590487519403368"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.9494209754238183"}],"style":{"align":"center"},"id":"n0.19546139395537332"}],"shape":{"data":{"p":{"x":150.58166565657575,"y":218.18984940756428},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de311792193101031":{"id":"de311792193101031","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.6057829974237232"}],"id":"n0.7516130028137709"}],"id":"n0.6909822130568688"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.18647341392534633"}],"style":{"align":"center"},"id":"n0.11009329718912242"}],"shape":{"data":{"p":{"x":60.5752569651695,"y":257.96795654296875},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de6715154092032498":{"id":"de6715154092032498","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|S|×|A|","id":"n0.002121963406264138"}],"id":"n0.12942752166974025"}],"id":"n0.608719912583584"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.5822546705489986"}],"style":{"align":"center"},"id":"n0.7119450236672624"}],"shape":{"data":{"p":{"x":180.31076744317738,"y":258.2583716044299},"rotation":359.98},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de4793583580341598":{"id":"de4793583580341598","lines":[{"blocks":[{"text":"Nested MDP module","style":{"fontSize":"\\tiny"},"id":"n0.8448358206245414"}],"style":{"align":"center"},"id":"n0.5997765310201999"}],"shape":{"data":{"p":{"x":288.1061553955079,"y":204.60139017105115},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de5251325581597752":{"id":"de5251325581597752","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"One hot mapping","id":"n0.1311128344440089"}],"id":"n0.9208219994297089"}],"shape":{"data":{"p":{"x":158.0172119140625,"y":48.78239979743955},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de047770060574601425":{"id":"de047770060574601425","lines":[{"blocks":[{"style":{"fontSize":{"value":0.4}},"text":"Depth: ","id":"n0.8608065394806057"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"|A","id":"n0.1517757797109054"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"i","id":"n0.5305308657982704"}],"id":"n0.8293462318848102"}],"id":"n0.46725334418639997"}},"id":"n0.14390605202063256"},{"text":"|","id":"n0.4459980056293207"}],"id":"n0.9142747805274785"}],"id":"n0.6638238662000462"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}},"id":"n0.053809341239267505"},{"id":"n0.06962374744131217","text":",","style":{"fontSize":{"value":0.4}}},{"id":"n0.23137954604272326","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.27431182150181543","lines":[{"id":"n0.9452261389098291","blocks":[{"id":"n0.6323810685373348","text":"|A"},{"id":"n0.7581772681461316","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6622233094117673","lines":[{"id":"n0.019564322462538808","blocks":[{"id":"n0.2997409476047901","text":"j"}]}]}}},{"text":"|","id":"n0.2897989632134057"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":{"value":0.4}}}],"id":"n0.0012820744010371143"}],"shape":{"data":{"p":{"x":151.0172119140625,"y":51.28239979743955},"rotation":90},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di3840833210691088","items":[],"style":{}},"shapes":[{"id":"dp47291887025148904","type":"rectangle","data":{"p1":{"x":32.21372256017689,"y":176.57503948597804},"p2":{"x":61.536182406122975,"y":205.89749933192408}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp33270367186104255","type":"rectangle","data":{"p1":{"x":178.53618240612298,"y":177.57503948597804},"p2":{"x":207.85864225206907,"y":206.89749933192408}},"style":{"fillColor":[248,231,28,1],"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]}}},{"id":"dp3686329362905836","type":"doc-rounded-rect","data":{"p1":{"x":273.39875726699836,"y":204.36876454353347},"p2":{"x":379.02362060546886,"y":230.0662476062774}},"style":{"fillColor":[140,200,240,1]}},{"id":"dp5007381791832946","type":"doc-rounded-rect","data":{"p1":{"x":274.39875726699825,"y":168.188744354248},"p2":{"x":377.026611328125,"y":193.88622741699214}},"style":{"fillColor":[140,200,240,1]}},{"id":"da6392114586352498","data":[{"x":61.0093994140625,"y":192.28239979743955},{"x":177.026611328125,"y":192.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp5349757603446712","type":"square","data":{"p1":{"x":62.0172119140625,"y":45.28239979743955},"p2":{"x":74.5172119140625,"y":57.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp7720825853344573","type":"rectangle","data":{"p1":{"x":133.0172119140625,"y":50.78239979743955},"p2":{"x":149.02362060546875,"y":99.78239979743955}}},{"id":"da030927197472309542","data":[{"x":33.0093994140625,"y":105.28239979743955},{"x":95.0093994140625,"y":105.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da953350202160437","data":[{"x":69.0093994140625,"y":83.28239979743955},{"x":132.0093994140625,"y":83.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da11428665306721131","data":[{"x":149.02362060546875,"y":86.28239979743955},{"x":162.02362060546875,"y":86.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg8117454392492514","entities":[{"id":"dp6894444328881189","type":"rectangle","data":{"p1":{"x":163.0172119140625,"y":78.7643699028738},"p2":{"x":175.67437264612136,"y":91.42153063493265}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp7867069659758521","type":"rectangle","data":{"p1":{"x":164.59935700556986,"y":80.34651499438115},"p2":{"x":177.2565177376287,"y":93.00367572644001}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp8906719224066897","type":"rectangle","data":{"p1":{"x":166.1815020970772,"y":81.92866008588851},"p2":{"x":178.83866282913607,"y":94.58582081794736}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dg025260480365929094","entities":[{"id":"dg6091432848288012","entities":[{"id":"dp898136671828403","type":"rectangle","data":{"p1":{"x":200.0172119140625,"y":96.7643699028738},"p2":{"x":212.67437264612136,"y":109.42153063493265}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp6715600294846531","type":"rectangle","data":{"p1":{"x":201.59935700556986,"y":98.34651499438115},"p2":{"x":214.2565177376287,"y":111.00367572644001}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp99606808320349","type":"rectangle","data":{"p1":{"x":203.1815020970772,"y":99.92866008588851},"p2":{"x":215.83866282913607,"y":112.58582081794736}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl11878088651665242","linkedId":"de9077288866210012"}]},{"id":"da49805112140537133","data":[{"x":111.0093994140625,"y":105.28239979743955},{"x":199.0172119140625,"y":105.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp8861163273406749","type":"square","data":{"p1":{"x":77.0172119140625,"y":45.28239979743955},"p2":{"x":89.5172119140625,"y":57.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp42447876275798024","type":"square","data":{"p1":{"x":107.0172119140625,"y":45.28239979743955},"p2":{"x":119.5172119140625,"y":57.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"da5907703484136553","data":[{"x":97.9664306640625,"y":34.3687645435333},{"x":352.026611328125,"y":34.3687645435333}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da12041695999585555","data":[{"x":97.9664306640625,"y":34.3687645435333},{"x":97.9664306640625,"y":38.4984032154083}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg8979656007400847","entities":[{"id":"dp8714920450744359","type":"rectangle","data":{"p1":{"x":95.0172119140625,"y":86.78239979743955},"p2":{"x":111.02362060546875,"y":135.78239979743955}}},{"id":"dl3810803124023281","linkedId":"de8769763256636647"},{"id":"dl8502562526816417","linkedId":"de766426490560322"}]},{"id":"dp2743939152477397","type":"doc-rounded-rect","data":{"p1":{"x":228.3987572669983,"y":72.3687645435333},"p2":{"x":387.346923828125,"y":98.06624760627744}},"style":{"fillColor":[140,200,240,1]}},{"id":"dp13836120411734676","type":"doc-cube","data":{"p1":{"x":66.0172119140625,"y":138.24594116210938},"p2":{"x":104.10756690024687,"y":175.95588793598483},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da9034582338657684","data":[{"x":179.02362060546875,"y":86.28239979743955},{"x":228.0093994140625,"y":86.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da3568795922343908","data":[{"x":208.026611328125,"y":92.58582081794736},{"x":228.026611328125,"y":92.58582081794736}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp5854503391049615","type":"doc-cube","data":{"p1":{"x":411.0172119140625,"y":65.24594116210938},"p2":{"x":449.10756690024687,"y":102.95588793598483},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da15955639931239407","data":[{"x":388.0172119140625,"y":85.28239979743955},{"x":411.0093994140625,"y":85.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da0683073607586604","data":[{"x":245.026611328125,"y":155.3687645435333},{"x":245.026611328125,"y":98.53384399414062}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da8342047457852937","data":[{"x":250.026611328125,"y":59.3687645435333},{"x":430.026611328125,"y":59.3687645435333}],"head":"no","tail":"no","shaft":{"type":"dash","pattern":[5,4,10,2]},"headScale":0.6},{"id":"da1240180229856167","data":[{"x":250.026611328125,"y":59.3687645435333},{"x":250.026611328125,"y":71.40420532226562}],"head":"fh>","tail":"no","shaft":{"type":"dash","pattern":[5,4,10,2]},"headScale":0.6},{"id":"da35220081363584743","data":[{"x":430.026611328125,"y":65.61519384384155},{"x":430.026611328125,"y":59.3687645435333}],"head":"no","tail":"no","shaft":"--","headScale":0.6},{"id":"da3297076579890863","data":[{"x":430.026611328125,"y":102.61519384384155},{"x":430.026611328125,"y":141.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da3354121762434161","data":[{"x":486.026611328125,"y":48.3687645435333},{"x":458.026611328125,"y":48.3687645435333}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp9444187807371747","type":"doc-rounded-rect","data":{"p1":{"x":352.3987572669983,"y":27.368764543533302},"p2":{"x":458.02362060546875,"y":53.06624760627744}},"style":{"fillColor":[255,100,100,1]}},{"id":"dp14401954448631438","type":"doc-rounded-rect","data":{"p1":{"x":466.026611328125,"y":1.5379272937775},"p2":{"x":545.026611328125,"y":26.368764543533302}},"style":{"fillColor":[255,100,100,1]}},{"id":"dg5964008931601581","entities":[{"id":"dg13729603557708514","entities":[{"id":"dp8608226067570728","type":"rectangle","data":{"p1":{"x":524.9827880859375,"y":40.764369902873796},"p2":{"x":537.6399488179964,"y":53.42153063493265}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp33308955013887354","type":"rectangle","data":{"p1":{"x":526.5649331774448,"y":42.34651499438115},"p2":{"x":539.2220939095037,"y":55.00367572644001}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp08325441009202605","type":"rectangle","data":{"p1":{"x":528.1470782689522,"y":43.92866008588851},"p2":{"x":540.8042390010111,"y":56.585820817947365}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl04227117205865438","linkedId":"de7333755688576151"}]},{"id":"dg07971275407612999","entities":[{"id":"dg10005593632932497","entities":[{"id":"dp2595396412152444","type":"rectangle","data":{"p1":{"x":491.9827880859375,"y":40.42916718304414},"p2":{"x":504.63994881799636,"y":53.335634957633346}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp7503940593260996","type":"rectangle","data":{"p1":{"x":493.5649331774448,"y":42.042475654867786},"p2":{"x":506.22209390950366,"y":54.94894342945699}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp4255756058740263","type":"rectangle","data":{"p1":{"x":495.1470782689522,"y":43.65578412669143},"p2":{"x":507.80423900101107,"y":56.562251901280646}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{"rotation":0}},{"id":"dl6550347857907792","linkedId":"de11067232215210976"}]},{"id":"dp7344263155280306","type":"square","data":{"p1":{"x":529,"y":194.0137939453125},"p2":{"x":541.5,"y":206.5137939453125}},"style":{"fillColor":[248,231,28,1]}},{"id":"da6087127329803084","data":[{"x":473.026611328125,"y":180.76184458732604},{"x":514.9260864257812,"y":180.76184458732604}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg28665975456564574","entities":[{"id":"dg1220839973179737","entities":[{"id":"dp02859167077177971","type":"rectangle","data":{"p1":{"x":457,"y":172.49576405074674},"p2":{"x":469.65716073205886,"y":185.1529247828056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp7557740031830245","type":"rectangle","data":{"p1":{"x":458.5821450915073,"y":174.0779091422541},"p2":{"x":471.23930582356616,"y":186.73506987431296}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp05921587767632008","type":"rectangle","data":{"p1":{"x":460.1642901830147,"y":175.66005423376146},"p2":{"x":472.82145091507357,"y":188.3172149658203}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl7884950672888991","linkedId":"de5551324285345347"}]},{"id":"da4360362968208855","data":[{"x":514.9260864257812,"y":180.76184458732604},{"x":514.9260864257812,"y":66.08636474609375}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da1365254495516297","data":[{"x":406.026611328125,"y":27.615193843841553},{"x":406.026611328125,"y":14.316253662109375}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7266274650303373","data":[{"x":406.026611328125,"y":14.316253662109375},{"x":465.026611328125,"y":14.316253662109375}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da7146537518216651","data":[{"x":47.026611328125,"y":155.3687645435333},{"x":65.026611328125,"y":155.3687645435333}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da3822054179326899","data":[{"x":47.026611328125,"y":176.08636474609375},{"x":47.026611328125,"y":155.3687645435333}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dg31479627254461207","entities":[{"id":"dg04182556084429523","entities":[{"id":"dp8222555557078086","type":"rectangle","data":{"p1":{"x":126.2857093811034,"y":267.5552864074705},"p2":{"x":135.42856979370129,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[248,231,28,1]}},{"id":"dl8712823427166769","linkedId":"de157530155636616"}]},{"id":"dg039684418290218515","entities":[{"id":"dp8400337706125396","type":"rectangle","data":{"p1":{"x":191.2857093811034,"y":267.5552864074705},"p2":{"x":200.42856979370129,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[80,227,194,1]}},{"id":"dl9055472886924096","linkedId":"de9474792898469997"}]},{"id":"dg9466631126217466","entities":[{"id":"dp052026641018338315","type":"rectangle","data":{"p1":{"x":321.2857093811034,"y":267.5552864074705},"p2":{"x":330.4285697937013,"y":330.5552864074705},"rotation":270}},{"id":"dl1370376181394557","linkedId":"de38901163369922753"}]},{"id":"dg00781979238143271","entities":[{"id":"dp779255616671013","type":"rectangle","data":{"p1":{"x":386.2857093811034,"y":267.5552864074705},"p2":{"x":395.4285697937013,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[184,233,134,1]}},{"id":"dl7466420505056555","linkedId":"de7846039342937636"}]},{"id":"dg6978924027490241","entities":[{"id":"dp2553832889138268","type":"rectangle","data":{"p1":{"x":516.2857093811034,"y":267.5552864074705},"p2":{"x":525.4285697937013,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[255,100,100,1]}},{"id":"dl5551832308589866","linkedId":"de6916130444344799"}]},{"id":"dg27173311021871127","entities":[{"id":"dp5838520968227427","type":"rectangle","data":{"p1":{"x":581.2857093811034,"y":267.5552864074705},"p2":{"x":590.4285697937013,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[74,144,226,0.5]}},{"id":"dl5405692283635466","linkedId":"de6830316854968421"}]},{"id":"dg818223334097526","entities":[{"id":"dp09610739516205102","type":"rectangle","data":{"p1":{"x":451.2857093811034,"y":267.5552864074705},"p2":{"x":460.4285697937013,"y":330.5552864074705},"rotation":270},"style":{"fillColor":[180,180,180,1]}},{"id":"dl677683996301746","linkedId":"de6581424833173313"}]},{"id":"dg8743036343367914","entities":[{"id":"dp8550898217750769","type":"rectangle","data":{"p1":{"x":256.2857093811034,"y":267.53902053832985},"p2":{"x":265.4285697937013,"y":330.53902053832985},"rotation":270},"style":{"fillColor":[245,166,35,1]}},{"id":"dl5117518334725439","linkedId":"de03535318107247609"}]}]},{"id":"dp36530934611293553","type":"doc-cube","data":{"p1":{"x":175.0172119140625,"y":135.24594116210938},"p2":{"x":213.10756690024687,"y":172.95588793598483},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[80,227,194,1]}},{"id":"da9137409352026389","data":[{"x":159.0093994140625,"y":155.3687645435333},{"x":175.026611328125,"y":155.3687645435333}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp3354267807849822","type":"square","data":{"p1":{"x":62,"y":66.28239979743955},"p2":{"x":74.5,"y":78.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"da5895173336123907","data":[{"x":47.026611328125,"y":206.61519384384155},{"x":47.026611328125,"y":244.89722917234633}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da4759367535608223","data":[{"x":104.026611328125,"y":155.3687645435333},{"x":136.0093994140625,"y":155.3687645435333}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da23401725323007638","data":[{"x":69.0172119140625,"y":57.78239979743955},{"x":69.0093994140625,"y":62.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da4417642064933385","data":[{"x":69.0093994140625,"y":62.21600341796875},{"x":132.0093994140625,"y":62.21600341796875}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da16723585432262245","data":[{"x":149.02362060546875,"y":62.28239979743955},{"x":162.02362060546875,"y":62.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg6204603852043595","entities":[{"id":"dg34507822073433725","entities":[{"id":"dp6767493988125446","type":"rectangle","data":{"p1":{"x":163.0172119140625,"y":54.764369902873796},"p2":{"x":175.67437264612136,"y":67.42153063493265}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp8378712102252863","type":"rectangle","data":{"p1":{"x":164.59935700556986,"y":56.34651499438115},"p2":{"x":177.2565177376287,"y":69.00367572644001}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}},{"id":"dp9340856766244212","type":"rectangle","data":{"p1":{"x":166.1815020970772,"y":57.92866008588851},"p2":{"x":178.83866282913607,"y":70.58582081794736}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[180,180,180,1]}}],"data":{}},{"id":"dl5674564919174834","linkedId":"de27900670992145105"}]},{"id":"da8657778222710852","data":[{"x":206.0093994140625,"y":79.50826115608213},{"x":228.3987572669983,"y":79.50826115608213}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9090319524213821","data":[{"x":179.02362060546875,"y":62.28239979743955},{"x":206.0093994140625,"y":62.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7933468941224051","data":[{"x":206.0093994140625,"y":79.50826115608213},{"x":206.0093994140625,"y":62.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da2634070014092007","data":[{"x":172.0172119140625,"y":70.78239979743955},{"x":172.0093994140625,"y":75.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da5045693654670567","data":[{"x":172.0172119140625,"y":94.78239979743955},{"x":172.0093994140625,"y":102.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7005836873374018","data":[{"x":172.0093994140625,"y":75.21600341796875},{"x":189.0093994140625,"y":75.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9975072723287093","data":[{"x":172.0093994140625,"y":102.21600341796875},{"x":189.0093994140625,"y":102.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9717334391214678","data":[{"x":189.0093994140625,"y":131.21600341796875},{"x":189.0093994140625,"y":75.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da23462799332701567","data":[{"x":189.0093994140625,"y":131.21600341796875},{"x":305.0093994140625,"y":131.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da05639754580279521","data":[{"x":233.0093994140625,"y":178.28239979743955},{"x":273.92608642578125,"y":178.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da41048600073210206","data":[{"x":194.0093994140625,"y":221.32824096679684},{"x":273.39875726699836,"y":221.32824096679684}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da4130143203023442","data":[{"x":327.39875726699825,"y":141.28239979743955},{"x":430.026611328125,"y":141.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da027523619528937227","data":[{"x":379.1072021484375,"y":217.35307836532593},{"x":416.9921875,"y":217.35307836532593}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg9275159137300206","entities":[{"id":"dg03931437452152142","entities":[{"id":"dp2612886007456432","type":"rectangle","data":{"p1":{"x":417.9827880859375,"y":209.49576405074674},"p2":{"x":430.63994881799636,"y":222.1529247828056}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp703123805601543","type":"rectangle","data":{"p1":{"x":419.5649331774448,"y":211.0779091422541},"p2":{"x":432.22209390950366,"y":223.73506987431296}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp7783348813475786","type":"rectangle","data":{"p1":{"x":421.1470782689522,"y":212.66005423376146},"p2":{"x":433.80423900101107,"y":225.3172149658203}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl9045323818869151","linkedId":"de5137422723619176"}]},{"id":"da76520212951226","data":[{"x":327.39875726699825,"y":168.32824096679684},{"x":327.39875726699825,"y":141.28239979743955}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da8231706178092588","data":[{"x":327.39875726699825,"y":193.32824096679684},{"x":327.39875726699825,"y":199.76184458732604}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8843110333077893","data":[{"x":327.39875726699825,"y":199.76184458732604},{"x":529.026611328125,"y":199.76184458732604}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da5408394447346849","data":[{"x":377.39875726699825,"y":180.76184458732604},{"x":457.026611328125,"y":180.76184458732604}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dg010187030176750156","entities":[{"id":"dg7740502244820402","entities":[{"id":"dp30502397317802865","type":"rectangle","data":{"p1":{"x":584.9827880859375,"y":28.764369902873796},"p2":{"x":597.6399488179964,"y":41.42153063493265}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp6929910450011407","type":"rectangle","data":{"p1":{"x":586.5649331774448,"y":30.346514994381153},"p2":{"x":599.2220939095037,"y":43.00367572644001}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp14312062962951622","type":"rectangle","data":{"p1":{"x":588.1470782689522,"y":31.92866008588851},"p2":{"x":600.8042390010111,"y":44.585820817947365}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{}},{"id":"dl937254962591253","linkedId":"de13864094431472274"}]},{"id":"dg14381181430645285","entities":[{"id":"dg851948865293015","entities":[{"id":"dp6449076364831263","type":"rectangle","data":{"p1":{"x":551.9827880859375,"y":28.429167183044143},"p2":{"x":564.6399488179964,"y":41.335634957633346}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp5027674435197778","type":"rectangle","data":{"p1":{"x":553.5649331774448,"y":30.042475654867786},"p2":{"x":566.2220939095037,"y":42.94894342945699}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}},{"id":"dp5393966062547468","type":"rectangle","data":{"p1":{"x":555.1470782689522,"y":31.65578412669143},"p2":{"x":567.8042390010111,"y":44.562251901280646}},"style":{"boxShadow":{"xOffset":0,"yOffset":0,"fill":[0,0,0,1]},"fillColor":[248,231,28,1]}}],"data":{"rotation":0}},{"id":"dl9970922422977695","linkedId":"de130364287178661"}]},{"id":"da7287519209547981","data":[{"x":574.9260864257812,"y":217.35307836532593},{"x":574.9260864257812,"y":55.08636474609375}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da8134947108062274","data":[{"x":433.9921875,"y":217.35307836532593},{"x":574.9260864257812,"y":217.35307836532593}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9462672208237359","data":[{"x":327.39875726699825,"y":244.89722917234633},{"x":327.39875726699825,"y":229.76184458732604}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da9177471098672696","data":[{"x":181.26448952199212,"y":244.89722917234633},{"x":327.39875726699825,"y":244.89722917234633}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7862100457272858","data":[{"x":305.0093994140625,"y":168.08636474609375},{"x":305.0093994140625,"y":131.21600341796875}],"head":"no","tail":"fh<","shaft":"-","headScale":0.6},{"id":"da8237929411758496","data":[{"x":545.9260864257812,"y":36.50826115608213},{"x":458.02362060546875,"y":36.50826115608213}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da784974372238094","data":[{"x":213.0093994140625,"y":155.3687645435333},{"x":245.026611328125,"y":155.3687645435333}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da5017675230909444","data":[{"x":261.0093994140625,"y":212.08636474609375},{"x":261.0093994140625,"y":131.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da7847399800114798","data":[{"x":261.0093994140625,"y":212.50826115608226},{"x":273.39875726699836,"y":212.50826115608226}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da04620954595561888","data":[{"x":254.39875726699825,"y":245.21600341796875},{"x":254.39875726699825,"y":185.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da3986932486764072","data":[{"x":254.39875726699825,"y":185.28239979743955},{"x":273.66242184638975,"y":185.28239979743955}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"dp8618704677398219","type":"square","data":{"p1":{"x":77.0172119140625,"y":66.28239979743955},"p2":{"x":89.5172119140625,"y":78.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp4220243817144764","type":"square","data":{"p1":{"x":107.0172119140625,"y":66.28239979743955},"p2":{"x":119.5172119140625,"y":78.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"da6000787670579764","data":[{"x":69.0093994140625,"y":83.28239979743955},{"x":69.0093994140625,"y":79.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp40504580124109624","type":"square","data":{"p1":{"x":26.0172119140625,"y":88.28239979743955},"p2":{"x":38.5172119140625,"y":100.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp05521779590020026","type":"square","data":{"p1":{"x":41.0172119140625,"y":88.28239979743955},"p2":{"x":53.5172119140625,"y":100.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"dp5297858632182728","type":"square","data":{"p1":{"x":71.0172119140625,"y":88.28239979743955},"p2":{"x":83.5172119140625,"y":100.78239979743955}},"style":{"fillColor":[248,231,28,1]}},{"id":"da9760486685833776","data":[{"x":33.0093994140625,"y":105.28239979743955},{"x":33.0093994140625,"y":101.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da5414642445065745","data":[{"x":233.0093994140625,"y":168.21600341796875},{"x":252.0093994140625,"y":168.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da8874845382551191","data":[{"x":252.0093994140625,"y":168.21600341796875},{"x":252.0093994140625,"y":98.21600341796875}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da3614163071748169","data":[{"x":194.0093994140625,"y":221.32824096679684},{"x":194.0093994140625,"y":207.28239979743955}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da6285132337880759","data":[{"x":233.0093994140625,"y":192.21600341796875},{"x":233.0093994140625,"y":168.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da36703405582495274","data":[{"x":208.0093994140625,"y":192.21600341796875},{"x":233.0093994140625,"y":192.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"dp31192838658068833","type":"doc-cube","data":{"p1":{"x":80.31076744317738,"y":229.9559559513225},"p2":{"x":118.40112242936175,"y":267.66590272519784},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp21586068142524484","type":"doc-cube","data":{"p1":{"x":80.31076744317738,"y":197.65354029821492},"p2":{"x":118.40112242936175,"y":235.36348707209038},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp3674475134050299","type":"doc-cube","data":{"p1":{"x":90.99359130859375,"y":240.2549580112808},"p2":{"x":129.08394629477812,"y":277.96490478515625},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp5033659830497497","type":"doc-cube","data":{"p1":{"x":90.99359130859375,"y":208.2549580112808},"p2":{"x":129.08394629477812,"y":245.96490478515625},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"dp23700482503033227","type":"doc-cube","data":{"p1":{"x":132.49131067039139,"y":230.48331622683804},"p2":{"x":170.58166565657575,"y":268.1932630007134},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp6002948552391556","type":"doc-cube","data":{"p1":{"x":132.49131067039139,"y":198.18090057373047},"p2":{"x":170.58166565657575,"y":235.89084734760593},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1]}},{"id":"dp21640677116835727","type":"doc-cube","data":{"p1":{"x":143.17413453580775,"y":241.2549580112808},"p2":{"x":181.26448952199212,"y":278.96490478515625},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[230,240,210,1],"strokeType":"-"}},{"id":"dp23699338099923106","type":"doc-cube","data":{"p1":{"x":143.17413453580775,"y":209.2549580112808},"p2":{"x":181.26448952199212,"y":246.96490478515625},"flipX":true,"percentage":0.22295261171231578},"style":{"fillColor":[184,233,134,1]}},{"id":"da6761432924104998","data":[{"x":47.026611328125,"y":244.89722917234633},{"x":80.0093994140625,"y":244.89722917234633}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da05559165748430894","data":[{"x":208.0093994140625,"y":96.50826115608213},{"x":208.0093994140625,"y":92.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da5357038925844808","data":[{"x":124.0093994140625,"y":184.21600341796875},{"x":124.0093994140625,"y":126.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da07608551579945444","data":[{"x":124.0093994140625,"y":126.21600341796875},{"x":238.026611328125,"y":126.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da9064000025688352","data":[{"x":238.026611328125,"y":126.21600341796875},{"x":238.026611328125,"y":98.53384399414062}],"head":"fh>","tail":"no","shaft":"-","headScale":0.6},{"id":"da00021660160795677896","data":[{"x":98.0093994140625,"y":184.21600341796875},{"x":124.0093994140625,"y":184.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6},{"id":"da6273542180639886","data":[{"x":98.0093994140625,"y":197.21600341796875},{"x":98.0093994140625,"y":184.21600341796875}],"head":"no","tail":"no","shaft":"-","headScale":0.6}],"settings":{"grid":true,"diagramHeight":304.9266357421875}}]},{"id":"n0.9182410738498363","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":5062,"delayRenderCache":{"av":5062,"map":{"n0.2798165469167486":{"n0.8584969463576833":{"w":11.3661,"h":8.4545,"bl":0.8214}},"n0.0956182946294597":{"n0.35156619811075585":{"w":11.6193,"h":8.4545,"bl":0.8214}},"n0.4915964638796144":{"n0.6764598294619883":{"w":13.4368,"h":41.6667,"bl":0.8333}},"n0.44181901465933904":{"n0.19455039516198558":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.8377316246435462":{"n0.8879719304316316":{"w":11.6193,"h":8.4545,"bl":0.8214}},"n0.6638238662000462":{"n0.9142747805274785":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.8656149269890585":{"n0.2421330624441942":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.6037157092616128":{"n0.6856134748473006":{"w":11.122,"h":8.4545,"bl":0.8214}},"n0.7968369877522394":{"n0.9903605090117544":{"w":7.5955,"h":8.988,"bl":0.7726}},"n0.43200332154226206":{"n0.6777525444975907":{"w":7.7673,"h":8.988,"bl":0.7726}},"n0.7879157549084901":{"n0.574213430457988":{"w":7.5955,"h":8.988,"bl":0.7726}},"n0.6909822130568688":{"n0.7516130028137709":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.608719912583584":{"n0.12942752166974025":{"w":24.3236,"h":8.1019,"bl":0.8571}},"n0.9805767880860297":{"n0.8796898714453854":{"w":10.6518,"h":9.1146,"bl":0.7619}},"n0.8192672737499627":{"n0.4046619303284873":{"w":5.3982,"h":9.1146,"bl":0.7619}},"n0.8865234094211434":{"n0.7670471443345628":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.9553225079236318":{"n0.36904407403017525":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.07663451775769459":{"n0.21276920260652177":{"w":6.7184,"h":9.1146,"bl":0.7619}},"n0.05892219861296333":{"n0.6634858829152157":{"w":16.8457,"h":12.5054,"bl":0.7021}},"n0.8095639861826163":{"n0.6922443966909593":{"w":15.8511,"h":12.5054,"bl":0.7021}},"n0.7620537820832181":{"n0.6042093799923687":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.9087874361013744":{"n0.31153597860941096":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.678448619782392":{"n0.07297285074437698":{"w":5.3982,"h":9.1146,"bl":0.7619}},"n0.2860407715183735":{"n0.4675833849066542":{"w":22.4157,"h":12.5054,"bl":0.7021}},"n0.8842098281055866":{"n0.7129346546594733":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.6926625074118744":{"n0.8820827388445249":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.19734605494092916":{"n0.6878304647006728":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.11712223778126041":{"n0.560660220226239":{"w":7.4599,"h":9.6481,"bl":0.7198}},"n0.7646762117471588":{"n0.2652112962808757":{"w":10.6518,"h":9.1146,"bl":0.7619}},"n0.8432401649435193":{"n0.3745027443049487":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.865317173645763":{"n0.43454788566174973":{"w":11.0315,"h":9.6481,"bl":0.7198}},"n0.6370642722097213":{"n0.9405832457870693":{"w":7.6317,"h":9.6481,"bl":0.7198}},"n0.7046338254291307":{"n0.4472116882434696":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.7689628952048579":{"n0.49535503691405913":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.5800614332963825":{"n0.7399053922658398":{"w":7.6317,"h":9.6481,"bl":0.7198}},"n0.5054730445479463":{"n0.7748604418054355":{"w":7.6317,"h":9.6481,"bl":0.7198}},"n0.3935563474086412":{"n0.7205301889098097":{"w":5.3982,"h":9.1146,"bl":0.7619}},"n0.9680449396846869":{"n0.639855730025886":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.4581428332056161":{"n0.5961478322886438":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.39136111084628955":{"n0.37647153187475135":{"w":6.7184,"h":9.1146,"bl":0.7619}},"n0.09302421410022554":{"n0.6389586816019504":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.13123680074453592":{"n0.9518648643126093":{"w":6.5014,"h":20.2546,"bl":0.8286}},"n0.9901597008831791":{"n0.6003475309273705":{"w":5.3982,"h":9.1146,"bl":0.7619}},"n0.9801920815872638":{"n0.3470720973214332":{"w":10.9502,"h":9.1146,"bl":0.7619}},"n0.7593809752282012":{"n0.9544275247121161":{"w":12.2703,"h":9.1146,"bl":0.7619}},"n0.3132924567681319":{"n0.15940430690943685":{"w":23.8082,"h":9.9736,"bl":0.6963}},"n0.7590487519403368":{"n0.3226085603936859":{"w":24.2965,"h":9.9736,"bl":0.6963}},"n0.27431182150181543":{"n0.9452261389098291":{"w":11.3661,"h":8.4545,"bl":0.8214}}}}}
